Parallel Statistical Model Checking for Safety Verification in Smart Grids

By using small computing devices deployed at user premises, Autonomous Demand Response (ADR) adapts users electricity consumption to given time-dependent electricity tariffs. This allows end-users to save on their electricity bill and Distribution System Operators to optimise (through suitable time-dependent tariffs) management of the electric grid by avoiding demand peaks. Unfortunately, even with ADR, users power consumption may deviate from the expected (minimum cost) one, e.g., because ADR devices fail to correctly forecast energy needs at user premises. As a result, the aggregated power demand may present undesirable peaks. In this paper we address such a problem by presenting methods and a software tool (APD-Analyser) implementing them, enabling Distribution System Operators to effectively verify that a given time-dependent electricity tariff achieves the desired goals even when end-users deviate from their expected behaviour. We show feasibility of the proposed approach through a realistic scenario from a medium voltage Danish distribution network.

==> 10_introduction/content.tex <==
% !TEX root = ../root.tex

%briefly sketched
%predicted pp
%DAGUM l'algo 1 nostro sia quello
%l'algo 2,3,4 versione parallels di 1, check.

\Input{framework.tex}

\SectionInput[sec:intro:motivations]{Motivations}{motivations.tex}

\SectionInput[sec:intro:contributions]{Contributions}{contributions.tex}


\endinput

\Comment{%%%%%%%%%%%%%%%%%%%%%%%%%%
As deviations are unpredictable, in this paper we define a \emph{probabilistic model} for them and v

As an example, we can say that with 10\% probability a user actual power profile will consume 40\% more than the corresponding collaborative power profile, and so on. This generates a {\em probability distribution} on the resulting aggregated
power demand on the given substation. Thus, in order to 
investigate the consequences of users deviations from collaborative power profiles, we need to compute such a probability distribution, given the probabilistic model for
users deviations (which we call {\em disturbance model}).
%disturbance model is better, since it is consistent with the terminology we use in other papers are with model checking jargon.

A computational service, called {\em \Ac{PPSV} service}, able to compute such a probability distribution, given the collaborative power profiles for each user and a disturbance model for user deviations, has been presented in~\cite{mancini-etal:2014:smartgridcomm}. Namely, \Ac{PPSV} uses a {\em statistical model checking} approach~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}
%Borrowing the main idea from~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}, \Ac{PPSV} also requires in input two real numbers $\epsilon, \delta \in [0, 1]$. As a result, the probability distribution returned as output is correct, up to a tolerance factor $\epsilon$, with confidence $1 - \delta$. Following the Monte Carlo-like approach in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}, \Ac{PPSV} achieves such a goal by generating $N = f(\delta, \epsilon)$ random values for the aggregated power demand $P$ (at the substation level) under the given disturbance model. Here, $N$ depends not only on $\delta$ and $\epsilon$ but also on the outcomes of previous samples (this technique is known as {\em sequential analysis}). If $S$ is the number of times that $P$ results to be in a given interval aggregated demand interval $I$, then the probability of $I$ is $\frac{S}{N}$. The whole process must be repeated for all intervals $I$.

However, the \Ac{PPSV} algorithm %(also briefly sketched in~\cite{mancini-etal:2014:smartgridcomm})
performs a sequential computation. This may require a very long computation time as a more precise output is required (i.e., as $\epsilon, \delta$ decrease). As an example, \Ac{PPSV} needs ... days to compute the output probability distribution with $\epsilon = ..., \delta = ...$, when applied to a meaningful and realistic scenario, taken from an existing Danish subnetwork with 130 users connected to a single substation. Thus, a more effective algorithm (and tool) is needed in order to enable \Acp{DSO} to actually use \Ac{PPSV}.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \Comment{
%% It has recently been proposed~\cite{mancini-etal:2014:smartgridcomm} to counteract this problem with a methodology based on three integrated services. In a nutshell, the first service, called \Ac{EVT}, focus on the whole \Ac{EDN} and computes, for each substation (feeder), the power safety threshold not to be exceeded by residential users connected to it. The second service, called \Ac{DAPP}, focus on a single substation $s$ at a time, redistributing the 
%% power demand ({\em load shifting}) so that the constraints on the input substation $s$ are fulfilled. This is done by computing, for each residential home $u$ connected to $s$, an {\em individualized %suggested
%%   power profile} $P_u$ (that is, different users may get different power profiles), so that if all users follow their power profile then the safety threshold on $s$ is not violated (that is, the {\em aggregated power demand} on $s$ is always below the safety threshold $s$). Each user $u$ is motivated to follow the individualised power profile $P_u$ by an {\em individualised price policy} based on $P_u$.
%% Note that proposing individualised price policies avoids that power demand peaks are simply shifted through the day (power demand {\em rebounds}),
%% which would again violate constraints on substations.

%% Unfortunately, since users are not forced to follow their individualised power profiles, they may {\em deviate}, thus causing a substation safety failure, and thus an economical damage if such failures are too frequent. In order to 
%% investigate the consequences of users deviations from individualised power profiles, the last service, called \Ac{PPSV} computes the probability distribution of the resulting aggregated
%% power demand on $s$, given a probabilistic model for such
%% deviations ({\em disturbance model}). 

%% In this paper we focus on the \Ac{PPSV} service. Borrowing the main idea from~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}, the \Ac{PPSV} service also requires in input two real numbers $\epsilon, \delta \in [0, 1]$. As a result, the probability distribution returned as output is correct, up to a tolerance factor $\epsilon$, with confidence $1 - \delta$. However, the first version of the \Ac{PPSV} algorithm sketched in~\cite{mancini-etal:2014:smartgridcomm} performs a sequential computation. This may require a very long computation time as a more precise output is required (i.e., as $\epsilon, \delta$ decrease). Finally, note that \Ac{PPSV} service may be used also in other contexts, namely to check deviations of users from power profiles which have not been computed by \Ac{DAPP}, as well as using substation safety thresholds not computed by \Ac{EVT}.
%% }




\begin{Section}{Paper Overview}
\DraftWarning{To be done}
The paper is organised as follows.
After introducing the required background (\cref{sec:background}),
we define the problem (\cref{sec:ppsv}) 
and
we describe our new algorithm % implementation 
as a \emph{distributed multi-core} computational service (\cref{sec:algo}).
We then draw experimental results on a \emph{realistic} case study encompassing a substation line with 130 houses in Denmark (\cref{sec:expres}), showing that
%We show that 
our implementation scales well with the number of the computational cores available, as the workload is dynamically distributed by an Orchestrator process among the available slave processes.
%This implies that the computation is efficient also on \emph{heterogeneous} clusters (as ours). 
Finally, we discuss related work in \cref{sec:relwork}.


\Comment{%%%%%%%%%%%%%%%%%%%%%%%
In order to overcome the above described obstruction, and thus make \Ac{PPSV} effectively usable by \Acp{DSO}, in this paper we present a parallel (for clusters of computers with distributed memory) re-engineering of the algorithm for the \Ac{PPSV} service in~\cite{mancini-etal:2014:smartgridcomm}. We call such algorithm {\em \Ac{pPPSV}}. By employing \Ac{pPPSV}, it is possible to obtain the probability distribution for the case study discussed above in ... minutes instead of ... days, by employing 80 cores in a cluster of computers.

%\Ac{pPPSV} is designed so as to efficiently compute a probability distribution, rather than a single expected value as in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}. Moreover,  we show that \Ac{pPPSV} is correct w.r.t. the sequential version in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.

In a nutshell, \Ac{pPPSV} distributes the generation of the $N$ samples among the available cores. The workload is dynamically distributed by an {\em orchestrator} process, so that the computation is efficient also on heterogeneous clusters. Moreover, also if \Ac{pPPSV} is run on 1 core, it obtains a gain w.r.t the original \Ac{PPSV} service, as it computes the output probability in an optimised way. Namely, the sampling is organised so that outer cycle on all power intervals $I$ is avoided. We formally prove that, with such optimization, \Ac{pPPSV} is still correct w.r.t. the sequential version in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\Comment{%%%%%%%%%%%%%%%%%%
  %% Move this before!
In order to understand the main idea underneath \Ac{pPPSV}, we first have to explain how the sequential \Ac{PPSV} works. Following the Monte Carlo-like approach in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}, \Ac{PPSV} generates $N = f(\delta, \epsilon)$ random values for the aggregated power demand $P$ (at the substation level) under the given disturbance model. Here, $N$ depends not only on $\delta$ and $\epsilon$ but also on the outcomes of previous samples (this technique is known as {\em sequential analysis}). If $S$ is the number of times that $P$ results to be in a given interval aggregated demand interval $I$, then the probability of $I$ is $\frac{S}{N}$. The whole process must be repeated for all intervals $I$.

\Ac{pPPSV} improves \Ac{PPSV} on two key features. First of all, \Ac{pPPSV} makes the computation parallel, by distributing the generation of the $N$ samples among the available cores. The workload is efficiently dynamically distributed by an {\em orchestrator} process, so that the computation is efficient also on heterogeneous clusters. Second, \Ac{pPPSV} is designed so as to avoid the outer cycle on all intervals $I$, that is, the probability distribution required in output is computed in one step. 
}%%%%%%%%%%%%%%%%%%%%%


%Finally, we experimentally evaluate \Ac{pPPSV} on the meaningful and realistic scenario mentioned above, taken from an existing Danish \Ac{EDN}. As an example, using \Ac{pPPSV} we are able to...
\end{Section} %% Contributions


%\begin{Section}{Paper Overview}
%This paper is organised as follows. 
%\Cref{sec:background} introduces the background needed to understand the paper, i.e., the algorithms for Monte Carlo estimation in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola,grosu-etal:2005:tacas}. 
%%
%\Cref{sec:ppsv} gives input and output of \Ac{PPSV}, 
%\cref{sec:algo} describes our new parallel algorithm, %, whose correctness is shown in  
%%
%%\cref{sec:correctness}.
%%that the probability distribution computed \Ac{PPSV} approximates the real probability distribution with arbitrarily high precision.
%%\wrt the sequential version in~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.  ????????
%%
%\cref{sec:expres} describes our experimental evaluation.
%Finally, \cref{sec:relwork} reports on related work.
%\end{Section}


%\SectionInput[sec:relwork]{Related Work}{related_work.tex}


==> 10_introduction/contributions.tex <==
%!TEX root = ../root.tex
In this paper we propose \emph{\Ac{PPSV}}, a \Ac{HPC}-based software system aimed at supporting \Acp{DSO} in analysing the possible aggregated effects, on the \Ac{EDN} substation, of individualised price policies for electricity end-users, designed for highly dynamic \Ac{ADR} schemes.

In particular, \Ac{PPSV} allows \Acp{DSO} to compute a portfolio of \Acp{KPI} over the \emph{probability distribution of the \Ac{APD}}, %, and to estimate their values under the candidate portfolio of price policies at hand, 
subject to probabilistic deviations of end-users from their predicted behaviours under the given price policies.

\Ac{PPSV} can then act both as a \emph{\Ac{DSS}} allowing \emph{what-if analyses}, and as an \emph{automated verifier} for the safety of an envisioned set of price policies.
In particular, \Ac{PPSV} enables safety assessment of the price policies computed through automated methods (\eg~\cite{hayes-etal:2016:tsg} and references therein). 

% , hence supporting automated optimisation methods (\eg~\cite{hayes-etal:2016:tsg}) for the computation of optimal and \emph{safe} sets of price policies to be deployed (\eg each day) to end-users as part of a highly dynamic \Ac{ADR} schema.




%, \eg exploiting electricity day-ahead market prices.

\endinput





probability that the \Ac{APD} for the \Ac{EDN} substation under analysis exceeds the substation safety threshold, given that the users are subject to the given price policies.

To perform its risk analysis, our system takes as input:
\begin{enumerate*}[(i)]
\item the set of price policies to be analysed; 
\item the \emph{expected behaviour} of end-users under the new price policies (as \eg computed by \cite{hayes-etal:2016:tsg});
\item the \Ac{EDN} substation safety requirements;
\item a \emph{probabilistic model} of end-users deviations from their expected behaviours.
\end{enumerate*}

Using algorithms based on statistical model-checking and deployed on a \Ac{HPC} infrastructures, \Ac{PPSV} computes an estimation of the probability distribution of the \Ac{APD}, and provides \Acp{DSO} with an estimation of the \emph{probability} that the substation safety requirements will be violated 
about the end-user deviation model.

Hence, by exploiting \Ac{PPSV}, \Acp{DSO} have immediately usable means to evaluate the risk (in terms of substation safety requirements violations) associated to the deployment of a new set of price policies.



%Our method is a \emph{new parallel algorithm}, explicitly designed to run on a cluster of machines, which relies on a \emph{parallelisation} of two different \emph{statistical model checking} approaches~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.

%In this paper we propose a \emph{new parallel algorithm} for \Ac{PPSV} which relies on a \emph{parallelisation} of two different \emph{statistical model checking} approaches~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.
%
%Our new algorithm has been explicitly designed to run on a cluster of machines.
%, and is much faster than the algorithm sketched in~\cite{mancini-etal:2014:smartgridcomm} also when run in a \emph{sequential} fashion.

==> 10_introduction/framework.tex <==
%!TEX root = ../root.tex
One of the most challenging problems in the management of modern electric smart grids is to find a trade-off between two conflicting goals. On one hand both the energy retailer, who sells energy, and the \Ac{DSO}, who manages the \Ac{EDN}, want to sell as much energy as possible, without forcing %residential 
end-users to cut their power demands. 
On the other hand, if all users require power at the same time (\emph{peak time}), this may result in higher costs for the \Ac{DSO} (due to, \eg the need of suddenly activating additional power plants to face such peaks), and possible service and/or infrastructure disruption (due to, \eg feeder damage or reduced life-time~\cite{hilshey-etal:2013:tsg}).
%
In fact, the maximum power that can be safely provided by an \Ac{EDN} (\ie without stressing the infrastructure devices) is \emph{significantly less} than the power that would be needed in the most demanding scenario, when all users request their maximum allowed power simultaneously~\cite{kersting:2013:book}. 
%
% Uhm, penso che il problema vero è che la network è stata progettata a suo tempo per una domanda media di energia ben minore di quella attuale:
%This is because a \emph{cost-effective} design of an \Ac{EDN} heavily relies on the assumption that user demands are quite different from each other for most of the time.



\Ac{DSM}~\cite{vlot-etal:2013:tsg} approaches are used to achieve the objective of reducing/avoiding the presence of dangerous peaks in the \Ac{APD} (thus performing what is called \emph{peak shaving}).
%
%\Ac{DSM}~\cite{vlot-etal:2013:tsg} approaches are used to counteract such a problem by acting, directly or indirectly, on end users.
%There are two main approaches to \Ac{DSM}:
%\Ac{DLC} and \Ac{DR}.
%With \Ac{DLC}, %(see, e.g.,~\cite{douglass-etal:2013:tsg})
%the \Ac{DSO} \emph{directly} controls user consumption
%by remotely curtailing high-load appliances when needed.
%%
%With \Ac{DR} instead, each user receives
%a time-dependent tariff (called a \emph{price policy}) for the next future period (typically, one month). 
An increasingly popular approach to \Ac{DSM} is \Ac{DR} (see, \eg \cite{hayes-etal:2016:tsg} and references therein).
%
%Differently than with \Ac{DLC} (see, \eg~\cite{douglass-etal:2013:tsg}), where the \Ac{DSO} \emph{directly} controls user consumption by remotely curtailing high-load appliances when needed, 
%\Ac{DR} techniques are \emph{non-invasive} (\wrt \Ac{DLC} approaches, \eg \cite{douglass-etal:2013:tsg}) means for the \Acp{DSO} to steer aggregate power demand. \Ac{DR} is of course the only viable method to keep the aggregate power demand under control for most types of end-users (residential or commercial), who would not accept a direct control of their appliances by the \Ac{DSO}.
%
%The key enabler for \Ac{DR} are \emph{\Ac{IBR}} (see, \eg~\cite{reiss-white:2005:res}) or \emph{time-dependent tariffs} (see, \eg~\cite{????}) computed by the \Ac{DSO} and proposed to the users.
%
In a \Ac{DR} setting, \emph{\Ac{IBR}} %(see, \eg~\cite{reiss-white:2005:res}) 
or \emph{time-dependent tariffs} are computed by the \Ac{DSO} and proposed to the users, with the goal of \emph{indirectly steering} their individual power demands in such a way that the \Ac{APD} satisfies \Ac{EDN} constraints.

Classically, \Ac{DR} has been implemented by directly including such tariffs in the user contracts.
%
However, this approach poses two main problems: 
\begin{enumerate*}
\item tariffs explicitly included in the user contracts are long-term and \emph{static}, as users must be able to get used to and comfortably follow them;
\item such tariffs might not be enough to sufficiently diversify the individual user power demands, thus simply resulting in peak rebounds (see, \eg~\cite{li-etal:2012:automated}), where the critical peaks of the \Ac{APD} at the substation level are not removed, but just shifted in time.
\end{enumerate*}	

==> 10_introduction/motivations.tex <==
%!TEX root = ../root.tex

Recent advancements in energy storage technology and electricity usage control algorithms enabled innovative approaches to \Ac{DR} (see, \eg~\cite{mishra-etal:2012:e-energy,erdinc-etal:2015:smart,chau-etal:2016:cost,lujano-etal:2017:optimizing}) where small computing devices (in the following: \Acp*{HEC}) are deployed at user premises to \emph{autonomously} shift high loads (\eg charging of \Acp*{PEV}, or heating), control local electricity generators (\eg \Ac*{PV}[,] panels) and storage (\eg batteries), compatibly with user actual behaviour and device capabilities (\eg capacities and power rates of installed batteries), while reacting to electricity price changes. Their ultimate goal is to minimise the user electricity bills. 
% \Acp{HEC} take care of automatically shifting loads that can be delayed to low-tariff time slots (\eg charge \Acp*{PEV}), and control the charge/discharge of installed batteries in order, \eg to use the accumulated electricity when the buy-price is high, with the goal of minimising the user electricity bill.

In such \emph{\Ac{ADR}} settings, the users are freed from the burden to manually adapting their electricity consumption behaviours, as reactions to price changes are handled automatically.
%
All this allows \Acp{DSO} to propose time-dependent tariffs envisioning \emph{high-frequency} fluctuations (\eg a new price every 15 minutes) announced with short notice (\eg 24 hours in advance), exploiting, \eg quotes of the day-ahead market (see, \eg \cite{mohsenian-etal:2010:optimal}). 
%
Also, such \emph{price policies} can be diversified among users connected to the same \Ac{EDN} substation (under non-discrimination requirements, see \eg~\cite{hayes-etal:2016:tsg}) in order to induce their \Acp{HEC} to react in complementary ways, ultimately producing an \Ac{APD} compatible with the grid safety constraints. 
To this end, designed price policies must take into consideration %non-discrimination issues among users and 
suitable short-term forecasts of each user power demand (which are typically based on historical demand plus, possibly, other data, see, \eg~\cite{decastro-cramton:2012:allerton}).
%, in order to require just \emph{small} corrective actions for them to yield their full economic saving (hence, easily implementable by the user or, automatically, by the installed \Acp{HEC}). 

In this paper we focus on such \Ac{ADR} scenarios.
The design of \emph{short-term}, \emph{individualised} price policies based on single user power demand forecasts and envisioning \emph{highly fluctuating} prices poses several computational challenges for the \Ac{DSO}.
%
In previous work \cite{hayes-etal:2016:tsg} we proposed global optimisation algorithmic methods to support the price policy design phase, building on mature technologies widely used in many diverse application domains (see, \eg \cite{mancini-etal:2012:sac,mancini:2016:negotiation,mancini-etal:2018:ismis,mancini-etal:2018:rcra-relay}).
%
Anyway, although global optimisation guarantees to return a set of policies (if one such set exists) that would satisfy all the requirements, in practice the grid safety is still not guaranteed.
This is because, due to the limits of \Ac{HEC} capabilities, the actual user power demands may \emph{not} follow the power profiles expected by the \Ac{DSO} as a result of the proposed price policies.
%



% to adapt their power demand to their price policies, they might sometimes behave in unexpected ways, \eg preferring to use more expensive electricity rather than shifting in time some of their loads. 
%
%Second, optimisation of individual price policies are computed starting from forecasts of each user power demand in the next time period, %(\eg the next 24 hours), 
%and the amount of uncertainty in such forecasts (typically based on historical demand plus, possibly, other data, see, \eg~\cite{decastro-cramton:2012:allerton}), could be substantial.

Although the \Ac{DSO} can perform a \emph{worst case analysis} (as in, \eg \cite{mancini-etal:2015:dsd}) of the impact of the envisioned set of price policies on the \Ac{EDN} safety, such an analysis could be too pessimistic and prevent the \Ac{DSO} from fully exploiting the opportunities stemming from highly fluctuating tariffs and its own investments on the \Ac{EDN}.


\endinput






\Cref{fig:dapp_eval_aggr} shows an example of peak shaving obtained by \Ac{ADR}: the yellow curve shows the predicted \Ac{APD} over several months for 130 residential end users in Denmark (our case study in \cref{sec:expres}) connected to a substation designed as to provide up to \Pretty[style=kw]{400} in safe conditions (\emph{safety threshold}).
Several peaks (much beyond the substation safety threshold) can be observed.
%The presence of peaks in the \Ac{APD} higher than the substation safety threshold triggers the activation of additional power plants (called \emph{peak plants}) when there is need of more power and increases the probability of damage in the infrastructure (\eg the feeder), leading to higher costs for the \Ac{DSO} and higher risks of service disruption.
By using demand-aware individualised price policies~\cite{hayes-etal:2016:tsg}, the \Ac{DSO} is able to \emph{shave} such peaks in power demand almost completely (see the blue curve in \cref{fig:dapp_eval_aggr}). Such price policies only require small corrective actions by each user, easily implementable by an automous system as a \Ac{HEC}.


\begin{Figure}
	\IncludeGraphics[absolute=true, width=\linewidth]{figures/APD/apd.pdf}
	\caption{%
		Predicted \Acf{APD} (yellow) from 130 homes in Denmark connected to a substation (our case study in \cref{sec:expres}) under no \Acf{DR}. 
		The substation safety threshold of \Pretty[style=kw]{400} is violated several times. As a consequence of using \Acs{DR}, the \Acs{APD} becomes that shown in blue (no peaks over the safety threshold).
	}
	\label{fig:dapp_eval_aggr}
\end{Figure}




Price policies are typically defined by using either \Acp{IBR} tariffs (where the per-unit energy tariff is dependent on the power demand, see~\cite{reiss-white:2005:res}), or time-dependent tariffs (where the per-unit energy tariff is dependent on the time of the day), or both (see~\cite{hayes-etal:2016:tsg}). 

Starting from the estimation of the power demand of a user $u$ in the incoming time period (\eg from historical and other data \cite{decastro-cramton:2012:allerton}) and on an envisioned price policy for $u$, a \Ac{DSO} can predict the power profile that $u$ will have \emph{if} that price policy were in charge. This is called the (predicted) \emph{\Ac{CPP}} for user $u$ \cite{hayes-etal:2016:tsg}.
%
Of course, there is \emph{no} guarantee that users will actually follow their predicted collaborative profiles. 
%
This is due to two main reasons. 
%
First, users may sometimes prefer to use more expensive electricity rather than shifting in time some of their loads. 
%
Second, collaborative profiles are computed starting from predictions of the user power demand in the future (\eg the next month), and the amount of uncertainty in such predictions is substantial.
%
% on a prediction (the typical scenario is that the price policy will be applied in the incoming month, thus a prediction for the user power demand in the incoming month is needed), which cannot be 100\% accurate. 

Thus, although the \Ac{DSO} might, in some cases, design price policies that completely avoid peaks of the \Ac{APD}, the \Ac{EDN} may still be at risk, because the actual users might \emph{deviate} from their predicted collaborative power profiles.

==> 20_system/content.tex <==
%!TEX root = ../root.tex

%In this section we define the inputs and outputs of \Ac{PPSV} and give a high-level overview of its architecture and underlying algorithms. 

In this section we describe the input required and the output provided by \Ac{PPSV}. 
%
In the following, we denote with 
	\Reals, 
	%\RealsGEZ,
	\RealsGZ, \Naturals
the sets of, \respectively, 
	all real,
	%, non-negative real and 
	strictly positive real,
	and non-negative integer numbers.
% and with
% 	\Naturals, 
% 	\NaturalsZ,
% 	\Integers
% 	%
% the sets of, \respectively, 
% 	all integers, 
% 	strictly positive integers and
% 	non-negative integers.

% \DraftWarning{Remove unused sets.}	


We assume that the period for which we want to compute the \Ac{APD} probability distribution (\eg the next day) is split into a set $\SetTimeSlots$ of time slots of equal duration (\eg 15 minutes).


Given $\SetTimeSlots$, a \emph{power profile} is a function $\PowerProfile: \SetTimeSlots \to \Reals$.
For each $\TimeSlot \in \SetTimeSlots$, $\PowerProfile(\TimeSlot)$ denotes a power value (in kW). 
We use such functions to model both the users' \Acp{EPP} (in this case $\PowerProfile(\TimeSlot)$ gives the average power demanded by a given user during time slot $\TimeSlot$) and the substation safety threshold (in this case $\PowerProfile(\TimeSlot)$ gives the maximum average power that the substation can provide during time slot $\TimeSlot$ in safe conditions).

% %Given values for $\Tolerance$ and $\Confidence$ in $(0,1)$, 
% \Ac{PPSV} % computes, with confidence $1 - \Confidence$ and tolerance $\Tolerance$, 
% computes a suitable estimation of
% the probability distribution values of the \Ac{APD} to a given \Ac{EDN} substation $\Substation$, taking as input the \Acp{EPP} for all users connected to $\Substation$ and a probabilistic model of their deviations from such predictions.



\SectionInput[sec:system:input]{Inputs}{input/content.tex}

\SectionInput[sec:system:output]{Outputs}{output/content.tex}

==> 20_system/input/content.tex <==
%!TEX root = ../../root.tex

The system requires the \Ac{DSO} to provide various inputs and configuration options, the most important of which are briefly outlined in the following.

\SectionInput[sec:system:input:users]{\Ac{EDN} substation end-users}{substation-and-users.tex}

\SectionInput[sec:system:input:period]{Analysis time period}{time.tex}

\SectionInput[sec:system:input:epp]{\Acfp{EPP}}{user-profiles.tex}

\SectionInput[sec:system:input:deviation-model]{Users deviation model}{deviation-model.tex}

\SectionInput[sec:system:input:substation]{Substation safety requirements}{substation.tex}

\SectionInput[sec:system:input:kpi]{\Acp{KPI}}{kpi.tex}

\SectionInput[sec:system:input:parameters]{Parameters}{parameters.tex}






==> 20_system/input/deviation-model.tex <==
%!TEX root = ../../root.tex
%
A \emph{probabilistic model} of end-user deviations \wrt their expected behaviours, 
%
given in terms of a function $\DeviationModel{\User}: \DomainDeviations{\User} \to [0,1]$ for each $\User \in \SetUsers$, where $\DomainDeviations{\User}$ is a bounded interval of real values defining possible deviations of $\User$ \wrt \Ac{EPP} $p_u$.
For each user $\User \in \SetUsers$, $\DeviationModel{\User}$ defines a probability density function (over bounded support $\DomainDeviations{\User}$), hence $\int_{\DomainDeviations{\User}} \DeviationModel{\User}(x) \text{d}x = 1$.
%
For each $\User \in \SetUsers$ and $a,b \in \DomainDeviations{\User}$ ($a < b$), 
$\int_{a}^{b} \DeviationModel{\User}(x) \text{d}x$ defines the probability that $\User$ will deviate from their \Ac{EPP} by a factor between $a$ and $b$, 
\ie that in any time slot $\TimeSlot \in \SetTimeSlots$, the actual power demand of $\User$ is within $[(1 + a)\EPP{\User}(\TimeSlot), (1 + b)\EPP{\User}(\TimeSlot)]$. 
%
User deviation probabilities can be retrieved from historical data, \eg by comparing past users' \Acp{EPP} to their actual behaviours.
%
Also, to overcome the intrinsic uncertainty of users behaviour predictability, sets $\DomainDeviations{\User}$ of users' possible deviations can be rather generous (\eg in our case study of \cref{sec:expres} we allowed, for \emph{all} users, deviations as high as $\pm40\%$ \wrt their \Acp{EPP}).



==> 20_system/input/kpi.tex <==
%!TEX root = ../../root.tex
%
A finite set $\SetKPIs$ of \Acp{KPI} defined over the probability distribution of the \Ac{APD} of the \Ac{EDN} substation, for different values of the substation safety requirements $\SubstationProfile$.
%
% Formally, let $\SetAPDDensities$ be the set of all possible probability density functions of the \Ac{APD}:
% \begin{equation*}
% \SetAPDDensities = \left\{
% 	\APDDensity : \APDDensityDef ~\middle|~ \int_{-\infty}^{\infty} \APDDensity(x) ~\text{d} x = 1
% \right\}.
% \end{equation*}
% %
% Each \Ac{KPI} $\KPI \in \SetKPIs$ is defined as a function $\KPI: \SetAPDDensities \to \Reals$, mapping \Ac{APD} probability density functions to quality or cost measurements.

Defining \Acp{KPI} as general functions of the \Ac{APD} probability distributions %(for different values of the substation safety requirements) 
is a flexible way to take into account \Ac{DSO} requirements. 
%
As an example, a \Ac{KPI} might define the probability that the \Ac{APD} exceeds the substation safety power threshold when such a threshold is at most $v$. Other typical \Acp{KPI} would rank \Ac{APD} probability distributions according to their similarity to desired shapes (defined, \eg starting from the electricity quotations in the day-ahead market).

%\Acp{KPI} can be defined at different time scales (\ie for different sets of future time slots $\SetTimeSlots$) to account for different \Ac{DSO} requirements.

==> 20_system/input/parameters.tex <==
%!TEX root = ../../root.tex
Real-valued parameters
$\Tolerance, \Confidence \in (0,1)$ and $\DiscretisationStep \in \RealsGZ$ defining, \respectively, \emph{tolerance} and \emph{statistical confidence} of the computed estimated values of the \Ac{APD} probability distribution (see \cref{def:EDApproximation}) and its \emph{discretisation step} (see \cref{sec:system:output}).

==> 20_system/input/substation-and-users.tex <==
%!TEX root = ../../root.tex
%
The finite set $\SetUsers$ of end-users (households, commercial buildings, etc.) connected to the \Ac{EDN} substation of interest.

==> 20_system/input/substation.tex <==
%!TEX root = ../../root.tex
The substation safety thresholds during $\SetTimeSlots$, in terms of a power profile $\SubstationProfile : \SetTimeSlots \to \Reals$. 
To keep the substation line (and hence the \Ac{EDN}) safe, the \Ac{APD} must be less than or equal to $\SubstationProfile(\TimeSlot)$ in any time slot $\TimeSlot \in \SetTimeSlots$.

==> 20_system/input/time.tex <==
%!TEX root = ../../root.tex
%
The future period of interest, as a set of contiguous time slots $\SetTimeSlots$
of the same duration 
(\eg 15-minute time slots spanning the next day).

==> 20_system/input/user-profiles.tex <==
%!TEX root = ../../root.tex
%
The \Acp{EPP} of all end-users in $\SetUsers$, defined under the (optimistic) assumption that end-users will adhere to the price policies under analysis, as predicted by the \Ac{DSO}. Such \Acp{EPP} may be either computed by some grid-level service~\cite{hayes-etal:2016:tsg} or forecasted using, \eg users historical data or other information (see, \eg \cite{decastro-cramton:2012:allerton}). 
\Acp{EPP} are defined in terms of a power profile $\EPP{\User}$ over $\SetTimeSlots$ for each $\User \in \SetUsers$.
%
%% The \Acp{EPP} of all end-users along the substation line, as the result of a forecast using, \eg their historical data or other information (see, \eg \cite{decastro-cramton:2012:allerton}). 
%% Such users' \Acp{EPP} are defined in terms of a power profile $\EPP{\User}$ over $\SetTimeSlots$ for each $\User \in \SetUsers$.
%% %, encoding the average \emph{expected} power demand (in kW) of $\User$ for each time slot in the period of interest $\SetTimeSlots$. 
%% \Acp{EPP} are defined under the (optimistic) assumption that end-users will adhere to the price policies under analysis, as predicted by the \Ac{DSO}.
%
Note that \Acp{EPP} functions can take \emph{negative} power values, to account for, \eg power generation capabilities at end-user premises, for example \Ac{PV} installations.


==> 20_system/output/content.tex <==
%!TEX root = ../../root.tex
%
The goal of \Ac{PPSV} is to compute values for all the given \Acp{KPI} under the given inputs.
As \Acp{KPI} are functions of the \Ac{APD} probability distributions for different values of the substation safety requirements $\SubstationProfile$, the \emph{core} computational task of \Ac{PPSV} is to compute, for each value $v$ of the substation safety requirements, the probability distribution of the \Ac{APD} when the substation can safely provide power $v$. 
Such a distribution in turn depends on the \Acp{EPP} of all users 
%$\User \in \SetUsers$ 
and their probabilistic deviation models.
% $\DeviationModel{\User}$.

%Since the computation of the required \Ac{APD} probability distributions cannot be performed analytically, \Ac{PPSV} computes so called \EDApproximation{s} (\cref{def:EDApproximation}) of the probabilities of interest.

Unfortunately, an exact computation of the required \Ac{APD} probability distributions is prohibitive, because of its exponential dependence in the number of users and time-slots (see \cref{sec:expres:results} for an example). Hence, \Ac{PPSV} computes so called \EDApproximation{s} (\cref{def:EDApproximation}) of the probabilities of interest.

Formally, let $[\PowerValueMin, \PowerValueMax]$ be the interval enclosing all the possible values that the \Ac{APD} can take, given the users \Acp{EPP} and their deviation models (defining a bounded range of possible deviations $\DomainDeviations{\User}$ for each $\User \in \SetUsers$): 
%
$\PowerValueMin = \min_{\TimeSlot \in \SetTimeSlots} \left[ 
	\sum_{\User \in \SetUsers} (1 + \min(\DomainDeviations{\User})) 
		\EPP{\User}(\TimeSlot) 
\right]$
and
% \text{~and}
% %\\
$\PowerValueMax = \max_{\TimeSlot \in \SetTimeSlots} \left[ 
 	\sum_{\User \in \SetUsers} (1 + \max(\DomainDeviations{\User})) 
 		\EPP{\User}(\TimeSlot) 
 \right]$.
%
%
%
%It then computes a discretised covering of $[\Ac{APD}_{\text{min}}, \Ac{APD}_{\text{max}}]$ by a finite set $W$ of \emph{power slots}, i.e., contiguous intervals of length $\gamma$. 
Let $\SetPowerSlots$ be a covering
of $[\PowerValueMin, \PowerValueMax]$ into a finite set of disjoint and contiguous intervals of width $\DiscretisationStep$ (which we call \emph{power slots}), \ie
%
$%\begin{equation*}
\SetPowerSlots = \left\{ 
	%\PowerSlot = 
	[x, x + \DiscretisationStep) ~\middle|~ 
		%\begin{array}{l}
		x < \PowerValueMax, %\\ %it was \leq
		x = \PowerValueMin + k \DiscretisationStep, %\\
	 	k \in \Naturals%
	%\end{array}%
	%\right.%
\right\}.%
$%\end{equation*}

Let $V_\Substation = \left\{ v ~\middle|~ \SubstationProfile(\TimeSlot) = v, \TimeSlot \in \SetTimeSlots \right\}$ 
be the set of all the (distinct) values for the power safely provided by the substation in some time slot.
% (as defined by the substation safety requirements). 
%
%For each $v \in V_\Substation$, 
%let $\SetTimeSlots_v \subseteq \SetTimeSlots$ be the subset of time slots in which the substation %provides power safety threshold for \Ac{APD} is $v$, \ie $\SetTimeSlots_v = \left\{ \TimeSlot ~\middle|~ \TimeSlot \in \SetTimeSlots, \SubstationProfile(\TimeSlot) = v\right\}$. 
%
%Finally, f
Also, for each $v \in V_\Substation$ and $\PowerSlot \in \SetPowerSlots$, let $\APDDistribution_v(\PowerSlot)$ be the (exact but unknown) probability that the \Ac{APD} takes a value within power slot $\PowerSlot$ when the substation %provides power
safety threshold is $v$.

Then, \Ac{PPSV} returns a set of functions 
$%\begin{equation*}
\{ 
	\APDDistributionApprox_v : \SetPowerSlots \to \Reals \cup \{\bot\} 
		~|~ v \in V_\Substation
\}%
$ %\end{equation*}
%
(with $\bot$ being a distinguished value)
%Forthcoming \cref{thm:correctness} (see \cref{sec:correctness}) shows that,
%for each $v \in V_s$, function $\estPrAPD_v : W \to \Reals \cup \{\perp\}$ is such that:
%\noindent 
such that, 
for each $v \in V_\Substation$, 
$\APDDistributionApprox_v$ %: \SetPowerSlots \to \Reals \cup \{\bot\}$ 
has the following properties (see \cref{thm:correctness}):
\begin{itemize}
\item if $\APDDistributionApprox_v(\PowerSlot) = \bot$ for a power slot $\PowerSlot \in \SetPowerSlots$, then, with statistical confidence at least $1-\Confidence$, the probability $\APDDistribution_v(\PowerSlot)$
  %% that the \Ac{APD} takes a value within power slot $w$ when the substation %provides power
  %% safety threshold is $v$
  is less than $\Tolerance$;
\item for all the other power slots $\PowerSlot$, with statistical confidence at least $1-\Confidence$, value $\APDDistributionApprox_v(\PowerSlot)$ is 
%such that:
within $(1\pm\Tolerance) \APDDistribution_v(\PowerSlot)$.
%
% \begin{equation*}
% 	(1-\Tolerance) \APDDistribution_v(\PowerSlot)
% 	\leq
% 	\APDDistributionApprox_v(\PowerSlot)	
% 	\leq
% 	(1+\Tolerance) \APDDistribution_v(\PowerSlot)
% \end{equation*}
% %
% (\ie $\APDDistributionApprox_v(\PowerSlot)$ is an \emph{\EDApproximation} of $\APDDistribution_v(\PowerSlot)$, see \cref{def:EDApproximation}).
\end{itemize}











\endinput


\begin{definition}[\Ac{APD} \EDGApproximation]
\label{def:APD:EDGApproximation}
%
Let $\APDDistribution: \APDDistributionDef$ be an \Ac{APD} probability distribution, $\Tolerance, \Confidence \in (0,1)$ and $\DiscretisationStep \in \RealsGZ$.

A \EDGApproximation of $\APDDistribution$ is a function:
\begin{equation*}
	\APDDistributionApprox: \APDDistributionApproxDef
\end{equation*}
%
where $\SetPowerSlots = \SetPowerSlotsDef$ is a partition of the reals (electrical power values) into right-open $\DiscretisationStep$-wide \emph{power slots}.
%
For each $\PowerSlot \in \SetPowerSlots$ the following inequation holds: 
%
\begin{equation*}
	\Probability{
		(1-\Tolerance) \int_{\PowerSlot} \APDDistribution(w) ~\text{d}w
		\leq 
		\APDDistributionApprox(\PowerSlot)
		\leq 
		(1+\Tolerance) \int_{\PowerSlot} \APDDistribution(w) ~\text{d}w
	}
	\geq 1-\Confidence.
\end{equation*}
\end{definition}

\Cref{def:APD:EDGApproximation}


==> 30_approximation/content.tex <==
%!TEX root = ../root.tex
Many applications, as our \Ac{PPSV}, require the computation of the mean value $\mu_Z$ for a 0/1 random variable $Z$. 
%
When, as in our case, an exact computation is infeasible, Monte Carlo methods are often used to compute an approximation of this quantity~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.

The main idea is to consider $N$ \Ac{iid} random variables $Z_1, \ldots, Z_N$ identical to $Z$ (having  mean $\mu_Z$), or, equivalently, $N$ independent realisations (samples) of the random variable $Z$,
and to take $\tilde{\mu}_Z = \frac{(Z_1 + \cdots + Z_N)}{N}$ as an approximation of $\mu_Z$.

In order to have a formally guaranteed upper bound for the error of this approximated computation, we exploit the notion of \emph{\EDApproximation} of the mean value of a random variable (\cref{def:EDApproximation}).

\begin{definition}[\EDApproximation, \cite{dagum-etal:2000:sicomp}]
\label{def:EDApproximation}
Let $\mu_Z$ be the mean value for a 0/1 random variable $Z$ and 
$Z_1, \ldots, Z_N$ be $N$ independent realisations (samples) of $Z$. 
Given $\Tolerance$ (\emph{tolerance}) and $\Confidence$ (\emph{statistical confidence}) in $(0,1)$,
we say that $\tilde{\mu}_Z = \frac{(Z_1 + \cdots + Z_N)}{N}$ is an \EDApproximation of $\mu_Z$ if:
%
$%\begin{equation*}
	\Probability{
		(1-\Tolerance) \mu_Z
		\leq
		\tilde{\mu}_Z
		\leq
		(1+\Tolerance) \mu_Z
	} 
	\geq 1 - \Confidence.%
$%\end{equation*}
\end{definition}



==> 40_computing/content.tex <==
%!TEX root = ../root.tex
The \Ac{PPSV} Monte Carlo--based algorithm computes, for each distinct value $v \in V_\Substation$ of the substation safety threshold in $\SetTimeSlots$ and for each power slot $\PowerSlot \in \SetPowerSlots$, an \EDApproximation $\APDDistributionApprox_v(\PowerSlot)$ of the probability that the \Ac{APD} takes a value within $\PowerSlot$ when the substation safety threshold is $v$.

Given the huge number of samples to be generated and evaluated, a naive implementation of a Monte Carlo algorithm to estimate an \EDApproximation $\APDDistributionApprox_v(\PowerSlot)$ of $\APDDistribution_v(\PowerSlot)$ for each power slot $\PowerSlot \in \SetPowerSlots$ would be infeasible.
%

To this end, for each value $v \in V_\Substation$, our algorithm generates \Ac{iid} random samples of the \Ac{APD}, starting from the \Ac{EPP} and the deviation model of each $\User \in \SetUsers$. 
%
Each generated \Ac{APD} sample $\PowerSlot \in \SetPowerSlots$ is used to define the realisation of a set of $\SetCardinality{\SetPowerSlots}$ 0/1 random variables $\{ Z^i ~|~ i \in \SetPowerSlots\}$, one per power slot, where $Z^\PowerSlot$ is $1$ and all the others are 0. 
%
Given a set of $N$ \Ac{iid} samples $\PowerSlot_1, \ldots \PowerSlot_N$ (in $\SetPowerSlots$)
%(each of them being in $\SetPowerSlots$) 
generated as above, we have that, for each power slot $i \in \SetPowerSlots$, the 0/1 variables $\{Z^{i}_1, \ldots Z^{i}_N\}$ are \Ac{iid}. 
%
This results in our algorithm effectively computing \EDApproximation{s} $\APDDistributionApprox_v(\PowerSlot)$ of $\APDDistribution_v(\PowerSlot)$ for each power slot $\PowerSlot \in \SetPowerSlots$ using a \emph{single} set of samples in $\SetPowerSlots$.


\Ac{PPSV} combines two Statistical Model Checking approaches.
The first approach, based on the algorithm in \cite{dagum-etal:2000:sicomp}, %(also reported in \cite{grosu-etal:2004:isola}), 
restricted to 0/1 random variables, decides when to stop sampling.
%
The second approach, important to guarantee termination on zero/low-probability areas of the computed distribution, relies on Statistical Hypothesis Testing (along the lines of \cite{grosu-etal:2005:tacas,mancini-etal:2014:fmcad,mancini-etal:2015:iwbbio}).


Our method uses the condition in \cite{dagum-etal:2000:sicomp} to decide whether $N_i$ is sufficiently large to guarantee that
% (i.e., at least the value of $N$ in \cref{step:final_N} of \cref{algo:aa}), 
$\frac{1}{N_i}\sum_{j=1}^{N_i} Z^i_j$ is a \EDApproximation $\APDDistributionApprox_v(i)$ of the probability $\APDDistribution_v(i)$ that the \Ac{APD} takes a value within power slot $i$ when the substation %provides power
safety threshold is $v$.
%
At the same time, if after a sufficiently large number of samples $M_i$, 
%= \lceil\ln(\Confidence)/\ln(1-\Tolerance)\rceil$, %see \cref{sec:background:sht}), 
%see \cref{sec:orchestrator}, Phase 1),
$\sum_{j=1}^{M_i} Z^i_j$ is still 0 for some power slot $i$, 
%by Statistical Hypothesis Testing 
the algorithm concludes that, with confidence at least $1-\Confidence$, 
%the probability that the \Ac{APD} takes a value within power slot $i$ when the substation safety threshold is $v$ is less than $\Tolerance$. 
$\APDDistributionApprox_v(i) < \Tolerance$.


==> 40_preliminaries/content.tex <==
%!TEX root = ../root.tex




\endinput


\begin{definition}[Time slot]
\label{def:time-slot}
A time slot is a finite-size right-open interval $\TimeSlot = [a, b)$ of the non-negative real numbers (\ie $a, b \in \RealsGEZ$, $0 \leq a < b$. 
%
The \emph{duration} of $\TimeSlot$ is $|\TimeSlot| = b-a$.
\end{definition}

\begin{definition}[Power profile]
\label{def:power-profile}
Let $\SetTimeSlots$ be a finite set of non-overlapping time slots.
A \emph{power profile} over $\SetTimeSlots$ is a function
$\PowerProfile: \SetTimeSlots \to \Reals$ defining a power value (in kW) for each time slot in $\SetTimeSlots$. 
\end{definition}

\begin{definition}[Power profile probability distribution]
\label{def:power-profile:probability:distribution}
Let $\SetTimeSlots$ be a finite set of non-overlapping time slots and $\PowerProfile$ a power profile over $\SetTimeSlots$ (\cref{def:power-profile}).

The probability distribution associated to $\PowerProfile$ is:
\begin{equation*}
	\Probability{\PowerProfile}: 
		\SetPowerSlots \to [0,1]
\end{equation*}
where $\SetPowerSlots$ is the finite set of all-different values assumed by $\PowerProfile$ in $\SetTimeSlots$ and 
\begin{equation*}
	\Probability{\PowerProfile = w} = 
		\frac{\sum_{t \in \SetTimeSlots \text{~s.t.~} \PowerProfile(t) = w} |t|}
			 {\sum_{t \in \SetTimeSlots}{|t|}}
\end{equation*}
\end{definition}

From \cref{def:power-profile:probability:distribution} it follows that $\sum_{w \in W} \Probability{\PowerProfile = w} = 1$.


==> 50_algo/content.tex <==
%!TEX root = ../root.tex


Our \Ac{PPSV} algorithm has been designed as to be massively parallelised on a \Ac{HPC} infrastructure.

%Thus, if we take $\tilde{N} = \max_{i \in \SetPowerSlots}\max\{M_i, N_i\}$ 
%(see \cref{sec:orchestrator}, Phases 2 and 3), 
%and we maintain separately the counters needed for each power slot $i$, when $\tilde{N}$ samples have been generated, we can compute a \EDApproximation of $\APDDistributionApprox_v$.


To this end, the computation is split in many Workers (\cref{sec:workers}) and one Orchestrator (\cref{sec:orchestrator}).

\SectionInput[sec:workers]{Workers}{workers.tex}

\SectionInput[sec:orchestrator]{Orchestrator}{orchestrator/content.tex}



\SectionInput[sec:correctness]{Algorithm correctness}{correctness.tex}

==> 50_algo/correctness.tex <==
%!TEX root = ../root.tex
The following result holds (proof omitted for lack of space).

\begin{theorem}\label{thm:correctness}
For each $v \in V_\Substation$ and each $\PowerSlot \in \SetPowerSlots$, let $\APDDistributionApprox_v(\PowerSlot)$ be the (unknown) probability that the \Acf{APD} is within power slot $\PowerSlot$ in a time slot extracted from $\SetTimeSlots_v = \{\TimeSlot | \TimeSlot \in \SetTimeSlots, \SubstationProfile(\TimeSlot)=v\}$ uniformly at random, when each user $\User \in \SetUsers$ independently deviates from the predicted collaborative profile $\EPP{\User}$ according to the deviation model $\DeviationModel{\User}$.

Value $\APDDistributionApprox_v(\PowerSlot)$ computed by 
%\cref{algo:orchestrator,algo:processAnswer,algo:generateSamples}
the algorithm above is such that:
%
\begin{enumerate}
\item If $\APDDistributionApprox_v(\PowerSlot) = \bot$, then $\APDDistribution_v(\PowerSlot) < \Tolerance$ with confidence $\geq 1-\Confidence$.
%
\item Otherwise, $\APDDistributionApprox_v(\PowerSlot)$ is a \EDApproximation of $\APDDistribution_v(\PowerSlot)$.
\end{enumerate}
\end{theorem}

==> 50_algo/orchestrator/content.tex <==
% !TEX root =  ../../root.tex

The Orchestrator runs the two Statistical Model Checking algorithms 
by asking workers to generate new samples and by properly aggregating 
the results. 
%
The Orchestrator runs a \emph{round} of the above for each substation power value $v \in V_\Substation$.
%
For each round (\ie for each $v \in V_\Substation$) 
and for each power slot $\PowerSlot \in \SetPowerSlots$, 
the computation state of $\APDDistributionApprox_v(\PowerSlot)$ 
may be in one of two \emph{phases}, which evolve \emph{independently}. 
%as in \cref{fig:evolution}.
%
Also, for each power slot $\PowerSlot \in \SetPowerSlots$, the following \emph{null hypothesis} $\NullHyp{\PowerSlot}$ is formulated: ``$\APDDistribution_v(\PowerSlot) \geq \Tolerance$''.


% \begin{Figure}
%     \IncludeGraphics[width=\linewidth]{fsa.pdf}
%     \caption{Evolution of the computation process of $\APDDistributionApprox_v(\PowerSlot)$ for each power slot $\PowerSlot \in \SetPowerSlots$, given $v \in V_\Substation$.}
%     \DraftWarning{To be redone.}
%     \label{fig:evolution}
% \end{Figure}

\SectionInput*[sec:orchestrator:phase:1]{Phase 1}{phase_1.tex}

\SectionInput*[sec:orchestrator:phase:2]{Phase 2}{phase_2.tex}

%\SectionInput[sec:orchestrator:phase:1]{Phase 3}{phase_3.tex}


The Orchestrator terminates the round for $v \in V_\Substation$ when the computation process of $\APDDistributionApprox_v(\PowerSlot)$ is in state ``Done'' for \emph{all} power slots $\PowerSlot \in \SetPowerSlots$.





\endinput



\begin{algorithm}[t]
%
\AlgoFunction{\AlgoFun{orchestrator}(\AlgoVar{T}, $P_s$, \AlgoVar{userProf}, \AlgoVar{\dist}, $\epsilon$, $\delta$, $\gamma$)}{
	\KwIn{\AlgoVar{T}, a set of contiguous time slots}
	\KwIn{$P_s$, the substation power profile in $T$}
	\KwIn{\AlgoVar{userProf}, a set of predicted collaborative profiles $P_u$ in $T$, one for each user $u \in U$}
	\KwIn{\AlgoVar{\dist}, the user disturbance model}
	\KwIn{($\epsilon, \delta$), error and confidence level}
	\KwIn{$\gamma$, the discretisation step for values of the \Ac{APD}}
	
	\AlgoVarGets{W}{\AlgoFun{admissiblePowerSlots}(\AlgoVar{userProf}, \AlgoVar{\dist}, $\gamma$)}\;	
	\AlgoVarGets{$V_s$}{$\{ \AlgoVar{v} | P_s(\AlgoVar{t}) = \AlgoVar{v}, \AlgoVar{t} \in \AlgoVar{T}\}$}\;
	
	\KwOut{\estPrAPD, a function associating, to each $\AlgoVar{v} \in V_s$, a probability value to each power slot $\AlgoVar{w} \in \AlgoVar{W}$}

	\BlankLine		
	\ForEach{$\AlgoVar{v} \in V_s$}{	
		\tcp{Initialisation}
		\AlgoVarGets{status}{an array associating to each power slot $\AlgoVar{w} \in \AlgoVar{W}$
		a record (\AlgoVar{state}, \AlgoVar{N}, \AlgoVar{succ}, \AlgoVar{alt}, \AlgoVar{cnt})}\;
		
		\ForEach{$\AlgoVar{w} \in \AlgoVar{W}$}{
			\AlgoVarGets{\estPrAPD$_{\AlgoVar{v}}$(\AlgoVar{w})}{\KwNil}\;
			\AlgoVarGets{status[$w$]}{(``Phase 1'', 0, 0, 0, 0)}\;
		}
		\AlgoVarGets{done}{\AlgoVar{false}}\;
		\While{$\lnot \AlgoVar{done}$}{
			\AlgoVarGets{s}{find an idle slave}\;
			\uIf{\AlgoVar{s} has terminated some previous task}{
				\AlgoVarGets{answer}{get result from \AlgoVar{s}}\;
				\AlgoVarGets{done}{\AlgoFun{procAns}(%
					\AlgoVar{answer}, \AlgoVar{status}, $\estPrAPD_\AlgoVar{v}$)}\;
			}
			\uIf{$\lnot \AlgoVar{done}$}{
				\KwSend request \AlgoFun{genSamples}(%
					\AlgoVar{v}, \AlgoVar{\dist}, \AlgoVar{userProf}) 
					to \AlgoVar{s}\;
			}
		}
		\ForEach{slave \AlgoVar{s}}{
			\KwSend Halt command to \AlgoVar{s}\;
			delete any pending incoming answer from \AlgoVar{s}\;
		}	
	} %end for each v
	\Return \estPrAPD\;
} % end function orchestrator()
\caption{The Orchestrator main algorithm \label{algo:orchestrator}}
\end{algorithm}



\begin{algorithm}[t]
\AlgoFunction{\AlgoFun{procAns}(\AlgoVar{answer}, \AlgoVar{status}, $\estPrAPD_v$)}{
	\tcp{$\AlgoVar{answer} = (\AlgoVar{cnt}, \AlgoVar{succ}, \AlgoVar{alt})$}

	\AlgoVarGets{done}{\AlgoVar{true}}\;
	\nllabel{algo:processAnswer:line:aggregation}
	\ForEach{$\AlgoVar{w} \in \AlgoVar{W}$}{	
		\tcp{Update data in \AlgoVar{status[w]}}
		\AlgoVarGets{status[w].cnt}{$\AlgoVar{status[w].cnt} + \AlgoVar{answer.cnt}$}\;
		\AlgoVarGets{status[w].succ}{$\AlgoVar{status[w].succ} + \AlgoVar{answer.succ[w]}$}\;
		\AlgoVarGets{status[w].alt}{$\AlgoVar{status[w].alt} + \AlgoVar{answer.alt[w]}$}\;
	

		\Switch{\AlgoVar{status[w].state}}{	
			\uCase{``Phase 1''}{			
				\uIf{$\AlgoVar{status[w].succ} > \Upsilon_1(\min(1/2, \sqrt{\epsilon}), \delta/3)$}{
					\nllabel{algo:processAnswer:line:Phase1done}
					\AlgoVarGets{$\estPrAPD_\AlgoVar{v}(\AlgoVar{w})$}{%
						$\AlgoVar{state[w].succ} / \AlgoVar{status[w].cnt}$}\;
					\tcp{\Acs{SRA} in Phase 1 done}
					\AlgoVarGets{status[w].N}{%
						$2 \times \Upsilon_2(\epsilon,\delta) ~\times~%$ 
						%$~~~~~~~~~~~
						\epsilon / \estPrAPD_\AlgoVar{v}(\AlgoVar{w})$}\;
					\AlgoVarGets{status[w].(succ,cnt,alt)}{(0,0,0)}\;
					\AlgoVarGets{status[w].status}{``Phase 2''}\;					
				}
				\lElse{%
					\uIf{$\AlgoVar{status[w].succ} = 0$ and
						$\AlgoVar{status[w].cnt} > M$}{
							\nllabel{algo:processAnswer:line:H0rejected}
							\AlgoVarGets{$\estPrAPD_\AlgoVar{v}(\AlgoVar{w})$}{%
									$\perp$} \tcp*{$H_0(w)$ rejected}
							\AlgoVarGets{status[w].status}{``Done''}
				}}
				\KwBreak
			}			
			\uCase{``Phase 2''}{
				\uIf{$\AlgoVar{status[w].cnt} > \AlgoVar{status[w].N}$}{
					\nllabel{algo:processAnswer:line:Phase2done}
					\tcp{Phase 2 done}					
					%\AlgoVarGets{S}{$\AlgoVar{status[w].alt}/2$}\;
					\mbox{\AlgoVarGets{$\hat{\rho}$}{%
							$\max \left(%
								\frac{\AlgoVar{status[w].alt}}{  
								\AlgoVar{status[w].cnt}}, 
								\epsilon \times \estPrAPD_\AlgoVar{v}(\AlgoVar{w}) \right)$}%
					}\;
	
					\AlgoVarGets{status[w].N}{
						$\Upsilon_2(\epsilon,\delta) ~\times~%$
						%$~~~~~~~~~~~
						\hat{\rho} /
							[\estPrAPD_\AlgoVar{v}(\AlgoVar{w})]^2%
						$}\;
					\AlgoVarGets{status[w].(succ,cnt,alt)}{(0,0,0)}\;
					\AlgoVarGets{status[w].state}{``Phase 3''}\;
				}
				\KwBreak
			}	
			\uCase{``Phase 3''}{
				\uIf{$\AlgoVar{status[w].cnt} > \AlgoVar{status[w].N}$}{
					\tcp{Phase 3 done}
					\nllabel{algo:processAnswer:line:Phase3done}
					\AlgoVarGets{%
						$\estPrAPD_\AlgoVar{v}(\AlgoVar{w})$}{%
							$\AlgoVar{status[w].succ} / \AlgoVar{status[w].cnt}$}\;
					\AlgoVarGets{status[w].lastStep}{``Done''}\;
				}
				\KwBreak
			}		
		}
		\lIf {$\AlgoVar{status[w]} \neq \AlgoVar{``Done''}$}{
			\AlgoVarGets{done}{\AlgoVar{false}}
		}
	} %end foreach w	
	\Return \AlgoVar{done}\;
}

\caption{Function \AlgoFun{procAns}() on the Orchestrator side\label{algo:processAnswer}}
\end{algorithm}




==> 50_algo/orchestrator/phase_1.tex <==
%!TEX root = ../../root.tex

%A minimum number $N_1$ of 0/1 samples $Z_1^\PowerSlot, \ldots, Z_{N_1}^\PowerSlot$ is generated for $\PowerSlot$ (starting from $N_1$ samples over $\SetPowerSlots$ as described earlier) until one of two conditions arises:

0/1 samples are generated for $\PowerSlot$ (starting from the samples over $\SetPowerSlots$ as described earlier) until one of two conditions arises:

\begin{enumerate}[(a)]
\item 
\label[case]{item:algo:phase:1:sra}
$\Upsilon_1$ samples are 1 (where $\Upsilon_1$ is a function of $\Tolerance$ and $\Confidence$ as defined in \cite{dagum-etal:2000:sicomp}).
% 1 + 
% 	\frac{(1+\tilde{\Tolerance})
% 		  (4(e-2) \ln(2/\tilde{\Confidence})}
% 		 {\tilde{\Tolerance}^2)}$ of the generated samples belongs to power slot $\PowerSlot$, 
% with $\tilde{\Tolerance} = \min(\frac{1}{2}, \sqrt{\Tolerance})$ and $\tilde{\Confidence} = \frac{\Confidence}{3}$.

\item 
\label[case]{item:algo:phase:1:rejection}
The first $\lceil\ln(\Confidence)/\ln(1-\Tolerance)\rceil$ samples are all 0. 
\end{enumerate}

Let $N_{1}^{\PowerSlot}$ be the number of samples generated for $\PowerSlot$.
In \cref{item:algo:phase:1:sra}, a first estimation of $\APDDistribution_v(\PowerSlot)$ is computed as ratio $\frac{\Upsilon_1}{N_{1}^{\PowerSlot}}$, and the computation proceeds with ``Phase 2''.

In \cref{item:algo:phase:1:rejection}, the null hypothesis $\NullHyp{\PowerSlot}$ is \emph{rejected}, thus declaring that $\APDDistribution_v(\PowerSlot) < \Tolerance$.
%
This Statistical Hypothesis Rejection procedure is known to be a one-sided error decision algorithm, as it may introduce a \emph{type-I error} (\ie the algorithm might reject $\NullHyp{\PowerSlot}$ when it actually holds).
%
However, from \cite{grosu-etal:2005:tacas} it follows that the probability of such an error, %is at most $\Confidence$.
%Formally: 
$\Probability{Z_1^\PowerSlot = \cdots Z_{N_1}^\PowerSlot = 0 ~|~  \NullHyp{\PowerSlot}}  < \Confidence$.
%
This equivalently tells us that $\NullHyp{\PowerSlot}$ is rejected with confidence at least $1-\Confidence$. In \cref{item:algo:phase:1:rejection} value for $\APDDistributionApprox_v(\PowerSlot)$ is set to special value $\bot$ and the computation for power slot $\PowerSlot$ moves to state ``Done''.





==> 50_algo/orchestrator/phase_2.tex <==
%!TEX root = ../../root.tex

For any power slot $\PowerSlot$ for which the computation state of $\APDDistributionApprox_v(\PowerSlot)$ is ``Phase 2'', the Orchestrator waits until a number of samples greater than $N_{2}^{\PowerSlot}$ is collected. 
%
Value for $N_{2}^{\PowerSlot}$ is computed during ``Phase~1'', and depends on the first estimate of $\APDDistributionApprox_v(\PowerSlot)$ computed therein.
%
Value for $N_{2}^{\PowerSlot}$ is needed in Phase~2 to compute the number of \emph{additional} samples $N_{3}^{\PowerSlot}$ that must be generated to compute the final \EDApproximation of $\APDDistributionApprox_v(\PowerSlot)$.
%
When such additional $N_{3}^{\PowerSlot}$ 0/1 samples $\{Z_1^\PowerSlot, \ldots, Z_{N_{3}^{\PowerSlot}}^\PowerSlot\}$ are generated by the workers, the final $\APDDistributionApprox_v(\PowerSlot)$ is set to $\frac{1}{N_{3}^{\PowerSlot}} \sum_{i=1}^{N_{3}^{\PowerSlot}} Z_i^\PowerSlot$ and the computation for $\PowerSlot$ is set to state ``Done''.

\endinput


achieve the required precision given $\Tolerance$ and $\Confidence$. %(\ie the number required to reach $\tilde{N}$) 
is computed and the computation state for $\APDDistributionApprox_v(\PowerSlot)$ is set to ``Phase~3''.
%At this point, value $\hat{\rho}$ for power slot $w$ is computed following \Ac{AA}, counters in \AlgoVar{status[w]} are reset, and \AlgoVar{status[w].state} is set to ``Phase 3''.

==> 50_algo/orchestrator/phase_3.tex <==
%!TEX root = ../../root.tex
For any power slot $w$ for which the computation state of $\estPrAPD_v(w)$ is ``Phase 3'', the Orchestrator waits until additional samples (as computed at the end of ``Phase~2'') are generated and returned by the slaves. 
At this point, the final value for $\estPrAPD_v(w)$ is computed
as the number of generated samples within power slot $w$ divided by the number of generated samples
 % (see \cref{algo:processAnswer}, \cref{algo:processAnswer:line:Phase3done}) and \AlgoVar{status[w].state} 
and computation state of $\estPrAPD_v(w)$ is set to ``Done''.


==> 50_algo/workers.tex <==
% !TEX root =  ../root.tex

Each worker runs in parallel upon requests from the Orchestrator. 
To reduce the overhead due to network communication, each invocation to a worker triggers the generation of a high number $\NbSamplesPerCall$ 
of samples.
Each sample of the \Ac{APD} (when the substation %provides power
safety threshold is $v$) is generated %by function \AlgoFun{rndPowerSlot()} of \cref{step:rndpowerslot} of \cref{algo:generateSamples} 
as follows:
%
\begin{enumerate}
\item A time slot $\TimeSlot \in \SetTimeSlots_v = \{\TimeSlot | \TimeSlot \in \SetTimeSlots, \SubstationProfile(\TimeSlot) = v\}$ is extracted uniformly at random (as time slots have equal duration).
%
\item For each user $\User \in \SetUsers$, a deviation $\Deviation_\User \in \DomainDeviations{\User}$ is extracted according to the deviation model of $\User$ (\ie using probability density function $\DeviationModel{\User}$).
%
\item The \Ac{APD} value in time-slot $\TimeSlot$ resulting from the extracted user deviations is computed as $A = \sum_{\User \in \SetUsers} (1 + \Deviation_\User) \EPP{\User}(\TimeSlot)$ and associated to its power slot $\PowerSlot = [a, a+\DiscretisationStep) \in \SetPowerSlots$ (\ie $\PowerSlot$ is such that $a \leq A < a + \DiscretisationStep$).
\end{enumerate}

%Upon termination, a record is returned to the Orchestrator, with values for the number of samples generated (field \AlgoVar{cnt}, which will be exactly $k$) and, for each power slot $i \in W$, the number of samples within power slot $i$ (the $i$-th component $\AlgoVar{succ}[i]$ of the array field $\AlgoVar{succ}$, whose name stands for ``successes''), and the number of odd/even consecutive samples such that exactly one is within power slot $i$ (the $i$-th component $\AlgoVar{alt}[i]$ of array field $\AlgoVar{alt}$).

At the end of each sampling task, the $\NbSamplesPerCall$ generated samples (power slots) are sent back to the Orchestrator.


\endinput






\begin{algorithm}[t]
\AlgoFunction{\AlgoFun{genSamples}(\AlgoVar{v}, \AlgoVar{\dist}, \AlgoVar{userProfiles})}{

	\KwOut{$\AlgoVar{answer} = (\AlgoVar{cnt}, \AlgoVar{succ}, \AlgoVar{alt})$, where 
		\AlgoVar{cnt} is the number of samples generated,
		\AlgoVar{succ} and \AlgoVar{alt} are arrays associating, 
			to each $\AlgoVar{w} \in \AlgoVar{W}$,
			the number of generated samples within \AlgoVar{w} and the number of 
			pairs of consecutive odd/even samples s.t.\ exactly one of them is within \AlgoVar{w}
	}

	
	\KwParam{\AlgoVar{k}, number of samples to be generated as a single 
		computation bunch, $>0$ and even}\;

	\BlankLine	
	\AlgoVarGets{w\_lastOddSample}{\KwNil};
	\AlgoVarGets{answer.cnt}{0}\;
	\ForEach{$\AlgoVar{w} \in \AlgoVar{W}$}{
		\AlgoVarGets{answer.succ[w]}{0};
		\AlgoVarGets{answer.alt[w]}{0}\;
	}
	\ForEach{$\AlgoVar{j} \in 1..\AlgoVar{k}$}{
		\AlgoVarGets{w}{\AlgoFun{rndPowerSlot}(\AlgoVar{v}, \AlgoVar{W},
			\AlgoVar{\dist}, \AlgoVar{userProf})}\;\nllabel{step:rndpowerslot}
		\AlgoIncrVar{answer.cnt};
		\AlgoIncrVar{answer.succ[w]}\;
		\lIf{ \AlgoVar{j} is odd }{
			\AlgoVarGets{w\_lastOddSample}{\AlgoVar{w}}\;
		}
		\lElse{
			\If{$\AlgoVar{w} \neq \AlgoVar{w\_lastOddSample}$}{
				\AlgoIncrVar{answer.alt[w\_lastOddSample]}\;
				\AlgoIncrVar{answer.alt[w]}			
			}
		}
	}
	\Return \AlgoVar{answer}\;
}
\caption{Function \AlgoFun{genSamples}() on the worker side\label{algo:generateSamples}}
\end{algorithm}





==> 60_expres/content.tex <==
% !TEX root =  ../root.tex

In this section we present experiments aiming at
evaluating %the effectiveness of 
our C implementation of \Ac{PPSV} in computing an \EDApproximation of \Ac{APD} probability values and the computational scalability of our parallel algorithm.

%We developed our system in the C programming language.
% using an implementation of the \Acf{MPI} (see, e.g., \cite{snir-etal:1998:mpi}) to enable the communication between the Orchestrator and a battery of slave processes spread on multiple machines connected by a network. 
 
\SectionInput[sec:expres:data]{Case study}{data.tex}

\SectionInput[sec:expres:settings]{Experimental setting}{setting.tex}

\SectionInput[sec:expres:results]{Computation of \Ac{APD} probability distributions}{results.tex}


\SectionInput[sec:expres:scalability]{Scalability analysis}{scalability/content.tex}






==> 60_expres/data.tex <==
% !TEX root =  ../root.tex

For our case study, we used real electricity usage data from 130 residential households (set $\SetUsers$) connected to a substation of a medium voltage distribution network in Denmark (data courtesy of SEAS-NVE). 
\Acp{EPP} for all users are %over 24 hours,
defined with a granularity of 60 minutes.
%
The (constant) safety threshold for \Ac{APD} is 400 kW,
as this is the substation nominal power.
%% The substation nominal power is 400 kW, which %we used as
%% is our (constant) safety threshold for \Ac{APD}.

We adopted the same deviation model for all users $\User \in \SetUsers$, which defines the range of possible deviations as $\DomainDeviations{\User} = [-0.4, 0.4]$ and density function $\DeviationModel{\User}$ defined as: 
$	\DeviationModel{\User}(x) =
		0.4 \DiracDeltaFunction(x)	+
		0.2 \DiracDeltaFunction(x - 0.2) +
		0.2 \DiracDeltaFunction(x + 0.2) +
		0.1 \DiracDeltaFunction(x - 0.4) +
		0.1 \DiracDeltaFunction(x + 0.4)
$
(where $\DiracDeltaFunction(x)$ is the Dirac delta function). That is, users can deviate from their \Acp{EPP} with non-zero probability in 5 possible ways, although very generously (as the largest possible deviations are as large as $\pm 40\%$ and occur with probability as high as $10\%$). 
Using a finite number of user deviations was dictated by the structure of our data and specifications from the \Ac{DSO}. However, we stress that such a choice has no impact on the performance of our tool, which uses standard libraries for the efficient sampling from continuous distributions.


%% Using a finite number of user deviations (instead of a continuous density function) was dictated by the structure of our data. However, we stress that such a choice has no impact on the computational complexity of the algorithm.



==> 60_expres/results.tex <==
% !TEX root =  ../root.tex


In order to assess effectiveness of our parallel algorithm to compute \EDApproximation{s} of the \Ac{APD} probability distribution values, we considered a very challenging scenario from our case study.

In particular, using data from all the 130 users in our dataset, we computed \EDApproximation{s} of the \Ac{APD} probability distribution values for each month of the year (time slot duration: 1 day). 
%This means that, each experiment (referring to one of the 12 months) envisions 30 or 31 time slots. 
As each of the 130 users can independently deviate from their \Acp{EPP} by 5 possible factors for each time slot, the overall allowed number of combinations of user deviations is approximately $5^{30 \times 130}$. This makes an exhaustive exploration of the space of user deviations (hence an exact computation of the \Ac{APD} distribution) clearly impossible.
%
%To further stress our algorithm, w
We set $\Tolerance$, $\Confidence$ and $\DiscretisationStep$ to small values, namely $\Tolerance = \Confidence = 5\%$ ($5 \times 10^{-2}$), $\DiscretisationStep = 20$~kW (\ie 5\% of the substation nominal power).
% era: 10^3 e 10 kW
Finally, to reduce network overhead, we set each worker as to generate $\NbSamplesPerCall = \NbSamplesPerCallDef$ samples per single Orchestrator request.


\Cref{fig:apd} shows the \Ac{APD} probability distribution computed by our algorithm for each month under these settings.
%
Each of the 12 computations took %\MathSecondsToHMS{243562} (h:m:s) 
between 
	\Pretty[unit={seconds}]{4782} 
	and 
	\Pretty[unit={seconds}]{6448} 
	(average: \Pretty[unit={seconds}]{5297}, \ie \Pretty[style=timeprose]{5297}) 
using \DataGet<exps>{workers/number} workers, and involved the generation of a number of samples ranging from 
	$\approx 1.6 \times 10^{9}$ 
	to 
	$\approx 2.2 \times 10^{9}$ 
	(average: $\approx 1.8 \times 10^{9}$ samples).

With current \Ac{IaaS} pricing schemes, the cost for such a computation would be of around \Pretty[style=eur]{2.80}, \ie as small as \Pretty[style=eur]{0.02} per user per day.%
	\footnote{%
		\label{footnote:iaas}%
		June 2018 prices for 80 Google g1-small nodes for 90 minutes, see \url{https://cloud.google.com/products/calculator}}
%(\eg 1000 Google n1-standard-1 nodes would cost just $\approx 800$ USD/day

\begin{Figure}[position=H]
	\IncludeGraphics[width=0.8\linewidth]{figures/12-months/dataTSind-12-G20.pdf}
	\caption{Monthly \Ac{APD} (in kW) probability distributions, as computed by our algorithm ($\Tolerance = \Confidence = 5\%$, $\DiscretisationStep = 20$~kW) on our case study scenarios.}
	\label{fig:apd}
\end{Figure}


\Comment{
	epsilon=delta=10^-3, gamma=10, k=80:
		- 3 days 
		$\approx 6.5 \times 10^{9}$ to $\approx 2.5 \times 10^{10}$ (average: $\approx 1.5 \times 10^{10}$ samples).

	epsilon=delta=5\%, gamma=40, k=80:
		between \Pretty[unit={seconds}]{98} and \Pretty[unit={seconds}]{201} (average: \Pretty[style=timeprose]{144}) 
	(using \DataGet<exps>{workers/number} workers) and involved the generation of a number of samples ranging from 
	$\approx 1.4 \times 10^{6}$ to $\approx 2.8 \times 10^{7}$ (average: $\approx 2 \times 10^{7}$ samples).


	epsilon=delta=5\%, gamma=20, k=80:
		between \Pretty[unit={seconds}]{...} and \Pretty[unit={seconds}]{...} (average: \Pretty[style=timeprose]{...}) 
	(using \DataGet<exps>{workers/number} workers) and involved the generation of a number of samples ranging from 
	$\approx XX \times 10^{XX}$ to $\approx XX \times 10^{XX}$ (average: $\approx XX \times 10^{XX}$ samples).
}






\endinput






%\endinput

\Cref{fig:distribution} shows the probability distribution of the \Ac{APD} computed using all the available cores (Orchestrator plus 80 slave processes) with $\epsilon = \delta = 10^{-3}$. 

\begin{Figure}
%	\IncludeGraphics[width=0.75\linewidth]{figures/distributionFeb2013.pdf}
	\IncludeGraphics[width=0.85\linewidth]{figures/dataTSind-2-2013.pdf}
	\caption{Probability distribution of the \Ac{APD}, as computed by our algorithm ($\epsilon = \delta = 10^{-3}$) on our case study scenario.}
	\label{fig:distribution}
\end{Figure}


In order to evaluate how our algorithm behaves when varying the number of parallel slaves (hence, cores) used, we ran additional (shorter) experiments, by setting $\epsilon = \delta = 10^{-1}$.
Results are in \cref{tab:results}.
%Each run of the algorithm generated about $1.5 \times 10^8$ samples. %149,720,000.

To perform a fair evaluation of our algorithm using different numbers of slaves, we have to deal with the fact that, since each slave uses its \emph{own independent} pseudo-random number generator, it is not possible to repeat the \emph{same} computation process (i.e., to generate the same sequence of random samples of the \Ac{APD}) when varying the number of slaves (even starting from the same random seed).

%To perform a fair evaluation of our algorithm using different numbers of slaves, we have to deal with two issues:
%%
%\begin{enumerate}
%\item our cluster machines have different characteristics (see \cref{tab:machines});
%%
%\item since each slave uses its \emph{own independent} pseudo-random number generator, it is not possible to repeat the \emph{same} computation process (i.e., to generate the same sequence of random samples of the \Ac{APD}) when varying the number of slaves (even starting from the same random seed). 
%\end{enumerate}

%Our methodology is thus as follows. For each run of the algorithm using $k$ slaves (hence $k$ computational cores):
%
%\begin{enumerate}
%\item we used the \emph{same} proportion of cores of (machines in) each category A, B, and C, i.e., 7.5\% of cores of category A, 17.5\% of cores of category B, and 75\% of cores of category C 
%(see columns ``\emph{\# slaves per machine category}'' in \cref{tab:results});
%
%\item we computed the \emph{speedup} as $s_k/s_1$, with $s_k$ and $s_1$ being the number of \emph{samples per second} received and aggregated by the Orchestrator when using, respectively, $k$ and $1$ slave processes. In other words, we used a definition of the speedup in terms of \emph{throughput} (work units completed per unit of time) \cite{baer:2009:microprocessor} rather than in terms of execution time (as this more common definition is not applicable in our context).
%\end{enumerate}

Our methodology is thus as follows. For each run of the algorithm using $k$ slaves (hence $k$ computational cores)
we computed the \emph{speedup} as $s_k/s_1$, with $s_k$ and $s_1$ being the number of \emph{samples per second} received and aggregated by the Orchestrator when using, respectively, $k$ and $1$ slave processes. In other words, we used a definition of the speedup in terms of \emph{throughput} (work units completed per unit of time) \cite{baer:2009:microprocessor} rather than in terms of execution time (as this more common definition is not applicable in our context).

We computed the number of samples per second in the one-core scenario (\emph{sequential algorithm}, our reference value when computing the speedups) to be $s_1 = 960.547$.

\Comment{
The computation of the number $s_1$ of samples per second in the one-core scenario (\emph{sequential algorithm}, our reference value when computing the speedups) also needs some comments.
In fact, given the heterogeneity of our cluster machines, the number of samples per second generated by the sequential algorithm varies depending on whether the (single) slave resides on a core of a machine of category A, B, or C. 
%\cref{tab:sequential} reports such values, to which we refer as $s_1^A, s_1^B, s_1^C$.
Such values are as follows: $s_1^A = 1122.153$, $s_1^B = 1040.217$, $s_1^C = 925.796$ samples/sec for a core in a machine of category, respectively, A, B, and C.
%
We computed an unbiased value for $s_1$ by averaging $s_1^A, s_1^B, s_1^C$, using, as weights, the ratio of cores of each machine category available to slave processes, i.e.: $s_1 = 7.5\% s_1^A + 17.5\% s_1^B + 75\% s_1^C = 960.547$. We then used this value for $s_1$ in speedup computation (\cref{tab:results}).
}

Finally, from each value of the speedup computed as above, we computed the \emph{efficiency} as typically done in the evaluation of parallel algorithms, by dividing the speedup by the number $k$ of the parallel slaves used (see column ``\emph{efficiency}'' in \cref{tab:results}).



\begin{table}
\newcommand{\thisTableSequential}{960.547} 
\gdef\thisTableRow#1#2{%
	% #1: nb slaves
	% #2 execution time
\xdef\thisTableNbSlaves{#1}% 
\xdef\thisTableExectime{#2}%
\FPeval\thisTableSpeedup{round(thisTableExectime/thisTableSequential:2)}%
\xdef\thisTableSpeedup{\thisTableSpeedup}%
\FPeval\thisTableEfficiency{round((thisTableSpeedup*100/thisTableNbSlaves):2)}%
\xdef\thisTableEfficiency{\thisTableEfficiency}%
%
\centering\thisTableNbSlaves
	&  \thisTableExectime
	&   \thisTableSpeedup$\times$ 
	&  \thisTableEfficiency\%
}


\begin{minipage}{\linewidth}
\begin{center}
{ \addtolength{\tabcolsep}{-4pt}
\begin{tabular}{c|ccc}
\toprule
	\textbf{\# slaves} &
	\textbf{samples/sec} & 
	\textbf{speedup} &
	\textbf{efficiency}
\\
\midrule
\centering 1 
	& \emph{\thisTableSequential}
	& 1$\times$ & 100\%
\\
\thisTableRow{20}{12852.984} \\
\thisTableRow{40}{26355.499} \\
\thisTableRow{60}{41788.824} \\
\thisTableRow{80}{54446.999} \\
\bottomrule
\end{tabular}

}
\end{center} 
\end{minipage}
\caption{Samples per second received by the Orchestrator when using different numbers of slaves.\label{tab:results}}
\end{table}



\Comment{
\begin{table}
\newcommand{\thisTableSequential}{960.547} 
\gdef\thisTableRow#1#2#3#4#5{%
	% #1: nb slaves
	% #2, #3, #4: slaves alloc
	% #5 execution time
\xdef\thisTableNbSlaves{#1}% 
\xdef\thisTableExectime{#5}%
\FPeval\thisTableSpeedup{round(thisTableExectime/thisTableSequential:2)}%
\xdef\thisTableSpeedup{\thisTableSpeedup}%
\FPeval\thisTableEfficiency{round((thisTableSpeedup*100/thisTableNbSlaves):2)}%
\xdef\thisTableEfficiency{\thisTableEfficiency}%
%
\centering\thisTableNbSlaves &   \centering#2 & \centering#3 & \centering#4 
	&  \thisTableExectime
	&   \thisTableSpeedup$\times$ 
	&  \thisTableEfficiency\%
}


\begin{minipage}{\linewidth}
\begin{center}
{ \addtolength{\tabcolsep}{-4pt}
\begin{tabular}{c|p{3em}p{3em}p{3em}ccc}
\toprule
	& 
	\multicolumn{3}{p{10em}}{\centering \textbf{\# slaves per mach. cat.}} &
	&
	&	
\\ \cmidrule{2-4}
	\textbf{\# slaves} &
	\centering \textbf{A} & 
	\centering \textbf{B} & 
	\centering \textbf{C} & 
	\textbf{samples/sec} & 
	\textbf{speedup} &
	\textbf{efficiency}
\\
\midrule
\centering 1 & \centering -- & \centering -- & \centering --    
	& \emph{\thisTableSequential} %$^{\text{(*)}}$
	& 1$\times$ & 100\%
\\
\thisTableRow{20}{1}{4}{15}{12852.984} \\
\thisTableRow{40}{3}{7}{30}{26355.499} \\
\thisTableRow{60}{4}{11}{45}{41788.824} \\
\thisTableRow{80}{6}{14}{60}{54446.999} \\
\bottomrule
\end{tabular}

%\scriptsize{(*) Weighted average of data from \cref{tab:sequential}}
}
\end{center} 
\end{minipage}
\caption{Samples per second received by the Orchestrator when using different numbers of slaves.\label{tab:results}}
\end{table}
}

\Comment{%%%%%%%%%%%%%%%%%%
\begin{table}[tp]
\begin{center}
\begin{tabular}{Hcc}
\toprule
	&
	\textbf{machine } &
	\textbf{samples/sec}
	\\
	\textbf{value id} & 
	\textbf{category} &
	\textbf{(one slave)}
	\\
\midrule 
	$s_1^A$ & A & 1122.153
	\\
	$s_1^B$ & B & 1040.217
	\\
	$s_1^C$ & C & 925.796
	\\	
\bottomrule	
\end{tabular}
\caption{Sequential algorithm: number of samples per second received by the Orchestrator when using a single slave allocated to a core of each machine category\label{tab:sequential}}
\end{center}
\end{table}
}%%%%%%%%%%%%%%%%%%%%%%%%%


\Comment{ %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\subfloat[][Speedup]{
	\framebox{\begin{minipage}{4cm}\hspace{4cm}\vspace{15ex}\end{minipage}}
	\label{fig:speedup}
}
%
\subfloat[][Efficiency]{
	\framebox{\begin{minipage}{4cm}\hspace{4cm}\vspace{15ex}\end{minipage}}
	\label{fig:efficiency}
}
\end{center}
\end{figure}


\Cref{fig:speedup,fig:efficiency} graphically plot the speedup and the efficiency achieved by our algorithm, as a function of the number of parallel \Ac{BA} verifiers used in our experiments.
} %%%%%%%%%%%%


From \cref{tab:results} we can see that our distributed multi-core implementation of our algorithm
scales well with the number of used parallel slaves instances. 
The observed efficiency reduction (around 30\%) is typical in a cluster environment, being mostly due to network delays.
%
RAM requirements are negligible.


==> 60_expres/scalability/content.tex <==
%!TEX root = ../../root.tex
In order to evaluate the scalability of our parallel algorithm, we ran additional experiments %, by setting $\epsilon = \delta = 10^{-1}$ 
by varying $\NbWorkers$, the number of used parallel workers/computational nodes ($\NbWorkers \in \{1,20,40,60,80\}$), and measuring the number of samples per second generated (and processed by the Orchestrator) in each configuration. 
%to be $s_1 = 960.547$.
%
%Then, for different values of $\NbWorkers$ (number of parallel workers, \ie computational nodes), we 
For each value of $\NbWorkers$, we computed the \emph{speedup} and \emph{efficiency} of our parallel algorithm as $\frac{s_\NbWorkers}{s_1}$ and $\frac{s_\NbWorkers}{s_1 \times \NbWorkers}$ \respectively, where $s_\NbWorkers$ and $s_1$ are the number of \emph{samples per second} received and aggregated by the Orchestrator when using, respectively, $\NbWorkers$ and $1$ workers (see, \eg \cite{baer:2009:microprocessor}).  
%
%In other words, we used a definition of the speedup in terms of \emph{throughput} (work units completed per unit of time) \cite{baer:2009:microprocessor} rather than in terms of execution time (as this more common definition is not applicable in our context).

\Cref{tab:scalability} shows that our parallel algorithm scales very well with the number of workers (computational nodes), with 
% the good scalability capabilities of our algorithm,
%Thanks to the fact that worker-orchestrator communication occurs rarely (only every $\NbSamplesPerCall = \NbSamplesPerCallDef$ samples in our setting), 
efficiency values stabilising at around $70\%$, 
%when the number of workers is $\geq 40$. %Using larger values for $\NbSamplesPerCall$ would further increase efficiency.
%Such values are standard in \Ac{HPC} applications.
a typical value in cluster environments.




%We used such knowledge about the scalability of our parallel approach to perform a \emph{dimensioning assessment} of the \Ac{HPC} infrastructure needed to run \Ac{PPSV} in a \emph{production scenario}, where, as anticipated in \cref{sec:introduction}, in order to exploit the opportunities of the day-ahead market, \Acp{DSO} would be interested in estimating the \Ac{APD} probability distribution (and the values for the associated defined \Acp*{KPI}) for the next day, and hence with a computation of a few hours.

%\Cref{fig:completion-time} shows the \emph{expected completion time} for \Ac{PPSV} as a function of the number $\NbWorkers$ of parallel workers. 
%The estimations have been performed by considering an efficiency of the algorithm of 70\% (as assessed above) and an expected number of samples to be generated equal to $1.4 \times 10^{10}$ (the value for our experiments in \cref{sec:expres:results} closest to the average number of samples, corresponding to February). Again, $\Tolerance = \Confidence = 10^{-3}$. 
%
%The figure shows that around 600 workers (computational nodes) are sufficient to keep the overall expected computation time under 10 hours, and 1000 workers would keep it under just \emph{5 hours}. It is worth noting that such numbers of computational nodes are to date very affordable under current Infrastructure as a Service pricing schemes. 
%(\eg 1000 Google n1-standard-1 nodes would cost just $\approx 800$ USD/day, while ).
%(\eg 1000 Google g1-small machines would cost just $\approx 450$ USD/day).
%(\eg 1000 Google f1-micro machines would cost around \Pretty[style=eur0]{110} per day, \ie less than \Pretty[style=eur0]{1} per user per day).
%(\eg 1000 Google g1-small machines would cost around \Pretty[style=eur0]{115} for a 5-hour computation.
%, \ie less than \Pretty[style=eur]{0.60} per user per day).

%Also, by lowering accuracy requirements (\ie by increasing $\Tolerance$ and $\Confidence$ which we set to very low values), and by increasing the power values discretisation step (now set to a value as tiny as $\DiscretisationStep = 10$~kW), computation time can be substantially reduced.
%

The short computation time needed by \Ac{PPSV} clearly enables its \emph{online} usage, in order to compute the \Ac{KPI} values for \emph{multiple} candidate price policies, 
% Toni: removed, to be introduced in the journal version
%and to assist the \Ac{DSO} in designing \emph{Pareto-optimal} price policies.
%
hence assisting the \Ac{DSO} in price policy \emph{design}.
%
To this end, it is worth noting that the stable efficiency of our parallel algorithm (as shown in \cref{tab:scalability}) allows \Acp{DSO} to compress computation times by increasing the number of computational nodes used (with no substantial additional \Ac*{IaaS}[,] cost). For example, using 501 computational cores (\ie 1 Orchestrator and 500 Workers) and assuming an efficiency of 70\%, the expected computation time would have been of just 15 minutes (for an \Ac{IaaS} cost of around \Pretty[style=eur]{2.90} per day, \ie \Pretty[style=eur]{0.02} per user per day, see \cref{footnote:iaas}).

% 200 worker --> 36 min
% 500 worker --> 868 sec
	
% Toni: Removed in final version, both to save space and to keep it for the journal version (where we can even define power slots of different widths)
%Finally, our system can be configured as to take as input a \emph{set} of $(\Tolerance, \Confidence)$ pairs and to proceed at computing multiple \EDApproximation{s} of \Ac{APD} probability distribution values (one set of values for each $(\Tolerance, \Confidence)$ pair) \emph{simultaneously}, by using the \emph{same} sequence of generated samples, with \emph{no} additional computational cost. Hence, the computation can be stopped as soon as, for each power slot of the \Ac{APD} probability distribution, a satisfactory \EDApproximation (with varying values for $\Tolerance$ and $\Confidence$) is computed. All this makes \Ac{PPSV} an extremely versatile service.




\begin{Table}[position=H]
	\Input{efficiency-table.tex}

	\caption{\Ac{PPSV} parallel algorithm scalability.}
	\label{tab:scalability}
\end{Table}	



\endinput


Results are in \cref{tab:results}.
%Each run of the algorithm generated about $1.5 \times 10^8$ samples. %149,720,000.

To perform a fair evaluation of our algorithm using different numbers of slaves, we have to deal with the fact that, since each slave uses its \emph{own independent} pseudo-random number generator, it is not possible to repeat the \emph{same} computation process (i.e., to generate the same sequence of random samples of the \Ac{APD}) when varying the number of slaves (even starting from the same random seed).

%To perform a fair evaluation of our algorithm using different numbers of slaves, we have to deal with two issues:
%%
%\begin{enumerate}
%\item our cluster machines have different characteristics (see \cref{tab:machines});
%%
%\item since each slave uses its \emph{own independent} pseudo-random number generator, it is not possible to repeat the \emph{same} computation process (i.e., to generate the same sequence of random samples of the \Ac{APD}) when varying the number of slaves (even starting from the same random seed). 
%\end{enumerate}

%Our methodology is thus as follows. For each run of the algorithm using $k$ slaves (hence $k$ computational cores):
%
%\begin{enumerate}
%\item we used the \emph{same} proportion of cores of (machines in) each category A, B, and C, i.e., 7.5\% of cores of category A, 17.5\% of cores of category B, and 75\% of cores of category C 
%(see columns ``\emph{\# slaves per machine category}'' in \cref{tab:results});
%
%\item we computed the \emph{speedup} as $s_k/s_1$, with $s_k$ and $s_1$ being the number of \emph{samples per second} received and aggregated by the Orchestrator when using, respectively, $k$ and $1$ slave processes. In other words, we used a definition of the speedup in terms of \emph{throughput} (work units completed per unit of time) \cite{baer:2009:microprocessor} rather than in terms of execution time (as this more common definition is not applicable in our context).
%\end{enumerate}

Our methodology is thus as follows. 


==> 60_expres/scalability/efficiency-table.tex <==
%!TEX root = ../../root.tex
%\begin{table}
\newcommand{\thisTableSequential}{5924.89}%{960.547}% 
\gdef\thisTableRow#1#2{%
	% #1: nb slaves
	% #2 execution time
	\xdef\thisTableNbSlaves{#1}% 
	\xdef\thisTableExectime{#2}%
	\FPeval\thisTableSpeedup{round(thisTableExectime/thisTableSequential:2)}%
	\xdef\thisTableSpeedup{\thisTableSpeedup}%
	\FPeval\thisTableEfficiency{round((thisTableSpeedup*100/thisTableNbSlaves):2)}%
	\xdef\thisTableEfficiency{\thisTableEfficiency}%
%
	\centering\thisTableNbSlaves
		&  \thisTableExectime
		&   \thisTableSpeedup$\times$ 
		&  \thisTableEfficiency\%
}%
%
%
{ \addtolength{\tabcolsep}{-4pt}%
\begin{tabular}{c|ccc}
\toprule
	\textbf{\# workers} &
	\textbf{samples/sec} & 
	\textbf{speedup} &
	\textbf{efficiency}
\\
\midrule
\centering 1 
	& \emph{\thisTableSequential}
	& 1$\times$ & 100\%
\\
\thisTableRow{20}{79275.028} \\ %{12852.984} \\
\thisTableRow{40}{162578.98} \\ %{26355.499} \\
\thisTableRow{60}{257791.96} \\ %{41788.824} \\
\thisTableRow{80}{335823.24} \\ %{54446.999} \\
\bottomrule
\end{tabular}
}
%\end{table}

==> 60_expres/setting.tex <==
% !TEX root =  ../root.tex

We ran our \Ac{PPSV} on a \Ac{HPC} infrastructure, allocating up to \DataGet<exps>{nodes/number} nodes (1 Orchestrator and up to \DataGet<exps>{workers/number} workers).
Each process ran on a node consisting of an Intel(R) Xeon(R) CPU with a frequency varying within 2.27--2.83 GHz, and had access to 1 GB of RAM.
%The single Orchestrator process was always run on a single core.

\endinput

Experiments have been carried out on
a cluster of 7 Linux heterogeneous machines, whose configurations are shown in \cref{tab:machines}.
We used a maximum number of 81 CPU cores (7 out of the 8 available cores for machines of categories A and B and 15 out of the 16 available cores for machines of category C).
%
The single Orchestrator process was always run on a core of Machine 0.
%
This means that we have 6 (i.e., 7.5\%) cores of (machines of) category A, 14 (i.e., 17.5\%) cores of category B, and 60 (i.e., 75\%) cores of category C available for slave processes.


%an Intel(R) Xeon(R) CPU @ 2.27GHz, 
%with 23GB of RAM, Kernel: Linux 2.6.32-5-686-bigmem, distribution Debian GNU/Linux 6.0.3 (squeeze).
\Comment{
\begin{table}[tp]
\begin{center}
{\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{c|ccccH|c}
\toprule
	\textbf{machine} & 
	%\multicolumn{2}{c}{\textbf{CPUs}} &	
	\textbf{Type and} & \textbf{\# CPUs} &
	\textbf{total} &	
	\multicolumn{2}{c}{\textbf{overall}} &
	\textbf{machine} 
\\
%\cmidrule{2-3} %\cmidrule{5-6}
	\textbf{id} & 
	\textbf{of CPUs} & \textbf{frequency} &
	\textbf{\# cores} &	
		\Comment{\textbf{overall}} \textbf{RAM} & 
		\Comment{\textbf{per core}} &
	\textbf{category}
\\
%
\midrule
0   &  2 $\times$ Intel(R) Xeon(R) & 2.83 GHz  &  8  &  8 GB   & 1 GB  & A \\
1   &  2 $\times$ Intel(R) Xeon(R) & 2.66 GHz  &  8  &  32 GB   & 4 GB & B\\	
2   &  2 $\times$ Intel(R) Xeon(R) & 2.66 GHz  &  8  &  32 GB   & 4 GB & B \\	
3   &  2 $\times$ Intel(R) Xeon(R) & 2.27 GHz  &  16  &  24 GB   & 1.5 GB & C \\	
4   &  2 $\times$ Intel(R) Xeon(R) & 2.27 GHz  &  16  &  24 GB   & 1.5 GB & C  \\
5   &  2 $\times$ Intel(R) Xeon(R) & 2.27 GHz  &  16  &  24 GB   & 1.5 GB & C  \\
6   &  2 $\times$ Intel(R) Xeon(R) & 2.27 GHz  &  16  &  24 GB   & 1.5 GB & C  \\
\bottomrule
\end{tabular}
}
\caption{Description of our cluster machines.}
\label{tab:machines}
\end{center}
\end{table}
}



\Comment{%%%%%%%%%%%%%%%%%%%
\begin{table}[tp]
\begin{center}
{\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{ccc}
\toprule
	\textbf{machine} & &
	\\
	\textbf{category} &	 
	\textbf{number} &
	\textbf{\%} 
	\\
\midrule
A   &  6	& 7.5 \% \\
B   &  14	& 17.5 \% \\
C   &  60	& 75.0 \% \\
\bottomrule
\end{tabular}
}
\caption{Number and \% of cores available to run slave processes for each machine category\label{tab:slaves}}
\end{center}
\end{table}
}%%%%%%%%%%%%%%%%%%%%%%%



==> 90_background/content.tex <==
% !TEX root =  ../root.tex

%\begin{Section}{Notation}
In the following, we denote with \Reals, \RealsGZ, \Naturals, and \NaturalsZ the sets of, respectively, all real, strictly positive real, strictly positive natural numbers and natural numbers including zero.
%\end{Section}

%\InputSection[sec:background:mc]{Optimal Monte Carlo Estimation}{montecarlo.tex}
\Input{montecarlo.tex}


==> 90_background/montecarlo.tex <==
% !TEX root =  ../root.tex

Many applications require the computation of the mean value $\mu_Z$ for a 0/1 random variable $Z$. 
When, as in our case, an exact computation is infeasible, Monte Carlo methods are often used to compute an approximation of this quantity~\cite{dagum-etal:2000:sicomp,grosu-etal:2004:isola}.
The main idea is to consider $N$ \Ac{iid} random variables $Z_1, \ldots, Z_N$ identical to $Z$ (having  mean $\mu_Z$), or, equivalently, $N$ independent realisations (samples) of the random variable $Z$,
and to take $\tilde{\mu}_Z = (Z_1 + \cdots + Z_N)/N$ as an approximation of $\mu_Z$.

In order to have a formally guaranteed upper bound for the error of this approximated computation, we employ an approach based on Statistical Model Checking which relies on the \Acf{AA} \cite{dagum-etal:2000:sicomp} (also reported in \cite{grosu-etal:2004:isola}), restricted to 0/1 random variables, and on Statistical Hypothesis Testing (along the lines of \cite{grosu-etal:2005:tacas}).
\footnote{For reviewing purposes, algorithmic versions of \Ac{AA} and of Statistical Hypothesis Testing are given in \cref{sec:background:aa,sec:background:sht}.}

\endinput

\begin{Section}[sec:background:aa]{\Acl{AA}}
Given two reals $\epsilon$ and $\delta$ in $(0,1)$, the \Acf{AA} \cite{dagum-etal:2000:sicomp} 
(also reported in \cite{grosu-etal:2004:isola}) computes a $(\epsilon, \delta)$-approximation $\tilde{\mu}_Z$ of $\mu_Z$, i.e., such that 
$
Pr[(1-\epsilon)\mu_Z \leq \tilde{\mu}_Z \leq (1+\epsilon)\mu_Z] \geq 1-\delta%
$.

%The algorithm, whose pseudo-code is reported as \cref{algo:aa}, 
%requires that $\mu_Z > 0$.
%It works in three phases (using a methodology known as \emph{sequential analysis}). 
%In Phase 1, it computes a first approximation $\tilde{\mu}_Z$ of $\mu_Z$ using the \Acf{SRA}. In Phase 2, it uses such a first approximation to compute a number of samples to be generated. It then generates that number of \Ac{iid} samples from $Z$ and computes (see variable \AlgoVar{alt}) the number of pairs of consecutive odd/even samples having different values. 
%In Phase 3, the algorithm uses such a value of \AlgoVar{alt} to compute a number of \emph{additional} samples that must be generated to achieve the required precision (given $\epsilon$ and $\delta$). It then generates such a number of additional samples and returns as $\tilde{\mu}_Z$ their mean value. 
%Value $\tilde{\mu}_Z$ is proved to be a $(\epsilon, \delta)$-approximation of $\mu_Z$ and the overall number of generated samples is proved to be optimal (up to a constant factor). The proof resorts to and generalises the zero-one estimator theorem~\cite{karp-etal:1989:jalgo}.

The \Acs{AA} algorithm requires that $\mu_Z > 0$.
It works in three phases (using a methodology known as \emph{sequential analysis}). 
In Phase 1, it computes a first approximation $\tilde{\mu}_Z$ of $\mu_Z$ using the \Acf{SRA}. 
In Phase 2, it uses such a first approximation to compute a number of samples to be generated. It then generates that number of \Ac{iid} samples from $Z$ and computes the number of pairs of consecutive odd/even samples having different values. 
In Phase 3, the algorithm uses such set of pairs to compute a number of \emph{additional} samples that must be generated to achieve the required precision (given $\epsilon$ and $\delta$). It then generates such a number of additional samples and returns as $\tilde{\mu}_Z$ their mean value. 
Value $\tilde{\mu}_Z$ is proved to be a $(\epsilon, \delta)$-approximation of $\mu_Z$ and the overall number of generated samples is proved to be optimal (up to a constant factor). The proof resorts to and generalises the zero-one estimator theorem~\cite{karp-etal:1989:jalgo}.

%\Input{montecarlo_AA.tex}

\end{Section}


\begin{Section}[sec:background:sht]{Statistical Hypothesis Testing}
%Function \AlgoFun{\Acs{SRA}()} used by \Ac{AA} (\cref{algo:aa}) does not terminate when the mean $\mu_Z$ of the input random variable $Z$ is \emph{zero} (as the termination condition is based on the number of successes going beyond a given positive threshold $\Upsilon_1$).
%Similarly, termination might require a huge number of samples in case the mean, although positive, is very low.

\Acf{SRA} used by \Acs{AA} does not terminate when the mean $\mu_Z$ of the input random variable $Z$ is \emph{zero} (as the termination condition is based on the number of successes going beyond a given positive threshold $\Upsilon_1$).
Similarly, termination might require a huge number of samples in case the mean, although positive, is very low.

To circumvent this limitation, our algorithm for \Ac{PPSV} (see forthcoming \cref{sec:algo}) also relies on a kind of Statistical Hypothesis Testing technique, along the lines of \cite{grosu-etal:2005:tacas,mancini-etal:2014:fmcad,mancini-etal:2015:iwbbio}. Such technique works as follows. 

Consider a 0/1 random variable $Z$ and the \emph{null hypothesis} $H_0$ which is true iff $\mu_Z \geq \epsilon$.
%
Given values $\epsilon$ and $\delta$ in $(0,1)$, if, after $M = \lceil\ln(\delta)/\ln(1-\epsilon)\rceil$ \Ac{iid} samples $Z_1\ldots, Z_M$ of $Z$, we have $\sum_{i=1}^M Z_i = 0$, we reject $H_0$, thus declaring that $\mu_Z < \epsilon$. 
This is known to be a one-sided error decision procedure, as it may introduce a \emph{type-I error} (i.e., we might reject $H_0$ when it actually holds).
%
However, \cite{grosu-etal:2005:tacas} shows that the probability of such an error is at most $\delta$.
Formally: 
$Pr[ Z_1 = \cdots Z_M = 0 ~|~  H_0]  < \delta$.
%
This equivalently tells us that $H_0$ is rejected with confidence at least $1-\delta$. 

\Comment{
Note that, in case $\sum_{i=1}^M Z_i > 0$ we do not accept $H_0$, but continue with the computation of an estimation $\hat{\mu}_Z$ of $\mu_Z$ according to \Ac{AA}. As a consequence, we never introduce a type-II error (i.e., we never accept $H_0$ when it does not hold).
}
\end{Section} %% statistical hyp testing







==> MCLabPaper_Acronym_2.tex <==
\MCLabPaper@RequirePackage{datatool}

\MCLabPaper@Set@Tutorial@Section{Acronym}{sec:acronym}

\DeclareDocumentCommand{\Debug@Out@Acronym}{o m}{%
	\Debug@Out{Acronym}[#1]{#2}%
}

\DiagDefineMsgType{missingacronym}{
	title={Undefined Acronym},
	backgroundcolor={yellow!30},
	linecolor={black!50}, 
	icon=\Diag@Image@Warning,
	die=false, 
	showinpdf=true, 
	showtutorialbutton=true, 
	showinlog=true
}


\DeclareDocumentCommand{\Acro@Diag@Undefined}{m}{%
	% Call \Diag@Message:
	%  - arg1: \BooleanTrue -> inline, \BooleanFalse -> banner
	%  - (arg2): options
	%  - arg3: module name
	%  - arg4: message to PDF
	%  - arg5: message to log
	\Diag@Message%
		{\BooleanFalse}% \BooleanTrue -> inline
		{missingacronym}%	message type
		()%		options
		{Acronym}%		module name
		{Acronym `#1' has not been defined. Use \DiagLatexCmd{NewAcronym} first.}%		message to PDF
		[Acronym `#1' has not been defined. Use \detokenize{\NewAcronym} first]% 		message to log (empty: use msg to PDF)
}


\def\MCLabPaper@Acro@plural@postfix{s}%
\def\MCLabPaper@listofacronymsname{List of Acronyms}%

\addto\captionsenglish{%
  \def\MCLabPaper@Acro@plural@postfix{s}%
  \def\MCLabPaper@listofacronymsname{List of Acronyms}%
}

\addto\captionsitalian{%
  \def\MCLabPaper@Acro@plural@postfix{}%
  \def\MCLabPaper@listofacronymsname{Elenco degli Acronimi}%  
}

\xdef\AcroPrefix{MCLabPaper/Acronyms}%

\CommaSepListNew{Acronyms@List}% contains short versions of acronyms, not acronyms
\define@cmdkey{NewAcronym}{shortplural}[]{}%
\define@cmdkey{NewAcronym}{longplural}[]{}%
\define@choicekey*{NewAcronym}{expand}[\NewAcro@expand\NewAcro@expand@idx]{auto, never, always}[auto]{}%

\newtoggle{Acro@is@new}%
\DeclareDocumentCommand{\NewAcronym}{m o m O{}}{%	
	\Debug@Out@Acronym[{NewAcronym(#1)[#2](#3)[#4]}]{Start}%
	% #1: Acronym
	% #2: Displayed acronym
	% #3: Long definition
	% #4: other options: shortplural=..., longplural=...	
	\def\NewAcro@acro{#1}%
	\IfValueTF{#2}{%
		\def\NewAcro@short{#2}%	
	}{%
		\def\NewAcro@short{#1}%
	}%
	\def\NewAcro@long{#3}%
	\setkeys{NewAcronym}{shortplural, longplural, expand}%
	\@expandtwoargs\setkeys{NewAcronym}{#4}%
	%
	\ifequals{\cmdKV@NewAcronym@shortplural}{}{%
		\edef\NewAcro@shortplural{\NewAcro@short\MCLabPaper@Acro@plural@postfix}%
	}{%
		\let\NewAcro@shortplural\cmdKV@NewAcronym@shortplural%
	}%
	\ifequals{\cmdKV@NewAcronym@longplural}{}{%
		\edef\NewAcro@longplural{\NewAcro@long\MCLabPaper@Acro@plural@postfix}%
	}{%
		\let\NewAcro@longplural\cmdKV@NewAcronym@longplural%
	}%	
	%
	\Debug@Out@Acronym[NewAcronym]{Defining acronym:}%
	\Debug@Out@Acronym[NewAcronym]{ - Acronym Id: '\NewAcro@acro'}%
	\Debug@Out@Acronym[NewAcronym]{ - Short: '\NewAcro@short'}%
	\Debug@Out@Acronym[NewAcronym]{ - Long: '\NewAcro@long'}%
	\Debug@Out@Acronym[NewAcronym]{ - Short plural: '\NewAcro@shortplural'}%
	\Debug@Out@Acronym[NewAcronym]{ - Long plural: '\NewAcro@longplural'}%
	\Debug@Out@Acronym[NewAcronym]{ - Expand policy: '\NewAcro@expand' (code = '\NewAcro@expand@idx')}%
	%
	\ifcsdef{\AcroPrefix/acronym/\NewAcro@acro/short}{%
		\togglefalse{Acro@is@new}%
		% Short acronym already defined. Definition will be overridden, but acronym is not added again to the list of acronyms.
	}{%
		\toggletrue{Acro@is@new}%
	}%
	%
	% Define acronym data
	%
	\csxdef{\AcroPrefix/acronym/\NewAcro@acro/short}{\NewAcro@short}%
	\csxdef{\AcroPrefix/acronym/\NewAcro@acro/long}{\NewAcro@long}%
	\csxdef{\AcroPrefix/acronym/\NewAcro@acro/shortplural}{\NewAcro@shortplural}%
	\csedef{\AcroPrefix/acronym/\NewAcro@acro/longplural}{\NewAcro@longplural}%
	%
	% Define macro whose name contains "expand policy" (fast testing with \ifcsdef --non-empty macro content is irrelevant).
	\csedef{\AcroPrefix/acronym/\NewAcro@acro/expand/\NewAcro@expand}{x}%
	\UtilGlobalDefinitions{%
		\providebool{\AcroPrefix/acronym/\NewAcro@acro/used}%
		\boolfalse{\AcroPrefix/acronym/\NewAcro@acro/used}%
	}%
	%
	% Undefine 'firstpagelabel'
	\csundef{\AcroPrefix/acronym/\NewAcro@acro/firstpagelabel}%
	%
	% Define mapping: short --> acronym-id
	\ifcsdef{\AcroPrefix/short/\NewAcro@short/acronym}{% 
		% Short value is already defined. 
		% Check that we are overriding acronym definition, 
		% not adding a new acronym with same short variant.
		\ifequals{\NewAcro@acro}{\csuse{\AcroPrefix/short/\NewAcro@short/acronym}}{}{%
			% not equal
			\DiagError{Acronym}{Acronym ID `\NewAcro@acro', when shortened to `\NewAcro@short', will appear identical to previously defined acronym ID `\csuse{\AcroPrefix/short/\NewAcro@short/acronym}'. This is not acceptable}%
		}%		
	}{}%
	\csxdef{\AcroPrefix/short/\NewAcro@short/acronym}{\NewAcro@acro}%
	\iftoggle{Acro@is@new}{%
		% If expand policy is != "always", 
		% add acro to the list of acronyms
		\ifcsundef{\AcroPrefix/acronym/\NewAcro@acro/expand/always}{%
			\CommaSepListAppend{Acronyms@List}[/.expanded]{\NewAcro@short}%
		}{}%
	}{}%
	%
	\IfDebugTF{Acronym}{%
		\CommaSepList{Acronyms@List}{\Acronyms@List}%
		\Debug@Out@Acronym[NewAcronym]{Done with '\NewAcro@acro'. List of short versions of acronyms defined so far: [\Acronyms@List]}%
	}{}%
	\Debug@Out@Acronym[{NewAcronym(#1)[#2](#3)[#4]}]{End}%
}

\DeclareDocumentCommand{\Ac@What}{m m m}{% 
	% #1: acro, 
	% #2: what={short, long}, 
	% #3={{}, plural}
	%
	%[acwhat(#1)(#2)(#3)]
	\ifcsdef{\AcroPrefix/acronym/#1/short}{%
		% Acronym is defined
		\letcs\Ac@what@result{\AcroPrefix/acronym/#1/#2#3}%
		%
		\Debug@Out@Acronym[Ac@what(#1)(#2)(#3)]{ --> '\Ac@what@result'}%
		\Ac@what@result%
		%
		% \ifcsundef{\AcroPrefix/acronym/#1/firstpagelabel}{%
		% 	%
		% 	%[firstpage undef]
		% 	\Debug@Out@Acronym[Ac@what(#1)(#2)(#3)]{firstpagelabel undefined}%
		% 	%
		% 	\ifstrequal{#2}{long}{%
		% 		%
		% 		%[long]
		% 			\edef\Acro@label{MCLabPaper_Acronyms:#1}%
		% 		%\noexpand{%
		% 			\label{\Acro@label}%
		% 			%[LABEL SET]%
		% 			\csxdef{\AcroPrefix/acronym/#1/firstpagelabel}{\Acro@label}%
		% 			%
		% 			%
		% 			\Debug@Out@Acronym[Ac@what(#1)(#2)(#3)]{First use of long version: saving current page via label '\Acro@label'}%
		% 		%}%
		% 	}{%
		% 		%[not long]
		% 		\Debug@Out@Acronym[Ac@what(#1)(#2)(#3)]{User requested '#2' version, not setting firstpagelabel}%
		% 	}%
		% }{%
		% 	%[firstpage already def]
		% 	\Debug@Out@Acronym[Ac@what(#1)(#2)(#3)]{firstpagelabel already set to '\csuse{\AcroPrefix/acronym/#1/firstpagelabel}'}%
		% }%
	}{%
		% Acronym undefined
		\Acro@Diag@Undefined{#1}%
		#1%
	}%
	%
}

%\provideboolean{ac used}%
\DeclareDocumentCommand{\Ac@Auto@Expand}{m m m O{}}{% 
		% #1: \Booleanfalse (default) or \Booleantrue (don't use parentheses)
		% #2: acro, 
		% #3={{}, plural}
		% [#4]: if alternative layout and full, what to be put after acro
	\ifcsdef{\AcroPrefix/acronym/#2/short}{%	
		% Acronym is defined	
		%
		% expand can be: auto, never, always
		%
		\Debug@Out@Acronym[{Ac@Auto@Expand(#1)(#2)(#3)[#4]}]{Start}%
		\ifcsdef{\AcroPrefix/acronym/#2/expand/always}{%
			% if expand policy = always --> long (not full)
			\Debug@Out@Acronym[{Ac@Auto@Expand(#1)(#2)(#3)[#4]}]{ - expand policy is 'always' --> long}%
			\Ac@What{#2}{long}{#3}%			
		}{%
			\ifcsdef{\AcroPrefix/acronym/#2/expand/never}{%
				% if expand policy = never --> short
				\Debug@Out@Acronym[{Ac@Auto@Expand(#1)(#2)(#3)[#4]}]{ - expand policy is 'never' --> short}%
				\Ac@What{#2}{short}{#3}%
			}{%
				% else (expand policy = auto): check if 'used'
				\Debug@Out@Acronym[{Ac@Auto@Expand(#1)(#2)(#3)[#4]}]{ - expand policy is 'auto' --> check used}%
				\ifbool{\AcroPrefix/acronym/#2/used}{%
					\Debug@Out@Acronym[{Ac@Auto@Expand(#1)(#2)(#3)[#4]}]{   - used is true --> short}%
					\Ac@What{#2}{short}{#3}%
				}{%
					\Debug@Out@Acronym[{Ac@Auto@Expand(#1)(#2)(#3)[#4]}]{   - used is false --> full}%
					\Acf@aux{#1}{#2}{#3}[#4]%					
				}%
			}%
		}%
		\AcronymUsed{#2}%	
	}{%
		% Acronym not defined
		\Acro@Diag@Undefined{#2}%
		#2%
	}%
	%\xspace%
}

\DeclareDocumentCommand{\Ac}{s m O{}}{% 
	% * --> alternative layout
	% #2: acro
	% [#3]: if alternative layout and full, what to be put after acro
	\Ac@Auto@Expand{#1}{#2}{}[#3]\xspace%
}
\DeclareDocumentCommand{\Acp}{s m O{}}{% 
	% * --> alternative layout
	% #2: acro
	% [#3]: if alternative layout and full, what to be put after acro
	\Ac@Auto@Expand{#1}{#2}{plural}[#3]\xspace%
}
\DeclareDocumentCommand{\Acs}{m}{% #1: acro
	\Ac@What{#1}{short}{}\xspace%
}
\DeclareDocumentCommand{\Acsp}{m}{% #1: acro
	\Ac@What{#1}{short}{plural}\xspace%
}

\DeclareDocumentCommand{\Acl}{m}{% #1: acro
	\Ac@What{#1}{long}{}\xspace%
}
\DeclareDocumentCommand{\Aclp}{m}{% #1: acro
	\Ac@What{#1}{long}{plural}\xspace%
}

\DeclareDocumentCommand{\Acf@aux}{m m m O{}}{% 
	% #1: BooleanT = alternative layout, i.e., with no parenthesis
	% #2: id
	% #3: what (long|short)
	% [#4]: if #1=true (alternative layout), what to be put after acronym (e.g., ",")%	
	\Debug@Out@Acronym[{Acf@aux(#1)(#2)(#3)[#4]}]{Start}%
	\IfBooleanTF{#1}{%  star: no pars
		\Debug@Out@Acronym[{Acf@aux(#1)(#2)(#3)[#4]}]{Don't use parentheses}%
		\Ac@What{#2}{long}{#3}, \Ac@What{#2}{short}{#3}#4%
	}{% default
		\Debug@Out@Acronym[{Acf@aux(#1)(#2)(#3)[#4]}]{Default format with parentheses}%			
		\Ac@What{#2}{long}{#3} (\Ac@What{#2}{short}{#3})%
	}%
	\Debug@Out@Acronym[{Acf@aux(#1)(#2)(#3)[#4]}]{End}%
	%\xspace%	
}

\DeclareDocumentCommand{\Acf}{s m O{}}{% 
		% #1: star --> don't use parentheses
		% #2: acro
		% [#3]: if #1=true (alternative layout), what to be put after acro
	%\Debug@Out@Acronym[{Acf(#1)(#2)[#3]}]{Start}%
	\Acf@aux{#1}{#2}{}[#3]\xspace%
	%\Debug@Out@Acronym[{Acf(#1)(#2)[#3]}]{End}%
}
\DeclareDocumentCommand{\Acfp}{s m O{}}{%
		% #1: star --> don't use parentheses
		% #2: acro
		% [#3]: if #1=true (alternative layout), what to be put after acro
	\Acf@aux{#1}{#2}{plural}[#3]\xspace%
}



\DeclareDocumentCommand{\AcronymReset}{m}{% #1: acro
	\Debug@Out@Acronym[AcronymReset(#1)]{Resetting acronym '#1'.}%
	\UtilGlobalDefinitions{%
		\boolfalse{\AcroPrefix/acronym/#1/used}% why \global produces error during acro reset upon \begin{Section} in \ListOfAcronyms??
	}%
	\Debug@Out@Acronym[AcronymReset(#1)]{Acronym '#1' has been reset.}%
}
\DeclareDocumentCommand{\AcronymUsed}{m}{% #1: acro	
	\Debug@Out@Acronym[AcronymUsed(#1)]{Start}%
	\UtilGlobalDefinitions{%
	 	\booltrue{\AcroPrefix/acronym/#1/used}%
	}%
	\Debug@Out@Acronym[AcronymUsed(#1)]{ - set 'used' to true (I'm not checking if this was really needed)}%
 	%
  	\ifcsundef{\AcroPrefix/acronym/#1/firstpagelabel}{%
		% Acro has been used for the *first* time in document
		% Set first-page label
		%
		\Debug@Out@Acronym[AcronymUsed(#1)]{ - acro has been used for the first time in document: setting firstpagelabel}%
		%
		\edef\Acro@label{MCLabPaper_Acronyms:#1}%
		\expandafter\label\expandafter{\Acro@label}%
		\csxdef{\AcroPrefix/acronym/#1/firstpagelabel}{\Acro@label}%
	}{%
		%[firstpage already def]
		\Debug@Out@Acronym[AcronymUsed(#1)]{ - firstpagelabel already set to '\csuse{\AcroPrefix/acronym/#1/firstpagelabel}'}%
	}%		
	%
	\Debug@Out@Acronym[AcronymUsed(#1)]{End}%
}

\DeclareDocumentCommand{\AcronymResetAll}{}{% #1: acro
	\Debug@Out@Acronym[AcronymResetAll]{Start}%
	\CommaSepList{Acronyms@List}{\Acronyms@List}%
	\ifequals{\Acronyms@List}{}{%
		\Debug@Out@Acronym[AcronymResetAll]{ - No acronyms defined}%
	}{%
		\xintFor ##9 in {\Acronyms@List} \do{% %\Acronyms@List contains short (not acronyms)
			\letcs\Acro@Reset@All@acro{\AcroPrefix/short/##9/acronym}%	
			\Debug@Out@Acronym[AcronymResetAll]{ - Resetting acronym '\Acro@Reset@All@acro'}%
			\AcronymReset{\Acro@Reset@All@acro}%
		}%
	}%
	\Debug@Out@Acronym[AcronymResetAll]{End}%
}

\newlist{listofacronyms}{description}{1}

\def\List@Of@Acronyms@layout{style={labelwidth=\widthof{MMMMMM}}, pages=true}%
\DeclareDocumentCommand{\AcronymListSetLayout}{m}{%
	\def\List@Of@Acronyms@layout{#1}%
}

\define@cmdkey{ListOfAcronyms}{style}[]{}
\define@boolkey{ListOfAcronyms}{pages}[true]{}
\newcommand{\ListOfAcronymsMark}[1]{}%
\DeclareDocumentCommand{\ListOfAcronyms}{O{}}{% 
	% #1: options: style=enumitem comma-sep list of options
	\Debug@Out@Acronym[ListOfAcronyms]{Start.}%
	\Debug@Out@Acronym[ListOfAcronyms]{Current document-wise layout: '\List@Of@Acronyms@layout'}%
	\Debug@Out@Acronym[ListOfAcronyms]{Explicit options given: '#1'}%
	\setkeys{ListOfAcronyms}{style, pages}%
	\@expandtwoargs\setkeys{ListOfAcronyms}{\List@Of@Acronyms@layout, #1}%
	\Debug@Out@Acronym[ListOfAcronyms]{Final list options:}%
	\Debug@Out@Acronym[ListOfAcronyms]{ - style = [\cmdKV@ListOfAcronyms@style]}%
	\Debug@Out@Acronym[ListOfAcronyms]{ - pages = [\ifKV@ListOfAcronyms@pages true\else false\fi]}%
	\CommaSepList{Acronyms@List}{\Acronyms@List}%
	\Debug@Out@Acronym[ListOfAcronyms]{List of short versions of all acronyms = [\Acronyms@List]}%
	%
	% First scan of acro list to retrieve only used %
	% (short versions of) acronyms.
	% In this way we can better understand if we need to print
	% list of acronyms or not.
	%
	\Debug@Out@Acronym[ListOfAcronyms]{Computing list of used acronym short versions}%
	\CommaSepListNew{Acronyms@List@Used}%
	\xintFor ##9 in {\Acronyms@List} \do{% 
		% \Acronyms@List contains short versions (not acronyms)
		\letcs\Acro@List@acro{\AcroPrefix/short/##9/acronym}%
		\ifcsdef{\AcroPrefix/acronym/\Acro@List@acro/firstpagelabel}{%
			\Debug@Out@Acronym[ListOfAcronyms]{ - Acronym ID '\Acro@List@acro' used, added to list}%
			% Append short version of \Acro@List@acro
			\CommaSepListAppend{Acronyms@List@Used}[/.expanded]{##9}%
		}{}% else don't add to list of used acronyms
	}%
	\CommaSepList{Acronyms@List@Used}{\Acronyms@List@Used}%
	\Debug@Out@Acronym[ListOfAcronyms]{List of short versions of used acronym: [\Acronyms@List@Used]}%
	%
	\ifequals{\Acronyms@List@Used}{}{%
		% empty list of used acronyms --> do nothing
		\DiagInfo{Acronym}{No acronyms have been used so far, hence the list of acronyms is not printed. Remove draft mode to hide this message and come out with a polished document.}
	}{%
		\Debug@Out@Acronym[ListOfAcronyms]{Creating Section for List of Acronyms}%
		\begin{Section}*{\MCLabPaper@listofacronymsname}%	
			\ListOfAcronymsMark{\MCLabPaper@listofacronymsname}%
			%\setlist[listofacronyms]{#1}%			
			% My datatool version is too old!
			\ifdef{\dtlsortlist}{%
				\Debug@Out@Acronym[ListOfAcronyms]{Sorting list of acronyms}%
				\dtlsortlist{\Acronyms@List@Used}{\dtlcompare}%
			}{%
				\PackageWarning{MCLabPaper}{You have an old version of the datatool package (older than 2016-07-28). Please, update your Latex Platform. As a result, the list of acronyms is not sorted.}%
				\DraftWarning[MCLabPaper]{You have an old version of the datatool package (older than 2016-07-28). Please, update your Latex Platform.\\ As a result, the list of acronyms is not sorted.}%
			}%
			\Debug@Out@Acronym[ListOfAcronyms]{Starting description list}%
			\expandafter\listofacronyms\expandafter[\cmdKV@ListOfAcronyms@style]
			\xintFor ##9 in {\Acronyms@List@Used} \do{% 
				% \Acronyms@List contains acronym short versions
				\letcs\Acro@List@acro{\AcroPrefix/short/##9/acronym}%
				\Debug@Out@Acronym[ListOfAcronyms]{ - \Acro@List@acro}%
				\letcs\Ac@short{\AcroPrefix/acronym/\Acro@List@acro/short}%
				\letcs\Ac@long{\AcroPrefix/acronym/\Acro@List@acro/long}%
				%
				\ifcsdef{\AcroPrefix/acronym/\Acro@List@acro/firstpagelabel}{%
					\letcs\Ac@firstpagelabel{\AcroPrefix/acronym/\Acro@List@acro/firstpagelabel}%
					%
					\Debug@Out@Acronym[ListOfAcronyms]{   - short: '\Ac@short'}%
					\Debug@Out@Acronym[ListOfAcronyms]{   - long: '\Ac@long'}%
					\Debug@Out@Acronym[ListOfAcronyms]{   - firstpagelabel: '\Ac@firstpagelabel'}%
					\item[\Ac@short] \Ac@long%
						\ifKV@ListOfAcronyms@pages%
							\dotfill\pageref{\Ac@firstpagelabel}%
						\fi%
					\par

				}{%
					\PackageError{MCLabPaper}{Acronym module error: acronym \Acro@List@acro\space never used, this should never happen.}%
					%\Debug@Out@Acronym{\space\space\space ---> \Acro@List@acro\space never used -> skipped}%
				}%
				%
			}% end for
			\endlistofacronyms%
			\Debug@Out@Acronym[ListOfAcronyms]{End}%
		\end{Section}%
	}%
}
\let\AcronymList\ListOfAcronyms%

% RESETTING ACRONYMS
\def\MCLabPaper@Acronym@Reset@At@Each{}
\DeclareDocumentCommand{\AcronymResetAllAtEach}{m}{%
	\ArrayPos[\MCLabPaper@Acronym@Reset@At@Each]{Sectioning}{#1}%
}
\AcronymResetAllAtEach{section} % DEFAULT

\newcommand{\MCLabPaper@Acronym@Possibly@Reset@All}{%
	\Debug@Out@Acronym[@Possibly@Reset@All]{Start. Starting Section at depth = \theSections@current@depth): 
		Should I reset acronyms (to be reset at depth \MCLabPaper@Acronym@Reset@At@Each)?}%
	\ifthenelse{\theSections@current@depth > \MCLabPaper@Acronym@Reset@At@Each}{%
		\Debug@Out@Acronym[@Possibly@Reset@All]{ --> No}%
	}{%
		\AcronymResetAll%
		\Draft@SystemNote{Acronyms reset}%
		\Debug@Out@Acronym[@Possibly@Reset@All]{ --> Yes}%
	}%
	\Debug@Out@Acronym[@Possibly@Reset@All]{End}%
}


\AtBeginDocument{%
	\ArrayLastIndex[\tmp@sectioning@maxlevel]{Sectioning}	
	\xintFor* #1 in {\xintSeq {1}{\tmp@sectioning@maxlevel}} \do{%
		%\Section@DebugOut{ - command at depth #1 is...}%
		\ArrayGet[\tmp@sectioning@section@command]{Sectioning}{#1}%
		%\Section@DebugOut{ ---> '\tmp@sectioning@section@command'}%
		\MCLabPaper@Sectioning@Hook@Name{\tmp@sectioning@hook@name}{\tmp@sectioning@section@command}%
		%
		\csappto{\tmp@sectioning@hook@name}{\MCLabPaper@Acronym@Possibly@Reset@All}%
	}%
}



%%% DEPRECATED COMMANDS

\DeclareDocumentCommand{\newacronym}{m o m}{%
	\DiagDeprecationSimple{Acronym}{newacronym}{NewAcronym}%
	\NewAcronym{#1}[#2]{#3}%
}
\DeclareDocumentCommand{\ac}{m}{%
	\DiagDeprecationSimple{Acronym}{ac}{Ac}%
	\Ac{#1}%
}
\DeclareDocumentCommand{\acp}{m}{%
	\DiagDeprecationSimple{Acronym}{acp}{Acp}%
	\Acp{#1}%
}
\DeclareDocumentCommand{\acs}{m}{%
	\DiagDeprecationSimple{Acronym}{acs}{Acs}%
	\Acs{#1}%
}
\DeclareDocumentCommand{\acsp}{m}{%
	\DiagDeprecationSimple{Acronym}{acsp}{Acsp}%
	\Acsp{#1}%
}
\DeclareDocumentCommand{\acl}{m}{%
	\DiagDeprecationSimple{Acronym}{acl}{Acl}%
	\Acl{#1}%
}
\DeclareDocumentCommand{\aclp}{m}{%
	\DiagDeprecationSimple{aclp}{Aclp}%
	\Aclp{#1}%
}
\DeclareDocumentCommand{\acf}{m}{%
	\DiagDeprecationSimple{Acronym}{acf}{Acf}%
	\Acf{#1}%
}
\DeclareDocumentCommand{\acfp}{m}{%
	\DiagDeprecationSimple{Acronym}{acfp}{Acfp}%
	\Acfp{#1}%
}
\DeclareDocumentCommand{\acused}{m}{%
	\DiagDeprecationSimple{Acronym}{acused}{AcronymUsed}%
	\AcronymUsed{#1}%
}
\DeclareDocumentCommand{\acresetall}{}{%
	\DiagDeprecationSimple{Acronym}{acresetall}{AcronymResetAll}%
	\AcronymResetAll%
}



==> MCLabPaper_Algo_2.tex <==
%% Toni: Finally it seems that algorithm2e has been amended with version 5.2 of 2017, but it is not yet included in our texlive/mactex
%\MCLabPaper@RequirePackage[noline,scleft,linesnumbered,noend]{MCLabPaper_algorithm2e}
\MCLabPaper@RequirePackage[noline,scleft,linesnumbered,noend]{algorithm2e}

\MCLabPaper@Set@Tutorial@Section{Algorithm}{sec:algo}

\SetAlgorithmName{Algorithm}{Algorithm}{List of Algorithms}

\addto\captionsenglish{%
  \SetAlgorithmName{Algorithm}{Algorithm}{List of Algorithms}
}
\addto\captionsitalian{%
    \SetAlgorithmName{Algoritmo}{Algoritmo}{Elenco degli Algoritmi}
}

%\DeclareDocumentCommand{\algoref}{m}{%
%	\smart@refs[\algorithmcfname]{#1}%
%}

\definecolor{MCLabPaper_CommentColor}{gray}{0.5}
\def\Algo@Comment@Sty#1{\textcolor{MCLabPaper_CommentColor}{\textit{#1}}}
\SetCommentSty{Algo@Comment@Sty}
\SetAlCapSkip{\abovecaptionskip} % same as figures (hence, they are tunable by using \SetCompact)

\SetInd{0.3em}{0.3em}
\SetKw{KwFunction}{function}
\SetKw{KwProcedure}{procedure}
\SetKw{KwMethod}{method}
\SetKw{KwClass}{class}
\SetKw{KwLet}{let}
\SetKw{KwNew}{new}
\SetKw{KwNil}{nil}
\SetKw{KwBreak}{break}
\SetKw{KwOutput}{output}
\SetKw{KwField}{field}
\SetKw{KwGlobal}{global}
\SetKw{KwMethod}{method}
\SetKw{KwParam}{param}
\SetKw{KwAssert}{assert}
\SetKw{KwReturns}{returns}
\SetKw{KwEnd}{end}
\SetKw{KwStatic}{static}
\SetKwRepeat{DoWhile}{do}{while}
\SetKwBlock{BeginNoEnd}{begin}{}
\SetKwBlock{EndNoBegin}{}{end}
\SetKwBlock{NoBeginNoEnd}{}{}

\SetKw{KwSend}{send}
\SetKw{KwRecv}{recv}
\SetKw{KwWait}{wait}

\DeclareDocumentCommand{\AlgoFunction}{m +m}{%
	\noindent%
	\KwFunction \AlgoFun{#1}%
	\EndNoBegin{#2}%
}
\DeclareDocumentCommand{\AlgoProcedure}{m +m}{%
	\noindent%
	\KwProcedure \AlgoProc{#1}%
	\EndNoBegin{#2}%
}

\DeclareDocumentCommand{\AlgoClass}{m +m}{%
	\noindent%
	\KwClass \AlgoFun{#1}%
	\EndNoBegin{#2}%
}
\DeclareDocumentCommand{\AlgoMethod}{m +m}{%
	\noindent%
	\KwMethod \AlgoFun{#1}%
	\EndNoBegin{#2}%
}



\newcommand{\AlgoFun}[1]{\ensuremath{\Fun{#1}}}
\newcommand{\AlgoProc}[1]{\ensuremath{\Fun{#1}}}
\newcommand{\AlgoType}[1]{\textbf{#1}}
\newcommand{\AlgoVar}[1]{\ensuremath{\Fun{#1}}}

\newcommand{\AlgoVarGets}[2]{\ensuremath{\AlgoVar{#1}\gets} #2}
\newcommand{\AlgoIncrVar}[1]{\ensuremath{\AlgoVar{#1}\text{++}}}
\let\AlgoVarIncr\AlgoIncrVar
\newcommand{\AlgoDecrVar}[1]{\ensuremath{\AlgoVar{#1}\text{-}{}\text{-}}}
\let\AlgoVarDecr\AlgoDecrVar

==> MCLabPaper_Array_2.tex <==
\PackageInfo{MCLabPaper}{Loading Module Array}%

% pgfkeys-based arrays
\xdef\pgfkeysArrayPrefix{\pgfkeysPrefix/arrays}

% Array positions from 0 to size-1
\DeclareDocumentCommand{\ArrayNew}{m}{%
	\xdef\arrayName{#1}%
	\pgfglobalkeys{\pgfkeysArrayPrefix/\arrayName/size/.initial=0}%
}
\DeclareDocumentCommand{\ArrayAdd}{m m}{%
	\xdef\@arrayName{#1}%
	\edef\@value{#2}%
	\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/size/.get=\@size}%
	\pgfmathsetmacro{\@newSize}{int(\@size+1)}%
	\pgfglobalkeys{%
		\pgfkeysArrayPrefix/\@arrayName/\@size/.initial/.expanded=\@value
	}%
	\pgfglobalkeys{%
		\pgfkeysArrayPrefix/\@arrayName/size/.expanded=\@newSize,
	}%
}
\DeclareDocumentCommand{\ArraySize}{o m}{%
	\edef\@arrayName{#2}%
	\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/size/.get=\array@size@value}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\array@size@value}%
	}{\array@size@value}%
}
\DeclareDocumentCommand{\ArrayLastIndex}{o m}{%
	\edef\@arrayName{#2}%
	\ArraySize[\array@lastIndex@size]{\@arrayName}%
	\ifnum \array@lastIndex@size > 0%
		\pgfmathsetmacro{\@lastIdx}{int(\array@lastIndex@size -1)}%
	\else%
		\def\@lastIdx{}%
	\fi%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\@lastIdx}%
	}{\@lastIdx}%
}

\DeclareDocumentCommand{\ArrayGet}{o m m}{%
	\edef\@arrayName{#2}%
	\ArraySize[\@size]{\@arrayName}%
	\def\ArrayGet@idx{#3}%
	%\@DebugOut{ArrayGet{#2}{#3}: start}%
	\ifthenelse{\ArrayGet@idx < 0 \OR \ArrayGet@idx > \@size \OR \ArrayGet@idx = \@size}{%
		\DiagError{Array}{ArrayGet asks the '\ArrayGet@idx'-th element of array '#2', but array size is \@size}%
	}{}%	
	\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/\ArrayGet@idx/.get=\ArrayGet@value}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\ArrayGet@value}%
	}{\ArrayGet@value}%
}
\DeclareDocumentCommand{\ArrayDump}{m}{%
	\edef\@arrayName{#1}%
	\ArraySize[\array@lastIndex@size]{\@arrayName}%
	\ifnum \array@lastIndex@size = 0%
		[array is empty]%
	\else%
		\begin{itemize}%
		\pgfmathsetmacro{\@lastIdx}{int(\array@lastIndex@size -1)}%
		\foreach \@i in {0, ..., \@lastIdx} {%
			\item (\@i) $\to$ ``\ArrayGet{\@arrayName}{\@i}''%
		}%
		\end{itemize}%
	\fi%
}
\DeclareDocumentCommand{\ArrayRemove}{o m m}{%
	\edef\@arrayName{#2}%
	\edef\@idx{#3}%
	\ArraySize[\array@remove@size]{\@arrayName}%
	\ifnum \array@remove@size = 0%
		\PackageError{MCLabPaper}{Trying to remove an element from an empty array}{Removing an element from an empty array results in an error. Please ensure with \IfArrayEmptyF that your array is not empty}%
		%\IfValueT{#1}{%
		%	\edef#1{}%
		%}%
	\else%
		\IfValueT{#1}{%
			\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/\@idx/.get=\@value}%
			\edef@macro{#1}{\@value}%
		}%
		\ArrayLastIndex[\@lastIdx]{\@arrayName}%
			\pgfmathsetmacro{\@nextIdx}{int(\@idx + 1)}%
			\ifnum \@nextIdx > \@lastIdx%
			\else%
				\foreach \@i in {\@nextIdx, ..., \@lastIdx} {%
					\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/\@i/.get=\@value}%
					\pgfmathsetmacro{\@prevIdx}{int(\@i - 1)}%
					\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/\@prevIdx/.expanded=\@value}%
				}%								
			\fi%			
			\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/\@lastIdx/.expanded=\pgfkeysnovalue}%
		\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/size/.expanded=\@lastIdx}%
	\fi%
}

\DeclareDocumentCommand{\ArrayPop}{o m}{%
	\edef\@arrayName{#2}%
	\ArraySize[\array@pop@size]{\@arrayName}%
	\pgfmathsetmacro{\@idx}{int(\array@pop@size-1)}%
	\IfValueTF{#1}{%
		\ArrayRemove[#1]{\@arrayName}{\@idx}%
	}{%
		\ArrayRemove{\@arrayName}{\@idx}%
	}%
}
\DeclareDocumentCommand{\ArrayTop}{o m}{%
	\ArrayLastIndex[\@idx]{#2}%
	\pgfglobalkeys{\pgfkeysArrayPrefix/\@arrayName/\@idx/.get=\@value}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\@value}%
	}{\@value}%
}



\DeclareDocumentCommand{\ArrayPush}{m m}{%
	\ArrayAdd{#1}{#2}%
}

\DeclareDocumentCommand{\IfArrayEmptyTF}{m +m +m}{%
	\ArraySize[\array@ifEmptyTF@size]{#1}%
	\ifnum \array@ifEmptyTF@size = 0%
		#2%
	\else%
		#3%
	\fi%
}
\DeclareDocumentCommand{\IfArrayEmptyT}{m +m}{%
	\IfArrayEmptyTF{#1}{#2}{}%
}
\DeclareDocumentCommand{\IfArrayEmptyF}{m +m}{%
	\IfArrayEmptyTF{#1}{}{#2}%
}



\DeclareDocumentCommand{\ArrayPos}{o m m}{%
	% #1: \macro storing result (optional)
	% #2: array
	% #3: value
	%
	\ArrayLastIndex[\array@pos@lastIndex]{#2}%
	\edef\array@pos@result{-1}%
	\foreach \array@pos@i in {0, ..., \array@pos@lastIndex} {%
		\ArrayGet[\@value]{#2}{\array@pos@i}%
		%
		\ifthenelse{\equal{\@value}{#3}}%
			{%
				%\typeout{ ---> ArrayPos: needle found at position \array@pos@i}%
				\xdef\array@pos@result{\array@pos@i}%
				\breakforeach%
			}%
			{%
				%\typeout{  --> ArrayPos: needle not found at position \array@pos@i}%
			}%
	}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\array@pos@result}%
	}{\array@pos@result}%
}%

\DeclareDocumentCommand{\ArrayClear}{m}{%
	\IfArrayEmptyF{#1}{\ArrayPop{#1}\ArrayClear{#1}}%
}


\PackageInfo{MCLabPaper}{Loading Module Array done}%

==> MCLabPaper_Biblio_2.tex <==
\MCLabPaper@RequirePackage{bibunits}

\DeclareDocumentCommand{\Debug@Out@Biblio}{o m}{%
	\Debug@Out{Biblio}[#1]{#2}%
}

\ArrayNew{biblioVerbosity}
\ArrayAdd{biblioVerbosity}{XS}
\ArrayAdd{biblioVerbosity}{S}
\ArrayAdd{biblioVerbosity}{L}



\DeclareDocumentCommand{\BibliographySource}{o D<>{\Bibliography@verbosity}}{% 
	% #1: [\result] #2: verbosity}
	\edef\Biblio@sources{mclab-flattened-#2.bib}%
	\IfValueTF{#1}{%
		\edef@macro#1{\Biblio@sources}%
	}{\Biblio@sources}%
}

\edef\Biblio@additional@sources{}
\DeclareDocumentCommand{\BibliographyAddLocalSource}{m}{%
	\Debug@Out@Biblio[BibliographyAddLocalSource(#1)]{Start}%
	\GetCurrentDir[\Biblio@add@local@src@cwd]%
	\ifequals{\Biblio@additional@sources}{}{%	
		\edef\Biblio@additional@sources{\Biblio@add@local@src@cwd/#1}%
	}{%
		\edef\Biblio@additional@sources{\Biblio@additional@sources, \Biblio@add@local@src@cwd/#1}%
	}%
	\Debug@Out@Biblio[BibliographyAddLocalSource(#1)]{ - additional sources now = '\Biblio@additional@sources'}%
	\Debug@Out@Biblio[BibliographyAddLocalSource(#1)]{End}%
}%

\edef\Bibliography@style{plain}
%\newtoggle{Biblio@DefaultStyle@Set}
%\togglefalse{Biblio@DefaultStyle@Set}
\DeclareDocumentCommand{\BibliographySetStyle}{m}{%
	\edef\Bibliography@style{#1}%
		% \bibliographystyle{#1}%		
		% 	\expandafter\defaultbibliographystyle\expandafter{#1}% in case bibunits are used
		% }%
	\Debug@Out@Biblio[BibliographySetStyle(#1)]{Style set to '#1'}%
}%


\define@cmdkey{Bibliography}{verbosity}[]{}
\define@cmdkey{Bibliography}{style}[\Bibliography@style]{}
\define@boolkey{Bibliography}{usedb}[true]{}


\DeclareDocumentCommand{\Bibliography}{O{}}{%
		\setkeys{Bibliography}{usedb, style, verbosity=\Bibliography@verbosity}%
		\setkeys{Bibliography}{#1}%
		%
		\edef\Bibliography@all@sources{\Biblio@additional@sources}%
		%
		\ifKV@Bibliography@usedb%
			% Add DB file to @all@sources
			\ArrayPos[\bib@arr@pos]{biblioVerbosity}{\cmdKV@Bibliography@verbosity}%
			\ifthenelse{\bib@arr@pos = -1}{%
				\PackageError{MCLabPaper}{Biblio verbosity level 
					`\cmdKV@Bibliography@verbosity' unknown}%
					{See the manual for the allowed bibliography verbosity levels}%
			}{%
				% Get DB file of requested verbosity
				\BibliographySource[\mclab@flattened@bib@file]%
					<\cmdKV@Bibliography@verbosity>%
				%
				\ifequals{\Bibliography@all@sources}{}{%
					\edef\Bibliography@all@sources{\mclab@flattened@bib@file}%	
				}{%
					\edef\Bibliography@all@sources{\Bibliography@all@sources, \mclab@flattened@bib@file}%	
				}%				
			}%
		\fi% end if 'usedb'
		%
		\StrRemoveSpacesFromCommaSepList{\Bibliography@all@sources}{\Bibliography@all@sources}%
		%
		% Set style (store value only)
		\BibliographySetStyle{\cmdKV@Bibliography@style}%
		%
		% BibUnits: set default sources in case 
		%\defaultbibliography{\Bibliography@all@sources}%
		%
		% 
		\iftoggle{Biblio@Is@Bib@Unit}{%
			% within bibunit
			\WriteToAuxFile{%
				\csxdef{Biblio@BibUnit@style@\arabic{Biblio@BibUnit@Counter}}%
					  {\Bibliography@style}%
			}%
			\putbib[\Bibliography@all@sources]%
		}{% 
			% global bibliography
			\bibliographystyle{\Bibliography@style}%
			\bibliography{\Bibliography@all@sources}%
		}
		\if@MCLabPaper@draft%
			\iftoggle{@MCLabPaper@draft@show@buttons}{%
				\ButtonBiblioProcess%
			}{}%
		\fi%
		%
}%


\DeclareDocumentCommand{\printbibliography}{O{}}{%
	\Deprecated@Notice{Use of command printbibliography is deprecated. Use Bibliography}%
	\Bibliography[#1]%
}


% \let\BibUnits@Cite@Cmd\cite%
% \def\Biblio@Global@Cite#1{\BibUnits@Cite@Cmd*{#1}}
% \def\Biblio@Local@Cite#1{\BibUnits@Cite@Cmd{#1}}


\newtoggle{Biblio@Is@Bib@Unit}
\togglefalse{Biblio@Is@Bib@Unit}
%\let\cite\Biblio@Global@Cite
\newcounter{Biblio@BibUnit@Counter}
\setcounter{Biblio@BibUnit@Counter}{0}
\DeclareDocumentEnvironment{BibliographyUnit}{}{%
	\stepcounter{Biblio@BibUnit@Counter}%
	\ifcsundef{Biblio@BibUnit@style@\arabic{Biblio@BibUnit@Counter}}{%
		\cslet{Biblio@BibUnit@style@\arabic{Biblio@BibUnit@Counter}}%
			  {\Bibliography@style}%
	}{}%
	\bibunit[\csuse{Biblio@BibUnit@style@\arabic{Biblio@BibUnit@Counter}}]%	
	\global\toggletrue{Biblio@Is@Bib@Unit}%
	%\let\cite\Biblio@Local@Cite{#1}%
}{%
	\endbibunit%
	\togglefalse{Biblio@Is@Bib@Unit}%
}

==> MCLabPaper_Cache_2.tex <==

\MCLabPaper@Set@Tutorial@Section{Cache}{sec:cache}


\DeclareDocumentCommand{\Debug@Out@Cache}{o m}{%
	\Debug@Out{Cache}[#1]{#2}%
}

\xdef\CachePrefix{\pgfkeysPrefix/Cache}%

\DeclareDocumentCommand{\CacheOn}{O{}}{%
	% [#1] comma sep list of cache names (empty = all)
	\ifequals{#1}{}{%
		\pgfglobalkeys{\CachePrefix/default/.initial = true}%
	}{%
		\xintFor ##9 in {#1} \do{%
			\pgfglobalkeys{\CachePrefix/##9/.initial = true}%
		}%
	}%
}%


\providetoggle{CacheEnabled}
\DeclareDocumentCommand{\IfCacheEnabledTF}{m +m +m}{%
	% #1 : cache name
	% #2 : code if cache true
	% #3 : code if cache false
	\pgfglobalkeysifdefined{\CachePrefix/default}{%
		\pgfglobalkeys{\CachePrefix/default/.get = \CacheEnabled@value}%
		\settoggle{CacheEnabled}{\CacheEnabled@value}%
	}{}%
	\pgfglobalkeysifdefined{\CachePrefix/#1}{%
		% override default
		\pgfglobalkeys{\CachePrefix/#1/.get = \CacheEnabled@value}%
		\settoggle{CacheEnabled}{\CacheEnabled@value}%	
	}{}%
	\iftoggle{CacheEnabled}{%
		\Debug@Out@Cache[IfCacheEnabledTF{#1}]{Cache enabled}%
		#2%
	}{
		\Debug@Out@Cache[IfCacheEnabledTF{#1}]{Cache disabled}%
		#3%
	}%
}

\newcommand{\Cache@File@Name}[1]{\jobname.#1.cache.aux}

\DeclareDocumentCommand{\CacheOrDo}{m +m}{%
	% #1: cache name
	% #2: what to do if cache is disabled or does not exist (it also stores in cache)
	\IfCacheEnabledTF{#1}{%
		%... load from cache
		\IfFileExists{\Cache@File@Name{#1}}{%
			\Debug@Out@Cache[CacheOrDo]{Reading from cache file \Cache@File@Name{#1}}%
			\input{\Cache@File@Name{#1}}%
			\Debug@Out@Cache[CacheOrDo]{Done reading from cache file \Cache@File@Name{#1}}%
		}{%
			\Debug@Out@Cache[CacheOrDo]{Cache file \Cache@File@Name{#1} does not exists: recomputing cache}%
			% real do
			#2%
		}%
	}{%
		% real do
		\Debug@Out@Cache[CacheOrDo]{No caching enabled for '#1'.}%
		#2%
	}%
}

\DeclareDocumentCommand{\CacheFileOpen}{m m D(){}}{%
	% #1: \handler  
	% #2: cache name
	% #3: (options)
	\FileOpen{#1}(#3){\Cache@File@Name{#2}}%
}

%\DeclareDocumentCommand{\CacheFileClose}{m}{%
%	\FileClose{\Cache@File@Name{#1}}%
%}

==> MCLabPaper_Capitalise_2.tex <==
\MCLabPaper@Set@Tutorial@Section{Capitalise}{sec:capitalise}

\MCLabPaper@RequirePackage{mfirstuc}

\addto\captionsenglish{%
	\MFUclear
	\MFUnocap{a}
	\MFUnocap{an}
	\MFUnocap{and}
	\MFUnocap{but}
	\MFUnocap{for}
	\MFUnocap{in}
	\MFUnocap{of}
	\MFUnocap{or}
	\MFUnocap{no}
	\MFUnocap{nor}
	\MFUnocap{so}
	\MFUnocap{some}
	\MFUnocap{the}
	\MFUnocap{with}
	\MFUnocap{yet}
}


\addto\captionsitalian{%
	\MFUclear
	\MFUnocap{il}
	\MFUnocap{lo}
	\MFUnocap{la}
	\MFUnocap{i}
	\MFUnocap{gli}
	\MFUnocap{le}
	\MFUnocap{un}
	\MFUnocap{uno}
	\MFUnocap{una}
	\MFUnocap{di}
	\MFUnocap{a}
	\MFUnocap{da}
	\MFUnocap{in}
	\MFUnocap{con}
	\MFUnocap{su}
	\MFUnocap{per}
	\MFUnocap{tra}
	\MFUnocap{fra}
}

%API from mfirstuc
%\[e]capitalisewords#1
%\[e]makefirstuc#1



\DeclareDocumentCommand{\Debug@Out@Capitalise}{o m}{%
	\Debug@Out{Capitalise}[#1]{#2}%
}

\DeclareDocumentCommand{\CapitaliseFirst}{o m}{%
	% [#1]: \result
	% #2: word
	\IfValueTF{#1}{%
		\edef@macro{#1}{\emakefirstuc{#2}}%
	}{\emakefirstuc{#2}}%
}

\DeclareDocumentCommand{\CapitaliseFirstAll}{o m}{%
	% [#1]: \result
	% #2: word
	\IfValueTF{#1}{%
		\edef@macro{#1}{\ecapitalisewords{#2}}%
	}{\ecapitalisewords{#2}}%
}


==> MCLabPaper_CommaSepList_2.tex <==
\PackageInfo{MCLabPaper}{Loading Module CommaSepList}%

\DeclareDocumentCommand{\Debug@Out@CommaSepList}{o m}{%
	\Debug@Out{CommaSepList}[#1]{#2}%
}

\xdef\commaSepListPrefix{\pgfkeysPrefix/CommaSepLists}%

% Create a new csl using name 'name'
% eg., \CommaSepListNew{my list}
\DeclareDocumentCommand{\CommaSepListNew}{m}{%
	%#1 : list name
	\pgfglobalkeys{\commaSepListPrefix/#1/.initial = {}}%
}	

% Put content of list #1 into macro #2
% eg., \CommaSepList{my list}{\mylist}
\DeclareDocumentCommand{\CommaSepList}{m m}{%
	\pgfglobalkeys{\commaSepListPrefix/#1/.get = #2}%
}
	
% Append #3 to csl #1 using handlers #2
% e.g., \CommaSepListsAppend{my list}{my new item}
% e.g., \CommaSepListsAppend{my list}[./expanded]{\mynewitem}
\DeclareDocumentCommand{\CommaSepListAppend}{m O{} m}{%
	% #1: list name 
	% #1: handlers (/.expanded, /.expand once, etc.)
	% #3: value
	\Debug@Out@CommaSepList[CommaSepListAppend(#1)[#2](#3)]{Start}%
	\pgfglobalkeys{\commaSepListPrefix/#1/.append to list#2 = #3}%
	\pgfglobalkeys{\commaSepListPrefix/#1/.get = \cslaList}%
	\Debug@Out@CommaSepList[CommaSepListAppend(#1)[#2](#3)]{End --> now list is: [\cslaList]}%
}

% Store size of list #2 in macro #1
% eg., \CommaSepListsSize[\listsize]{my list}
\DeclareDocumentCommand{\CommaSepListSize}{o m}{%
  {%\begingroup%
	\CommaSepList{#2}{\CommaSepListSize@list}%
	\IfValueTF{#1}{% value to be stored into macro
		\Comma@Sep@List@Size@raw[#1]{\CommaSepListSize@list}%
	}{%
		\Comma@Sep@List@Size@raw{\CommaSepListSize@list}%
	}%
  }%\endgroup%
}

%% Returns in #1 (or displays, if #1 is not given) the number of elements in #2 (separated by ',')
\newcounter{MCLab@CSL@size@cnt}%
\DeclareDocumentCommand{\Comma@Sep@List@Size@raw}{o m}{%
  {%\begingroup%
	\setcounter{MCLab@CSL@size@cnt}{0}%
	\xintFor ##9 in {#2} \do{%
		%(##9)%
		\stepcounter{MCLab@CSL@size@cnt}%
	}%
	\IfValueTF{#1}{% value to be stored into macro
		\xdef@macro{#1}{\theMCLab@CSL@size@cnt}%		
	}{%
		\theMCLab@CSL@size@cnt%
	}%
  }%\endgroup%
}


\addto\captionsenglish{%
  \def\MCLabPaper@and{and}%
}
\addto\captionsitalian{%
  \def\MCLabPaper@and{e}%
}

\DeclareDocumentCommand{\CommaSepListToProse}{o m}{%
	% #1: [\result]
	% #2: a list name (within pgfglobalkeys) or an explicit list "first, second, ..."
	\Debug@Out@CommaSepList[CommaSepListToProse(#2)]{Start}%
	\def\csltp@result{}%
	\pgfglobalkeysifdefined{\commaSepListPrefix/{#2}}{%
		\Debug@Out@CommaSepList[CommaSepListToProse(#2)]{ --> given pgfglobalkeys list name: [#2]}%
		\pgfglobalkeys{\commaSepListPrefix/#2/.get=\csltpList}%
	}{%
		\Debug@Out@CommaSepList[CommaSepListToProse(#2)]{ --> explicit list given [#2]}%
		\edef\csltpList{#2}%
	}%
	\xintFor ##9 in {\csltpList} \do{%
		\Debug@Out@CommaSepList[CommaSepListToProse(#2)]{ - processing item '##9'}%
		\xintifForLast{%
			\edef\@csltp@sep{\space\MCLabPaper@and\space}%
		}{%
			\edef\@csltp@sep{,\space}%
		}%
		\ifequals{\csltp@result}{}{%
			% prev. list is empty --> no separator		
			\edef\@csltp@sep{}%
		}{}%
		\Debug@Out@CommaSepList[CommaSepListToProse(#2)]{    --> separator before last item: [\@csltp@sep]}%		
		\protected@eappto{\csltp@result}{\@csltp@sep##9}%
		\Debug@Out@CommaSepList[CommaSepListToProse(#2)]{    --> now prose is: [\csltp@result]}%		
	}%
	\IfValueTF{#1}{% value to be stored into macro
		\expandafter\protected@xdef\csname\expandafter\@gobble\string#1\endcsname{\csltp@result}%
	}{%
		\csltp@result%
	}%
}


\PackageInfo{MCLabPaper}{Loading Module CommaSepList done}%

\endinput

%%%%OLD IMPLEMENTATION




\DeclareDocumentCommand{\CommaSepListNew}{m}{%
	%#1 : \macro
	\xdef@macro{#1}{}%
}	

\DeclareDocumentCommand{\CommaSepListAppend}{m m}{%
	\ifdefempty{#1}{%
		\xdef@macro{#1}{#2}%
	}{%
		\xdef@macro{#1}{#1,#2}%
	}%
}


\addto\captionsenglish{%
  \def\MCLabPaper@and{and}%
}
\addto\captionsitalian{%
  \def\MCLabPaper@and{e}%
}

\DeclareDocumentCommand{\CommaSepListToProse}{o m}{%
	\Debug@Out@CommaSepList{CommaSepListToProse(#2):}%
	\def\csltp@result{}%
	\xintFor ##9 in {#2} \do{%
		\Debug@Out@CommaSepList{ - processing item '##9'}%
		\xintifForLast{%
			\edef\@csltp@sep{\space\MCLabPaper@and\space}%
		}{%
			\edef\@csltp@sep{,\space}%
		}%
		\ifequals{\csltp@result}{}{%
			% prev. list is empty --> no separator		
			\edef\@csltp@sep{}%
		}{}%
		\Debug@Out@CommaSepList{    --> separator before last item: [\@csltp@sep]}%		
		\protected@eappto{\csltp@result}{\@csltp@sep##9}%
		\Debug@Out@CommaSepList{    --> now prose is: [\csltp@result]}%		
	}%
	\IfValueTF{#1}{% value to be stored into macro
		\expandafter\protected@xdef\csname\expandafter\@gobble\string#1\endcsname{\csltp@result}%
	}{%
		\csltp@result%
	}%
%	
%	
%	\CommaSepListSize[\MCLab@CSL@size]{\MCLab@CSL@list}%
%	%[\MCLab@CSL@size]
%	\ifthenelse{\MCLab@CSL@size=1}{%
%		#1%
%	}{%		
%		\foreach \@item [count=\MCLab@CSL@cnt] in \MCLab@CSL@list {%
%			\ifthenelse{\MCLab@CSL@cnt=\MCLab@CSL@size}{%
%					{} \MCLabPaper@and~%
%			}{%
%					\ifthenelse{\MCLab@CSL@cnt > 1}{,\space}{}%
%			}%
%			%
%			\@item%
%			%\DraftNote*{\@label}%
%		}%
%	}%
	%\xspace%
}%




==> MCLabPaper_Compact_2.tex <==

\MCLabPaper@Set@Tutorial@Section{Compact}{sec:compact}

\newif\ifcompactexpressions\compactexpressionsfalse

\define@boolkey{CompactOn}{expressions}[true]
	{\csname compactexpressions#1\endcsname}

\define@key{CompactOn}{abovecaption}[0pt]{%
	\addtolength{\abovecaptionskip}{-#1}%
}
\define@key{CompactOn}{belowcaption}[0pt]{%
	\addtolength{\belowcaptionskip}{-#1}%
}
\define@key{CompactOn}{stretch}[1]{%
	\renewcommand{\baselinestretch}{#1}%
}
\define@key{CompactOn}{parskip}[0pt]{%
	\addtolength{\parskip}{-#1}%
}

\gdef\Bibliography@verbosity{L}%
\define@key{CompactOn}{bibliography}[L]{%
	\gdef\Bibliography@verbosity{#1}%
}%



\DeclareDocumentCommand{\CompactOn}{m}{%
	\setkeys{CompactOn}{expressions, bibliography, abovecaption, belowcaption, stretch, parskip}% %defaults
	\setkeys{CompactOn}{#1}%
}	

\DeclareDocumentCommand{\SetCompact}{m}{%
	\DiagDeprecationSimple{Compact}{SetCompact}{CompactOn}%
	\CompactOn{#1}%
}




%\def\paragraph*#1{\par\bigskip\noindent\textbf{#1.}~}
%\def\subparagraph#1{#1}
%\def\subparagraph*#1{#1}
%\usepackage[compact]{titlesec}
%\titlespacing{\section}{0pt}{2ex}{1ex}
%\titlespacing{\subsection}{0pt}{1ex}{0ex}
%\titlespacing{\subsubsection}{0pt}{0.5ex}{0ex}
%\renewcommand{\baselinestretch}{0.978}
%\addtolength{\abovecaptionskip}{-5pt}
%\addtolength{\belowcaptionskip}{-10pt}
%\addtolength{\parskip}{-2pt}



%\DeclareDocumentCommand\SetCompact{m}{%	
%	\foreach \@c in {#1} {%
%		\ifthenelse{\equal{#1}{expressions}}{%
%			\@SystemNote{Compact mode ``expressions'' enabled}%		
%			\global\compactexpressionstrue%
%		}{}%
%		\ifthenelse{\equal{#1}{expressions}}{%
%			\@SystemNote{Compact mode ``expressions'' enabled}%		
%			\global\compactexpressionstrue%
%		}{}%
%		
%	}%
%}





\definecolor{compact-expression}{rgb}{0.0, 0.6, 0.6}
\DeclareDocumentCommand{\CompactDefineExpression}{m o m}{%
	% #1: command
	% #2: compact (optional)
	% #3: full 
	\expandafter\DeclareDocumentCommand{#1}{s}{%
		\ifcompactexpressions%
			\IfBooleanTF{##1}{%
				\Draft@Highlight{compact-expression}{#3}%
			}{%
				\IfValueTF{#2}{%
					\Draft@Highlight{compact-expression}{#2}%
				}{%
					\Draft@Highlight{compact-expression}{#3}%
				}%
			}%
		\else%
			\Draft@Highlight{compact-expression}{#3}%
		\fi%
		\xspace%
	}%
}

\DeclareDocumentCommand{\DefineCompactExpression}{m o m}{%
	\DiagDeprecationSimple{Compact}{DefineCompactExpression}{CompactDefineExpression}%
	\CompactDefineExpression{#1}[#2]{#3}%
}

\addto\captionsenglish{		
	\CompactDefineExpression{\wrt}[wrt.]{with respect to}
	\CompactDefineExpression{\wlossgen}[wlog.]{without loss of generality}
	\CompactDefineExpression{\respectively}[resp.]{respectively}
	\CompactDefineExpression{\eg}{\textit{e.g.},}
	\CompactDefineExpression{\ie}{\textit{i.e.},}
	\CompactDefineExpression{\suchthat}[s.t.]{such that}		
	\CompactDefineExpression{\ifandonlyif}[iff]{if and only if}		
}
\addto\captionsitalian{		
	\CompactDefineExpression{\wrt}[rispetto a]{rispetto a}
	\CompactDefineExpression{\wlossgen}[senza perdita di generalit\`a]{senza perdita di generalit\`a}
	\CompactDefineExpression{\respectively}[risp.]{rispettivamente}
	\CompactDefineExpression{\eg}{\textit{p.es.},}
	\CompactDefineExpression{\ie}{\textit{i.e.},}
	\CompactDefineExpression{\suchthat}[t.c.]{tale che}		
	\CompactDefineExpression{\ifandonlyif}[sse]{se e solo se}		
}


\def\defaultthickmuskip{\thickmuskip}
\def\defaultmedmuskip{\medmuskip}

\def\compactthickmuskip{1mu plus 1mu minus 2mu}
\def\compactmedmuskip{1mu plus 1mu minus 2mu}


\DeclareDocumentCommand\CompactMath{+m}{%	
	\begingroup
		\thickmuskip=\compactthickmuskip%
		\medmuskip=\compactmedmuskip%
		%
		#1%
	\endgroup%
}


==> MCLabPaper_Data_2.tex <==

\DeclareDocumentCommand{\Debug@Out@Data}{o m}{%
	\Debug@Out{Data}[#1]{#2}%
}


\edef\Data@FileName{\jobname.data}
\newif\if@Data@Frozen
\@Data@Frozenfalse
\newcommand{\DataFrozen}{%
	\@Data@Frozentrue%
	\IfFileExists{\Data@FileName}{%
		\Debug@Out@Data[DataFrozen]{Reading existing file '\Data@FileName'}%
		\input{\Data@FileName}%
	}{}%
}

\newwrite\@Data@File
\newtoggle{Data File Open}
\settoggle{Data File Open}{false}
\newcommand{\Add@To@Data@File}[1]{%
	\iftoggle{Data File Open}{}{%
		\immediate\openout\@Data@File=\Data@FileName%
		\settoggle{Data File Open}{true}%
	}%
	\write\@Data@File{#1}%
}



\DeclareDocumentCommand{\Data@Next@Data@csname}{o m}{%
	% [#1]: \result
	% #2: prefix, e.g., command name storing data, as DataGet or DataChildren
	\InputCurrentFilePath[\Data@infile]%
	\FileModTimeStamp[\Data@timestamp]{\Data@infile}%
	\xdef\Data@Next@Data@csname@result{#2:\Data@infile:\csuse{the#2Cnt}:\Data@timestamp}%
	\stepcounter{#2Cnt}%
	\IfValueTF{#1}{%
		\xdef@macro{#1}{\Data@Next@Data@csname@result}%
	}{\Data@Next@Data@csname@result}%
}



\xdef\DataPrefix{\pgfkeysPrefix/Data/}

\input{MCLabPaper_Data_Utils_\MCLabPaper@file@suffix.tex}
\input{MCLabPaper_Data_Metadata_\MCLabPaper@file@suffix.tex}
\input{MCLabPaper_Data_Get_\MCLabPaper@file@suffix.tex}

\input{MCLabPaper_Data_Put_\MCLabPaper@file@suffix.tex}
\input{MCLabPaper_Data_Input_\MCLabPaper@file@suffix.tex}



==> MCLabPaper_Data_Get_2.tex <==
\define@cmdkey{DataGet}{pretty}[]{}


\DeclareDocumentCommand{\DataGetCheckType}{o m m}{%
	% #1: [\result]: 0 = ok, a negative integer = error
	% #2: value
	% #3: type
	%\Debug@Out@Data[{DataGetCheckType[...]{#2}{#3}}]{Start}%
	\edef\DataGet@Check@Type@Result{}%
	\ifcsdef{DataGetCheckType@#3}{%
		\csuse{DataGetCheckType@#3}{\DataGet@Check@Type@Result}{#2}%
		\edef@macro{#1}{\DataGet@Check@Type@Result}%
	}{%
		\InputCurrentFilePath[\tmp@curr@file]%
		\DiagError{Data}{DataCheckType: type '#3' not recognised in file \RenderFileName{\tmp@curr@file}.}%
			[DataCheckType: type '#3' not recognised in file \tmp@curr@file]
	}%
}

\DeclareDocumentCommand{\DataGetCheckType@int}{m m}{%
	% #1: {\result}
	% #2: value
	\IfInteger{#2}{%
		\edef@macro{\DataGet@Check@Type@Result}{0}%
	}{%
		\edef@macro{\DataGet@Check@Type@Result}{-1}%
	}%
}
\DeclareDocumentCommand{\DataGetCheckType@real}{m m}{%
	% #1: {\result}
	% #2: value
	\IfDecimal{#2}{%
		\edef@macro{\DataGet@Check@Type@Result}{0}%
	}{%
		\edef@macro{\DataGet@Check@Type@Result}{-1}%
	}%
}
\DeclareDocumentCommand{\DataGetCheckType@nonempty}{m m}{%
	% #1: {\result}
	% #2: value
	\ifequals{#2}{}{%
		\Debug@Out@Data[DataGetCheckType]{'#2' is empty}%
		\edef@macro{\DataGet@Check@Type@Result}{-1}%
	}{%	
		%\Debug@Out@Data[DataGetCheckType]{'#2' is not empty}%
		\edef@macro{\DataGet@Check@Type@Result}{0}%
	}%
}
\DeclareDocumentCommand{\DataGetCheckType@any}{m m}{%
	% #1: {\result}
	% #2: value
	\edef@macro{\DataGet@Check@Type@Result}{0}%
}

%\newcounter{DataGetCnt}
%\setcounter{DataGetCnt}{0}

\define@boolkey{DataGet}{die}[true]{}
\define@boolkey{DataGet}{global}[false]{}
\define@cmdkey{DataGet}{checktype}[any]{}
\DeclareDocumentCommand{\DataGet}{o D(){} D<>{} m}{%
	% #1 [\result]
	% #2 (options): die=true|false, global=true|false
	% #3 <prefix>
	% #4 {key}
	%
	\setkeys{DataGet}{pretty, die, global, checktype}%	
	\setkeys{DataGet}{#2}%	
	\xdef\DataGet@user@prefix{#3}%
	%
	\Debug@Out@Data[DataGet(#2)<#3>{#4}]{Start}%
	%
	\DataNormalisePrefix{\DataGet@user@prefix}{\DataGet@user@prefix}%
	\xdef\DataGet@key{#4}%	
	\Debug@Out@Data[DataGet(#2)<\DataGet@user@prefix>%
		{\DataGet@key}]{Prefix normalised}%	
	%
	% check whether key is defined
	\DataIfKeyDefinedTF<\DataGet@user@prefix>{\DataGet@key}{%		
		\pgfglobalkeys{\DataPrefix\DataGet@user@prefix\DataGet@key/.get=%
			\DataGet@value}%
			%\Debug@Out@Data[DataGet(#2)<\DataGet@user@prefix>{\DataGet@key}]{  --> '\RenderLatex{\DataGet@value}'}%
		%		
		% Check that value type is as required	
		\DataGetCheckType[\tmp@error]{\DataGet@value}{\cmdKV@DataGet@checktype}%
		\ifnumless{\tmp@error}{0}{%
			\InputCurrentFilePath[\tmp@curr@file]%
			\DiagError{Data}{%
				Your command \DiagLatexCmd{DataGet(#2)<#3>\{#4\}} in file \RenderFileName{\tmp@curr@file} tries to read stored value '\DataGet@value' as if it were of type \cmdKV@DataGet@checktype.}%
				[Your command \string\DataGet(#2)<#3>{#4} in file \tmp@curr@file\space tries to read stored value '\RenderLatex{\DataGet@value}' as if it were of type \cmdKV@DataGet@checktype]%
		}{}%
		%
		%
		%
		\IfValueTF{#1}{%
			% returning value into macro #1
			%\Debug@Out@Data[DataGet(#2)<\DataGet@user@prefix>{\DataGet@key}]{Returning value [\RenderLatex{\DataGet@value}] into macro}%
			%
			\ifKV@DataGet@global
				\xdef@macro{#1}{\expandonce\DataGet@value}%
			\else%
				\edef@macro{#1}{\expandonce\DataGet@value}%
			\fi%
		}{%
			%
			% sending value to text-flow			
			\Debug@Out@Data[DataGet(#2)<\DataGet@user@prefix>{\DataGet@key}]{- sending value to text-flow (pretty option = '\cmdKV@DataGet@pretty')}%
			\IfStrEq{\cmdKV@DataGet@pretty}{none}{%
				\Draft@Data{\DataGet@value}%
			}{%
				\def\DataGet@pretty@db{}%
				\DataIfKeyDefinedTF<\DataGet@user@prefix>{\DataGet@key/pretty}{%
					\pgfglobalkeys{%
						\DataPrefix%
						\DataGet@user@prefix\DataGet@key/%
						pretty/.get=%
							\DataGet@pretty@db%
					}%
					\Debug@Out@Data[DataGet(#2)<\DataGet@user@prefix>{\DataGet@key}]{- pretty-printing options defined in key 
						'\DataGet@user@prefix\DataGet@key/%
							pretty': '\DataGet@pretty@db'}%
				}{%			
					\Debug@Out@Data[DataGet(#2)<\DataGet@user@prefix>{\DataGet@key}]{ - no pretty-printing options defined 
						(key '\DataGet@user@prefix\DataGet@key/%
							pretty' does not exist)}%
				}%
				%
				\edef\DataGet@pretty{\DataGet@pretty@db, 
					\cmdKV@DataGet@pretty}%
				\Draft@Data{\Pretty[\DataGet@pretty]{\DataGet@value}}%
				%					
			}%
			%
			%
		}%
	}{%
		% key not defined
		%
		%\InputCurrentFilePath[\tmp@curr@file]%
		\DiagError*(die=\ifKV@DataGet@die true\else false\fi){Data}{%
				Your command \DiagLatexCmd{DataGet(#2)<#3>\{#4\}} tries to get an undefined key}%
				[Your command \string\DataGet(#2)<#3>{#4} tries to get an undefined key]%		
	}%
\Debug@Out@Data[DataGet(#2)<#3>{#4}]{end.}%							
}


\DeclareDocumentCommand{\DataGetDieOnMissingKeyOn}{}{%
	%\define@cmdkey{DataGet}{dieifundefined}[true]{}
}
\DeclareDocumentCommand{\DataGetDieOnMissingKeyOff}{}{%
	%\define@cmdkey{DataGet}{dieifundefined}[false]{}
}

==> MCLabPaper_Data_Input_2.tex <==
% Possible DB file encodings
%\newcommand{\Data@Input@encoding@latex}{}
\newcommand{\Data@Input@encoding@text}{%
	\catcode`_=12%
	%\catcode`\\=12%
	%\catcode`\{=12%
	%\catcode`\}=12%
	%\catcode`\==12%
}

\newcommand{\Data@Input@encoding@latex}{%
	% do nothing
}





\define@cmdkey{DataInput}{format}[kvp]{}
\define@cmdkey{DataInput}{encoding}[text]{}
\define@cmdkey{DataInput}{key}[]{}
\define@cmdkey{DataInput}{absolute}[false]{}


\input{MCLabPaper_Data_Input_KVP_\MCLabPaper@file@suffix.tex}	
\input{MCLabPaper_Data_Input_CSV_\MCLabPaper@file@suffix.tex}	

\providetoggle{DataInputAbsolute}

\DeclareDocumentCommand{\DataInput}{O{} D<>{} m}{%
	%#1: options, <#2: optional prefix,  #3: rel/path/to/filename
	\if@Data@Frozen%
		\PackageWarning{MCLabPaper}{DataInput: skipping \string\DataInput[#1]<#2>{#3} as data files have been declared to be frozen}%
	\else%
		\setkeys{DataInput}{key, format, encoding, absolute}%	
		\setkeys{DataInput}{key=rows, #1}%
		\settoggle{DataInputAbsolute}{\cmdKV@DataInput@absolute}
		\DataNormalisePrefix{\DataInput@user@prefix}{#2}%
		%
		\bgroup%
			\iftoggle{DataInputAbsolute}{%
				\def\DataInput@file{#3}%
			}{%
				\GetCurrentDir[\DataInput@cwd]%
				\def\DataInput@file{\DataInput@cwd/#3}%
			}%
			%	
			\IfFileExists{\DataInput@file}{%
				% file exists
				\Debug@Out@Data[DataInput]{I'm going to open file '\DataInput@file'}%
				\Debug@Out@Data[DataInput]{ - format: '\cmdKV@DataInput@format'}%
				\Debug@Out@Data[DataInput]{ - encoding: '\cmdKV@DataInput@encoding'}%
				\Debug@Out@Data[DataInput]{ - prefix: '\DataInput@user@prefix'}%
				\Debug@Out@Data[DataInput]{ --> running 
					DataInput@\cmdKV@DataInput@format}%
				\def\DataInput@method{DataInput@\cmdKV@DataInput@format}%
				\ifcsdef{\DataInput@method}{%
					% set encoding
					\ifcsdef{Data@Input@encoding@\cmdKV@DataInput@encoding}{%
						\csuse{Data@Input@encoding@\cmdKV@DataInput@encoding}%
					}{%
						\DiagError{Data}{Command \DataInput[#1]<#2>{#3}.
						Cannot input database file: unknown encoding `\cmdKV@DataInput@encoding'}%
					}%
					% run format-specific function
					\csuse{\DataInput@method}<\DataInput@user@prefix>{\DataInput@file}% 
				}{%
					\DiagError{Data}{Command \DataInput[#1]<#2>{#3}.
						Cannot input database file: unknown format `\cmdKV@DataInput@format'}%
				}%
			}{%
				\DiagError{Data}{Command \DataInput[#1]<#2>{#3}.
						Cannot input database file: file `\DataInput@file' does not exist}%
			}%
		\egroup%
	\fi%
}%



==> MCLabPaper_Data_Input_CSV_2.tex <==
\let\DataToolLoadDBCommand\relax%
\let\Par\DTLpar%

\newcommand{\Data@Input@csv@encoding@text}{%
	\Debug@Out@Data[Data@Input@csv@encoding@text]{ - text encoding: specifying mapping of special chars}%
%	\DTLrawmap{à}{\`a}%
%	\DTLrawmap{è}{\`e}%
	\DTLrawmap{|par|}{\DTLpar}%
	\DTLrawmap{|Par|}{\DTLpar}%
	\global\let\DataToolLoadDBCommand\DTLloadrawdb%
}

\newcommand{\Data@Input@csv@encoding@latex}{%
	\Debug@Out@Data[Data@Input@csv@encoding@latex]{ - Latex encoding: specifying mapping of special chars}%
	\global\let\DataToolLoadDBCommand\DTLloaddb%
}



\DeclareDocumentCommand{\DataInput@csv}{D<>{} m}{%
	% #1: <prefix>
	%#2: full path to filename
	% (options come from \DataInput): \cmdKV@DataInput@key
	%
	\def\DataInput@csv@prefix{#1}%
	\edef\DataInput@csv@file{#2}%
	%
	% we already know that file exists
	\Debug@Out@Data[DataInput@csv]{Opening file '\DataInput@csv@file'}%
	%
	%
	% Handle special chars in file, as by 'encoding'
	\Debug@Out@Data[DataInput@csv]{=============================}	
	\ifcsdef{Data@Input@csv@encoding@\cmdKV@DataInput@encoding}{%	
		\csuse{Data@Input@csv@encoding@\cmdKV@DataInput@encoding}%
	}{%
		\DiagError{Data}{Encoding `\cmdKV@DataInput@encoding' unknown}%
	}
	\Debug@Out@Data[DataInput@csv]{---------------}%	
	%
	\DataToolLoadDBCommand{tempDB}{\DataInput@csv@file}%
	%
	\Debug@Out@Data[DataInput@csv]{ - File read}%
	%
%	%define 'key' field
	\DTLifhaskey{tempDB}{\cmdKV@DataInput@key}{%
		% key is a column of the CSV file
		\DTLgetcolumnindex{\csv@key@col@idx}{tempDB}{\cmdKV@DataInput@key}%
			\Debug@Out@Data[DataInput@csv]{   - key col idx: '\csv@key@col@idx'}%
		\def\DataInput@csv@key@value##1{%
			\DTLgetvalue{\csv@thisKeyValue}{tempDB}{\DTLcurrentindex}%
				{\csv@key@col@idx}%
			\Debug@Out@Data[DataInput@csv]{   - key value of current row: [\csv@thisKeyValue]}%
			\edef@macro{##1}{\cmdKV@DataInput@key/\csv@thisKeyValue}%
		}%
	}{%
		% key is NOT a column of the CSV file
		\def\DataInput@csv@key@value##1{%
			\Debug@Out@Data[DataInput@csv]{   - key value of current row: 
				[\cmdKV@DataInput@key/\DTLcurrentindex]}%
			\edef@macro{##1}{\cmdKV@DataInput@key/\DTLcurrentindex}%
		}%	
	}%
	%	
	\DTLforeach*{tempDB}{}{%
		\Debug@Out@Data[DataInput@csv]{ - Processing new line from CSV:}%
		%
		% Get value of 'key' field (if \cmdKV@DataInput@key != empty)
%		\ifequals{\cmdKV@DataInput@key}{}{%
%			% \DataInput@csv@key@value already assigned
%		}{%
%			\DTLgetcolumnindex{\thisKeyColIdx}{tempDB}{\cmdKV@DataInput@key}%
%			\Debug@Out@Data{   - key col idx: '\thisKeyColIdx'}%
%			\DTLgetvalue{\thisKeyValue}{tempDB}{\DTLcurrentindex}{\thisKeyColIdx}%
%			\Debug@Out@Data{   - key value of current row: [\thisKeyValue]}%
%			\def\DataInput@csv@key@value{\cmdKV@DataInput@key/%
%				\thisKeyValue}%
%		}%
		%
		\DataInput@csv@key@value{\this@key@value}%
		\DTLforeachkeyinrow{\thisColValue}{%
			% current field is in \dtlkey
			% current field number is \dtlcol
			% current field header is \dtlheader
			\Debug@Out@Data[DataInput@csv]{    - column found: 
				(dtlkey=\dtlkey, dtlcol=\dtlcol, dtlheader=\dtlheader, value=\thisColValue)}%
			\DataPut<\DataInput@csv@prefix\this@key@value>%
				{\dtlkey/.expand once = \thisColValue}%
		}%
	}%
	\DTLgdeletedb{tempDB}%
}
\endinput	


%		
%		%
%			%
%			%	(dtlkey=\dtlkey, dtlcol=\dtlcol, dtlheader=\dtlheader, value=\thisColValue)}%
%			%
%		%}%
%		\Debug@Out@Data{}%
%	}%
%	\DTLgdeletedb{tempDB}%
}%



==> MCLabPaper_Data_Input_KVP_2.tex <==
\newread\MCLab@Data@input@file%
\DeclareDocumentCommand{\DataInput@kvp}{D<>{} m}{%
	% #1: <prefix>
	%#2: full path to filename
	% (options come from \DataInput)
	% we are already in a group
	\let\Par\par%
	\catcode`\#=14%	
	\endlinechar=-1%	
	\def\DataInput@kvp@prefix{#1}%
	\edef\DataInput@kvp@file{#2}%
	%
	% we already know that file exists	
	\openin\MCLab@Data@input@file=\DataInput@kvp@file\relax%
	\Debug@Out@Data[DataInput@kvp]{Opening file '\DataInput@kvp@file'}%
		\loop%  
			\read\MCLab@Data@input@file to \in@line%
			\Debug@Out@Data[DataInput@kvp]{}%
			\Debug@Out@Data[DataInput@kvp]{new line read}%
			\Debug@Out@Data[DataInput@kvp]{   - read line '\RenderLatex{\expandonce\in@line}'}%
			%
			\saveexpandmode%
			\expandarg%	
			\StrPosition{\in@line}{=}[\in@eq@pos]%
			\Debug@Out@Data[DataInput@kvp]{    - '=' at position: '\in@eq@pos'}%			
			\ifthenelse{\in@eq@pos = 0}{%
				\Debug@Out@Data[DataInput@kvp]{    -> no '=' --> skipping line}%
				\restoreexpandmode%
			}{%
				\StrSplit{\in@line}{\in@eq@pos}{\in@key@eq}{\in@value}%
				\StrTrim[\in@value]{\in@value}%
				\restoreexpandmode%
				\Debug@Out@Data[DataInput@kvp]{    - key (+ '='): '\in@key@eq'}%
				\Debug@Out@Data[DataInput@kvp]{    - value (trimmed): '\RenderLatex{\expandonce\in@value}'}%
				%
				% Expand "\in@key@eq{\in@value}" (i.e, '<key/.handlers> = <trimmed value>' once 
				% and put it back to \in@line
				\StrExpand[1]{\in@key@eq{\in@value}}{\in@line}%
				%
				%\edef\in@line{\in@key@eq\in@value}%
				%
				\Debug@Out@Data[DataInput@kvp]{    - final in@line: '\RenderLatex{\expandonce\in@line}'}%
				\DataPut<\DataInput@kvp@prefix>{\in@line}%
				\Debug@Out@Data[DataInput@kvp]{    --> line done}%
			}%
		\unless\ifeof\MCLab@Data@input@file%
	\repeat%
	\closein\MCLab@Data@input@file%
	\Debug@Out@Data[DataInput@kvp]{Closing file '\DataInput@kvp@file'}%    
	\Debug@Out@Data[DataInput@kvp]{End.}%
}%



==> MCLabPaper_Data_Metadata_2.tex <==

\def\Data@metadata@children@postfix{@metadata/children}
\DeclareDocumentCommand{\Data@add@child@to@metadata}{D<>{} m}{% 	
	\bgroup%
	%#1: current level
	%#2: key going to be inserted (with full user prefix)
	\DataNormalisePrefix{\Data@add@child@to@metadata@currentlevel}{#1}%	
	\edef\Data@add@child@to@metadata@key{#2}%
	\Debug@Out@Data[{Data@add@child@to@metadata<\Data@add@child@to@metadata@currentlevel>{\Data@add@child@to@metadata@key}}]{Start}%
	%
	\IfStrEq{\Data@add@child@to@metadata@key}{}{%
		% if key is empty, return;
	}{%
		\StrPosition{\Data@add@child@to@metadata@key}{/}%
			[\Data@add@child@to@metadata@pos]%
		%
		\IfEq{\Data@add@child@to@metadata@pos}{0}{%
			% no occurrence of '/': key is a leaf:
			\Debug@Out@Data[{Data@add@child@to@metadata<\Data@add@child@to@metadata@currentlevel>{\Data@add@child@to@metadata@key}}]{ - key `\Data@add@child@to@metadata@key' is leaf}%
			\DataIfKeyDefinedTF%
				<\Data@add@child@to@metadata@currentlevel>%
				{\Data@add@child@to@metadata@key}{}{%
					\DataPut(metadata=false)%
						<\Data@add@child@to@metadata@currentlevel>%
						{\Data@metadata@children@postfix/.append to list/.expanded = %
							\Data@add@child@to@metadata@key}%
				}%
		}{%
			\StrSplit{#2}{\Data@add@child@to@metadata@pos}%
				{\Data@add@child@to@metadata@prefix}%
				{\Data@add@child@to@metadata@rest}%
			\DataNormalisePrefix{\Data@add@child@to@metadata@prefix}%
				{\Data@add@child@to@metadata@prefix}%
			%
			% prefix="key/" and rest={....}
			\DataIfKeyDefinedTF{%
				\Data@add@child@to@metadata@currentlevel%
				\Data@add@child@to@metadata@prefix%
				\Data@metadata@children@postfix%
			}{%
				% prefix (=key/) already exists in DB, hence metadata are up-to-date.
			}{%
				\DataPut(metadata=false)%
					<\Data@add@child@to@metadata@currentlevel>%
					{\Data@metadata@children@postfix/.append to list/.expanded = %
						\Data@add@child@to@metadata@prefix}%
			}%
			\Data@add@child@to@metadata%
				<\Data@add@child@to@metadata@currentlevel\Data@add@child@to@metadata@prefix>%
				{\Data@add@child@to@metadata@rest}%
		}%
	}%
	\Debug@Out@Data[{Data@add@child@to@metadata<\Data@add@child@to@metadata@currentlevel>{\Data@add@child@to@metadata@key}}]{End}%
	\egroup%
}

\define@cmdkey{DataChildren}{global}[false]{}
\define@cmdkey{DataChildren}{number}[]{} % macro *name* in which to return number of children
\newtoggle{DataChildren_global}
\DeclareDocumentCommand{\DataChildren}{o D(){} D<>{} m}{%
	% #1: return macro
	% #2: (options)
	% #3: <prefix>
	% #4: key dir
	%
	\setkeys{DataChildren}{global, number}%	
	\setkeys{DataChildren}{#2}%
	%
	\DataNormalisePrefix{\DataChildren@prefix}{#3}%
	\DataNormalisePrefix{\DataChildren@fulldir}{%
		\DataChildren@prefix#4}%
	\DataIfKeyDefinedTF{%
		\DataChildren@fulldir\Data@metadata@children@postfix}{%
		\DataGet[\DataChildren@result]{%
			\DataChildren@fulldir\Data@metadata@children@postfix}%
	}{%
		\def\DataChildren@result{}%		
	}%
	%
	% Return number of children, if requested
	\Debug@Out@Data[DataChildren(#2)<#3>{#4}]{Number=\cmdKV@DataChildren@number}%
	\ifequals{\cmdKV@DataChildren@number}{\relax}{%
		\Debug@Out@Data[DataChildren(#2)<#3>{#4}]{Number of children not requested, doing nothing}%
	}{%	
		\Debug@Out@Data[DataChildren(#2)<#3>{#4}]{Number of children requested to be stored into macro named \cmdKV@DataChildren@number}%
		\Comma@Sep@List@Size@raw[\DataChildren@result@number]{\DataChildren@result}%
		\Debug@Out@Data[DataChildren(#2)<#3>{#4}]{Number of children is \DataChildren@result@number}%
		%
		\csedef{\cmdKV@DataChildren@number}{\DataChildren@result@number}%
	}%
	%
	\IfValueTF{#1}{%
		\settoggle{DataChildren_global}{\cmdKV@DataChildren@global}%
		\iftoggle{DataChildren_global}{%
			\xdef@macro{#1}{\expandonce\DataChildren@result}%
		}{%
			\edef@macro{#1}{\expandonce\DataChildren@result}%
		}%
	}{%
		\DataChildren@result%
	}%
}

\DeclareDocumentCommand{\DataIfHasChildrenTF}{D<>{} m +m +m}{%
	% #1: <prefix>
	% #2: key
	% #3: then branch
	% #4: else branch
	\DataChildren[\Data@IfHasChildren]<#1>{#2}%
	\ifequals{\Data@IfHasChildren}{}{#4}{#3}%
}	

\newlist{data-print-all-description-list}{itemize}{20}
\setlist[data-print-all-description-list]{label={-}}

\DeclareDocumentCommand{\DataPrintAll}{D<>{} O{supercompact, align=left}}{%
	% #1: <initial prefix> (only this subtree is printed)
	% #2: list style
	\DataNormalisePrefix{\DataPrintAll@prefix}{#1}%
	\ifequals{\DataPrintAll@prefix}{}{%
		\DataPrintAll@Rec<\DataPrintAll@prefix>%
	}{%
		% initial prefix not-empty
		\begin{data-print-all-description-list}[#2]%
		\item \textbf{\DataPrintAll@prefix}\mbox{}%
			\DataPrintAll@Rec<\DataPrintAll@prefix>[#2]%
		\end{data-print-all-description-list}
	}%
}

\DeclareDocumentCommand{\DataPrintAll@Rec}{D<>{} O{}}{%
	% #1: common prefix
	% #2: list style
	\DataNormalisePrefix{\DataPrintAll@Rec@prefix}{#1}%
	%
	\DataChildren[\DataPrintAll@Rec@children]%
		{\DataPrintAll@Rec@prefix}%
	\ifequals{\DataPrintAll@Rec@children}{}{%
		% no children -> do nothing
	}{%
		\begin{data-print-all-description-list}[#2]%
		\xintFor ##9 in {\DataPrintAll@Rec@children} \do{%
			\item \textbf{##9}
			%\Debug@Out@Data{DataPrintAll: ##9}%
			\IfEndWith{##9}{/}{%
				\mbox{}% % to make a new line
				\bgroup
					%\Debug@Out@Data{DataPrintAll: recursing...}%
					\DataPrintAll@Rec<\DataPrintAll@Rec@prefix##9>[#2]%
				\egroup
			}{%
				\DataGet[\DataPrintAll@value]%
					<\DataPrintAll@Rec@prefix>{##9}%
				`\DataPrintAll@value'%
			}%
		}%
		\end{data-print-all-description-list}%
	}%
}


\DeclareDocumentCommand{\DataSave}{D<>{} m}{%
	% #1: <initial prefix> (only this subtree is stored)
	% #2: \fileHandler
	\DataNormalisePrefix{\DataSave@prefix}{#1}%
	\DataSave@Rec<\DataSave@prefix>{#2}%
}

\DeclareDocumentCommand{\DataSave@Rec}{D<>{} m}{%
	% #1: prefix
	% #2: \fileHandler
	\DataNormalisePrefix{\DataSave@Rec@prefix}{#1}%
	%
	\DataChildren[\DataSave@Rec@children]{\DataSave@Rec@prefix}%
	\Debug@Out@Data[DataSave@Rec]{Saving subtree rooted at <\DataSave@Rec@prefix> %
		which has children: [\DataSave@Rec@children]}%
	%
	\ifequals{\DataSave@Rec@children}{}{%
		% no children -> do nothing
		\Debug@Out@Data[DataSave@Rec]{ - no children, do nothing}%
	}{%		
		\xintFor ##9 in {\DataSave@Rec@children} \do{%
			\Debug@Out@Data[DataSave@Rec]{ - processing child '##9'}%
			\IfEndWith{##9}{/}{%
				\bgroup
					\Debug@Out@Data[DataSave@Rec]{ - child '##9' may have children, recursive call}%
					\DataSave@Rec<\DataSave@Rec@prefix##9>{#2}%
				\egroup
			}{%
				\DataGet[\DataSave@Rec@value]%
					<\DataSave@Rec@prefix>{##9}%
				%
				\Debug@Out@Data[DataSave@Rec]{ - child '##9' is leaf}% and has value '\DataSave@Rec@value'}%
				%\Debug@Out@Data[DataSave@Rec]{ - saving key='<\DataSave@Rec@prefix>{##9}' = '\DataSave@Rec@value' to cache file}%
				\protected@edef\DataSave@line{\string\DataPutDigested<\DataSave@Rec@prefix>{##9}{##9 = {\expandonce\DataSave@Rec@value}}}%
				%
				%\Debug@Out@Data[DataSave@Rec]{ - line to be saved: '\DataSave@line'}%
				\FileWriteLine{#2}{\expandonce\DataSave@line}%
			}%
		}%
	}%
	\Debug@Out@Data[DataSave@Rec]{End saving subtree rooted at <\DataSave@Rec@prefix>}%
}

==> MCLabPaper_Data_Put_2.tex <==


\providetoggle{metadata}%
\define@cmdkey{DataPutDigested}{metadata}[true]{}

\DeclareDocumentCommand{\DataPutDigested}{D(){} D<>{} m m}{%
	% #1: (options)
	% #2: prefix
	% #3: key/.../subkey only
	% #4: full assignment: key/.../subkey/.handlers = value
	%
	% first add metadata, if requested
	\def\Data@PutSimple@prefix{#2}%	
	\def\Data@PutSimple@key{#3}%	
	%\ifequals{#3}{}{%
	%	\edef\Data@PutSimple@handlers{}%
	%}{%
	%\def\Data@PutSimple@assignment{#4}%
	%}%
	%\def\Data@PutSimple@value{#4}%	
	%
	\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{Start}%
	\setkeys{DataPutDigested}{metadata}%	
	\setkeys{DataPutDigested}{#1}%
	\settoggle{metadata}{\cmdKV@DataPutDigested@metadata}%
	\iftoggle{metadata}{%
		\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{ - adding key to metadata}%
		\Data@add@child@to@metadata%
			{\Data@PutSimple@prefix\Data@PutSimple@key}%
	}{%
		\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{ - not adding key to metadata as requested}%
	}%
	%
	% then add key=value to database
	\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{ - key (without handlers): 
		'\Data@PutSimple@key'}%
	\pgfglobalkeysifdefined{\DataPrefix\Data@PutSimple@prefix\Data@PutSimple@key}{%
			% key already defined
	}{%
		% key not already defined: initialise it
		\pgfglobalkeys{\DataPrefix\Data@PutSimple@prefix\Data@PutSimple@key/.initial={}}%
		\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{ - new key created: 
			'\Data@PutSimple@prefix\Data@PutSimple@key'}%
	}%	
	\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{ storing '\DataPrefix\Data@PutSimple@prefix<key/handlers=value>'}%
	%
	\pgfglobalkeys{%
		\DataPrefix\Data@PutSimple@prefix#4%
	}%
	%
	% \IfDebugTF{Data}{%
	% 	\Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{...}]{ getting back stored value}%
	% 	\pgfglobalkeys{%
	% 		\DataPrefix\Data@PutSimple@prefix\Data@PutSimple@key/.get=\DataPutDigested@read}%
	% 	\Debug@Out@Data{ - key value stored: '\RenderLatex{\DataPutDigested@read}'}%
	% }{}%
	% \Debug@Out@Data[DataPutDigested(#1)<#2>{#3}{\RenderLatex{#4}}]{ done}%
}

\DeclareDocumentCommand{\DataPut}{D(){} D<>{} m}{%
	% #1 (options)
	% #2: <prefix> or <prefix/>
	% #3: comma sep. list of key/.handlers=value pairs	
	%
	%\setkeys{DataPut}{metadata}%	
	%\setkeys{DataPut}{#1}%
	%	
	\DataNormalisePrefix{\Data@Put@user@prefix}{#2}%
	%
	\xintFor ##9 in {#3} \do{%
	\bgroup% Toni: can be removed?
		% ##9: key=value
		\Debug@Out@Data[DataPut<#2>{...}]{}%
		\Debug@Out@Data[DataPut<#2>{...}]{}%		
		\Debug@Out@Data[DataPut<#2>{...}]{Start}%
		%
		\saveexpandmode%
		\noexpandarg%
		\StrBefore{##9}{=}[\Data@Put@key@and@handlers]%
		%\StrBehind{##9}{=}[\Data@Put@value]%
		\restoreexpandmode%
		%
		\StrTrim[\Data@Put@key@and@handlers]%
			{\Data@Put@key@and@handlers}%
		\Debug@Out@Data[DataPut<#2>{...}]{ - user prefix: `\Data@Put@user@prefix'}%
		\Debug@Out@Data[DataPut<#2>{...}]{ - key+handlers: `\Data@Put@key@and@handlers'}%
		%\Debug@Out@Data{DataPut<#2>{...} - value: `\RenderLatex{\Data@Put@value}'}%
		%
		\ifequals{\Data@Put@key@and@handlers}{}{%	
			% no '=' --> error		
			\Debug@Out@Data[DataPut<#2>{...}]{  - no '=' sign --> syntax error in line -> ignored}%
		}{%
			%
			\StrBefore{\Data@Put@key@and@handlers}{/.}[\Data@Put@key]%			
			\ifequals{\Data@Put@key}{}{%
				% no .handlers
				\Debug@Out@Data[DataPut<#2>{...}]{  - no handlers}%
				\gdef\Data@Put@key{\Data@Put@key@and@handlers}%
				%\gdef\Data@Put@handlers{}%
			}{% .handlers
				%\StrBehind{\Data@Put@key@and@handlers}{/.}[\Data@Put@handlers]%
				%\xdef\Data@Put@handlers{.\Data@Put@handlers}%
				%\Debug@Out@Data{DataPut<#2>{##9}:  - handlers: `\Data@Put@handlers'}%
			}%
			\Debug@Out@Data[DataPut<#2>{...}]{ - key: `\Data@Put@key'}%
			%
			\DataPutDigested(#1)<\Data@Put@user@prefix>{\Data@Put@key}{##9}%
			%
			%
			% % first add metadata, if requested			
\Comment{			
			\settoggle{metadata}{\cmdKV@DataPut@metadata}%
			\iftoggle{metadata}{%
				\Debug@Out@Data[DataPut<#2>{##9}]{ - adding key to metadata}%
				\Data@add@child@to@metadata%
					{\Data@Put@user@prefix\Data@Put@key}%
			}{%
				\Debug@Out@Data[DataPut<#2>{##9}]{ - not adding key to metadata as requested}%
			}%
			%
			% then add key=value to database
			\Debug@Out@Data[DataPut<#2>{##9}]{ - key (without handlers): 
				'\Data@Put@user@prefix\Data@Put@key'}%{}
			\pgfglobalkeysifdefined{\DataPrefix\Data@Put@user@prefix%
				\Data@Put@key}{%
					% key already defined
			}{%
				% key not already defined: initialise it
				\pgfglobalkeys{\DataPrefix\Data@Put@user@prefix%
					\Data@Put@key/.initial={}}%
				\Debug@Out@Data[DataPut<#2>{##9}]{ - new key created: 
					'\Data@Put@user@prefix\Data@Put@key'}%
			}%		
			%\Debug@Out@Data{ - pgfglobalkeys full cmd: '\DataPrefix\Data@Put@user@prefix##9'}%
			%			
			%
			%\edef\Data@Put@final@pgf@cmd{%
			%	\DataPrefix\Data@Put@user@prefix%
			%	\Data@Put@key@and@handlers = \Data@Put@value%
			%}%
			\pgfglobalkeys{%
				\DataPrefix\Data@Put@user@prefix%
				##9%
			}%
			%
			\IfDebug{Data}{%
				\pgfglobalkeys{%
					\DataPrefix\Data@Put@user@prefix%
						\Data@Put@key/.get=\DataPutNewLine@read}%
				\Debug@Out@Data[DataPut<#2>{##9}]{ - key value stored: '\DataPutNewLine@read'}%
			}{}%
			%
}%			
		}%
	\egroup%
	}%
}





==> MCLabPaper_Data_Utils_2.tex <==
% Ensure that prefix ends with '/''
\DeclareDocumentCommand{\DataNormalisePrefix}{ m m }{%
	%#1: result:   prefix/
	%#2:  prefix/ or prefix
	\IfEndWith{#2}{/}{%
		\edef@macro{#1}{#2}%
	}{%
		\IfStrEq{#2}{}{%
			\edef@macro{#1}{#2}%
		}{%
			\edef@macro{#1}{#2/}%
		}%
	}%
}

\DeclareDocumentCommand{\DataRemoveFinalSlash}{ m m }{%
	%#1: result:   prefix
	%#2:  prefix/ or prefix
	\IfEndWith{#2}{/}{%
		\StrGobbleRight{#2}{1}[#1]%
	}{%
		\edef@macro{#1}{#2}%
	}%
}


\DeclareDocumentCommand{\DataIfKeyDefinedTF}{ D<>{} m +m +m}{%
	\DataNormalisePrefix{\DataIfKeyDefinedTF@prefix}{#1}%
	\pgfglobalkeysifdefined{\DataPrefix\DataIfKeyDefinedTF@prefix#2}{#3}{#4}%	
}

\let\DataIfKeyExistsTF\DataIfKeyDefinedTF


==> MCLabPaper_DateTime_2.tex <==
\MCLabPaper@Set@Tutorial@Section{DateTime}{sec:datetime}

\MCLabPaper@RequirePackage{datetime2}

\DeclareDocumentCommand{\Debug@Out@DateTime}{o m}{%
	\Debug@Out{DateTime}[#1]{#2}%
}

\DeclareDocumentCommand{\Date@Parse}{m m m m}{%
	% #1: "dd/mm/yyyy"
	% #2: \day
	% #3: \month
	% #4: \year
	\Debug@Out@DateTime[Date@Parse(...)]{start: date is '#1'}%
	\edef\Date@Parse@userstring{#1}%
	\Debug@Out@DateTime[Date@Parse(\Date@Parse@userstring)(...)]{User date expanded: '\Date@Parse@userstring'}%
	\expandafter%
		\StrTrim\expandafter%
			[\expandafter\Date@Parse@user@string%
			\expandafter]\expandafter{\Date@Parse@userstring}%
	\StrCut[1]{\Date@Parse@user@string}{/}{#2}{\Date@Parse@Month@Year}%
	\Debug@Out@DateTime[Date@Parse(\Date@Parse@userstring)(...)]{day='#2', month+year='\Date@Parse@Month@Year'}%
	\StrCut[1]{\Date@Parse@Month@Year}{/}{#3}{#4}%
	\StrTrim[#2]{#2}%
	\StrTrim[#3]{#3}%
	\StrTrim[#4]{#4}%
	\IfInteger{#2}{%
		\MathStripLeadingZeroes{#2}{#2}% remove leading zeroes
	}{%
 		\DiagError{DateTime}{Day not integer in date '\Date@Parse@userstring'}%
 	}%
 	\IfInteger{#3}{%
 		\MathStripLeadingZeroes{#3}{#3}% remove leading zeroes
 	}{%
 		\DiagError{DateTime}{Month not integer in date '\Date@Parse@userstring'}%
 	}%
 	\IfInteger{#4}{}{%
 		\DiagError{DateTime}{Year not integer in date '\Date@Parse@userstring'}%
 	}%
	% \edef@macro{#2}{\Date@Parse@Day}%
	% \edef@macro{#3}{\Date@Parse@Month}%
	% \edef@macro{#4}{\Date@Parse@Year}%
	% %
	\Debug@Out@DateTime[Date@Parse(\Date@Parse@userstring)(...)]{day='#2', month='#3', year='#4'}%	
	\If@Is@Date@TF{#2}{#3}{#4}%
		{}% %ok
		{%
			\DiagError{DateTime}{String '#1' is not a valid date, although it has been successfully parsed as '#2/#3/#4'. Returning empty macros}%
			\edef@macro{#2}{}%
			\edef@macro{#3}{}%
			\edef@macro{#4}{}%
		}%
}



%% Checks whether #1 (dd/mm/yyyy) is a valid date
\DeclareDocumentCommand{\IfIsDateTF}{m +m +m}{%
	\Date@Parse{#1}%
		{\IfIsDate@day}%
		{\IfIsDate@month}%
		{\IfIsDate@year}%
	\If@Is@Date@TF%
		{\IfIsDate@day}%
		{\IfIsDate@month}%
		{\IfIsDate@year}%
		{#2}{#3}%
}

\newif\ifDateTime@Is@Date
\DeclareDocumentCommand{\If@Is@Date@TF}{m m m +m +m}{%
	% #1: day
	% #2: month 
	% #3: year
	% #4: true branch
	% #5: false branch
	%
	\DateTime@Is@Datetrue%
	%
	\ifnumcomp{#2}<{1}%
		{\DateTime@Is@Datefalse}%
		{%
			\ifnumcomp{#2}>{12}%
				{\DateTime@Is@Datefalse}%
				{%			
					\ifnumcomp{#1}<{1}%
						{\DateTime@Is@Datefalse}%
						{%
							\DateTime@Max@Day@In@Month%
								{#2}%
								{#3}%
								{\IfIsDate@max@day@in@month}%
							\ifnumcomp{#1}>{\IfIsDate@max@day@in@month}
								{\DateTime@Is@Datefalse}%
								{\DateTime@Is@Datetrue}%
						}%
				}%
		}%
	\ifDateTime@Is@Date%
		#4%
	\else%
		#5%
	\fi%
}



\DeclareDocumentCommand{\DateTime@Max@Day@In@Month}{m m m}{%
	% #1: month (1--12)
	% #2: year
	% #3: \result
	\ifcase#1%
  		% Case 0
  		\edef@macro{#3}{0}%
	\or%
  		% Case 1
  		\edef@macro{#3}{31}%
	\or%
		% Case 2
		\DateTime@If@Is@Year@Leap@TF{#2}%
			{\edef@macro{#3}{29}}%
			{\edef@macro{#3}{28}}%
	\or%
		% Case 3
  		\edef@macro{#3}{31}%
	\or%
		% Case 4
  		\edef@macro{#3}{30}%
	\or%
		% Case 5
  		\edef@macro{#3}{31}%
	\or%
		% Case 6
  		\edef@macro{#3}{30}%
	\or%
		% Case 7
  		\edef@macro{#3}{31}%  		
	\or%
		% Case 8
  		\edef@macro{#3}{31}%
	\or%
		% Case 9
  		\edef@macro{#3}{30}%
	\or%
		% Case 10
  		\edef@macro{#3}{31}%
	\or%
		% Case 11
  		\edef@macro{#3}{30}%
	\or%
		% Case 12
  		\edef@macro{#3}{31}%
	\else%
		\edef@macro{#3}{0}%
	\fi%
}


\newif\ifDateTime@Is@Leap@Year
\DeclareDocumentCommand{\DateTime@If@Is@Year@Leap@TF}{m +m +m}{%
	% #1: year
	% #2: then branch
	% #3: else branch
	%
	% Algorithm:
	% if (year is not divisible by 4) then (it is a common year)
	% else if (year is not divisible by 100) then (it is a leap year)
	% else if (year is not divisible by 400) then (it is a common year)
	%else (it is a leap year)
	%
	%
	\DateTime@Is@Leap@Yearfalse%
	%if (year is not divisible by 4) then (it is a common year)
	\MathMod[\DateTime@Is@Y@L@mod@four]{#1}{4}%
	\ifnumcomp{\DateTime@Is@Y@L@mod@four}={0}%
		{%	year is divisible by 4:
			%
			\MathMod[\DateTime@Is@Y@L@mod@hundred]{#1}{100}%
			\ifnumcomp{\DateTime@Is@Y@L@mod@hundred}={0}%
				{%	year divisible by 4 and by 100				
					\MathMod[\DateTime@Is@Y@L@mod@fourhundreds]{#1}{400}%
					\ifnumcomp{\DateTime@Is@Y@L@mod@fourhundreds}={0}%
						{%	year divisible by 4, 100, and 400 --> not leap
							\DateTime@Is@Leap@Yeartrue%
						}%
						{% year divisible by 4, 100, but NOT 400 --> leap							
							\DateTime@Is@Leap@Yearfalse%
						}%
				}%
				{%   year divisible by 4 but NOT by 100 --> leap
					\DateTime@Is@Leap@Yeartrue%
				}%
		}%
		{%	year is NOT divisible by 4 --> not leap
			\DateTime@Is@Leap@Yearfalse%
		}%
	%
	\ifDateTime@Is@Leap@Year%
		#2%
	\else%
		#3%
	\fi%
}


\DeclareDocumentCommand{\DateCompare}{m m m}{%
	% #1: dd/mm/yyyy
	% #2: dd/mm/yyyy
	% #3: result: -1, 0, 1  (if resp. <, =, >)
	% \edef\DateCompare@day@a{}%
	% \edef\DateCompare@month@a{}%
	% \edef\DateCompare@year@a{}%
	% \edef\DateCompare@day@b{}%
	% \edef\DateCompare@month@b{}%
	% \edef\DateCompare@year@b{}%
	%
	\Date@Parse{#1}%
		{\DateCompare@day@a}%
		{\DateCompare@month@a}%
		{\DateCompare@year@a}%
	\Date@Parse{#2}%
		{\DateCompare@day@b}%
		{\DateCompare@month@b}%
		{\DateCompare@year@b}%
	\Date@Compare%
		{\DateCompare@day@a}%
		{\DateCompare@month@a}%
		{\DateCompare@year@a}%
		{\DateCompare@day@b}%
		{\DateCompare@month@b}%
		{\DateCompare@year@b}%
		{#3}%
}

\newcommand{\Date@Compare}[7]{%
	% #1/#2/#3  <, =, > #4/#5/#6  
	% #7: result: -1, 0, +1
	%
	\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{Start}%
	\ifnumcomp{#3}{<}{#6}{%
		\edef\Date@Compare@Result{-1}%
		\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - year #3 < year #6: --> -1}%
	}{%
		\ifnumcomp{#3}{>}{#6}{%
			\edef\Date@Compare@Result{1}%
			\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - year #3 > year #6: --> +1}%
		}{%
			% same year
			\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - year #3 = year #6: --> need to check month}%
			\ifnumcomp{#2}{<}{#5}{%
				\edef\Date@Compare@Result{-1}%
				\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - month #2 < month #5: --> -1}%
			}{%
				\ifnumcomp{#2}{>}{#5}{%
					\edef\Date@Compare@Result{1}%
					\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - month #2 > month #5: --> +1}%
				}{%
					% same month
					\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - month #2 = month #5: --> need to check days}%
					\ifnumcomp{#1}{<}{#4}{%
						\edef\Date@Compare@Result{-1}%
						\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - day #1 < day #4: --> -1}%
					}{%
						\ifnumcomp{#1}{>}{#4}{%
							\edef\Date@Compare@Result{1}%
							\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - day #1 > day #4: --> +1}%
						}{%
							% same day
							\edef\Date@Compare@Result{0}%
							\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{ - day #1 = day #4: --> 0}%
						}%
					}%
				}%
			}%
		}%
	}%
	\edef@macro{#7}{\Date@Compare@Result}%
	\Debug@Out@DateTime[Date@Compare(#1/#2/#3 compared to #4/#5/#6)]{End. Result = [#7]}%
}




\PrettyDefineStyle{ddmmyyyy}{unit={}, unitpos=after, decimaldigits=0, convert=\Pretty@ddmmyyyy@Convert}

\def\Pretty@ddmmyyyy@Convert#1#2{%
	% stores in macro #1 user string #2 converted into a date
	\Date@Parse{#2}%
		{\TimeDate@Pretty@Convert@day}%
		{\TimeDate@Pretty@Convert@month}%
		{\TimeDate@Pretty@Convert@year}%	
	\If@Is@Date@TF%
		{\TimeDate@Pretty@Convert@day}%
		{\TimeDate@Pretty@Convert@month}%
		{\TimeDate@Pretty@Convert@year}%
			{%
				%
				\ifnumcomp{\TimeDate@Pretty@Convert@day}<{10}%
					{\edef\TimeDate@Pretty@Convert@day{0\TimeDate@Pretty@Convert@day}}%
					{}%
				\ifnumcomp{\TimeDate@Pretty@Convert@month}<{10}%
					{\edef\TimeDate@Pretty@Convert@month{0\TimeDate@Pretty@Convert@month}}%
					{}%
				%
				%
				\edef@macro{#1}{%
					\TimeDate@Pretty@Convert@day/%
					\TimeDate@Pretty@Convert@month/%
					\TimeDate@Pretty@Convert@year%
				}%
			}%
			{%
				\DiagError{Pretty}{\DiagLatexCmd{Pretty[style=ddmmyyyy...]\{#2\}}: Value must be in the form d/m/y and be a valid date}[\ Pretty[style=ddmmyyyy...]{#2}: Value must be in the form d/m/y and be a valid date]%
			}%
}


\PrettyDefineStyle{dmyyyy}{unit={}, unitpos=after, decimaldigits=0, convert=\Pretty@dmyyyy@Convert}

\def\Pretty@dmyyyy@Convert#1#2{%
	% stores in macro #1 user string #2 converted into a date
	\Date@Parse{#2}%
		{\TimeDate@Pretty@Convert@day}%
		{\TimeDate@Pretty@Convert@month}%
		{\TimeDate@Pretty@Convert@year}%	
	\If@Is@Date@TF%
		{\TimeDate@Pretty@Convert@day}%
		{\TimeDate@Pretty@Convert@month}%
		{\TimeDate@Pretty@Convert@year}%
			{%
				%
				\edef@macro{#1}{%
					\TimeDate@Pretty@Convert@day/%
					\TimeDate@Pretty@Convert@month/%
					\TimeDate@Pretty@Convert@year%
				}%
			}%
			{%
				\DiagError{Pretty}{\DiagLatexCmd{Pretty[style=dmyyyy...]\{#2\}}: Value must be in the form d/m/y and be a valid date}[\ Pretty[style=dmyyyy...]{#2}: Value must be in the form d/m/y and be a valid date]%
			}%
}

\endinput

%%% OLD STUFF

% \def\Date@Parse@Aux#1/#2/#3{%
% 	\IfInteger{#1}{}{%
% 		\DiagError{DateTime}{Day not integer in date '#1/#2/#3'}%
% 	}%
% 	\IfInteger{#2}{}{%
% 		\DiagError{DateTime}{Month not integer in date '#1/#2/#3'}%
% 	}%
% 	\IfInteger{#3}{}{%
% 		\DiagError{DateTime}{Year not integer in date '#1/#2/#3'}%
% 	}%
% 	%
% 	\edef\Date@Parse@Day{#1}%
%   	\edef\Date@Parse@Month{#2}%
%   	\edef\Date@Parse@Year{#3}%
%   	%
% 	\Debug@Out@DateTime[Date@Parse@Aux(#1/#2/#3)]{day='\Date@Parse@Day', month='\Date@Parse@Month', year='\Date@Parse@Year'}%	
% }

==> MCLabPaper_Debug_2.tex <==
\PackageInfo{MCLabPaper}{Loading Debug.tex}%

\DeclareDocumentCommand{\Debug@Out@Debug}{o m}{%
	\PackageInfo{MCLabPaper.Debug}{#1: #2}%
}

\DeclareDocumentCommand{\DebugOn}{o}{%
	% [#1]: list of module names (not given = all)
	\Debug@Out@Debug[DebugOn]{Start}%
	\Debug@Set[#1]{1}%
	\Debug@Out@Debug[DebugOn]{End}%
}
\DeclareDocumentCommand{\DebugOff}{o}{%
	% [#1]: list of module names (not given = all)
	\Debug@Out@Debug[DebugOff]{Start}%
	\Debug@Set[#1]{0}%
	\Debug@Out@Debug[DebugOff]{End}%
}


% #1: module name
% [#2]: function name
% #3: message
\DeclareDocumentCommand{\Debug@Out@Off}{o m}{}%
\DeclareDocumentCommand{\Debug@Out}{m O{} m}{%
	\typeout{*MCLabPaper.#1. #2: #3}%
}%


\DeclareDocumentCommand{\Debug@Set}{O{} m}{%
	% #1: list of module names (not given = all)
	% #2: >0 (=On), or 0 (=Off)
	\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{Start}%
	\ifequals{#1}{}{%
		\pgfglobalkeys{%
			\MCLabPaper@Modules@Prefix/.list/.get = \MCLabPaper@Modules@list
		}%
		\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{No modules are given, assuming all loaded modules}%
	}{%
		\edef\MCLabPaper@Modules@list{#1}%
		\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{Some modules are given}%
	}%
	\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{Setting Debug mode to '#2' for the following modules: [\MCLabPaper@Modules@list]}%
	%
	%
	\ifnumcomp{#2}{=}{0}{%
		\edef\Debug@State{false}%
	}{%
		\edef\Debug@State{true}%
	}%
	\xintFor ##9 in {\MCLabPaper@Modules@list} \do{%
		% \let\Debug@Out@<MODULE>\Debug@Out@<MODULE><On|Off>
		% method \*On is \let'd in \MCLabPaper@Load@All@Modules
		\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{Setting bool 'Debug@State@##9' to '\Debug@State'}%
		\setbool{Debug@State@##9}{\Debug@State}%
		%
		\ifbool{Debug@State@##9}{%
			% Debug On
			\csletcs{Debug@Out@##9}{Debug@Out@##9@On}%
			\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{Macro 'Debug@Out@##9' redefined as 'Debug@Out@##9@On'}%
		}{%
			% Debug Off
			\csletcs{Debug@Out@##9}{Debug@Out@Off}%
			\Debug@Out@Debug[{Debug@Set[#1]{#2}}]{Macro 'Debug@Out@##9' redefined as 'Debug@Out@Off'}%
		}%
	}%		
}%


\DeclareDocumentCommand{\IfDebugTF}{m +m +m}{%
	% #1: module name
	% #2: then branch
	% #3: else branch
	\ifbool{Debug@State@#1}{#2}{#3}%
}


\PackageInfo{MCLabPaper}{Loading Debug.tex done}%

==> MCLabPaper_Diagnostics_2.tex <==
\DeclareDocumentCommand{\Debug@Out@Diag}{o m}{%
	\Debug@Out{Diagnostics}[#1]{#2}%
}

\def\Diag@Image@Warning{pkg-warning-1.pdf}
\def\Diag@Image@Error{pkg-error-2.pdf}
\def\Diag@Image@Deprecation{pkg-deprecation-2.pdf}




\newcommand{\DiagLatexCmd}[1]{\textcolor{\LatexColor}{\textbackslash#1}}

\mdfdefinestyle{diagmessage}{skipabove=2pt, skipbelow=2pt, innertopmargin=4pt, innerbottommargin=4pt, nobreak=true}

\def\Diag@Prefix{\pgfkeysPrefix/diagnostics}

\define@cmdkey{DiagDefineMsgType}{title}[]{}
\define@cmdkey{DiagDefineMsgType}{backgroundcolor}[]{}
\define@cmdkey{DiagDefineMsgType}{linecolor}[]{}
\define@cmdkey{DiagDefineMsgType}{icon}[]{}
\define@choicekey*{DiagDefineMsgType}{die}%
	[\cmdKV@DiagDefineMsgType@die]{,true,false}[]{}
\define@choicekey*{DiagDefineMsgType}{showinpdf}%
	[\cmdKV@DiagDefineMsgType@showinpdf]{,true,false}[]{}
\define@choicekey*{DiagDefineMsgType}{showtutorialbutton}%
	[\cmdKV@DiagDefineMsgType@showtutorialbutton]{,true,false}[]{}
\define@choicekey*{DiagDefineMsgType}{showinlog}%
	[\cmdKV@DiagDefineMsgType@showinlog]{,true,false}[]{}

\DeclareDocumentCommand{\DiagDefineMsgType}{m m}{%
	% #1: message type
	% #2: options (key=value list)
	\Debug@Out{Diagnostics}[DiagDefineMsgType(#1)]{Start: options = '#2'}%
	\def\Diag@Define@Msg@Type@all@options%
		{title, backgroundcolor, linecolor, icon, 
		die, showinpdf, showtutorialbutton, showinlog}%
	%
	\@expandtwoargs\setkeys{DiagDefineMsgType}{\Diag@Define@Msg@Type@all@options}%
	\setkeys{DiagDefineMsgType}{#2}%
	%
	\xintFor ##9 in {\Diag@Define@Msg@Type@all@options} \do{
			\ifequals{\csuse{cmdKV@DiagDefineMsgType@##9}}{}{}{%
				\pgfglobalkeys{%
					\Diag@Prefix/types/#1/##9/.initial/.expanded=%
						\csuse{cmdKV@DiagDefineMsgType@##9}
				}%
				\Debug@Out{Diagnostics}[DiagDefineMsgType(#1)]%
					{ - ##9 now set to 
						\csuse{cmdKV@DiagDefineMsgType@##9}}%
			}%
	}%	
	\Debug@Out{Diagnostics}[DiagDefineMsgType(#1)]{Done.}%
}

%% Built-in diag message types
\DiagDefineMsgType{deprecation}{%
	title={Deprecation notice},
	backgroundcolor={yellow!30}, 
	linecolor={black!50}, 
	icon=\Diag@Image@Deprecation,
	die=false, 
	showinpdf=true, 
	showtutorialbutton=true, 
	showinlog=true
}
\DiagDefineMsgType{warning}{%
	title={Warning},
	backgroundcolor={orange!30}, 	
	linecolor={black!50}, 
	icon=\Diag@Image@Warning,
	die=false, 
	showinpdf=true, 
	showtutorialbutton=true, 
	showinlog=true
}
\DiagDefineMsgType{error}{%
	title={Error},
	backgroundcolor={red!30}, 	
	linecolor={black!50}, 
	icon=\Diag@Image@Error,
	die=true, 
	showinpdf=true, 
	showtutorialbutton=true, 
	showinlog=true
}

\DiagDefineMsgType{info}{%
	title={Info},
	backgroundcolor={green!30}, 	
	linecolor={black!50}, 
	icon=\Diag@Image@Warning,
	die=false, 
	showinpdf=true, 
	showtutorialbutton=true, 
	showinlog=true
}


%% Queue of diag messages generated in the preamble (whose showing is postponed at begin-document)
\pgfglobalkeys{\Diag@Prefix/preamble/messages/.initial = {}}


\newlength{\Diag@Msg@img@width}%
\setlength{\Diag@Msg@img@width}{2cm}

\newlength{\Diag@Msg@msg@width}%


\DeclareDocumentCommand{\DiagInfo}{s D(){} m +m O{}}{%
	% #1: star -> inline
	% (#2): options
	% #3: module name
	% #4: message to PDF
	% #5: message to log
	\Diag@Message%
		{#1}%		{star?} -> inline
		{info}%	message type
		(#2)%		options
		{#3}%		module name
		{#4}%		message to PDF
		[#5]% 		message to log (empty: use msg to PDF)
}

\DeclareDocumentCommand{\DiagWarning}{s D(){} m +m O{}}{%
	% #1: star -> inline
	% (#2): options
	% #3: module name
	% #4: message to PDF
	% #5: message to log
	\Debug@Out{Diagnostics}[DiagWarning(#1)(#2)(#3)(long msg to pdf)[#5]]{Start}%
	\Diag@Message%
		{#1}%		{star?} -> inline
		{warning}%	message type
		(#2)%		options
		{#3}%		module name
		{#4}%		message to PDF
		[#5]% 		message to log (empty: use msg to PDF)
	\Debug@Out{Diagnostics}[DiagWarning(#1)(#2)(#3)(long msg to pdf)[#5]]{End}%
}

\DeclareDocumentCommand{\DiagError}{s D(){} m +m O{}}{%
	% #1: star -> inline
	% (#2): options	
	% #3: module name
	% #4: message to PDF
	% #5: message to log
	% 
	\Diag@Message%
		{#1}%   	{star?} -> inline
		{error}% 	message type
		(#2)%		options
		{#3}%		module name
		{#4}%		message to PDF
		[#5]% 		message to log (empty: use msg to PDF)
}

\DeclareDocumentCommand{\DiagDeprecation}{s D(){} m +m O{}}{%
	% #1: star -> inline
	% (#2): options
	% #3: module name
	% #4: message to PDF
	% [#5]: message to log
	\Diag@Message%
		{#1}%   	{\BooleanTrue} -> inline
		{deprecation}% 	message type
		(#2)%		options
		{#3}%		module name
		{#4}%		message to PDF
		[#5]% 		message to log (empty: use msg to PDF)
}
\DeclareDocumentCommand{\DiagDeprecationSimple}{s m m m}{%
	% #1: star -> inline
	% #2: module name
	% #3: deprecated cmd
	% #4: new cmd
	\def\DiagDeprecationSimple@msg{Command \DiagLatexCmd{#3} is deprecated. 
		Use \DiagLatexCmd{#4} instead.}%
	\def\DiagDeprecationSimple@msg@log{Command \ #3 is deprecated. 
		Use \ #4 instead.}%
	%	
	\IfBooleanTF{#1}{%
		\DiagDeprecation*{#2}{\DiagDeprecationSimple@msg}[\DiagDeprecationSimple@msg@log]%
	}{%
		\DiagDeprecation{#2}{\DiagDeprecationSimple@msg}[\DiagDeprecationSimple@msg@log]%
	}%
}


% Explicitly given option (no default possible):
\define@cmdkey{Diag@Message}{tutorialdest}[]{} %a module of the tutorial. If not given, it will be the "module name" argument of \DiagXXX commands
\define@cmdkey{Diag@Message}{showinlog}[]{}% Overrides style def.
\define@cmdkey{Diag@Message}{die}[]{}% Overrides style def.


\DeclareDocumentCommand{\Diag@Message}{m m D(){} m +m O{}}{%
	% #1: \BooleanTrue -> inline
	% #2: message type
	% (#3): options
	% #4: module name
	% #5: message to PDF (long)
	% [#6]: message to log (empty: use #5)
	%
	\Debug@Out{Diagnostics}[Diag@Message(#1)(#2)(#3)(#4)(long msg to pdf)[#6]]{Start}%
	%
	\IfPreambleTF{%
		\pgfglobalkeys{%
			\Diag@Prefix/preamble/messages/.append = {%
				\Diag@Message%
					{#1}{#2}(#3){#4}{#5}[#6]%
			}%
		}%
	}{%
		\Diag@Message@Out%
			{#1}{#2}(#3){#4}{#5}[#6]%
	}%
	\Debug@Out{Diagnostics}[Diag@Message(#1)(#2)(#3)(#4)(long msg to pdf)[#6]]{End}%
}%

\newtoggle{Diag@Message@die}
\newtoggle{Diag@Message@showinpdf}
\newtoggle{Diag@Message@showtutorialbutton}
\newtoggle{Diag@Message@showinlog}
\DeclareDocumentCommand{\Diag@Message@Out}{m m D(){} m +m O{}}{%
	%
	\def\Diag@Msg@type{#2}%	
	\def\Diag@Msg@module{#4}%
	\def\Diag@Msg@msg@pdf{#5}%	
	%
	%
	\setkeys{Diag@Message}{tutorialdest, showinlog, die}%
	\setkeys{Diag@Message}{#3}%
	%
	% Set toggles using info from message type style
	\undef\Diag@Msg@title%
	\pgfglobalkeys{\Diag@Prefix/types/\Diag@Msg@type/.cd,
		title/.get = \Diag@Msg@title,
		die/.get = \Diag@Msg@die,
		showinpdf/.get = \Diag@Msg@showinpdf,
		showinlog/.get = \Diag@Msg@showinlog
	}%
	\Debug@Out{Diagnostics}[Diag@Message@Out(\Diag@Msg@type)]{Retrieved: %
		title='\Diag@Msg@title', die='\Diag@Msg@die'
	}%
	%
	\settoggle{Diag@Message@die}{\Diag@Msg@die}%
	\settoggle{Diag@Message@showinpdf}{\Diag@Msg@showinpdf}%
	\settoggle{Diag@Message@showinlog}{\Diag@Msg@showinlog}%
	%
	%
	% Process explicitly given options
	\ifequals{\cmdKV@Diag@Message@showinlog}{}{%
		% no overriding given, use default
	}{%
		% overriding given
		\settoggle{Diag@Message@showinlog}%
			{\cmdKV@Diag@Message@showinlog}%
	}%
	\ifequals{\cmdKV@Diag@Message@die}{}{%
		% no overriding given, use default
	}{%
		% overriding given
		\settoggle{Diag@Message@die}%
			{\cmdKV@Diag@Message@die}%
	}%
	%
	% Get name of current input file 
	\InputCurrentFilePath[\Diag@Msg@curr@file]%
	%
	% Produce log message if requested
	\iftoggle{Diag@Message@showinlog}{%
		%
		% Define log message
		\ifequals{#6}{}{%
			% No explicit message to log given, use msg to pdf.
			\def\Diag@Msg@msg@log{#5}%
		}{%
			% Explicit message to log given
			\def\Diag@Msg@msg@log{#6}%
		}%
		%
		\Diag@Message@Log%
			{\Diag@Msg@module}%
			{\Diag@Msg@title}%
			{\Diag@Msg@msg@log}%
			{\Diag@Msg@curr@file}%
			{Diag@Message@die}%
	}{%
		% do nothing if showinlog is false
	}%
	% Log message generation complete (if requested).
	\Debug@Out{Diagnostics}[Diag@Message@Out(\Diag@Msg@type)]{Log message generation complete (if requested)}%
	%
	%
	\iftoggle{Diag@Message@showinpdf}{%
		%
		% Show PDF message (banner or inline)
		\Diag@Message@Pdf%
			{#1}% \BooleanTrue --> inline
			{\Diag@Msg@type}%
			{\Diag@Msg@module}%
			{\Diag@Msg@title}%
			{\Diag@Msg@msg@pdf}%
			{\Diag@Msg@curr@file}%
			{\cmdKV@Diag@Message@tutorialdest}%
	}{%
		% do nothing if showinpdf is false
	}%
	\Debug@Out{Diagnostics}[Diag@Message@Out(\Diag@Msg@type)]{PDF message generation complete (if requested)}%
	%
	\iftoggle{Diag@Message@die}{%
		\GenericError{MCLabPaper}{Fatal error: Stopping compilation. See above errors (starting from the FIRST ONE!) for details.}%
		\relax%
		\stop%
	}{}%
	\Debug@Out{Diagnostics}[Diag@Message@Out(\Diag@Msg@type)]{End.}%
}


\DeclareDocumentCommand{\Diag@Message@Log}{m m m m m}{%
	\def\Diag@Msg@Log@module{#1}%
	\def\Diag@Msg@Log@title{#2}%
	\def\Diag@Msg@Log@msg{#3}%
	\def\Diag@Msg@Log@curr@file{#4}%
	\def\Diag@Msg@Log@die@toggle{#5}%
	%
	% Define right command to use: \PackageError or \PackageWarning depending on value of toggle '\Diag@Msg@die@toggle'
	\iftoggle{\Diag@Msg@Log@die@toggle}{%
		\let\Diag@Msg@Log@OutputCmd\PackageError%
	}{%
		\let\Diag@Msg@Log@OutputCmd\PackageWarning%
	}%
	%
	\typeout{}\typeout{}\typeout{}\typeout{}%
	\typeout{}\typeout{}\typeout{}\typeout{}%
	\typeout{?* =============================================================}%
	\Diag@Msg@Log@OutputCmd%
		{MCLabPaper.\Diag@Msg@Log@module}%
		{\Diag@Msg@Log@title: 
		 \Diag@Msg@Log@msg. 
		 Offending command is in file \Diag@Msg@Log@curr@file.}{}%
	\typeout{================================================================}%
	\typeout{}\typeout{}\typeout{}\typeout{}%
	\typeout{}\typeout{}\typeout{}\typeout{}%
}


\DeclareDocumentCommand{\Diag@Message@Pdf}{m m m m +m m m}{%
	\IfDraftTF{%
		\def\Diag@Msg@Pdf@star{#1}%
		\def\Diag@Msg@Pdf@type{#2}%
		\def\Diag@Msg@Pdf@module{#3}%
		\def\Diag@Msg@Pdf@title{#4}%
		\def\Diag@Msg@Pdf@msg{#5}%
		\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Start.}%
		\edef\Diag@Msg@Pdf@curr@file{#6}%
		\ifequals{#7}{}{%
			\let\Diag@Msg@Pdf@tutorialdest\Diag@Msg@Pdf@module%
		}{%
			\def\Diag@Msg@Pdf@tutorialdest{#7}%
		}%
		\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Tutorial dest: '\Diag@Msg@Pdf@tutorialdest'}%
		%
		% Set toggles using info from message type style
		\pgfglobalkeys{\Diag@Prefix/types/\Diag@Msg@Pdf@type/.cd,
			backgroundcolor/.get = \Diag@Msg@Pdf@bgcolor,
			linecolor/.get = \Diag@Msg@Pdf@color,
			icon/.get = \Diag@Msg@Pdf@icon,
			showtutorialbutton/.get = \Diag@Msg@Pdf@showtutorialbutton
		}%
		\settoggle{Diag@Message@showtutorialbutton}{\Diag@Msg@Pdf@showtutorialbutton}%
		%
		\def\Diag@Msg@Pdf@result{}%
		%
		\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Star is: '\Diag@Msg@Pdf@star'}%
		\IfBooleanTF{\Diag@Msg@Pdf@star}{% 
			% Inline mode
			\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Inline mode.}%
			\def\Diag@Msg@Pdf@result{%
				\expandafter\colorbox{\Diag@Msg@Pdf@bgcolor}{%
					\textbf{MCLabPaper.\Diag@Msg@Pdf@module}: \Diag@Msg@Pdf@msg{} % 
					\iftoggle{Diag@Message@showtutorialbutton}{%
						\ButtonTutorial*(\Diag@Msg@Pdf@tutorialdest)%
					}{}%
				}%
			}%
			\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Inline mode: result computed.}%
		}{%
			% Banner mode
			\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Banner mode.}%
			\edef\Diag@Msg@Pdf@banner@options{%
				style=diagmessage, 
				backgroundcolor=\Diag@Msg@Pdf@bgcolor,
				frametitle={MCLabPaper.\Diag@Msg@Pdf@module: 
					\Diag@Msg@Pdf@title}%
			}%
			\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Banner mode: options computed.}%
			\def\Diag@Msg@Pdf@result{%
				\par\noindent%
				\begin{minipage}{\linewidth}%
				\expandafter\mdframed\expandafter%
					[\Diag@Msg@Pdf@banner@options]%
					%
					%
					\begin{minipage}{\Diag@Msg@img@width}
						\includegraphics[width=\linewidth]%
							{\Diag@Msg@Pdf@icon}%
					\end{minipage}%
					%
					\setlength{\Diag@Msg@msg@width}{\linewidth}%
					\addtolength{\Diag@Msg@msg@width}{-\Diag@Msg@img@width}%
					%
					\begin{minipage}{\Diag@Msg@msg@width}%
						\Diag@Msg@Pdf@msg 
						\\ 
						Offending command is in file 
						\RenderFileName{\Diag@Msg@Pdf@curr@file}.%
						%
						\iftoggle{Diag@Message@showtutorialbutton}{%
							\begin{center}
								\ButtonTutorial(\Diag@Msg@Pdf@tutorialdest)
							\end{center}%
						}{}%
					\end{minipage}%
				\endmdframed%
				\end{minipage}%
			}%
			\Debug@Out{Diagnostics}[Diag@Message@Pdf]{Banner mode: result computed.}%
		}%
		%
		%
		\Diag@Msg@Pdf@result\relax%
	}{}%	
}



\AtBeginDocument{%
	\pgfglobalkeys{\Diag@Prefix/preamble/messages/.get=\Diag@Messages}%
	%\typeout{\DiagMessages}%
	\Diag@Messages%
}


==> MCLabPaper_Draft_2.tex <==
\MCLabPaper@RequirePackage[framemethod=tikz]{mdframed}

\MCLabPaper@Set@Tutorial@Section{Draft}{sec:draft}

\DeclareDocumentCommand{\Debug@Out@Draft}{o m}{%
	\Debug@Out{Draft}[#1]{#2}%
}


\newif\if@MCLabPaper@draft
\@MCLabPaper@draftfalse

\DeclareDocumentCommand{\IfDraftTF}{+m +m}{%
	\if@MCLabPaper@draft%
		#1%
	\else%
		#2%
	\fi%
}

\newtoggle{@MCLabPaper@draft@show@sysnotes}
\settoggle{@MCLabPaper@draft@show@sysnotes}{false}

\newtoggle{@MCLabPaper@draft@show@notes}
\settoggle{@MCLabPaper@draft@show@notes}{false}

\newtoggle{@MCLabPaper@draft@emph@data}
\settoggle{@MCLabPaper@draft@emph@data}{false}

\newtoggle{@MCLabPaper@draft@emph@math}
\settoggle{@MCLabPaper@draft@emph@math}{false}

\newtoggle{@MCLabPaper@draft@show@buttons}
\settoggle{@MCLabPaper@draft@show@buttons}{false}

\newtoggle{@MCLabPaper@draft@show@images}
\settoggle{@MCLabPaper@draft@show@images}{true}



\define@cmdkey{Draft}{sysnotes}[true]{}
\define@cmdkey{Draft}{data}[true]{}
\define@cmdkey{Draft}{math}[true]{}
\define@cmdkey{Draft}{buttons}[true]{}
\define@cmdkey{Draft}{notes}[true]{}
\define@cmdkey{Draft}{images}[true]{}

\def\@MCLabPaper@draft@options{}%

\DeclareDocumentCommand{\DraftOn}{O{}}{%
	\@MCLabPaper@drafttrue%
	\Debug@Out@Draft[DraftOn]{Enabling draft mode with options '#1'}%
	\def\@MCLabPaper@draft@options{#1}%
	\setkeys{Draft}{sysnotes, data, math, buttons, notes, images}%
	\setkeys{Draft}{#1}%
	\settoggle{@MCLabPaper@draft@show@notes}{\cmdKV@Draft@notes}%
	\settoggle{@MCLabPaper@draft@show@sysnotes}{\cmdKV@Draft@sysnotes}%
	\settoggle{@MCLabPaper@draft@emph@data}{\cmdKV@Draft@data}%		
	\settoggle{@MCLabPaper@draft@emph@math}{\cmdKV@Draft@math}%
	\settoggle{@MCLabPaper@draft@show@buttons}{\cmdKV@Draft@buttons}%	
	\settoggle{@MCLabPaper@draft@show@images}{\cmdKV@Draft@images}%
	%
	\Debug@Out@Draft[DraftOn]{ - sysnotes = \iftoggle{@MCLabPaper@draft@show@sysnotes}{true}{false}}%
	\Debug@Out@Draft[DraftOn]{ - draft notes = \iftoggle{@MCLabPaper@draft@show@notes}{true}{false}}%
	\Debug@Out@Draft[DraftOn]{ - data = \iftoggle{@MCLabPaper@draft@emph@data}{true}{false}}%	
	\Debug@Out@Draft[DraftOn]{ - math = \iftoggle{@MCLabPaper@draft@emph@math}{true}{false}}%
	\Debug@Out@Draft[DraftOn]{ - buttons = \iftoggle{@MCLabPaper@draft@show@buttons}{true}{false}}	
	\Debug@Out@Draft[DraftOn]{ - images = \iftoggle{@MCLabPaper@draft@show@images}{true}{false}}	
	%
}
\newcommand{\DraftOff}{\@MCLabPaper@draftfalse}

\DeclareDocumentCommand{\SetDraft}{}{%
	\Deprecated@Notice{Use of command SetDraft is deprecated. Use DraftOn}%
	\DraftOn%
}
\DeclareDocumentCommand{\SetNoDraft}{}{%
	\Deprecated@Notice{Use of command SetNoDraft is deprecated. Use DraftOff}%
	\DraftOff%
}


\appto\maketitle{%
	\if@MCLabPaper@draft%
		\iftoggle{@MCLabPaper@draft@show@buttons}{%
			\ButtonTutorial%
			~%
			\ButtonBiblio%
		}{}%
	\fi%
}




\DeclareDocumentCommand{\DraftGetCommandForCurrentStatus}{m}{%
	% #1: output macro 
	\if@MCLabPaper@draft%
		\xdef@macro{#1}{\DraftOn[\@MCLabPaper@draft@options]}%		
	\else%
		\gdef@macro{#1}{\DraftOff}%
	\fi%
}





% IMPLEMENTATION USING mdframed

%\MCLabPaper@RequirePackage{todonotes}
\MCLabPaper@RequirePackage{soulutf8} %soul (inline draft messages)

\mdfdefinestyle{draftmessage}{skipabove=2pt, skipbelow=2pt, innertopmargin=4pt, innerbottommargin=4pt}
\ArrayNew{DraftNoteStyle} % severity --> bg color
\ArrayAdd{DraftNoteStyle}{linecolor=black!20, skipabove=0.5pt, skipbelow=0.5pt, innertopmargin=2pt, innerbottommargin=2pt} % level 0: system notes
\ArrayAdd{DraftNoteStyle}{linecolor=black!50} % level 1: user notes
\ArrayAdd{DraftNoteStyle}{linecolor=black!50} % level 2: user warning
\ArrayAdd{DraftNoteStyle}{linecolor=red} % level 3: user serious errors

\ArrayNew{DraftNoteStyleColor}
\ArrayAdd{DraftNoteStyleColor}{black!3} % level 0: system notes
\ArrayAdd{DraftNoteStyleColor}{green!10} % level 1: user notes
\ArrayAdd{DraftNoteStyleColor}{orange!50} % level 2: user warning
\ArrayAdd{DraftNoteStyleColor}{red!40} % level 3: user serious errors


\DeclareDocumentCommand{\Draft@Message}{s o m +m}{%
	% #1: star --> inline 
	% #2: author (optional)
	% #3: severity level
	% #4: message
	\if@MCLabPaper@draft%
		\IfPreambleTF{}{%
			\ArrayGet[\Draft@Message@style]{DraftNoteStyle}{#3}%
			\ArrayGet[\Draft@Message@color]{DraftNoteStyleColor}{#3}%
			\IfBooleanTF{#1}{% star: inline
				\expandafter\colorbox{\Draft@Message@color}{%
					\IfValueT{#2}{\textbf{#2}: }#4%
				}%
			}{%
				% no star: DraftNote paragraph
				\xdef\Draft@Message@options{style=draftmessage, \Draft@Message@style, backgroundcolor=\Draft@Message@color}%
				%\Debug@Out@Draft{***** options [\Draft@Message@options]}%
				%\expandafter\todo\expandafter[\Draft@Message@options]{%
				%	\IfValueT{#2}{\textbf{#2}\newline}#4%
				%}%
				%
				\IfValueT{#2}{%
					\xdef\Draft@Message@options{\Draft@Message@options, frametitle={#2}}%
				}%
				%\Debug@Out@Draft{***** options [\Draft@Message@options]}%
				\expandafter\mdframed\expandafter[\Draft@Message@options]%
					#4%
				\endmdframed%
			}%
		}%
	\fi%
}
	
\DeclareDocumentCommand{\DraftNote}{s o +m}{%
	% #1: star -> inline
	% #2: author
	% #3: note
	\iftoggle{@MCLabPaper@draft@show@notes}{%
		\IfBooleanTF{#1}{% star: inline
			\Draft@Message*[#2]{1}{#3}%
		}{%
			\Draft@Message[#2]{1}{#3}%
		}%
	}{}%
}
\DeclareDocumentCommand{\DraftWarning}{s o +m}{%
	% #1: star -> inline
	% #2: author
	% #3: note
	\IfBooleanTF{#1}{% star: inline
		\Draft@Message*[#2]{2}{#3}%
	}{%
		\Draft@Message[#2]{2}{#3}%
	}%
}
\DeclareDocumentCommand{\DraftError}{s o +m}{%
	% #1: star -> inline
	% #2: author
	% #3: note
	\IfBooleanTF{#1}{% star: inline
		\Draft@Message*[#2]{3}{#3}%
	}{%
		\Draft@Message[#2]{3}{#3}%
	}%
}

	
\DeclareDocumentCommand{\Draft@SystemNote}{+m}{%
	\iftoggle{@MCLabPaper@draft@show@sysnotes}{%
		\Draft@Message{0}{\small{\textcolor{black!40}{\begin{scriptsize}#1\end{scriptsize}}}}%
	}{}%
}

\DeclareDocumentCommand{\Draft@Data}{+m}{%
	\IfDraftTF{%
		\iftoggle{@MCLabPaper@draft@emph@data}{%
			{\color{data}#1}%
			% Within tabulars \color{} messes with vertical alignment. 
			% Not solvable, as \textcolor{} (which does not have this 
			% problem, cannot be used, as data entries could be \long.
			% https://tex.stackexchange.com/questions/31547/color-changes-cell-height-in-tabular
		}{#1}%
	}{#1}%
}
\DeclareDocumentCommand{\Draft@Math}{+m}{%
	\IfDraftTF{%
		\iftoggle{@MCLabPaper@draft@emph@math}{%
			\textcolor{math}{#1}%
		}{#1}%
	}{#1}%
}


\newif\ifMathEval@Show@Computations
\MathEval@Show@Computationsfalse
\DeclareDocumentCommand{\DraftMathComputationsOn}{}{%
	\MathEval@Show@Computationstrue
}
\DeclareDocumentCommand{\DraftMathComputationsOff}{}{%
	\MathEval@Show@Computationsfalse
}

\DeclareDocumentCommand{\DraftShowMathComputations}{}{%
	\Deprecated@Notice{Use of command DraftShowMathComputations is deprecated. Use DraftMathComputationsOn}%
	\DraftMathComputationsOn%
}

\DeclareDocumentCommand{\DraftHideMathComputations}{}{%
	\Deprecated@Notice{Use of command DraftHideMathComputations is deprecated. Use DraftMathComputationsOff}%
	\DraftMathComputationsOff%
}
	
% Content categories (which are also color names)
\definecolor{data}{rgb}{0.47, 0.32, 0.66}
\definecolor{math}{rgb}{0.0, 0.47, 0.44}

\DeclareDocumentCommand{\Draft@Highlight}{m +m}{%
	% #1: category (which is also a color name)
	% #2: content
	\IfDraftTF{%
		\textcolor{#1}{#2}%
	}{#2}%
}


\DeclareDocumentCommand{\Draft@Image@Placeholder}{m}{%
	% #1: image filepath relative to current file
		\GetCurrentDir[\tmpCWD]%
		\begin{mdframed}[style=draftmessage, frametitle={Figure omitted}]%
			\begin{center}
				Here will go figure file \RenderFileName{#1}
				\par\medskip\par
				I checked: file file exists, relax!
			\end{center} 
			\par
			{\sloppy\tiny{Figure filepath from root folder is:
				\newline 
				\RenderFileName{\tmpCWD/#1}%
			}}%
		\end{mdframed}%
}%
	
\colorlet{textplaceholder}{black!30}
\DeclareDocumentCommand{\DraftTextPlaceholder}{m}{%
	% #1: number of lines
	\IfDraftTF{%
		\noindent%
		\xintFor* ##1 in {\xintSeq[1]{1}{#1}} \do{%
			\textcolor{textplaceholder}{(Line ##1)\dotfill}%
			\\%
		}%
	}{}%
}



%\ifdraft
%	
%%	\long\def\DraftNote#1{\todo[inline, color=green!15, bordercolor=black!50]{#1}}
%%	\long\def\DraftWarning#1{\todo[inline, color=orange!50, bordercolor=black!50]{#1}}	
%	%\long\def\@autoNote#1{\todo[inline, color=green!15, bordercolor=black!50]{#1}}
%\else
%%	\long\def\DraftNote#1{}
%%	\long\def\DraftWarning#1{}	
%	%\long\def\@autoNote#1{}
%\fi

\endinput








% IMPLEMENTATION ATTEMPT USING fixme PACKAGE 
\MCLabPaper@RequirePackage{fixme}
\DeclareDocumentCommand{\DraftNote}{+m}{%
	\begin{anfxnote}%
	#1%
	\end{anfxnote}%
}


\ifdraft
	\fxsetup{status=draft}
	\MCLabPaper@RequirePackage{todonotes}
	\long\def\@autoNote#1{\todo[inline, color=green!15, bordercolor=black!50]{#1}}
\else
		\fxsetup{status=final}
		\long\def\@autoNote#1{}
\fi		



\endinput


==> MCLabPaper_Figure_2.tex <==
\MCLabPaper@Set@Tutorial@Section{Figure}{sec:figure}


\DeclareDocumentCommand{\Debug@Out@Figure}{o m}{%
	\Debug@Out{Figure}[#1]{#2}%
}

%% STYLES
\def\Figure@Data@Prefix{MCLabPaper/Figure}

\define@cmdkey{FigureDefineStyle}{style}[default]{} %base style
\define@cmdkey{FigureDefineStyle}{columns}[\relax]{}
\define@cmdkey{FigureDefineStyle}{position}[\relax]{}
\define@cmdkey{FigureDefineStyle}{margin}[\relax]{}
\define@cmdkey{FigureDefineStyle}{colsep}[\relax]{}
\define@cmdkey{FigureDefineStyle}{valign}[\relax]{}
\DeclareDocumentCommand{\FigureDefineStyle}{m m}{
	% #1: style name
	% #2: options (key=value list)
	\setkeys{FigureDefineStyle}{style, columns, position, margin, colsep, valign}%
	\setkeys{FigureDefineStyle}{#2}%
	%
	\pgfglobalkeys{\Figure@Data@Prefix/style/#1/.cd,
		style/.initial/.expand once={\cmdKV@FigureDefineStyle@style}, 
		columns/.initial/.expand once={\cmdKV@FigureDefineStyle@columns}, 
		position/.initial/.expanded={\cmdKV@FigureDefineStyle@position},
		margin/.initial/.expand once={\cmdKV@FigureDefineStyle@margin}, 
		colsep/.initial/.expand once={\cmdKV@FigureDefineStyle@colsep},
		valign/.initial/.expand once={\cmdKV@FigureDefineStyle@valign},
	}%
}

\ifundef{\fps@figure}{%
	\def\fps@figure{tbp}%
}{}%

\FigureDefineStyle{default}{style={}, columns=1, position=\fps@figure, margin=30pt, colsep=20pt, valign=c}
\FigureDefineStyle{2columns}{style=default, columns=2}
\FigureDefineStyle{3columns}{style=default, columns=3}
\FigureDefineStyle{4columns}{style=default, columns=4}

% Counters and length for current figure (accessible to subfigures)
\newlength{\FigureMargin}
\newlength{\SubfigureColSep}
\newlength{\SubfigureWidth}
\newcounter{SubfigureCountInRow}

\define@cmdkey{Figure}{style}[default]{}
\define@cmdkey{Figure}{columns}[\relax]{}
\define@cmdkey{Figure}{position}[\relax]{}
\define@cmdkey{Figure}{margin}[\relax]{}
\define@cmdkey{Figure}{colsep}[\relax]{}
\define@cmdkey{Figure}{valign}[\relax]{}
\DeclareDocumentEnvironment{Figure}{s O{}}
	{% begin
		%
		% Redefine command \newpage inside Figure environment
		%\let\newpage\Figure@New@Page%
		%
		% Process options #2
		\setkeys{Figure}{style, columns, position, margin, colsep, valign}%
		\@expandtwoargs\setkeys{Figure}{style=default, #2}%
		%
		\Debug@Out@Figure[Figure]{Style = [\cmdKV@Figure@style]}%
		%
		\Figure@get@style@options{\cmdKV@Figure@style}%
		% sets vars \Figure@columns, \Figure@position, \Figure@margin, \Figure@colsep, \Figure@valign, 
		%
		% Override options if given
		\ifequals{\cmdKV@Figure@columns}{\relax}{}{%
			\Debug@Out@Figure[Figure]{Overriding columns=\cmdKV@Figure@columns}%
			\def\Figure@columns{\cmdKV@Figure@columns}%
		}%
		\ifequals{\cmdKV@Figure@position}{\relax}{}{%
			\Debug@Out@Figure[Figure]{Overriding position=\cmdKV@Figure@position}%
			\edef\Figure@position{\cmdKV@Figure@position}%
		}%
		\ifequals{\cmdKV@Figure@margin}{\relax}{}{%
			\Debug@Out@Figure[Figure]{Overriding margin=\cmdKV@Figure@margin}%
			\def\Figure@margin{\cmdKV@Figure@margin}%
		}%
		\ifequals{\cmdKV@Figure@colsep}{\relax}{}{%
			\Debug@Out@Figure[Figure]{Overriding colsep=\cmdKV@Figure@colsep}%
			\def\Figure@colsep{\cmdKV@Figure@colsep}%
		}%
		\ifequals{\cmdKV@Figure@valign}{\relax}{}{%
			\Debug@Out@Figure[Figure]{Overriding valign=\cmdKV@Figure@valign}%
			\def\Figure@valign{\cmdKV@Figure@valign}%
		}%
		%
		\Debug@Out@Figure[Figure]{Final values for options:}%
		\Debug@Out@Figure[Figure]{  - columns: [\Figure@columns]}%
		\Debug@Out@Figure[Figure]{  - position: [\Figure@position]}%
		\Debug@Out@Figure[Figure]{  - margin: [\Figure@margin]}%
		\Debug@Out@Figure[Figure]{  - colsep: [\Figure@colsep]}%
		\Debug@Out@Figure[Figure]{  - valign: [\Figure@valign]}%
		%
		\begingroup%
		% Define figure environment (figure or figure*)
		\def\tmpFigureEnv{figure}%
		\IfBooleanT{#1}{%
			\def\tmpFigureEnv{figure*}%
		}%
		%
		\setlength{\FigureMargin}{\Figure@margin}%
		\setlength{\SubfigureColSep}{\Figure@colsep}%
		% Define width of each subfigure:
		%  (\textwidth - 2*margin - (columns-1)*colsep) / columns
		% // \textwidth = with of text (and works also with Figure* in two column mode)
		\setlength{\SubfigureWidth}{%
			(\textwidth - 
				(\FigureMargin * 2) 
				- 
				(\SubfigureColSep * 
					((\Figure@columns) - 1)
				)
			) / (\Figure@columns)
		}%
		%
		% \begin{figure}, \begin{figure*}, \begin{figure}[...], \begin{figure*}[...]
		\Figure@begin@figure%
	}
	{% end
		\Figure@end@figure%		
		\endgroup%		
	}

\newcommand{\Figure@begin@figure}{%
	\ifequals{\Figure@position}{}{%
		\expandafter\csuse\expandafter{\expandafter\tmpFigureEnv\expandafter}%
	}{%
		\expandafter\csuse\expandafter{\expandafter\tmpFigureEnv\expandafter}%
			\expandafter[\Figure@position]%
	}%
	%
	\begin{center}%
		% position = [\Figure@position]
		% figure command: [\tmpFigureEnv]		
		% \par
		% columns = [\cmdKV@Figure@columns]
		% \par
		% colsep = [\cmdKV@Figure@colsep]
		% \par
		% margin = [\cmdKV@Figure@margin]
		% \par
		% width of page: [\the\linewidth]
		% \par
		% width of each subfigure: [\the\SubfigureWidth]
		% \par
		\global\setcounter{SubfigureCountInRow}{1}%
		\IgnoreFollowingSpacesAndPars%
}
\newcommand{\Figure@end@figure}{%
	\end{center}%		
	\csuse{end\tmpFigureEnv}%
}


\newcommand{\FigureNewPage}{%
	\Figure@end@figure%
	\par%
	\Figure@begin@figure\ContinuedFloat%
}

\DeclareCaptionLabelFormat{continued}{#1~#2 (continued)}
\captionsetup[ContinuedFloat]{labelformat=continued}


\newlength{\thisSubfigureWidth}
\define@cmdkey{Subfigure}{valign}[\relax]{}
\define@cmdkey{Subfigure}{columns}[1]{}
\DeclareDocumentEnvironment{Subfigure}{O{}}
	{% begin
		%
		% Process options #1
		\setkeys{Subfigure}{columns, valign}%
		\setkeys{Subfigure}{#1}%
		%
		\ifequals{\cmdKV@Subfigure@valign}{\relax}{%
			\edef\cmdKV@Subfigure@valign{\cmdKV@Figure@valign}%
		}{%
			\Debug@Out@Figure[Subfigure]{Overriding: valign=\cmdKV@Subfigure@valign{} in subfigure}%
		}%
		%
		\setlength{\thisSubfigureWidth}{%
			(\SubfigureWidth * \cmdKV@Subfigure@columns) + 
			(
				(\SubfigureColSep) * 
					(\cmdKV@Subfigure@columns-1)
			)
		}%
		%
		% Check if we need to add a hspace or \par
		\ifnumcomp{\Figure@columns}{<}{\theSubfigureCountInRow + \cmdKV@Subfigure@columns - 1}%
			{%	subfigure will not fit in current row
        		\global\setcounter{SubfigureCountInRow}{1}%
        		\par%
      		}{}%
      	% invariant: subfigure will fit in current row
      	\ifnumcomp{\theSubfigureCountInRow}{=}{1}{% 
      		% this is first subfig in row, nothing to do
      	}{%
      		% this is not the first subfig in current row -> add colsep space
  	      	\noindent\hspace{\SubfigureColSep}%
  	      	%|
        	%\the\SubfigureColSep%
        }%
      	% 
		%
		\begin{subfigure}[\cmdKV@Subfigure@valign]{\thisSubfigureWidth}%
		%\subcaptionbox{my caption}[\thisSubfigureWidth][c]\begingroup%
			%[\cmdKV@Subfigure@valign]
			%\noindent[startcol=\theSubfigureCountInRow; width=\the\thisSubfigureWidth]%
	}%
	{% end
		%\endgroup%
		\end{subfigure}%
        % increment counter to col of next subfig
        \global\addtocounter{SubfigureCountInRow}{\cmdKV@Subfigure@columns}%
      	\IgnoreFollowingSpacesAndPars%
	}


% sets vars \Figure@columns, \Figure@position, \Figure@margin, \Figure@colsep, \Figure@valign traversing styles hierarchy bottom-up
\newcommand{\Figure@get@style@options}[1]{ % #1: style name
	\begingroup%
	\edef\this@style{#1}%
	\pgfglobalkeys{\Figure@Data@Prefix/style/\this@style/style/.get=\Figure@base@style}%
	\ifequals{\Figure@base@style}{}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Base style = empty [\Figure@base@style]}%
	}{%
		% base style available: recursive call
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Base style=[\Figure@base@style] not empty -> recursive call}%
		%
		\Figure@get@style@options{\Figure@base@style}%
	}%
	%
	% override given options
	\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Check whether style specifies 'columns'}%
	\pgfglobalkeys{\Figure@Data@Prefix/style/\this@style/columns/.get=\Figure@columns@override}%
	\ifequals{\Figure@columns@override}{\relax}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{   - no 'columns'}%
	}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{   - overriding columns, now [\Figure@columns@override]}%
		\protected@xdef\Figure@columns{\Figure@columns@override}%
	}%
	%
	\pgfglobalkeys{\Figure@Data@Prefix/style/\this@style/position/.get=\Figure@position@override}%
	\ifequals{\Figure@position@override}{\relax}{}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Overriding position=\Figure@position@override}%
		\protected@xdef\Figure@position{\Figure@position@override}%
	}%
	%
	\pgfglobalkeys{\Figure@Data@Prefix/style/\this@style/margin/.get=\Figure@margin@override}%
	\ifequals{\Figure@margin@override}{\relax}{}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Overriding margin=\Figure@margin@override}%
		\protected@xdef\Figure@margin{\Figure@margin@override}%
	}%
	%
	\pgfglobalkeys{\Figure@Data@Prefix/style/\this@style/colsep/.get=\Figure@colsep@override}%
	\ifequals{\Figure@colsep@override}{\relax}{}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Overriding colsep=\Figure@colsep@override}%
		\protected@xdef\Figure@colsep{\Figure@colsep@override}%
	}%
	%
	\pgfglobalkeys{\Figure@Data@Prefix/style/\this@style/valign/.get=\Figure@valign@override}%
	\ifequals{\Figure@valign@override}{\relax}{}{%
		\Debug@Out@Figure[Figure@get@style@options(\this@style)]{Overriding valign=\Figure@valign@override}%
		\protected@xdef\Figure@valign{\Figure@valign@override}%
	}%
	\endgroup
}

==> MCLabPaper_File_2.tex <==

\MCLabPaper@Set@Tutorial@Section{File}{sec:file}


\DeclareDocumentCommand{\Debug@Out@File}{o m}{%
	\Debug@Out{File}[#1]{#2}%
}


% Creates a file handler
\DeclareDocumentCommand{\FileNewHandler}{m}{%
	\newwrite#1%
}

\newtoggle{FileOpen_absolute}
\define@cmdkey{FileOpen}{absolute}[false]{}
\DeclareDocumentCommand{\FileOpen}{m D(){} O{./} m}{%
	% #1: \handler  
	% #2: (options)
	% #3: [additional path] 
	% #4: filepath 
	\GetCurrentDir[\FileCreate@cwd]%
	\setkeys{FileOpen}{absolute}%	
	\setkeys{FileOpen}{#2}%
	\settoggle{FileOpen_absolute}{\cmdKV@FileOpen@absolute}%
	\iftoggle{FileOpen_absolute}{%
		\def\FileCreate@path{\FileCreate@cwd/#3}%
	}{%
		\def\FileCreate@path{#3}%
	}%
	\def\FileCreate@basename{#4}%
	%
	\edef\FileCreate@fullpathname{\FileCreate@path/\FileCreate@basename}%
	\immediate\openout#1=\FileCreate@fullpathname%
}

\DeclareDocumentCommand{\FileWriteLine}{m +m}{%
	% #1: \handler,  #2: text
	\immediate\write#1{#2}%
}

\DeclareDocumentCommand{\FileClose}{m}{%
	% #1: \handler
	\immediate\closeout#1%
}

\def\WriteToAuxFile@Delayed{\write\@auxout}% % check-out Data module for usage
\def\WriteToAuxFile{\immediate\write\@auxout}

% \DeclareDocumentCommand{\FileAppend}{m +m}{%
% 	% #1: filepath (relative to caller)
% 	% #2: content
% 	\GetCurrentDir[\Append@To@File@cwd]
% 	\Debug@Out@File{Append@To@File{#1}{#2}: start}%
% 	\protected@edef\Append@To@File@handler{\csname#1-handler\endcsname}%	
% 	\ifcsundef{file #1 open}{%
% 		\Debug@Out@File{Append@To@File: file '#1' is not already open}%
% 		\expandafter\newwrite\Append@To@File@handler%
% 		\immediate\expandafter\openout\Append@To@File@handler=\Append@To@File@cwd/#1%
% 		\Debug@Out@File{Append@To@File: file '#1' opened}%
% 		\csgdef{file #1 open}{}%
% 	}{}%
% 	\Debug@Out@File{Append@To@File: writing '#2' to file '#1'}%	
% 	\immediate\expandafter\write\Append@To@File@handler{#2}%
% 	\Debug@Out@File{Append@To@File{#1}{#2}: end}%
% }




\DeclareDocumentCommand{\ShellExec}{O{./} m}{%	
	\GetCurrentDir[\ShellExec@cwd]%
	\def\ShellExec@path{\ShellExec@cwd/#1}%
	\edef\ShellExec@fullcommand{pushd \ShellExec@path  ; #2 ; popd}%
	\typeout{Executing shell command: \ShellExec@fullcommand}%
	\immediate\write18{\ShellExec@fullcommand}%
}


\DeclareDocumentCommand{\FileModTimeStamp}{o m}{%
	\edef\FileModTimeStamp@result{\pdffilemoddate{#2}}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\FileModTimeStamp@result}%
	}{\FileModTimeStamp@result}%
}


==> MCLabPaper_Float_2.tex <==
\MCLabPaper@Set@Tutorial@Section{Float}{sec:float}


\DeclareDocumentCommand{\Debug@Out@Float}{o m}{%
	\Debug@Out{Float}[#1]{#2}%
}

%% STYLES (independent of float type)
\def\Float@Data@Prefix{MCLabPaper/Float}

\define@cmdkey{FloatDefineStyle}{style}[default]{} %base style
\define@cmdkey{FloatDefineStyle}{columns}[\relax]{}
\define@cmdkey{FloatDefineStyle}{position}[\relax]{}
\define@cmdkey{FloatDefineStyle}{margin}[\relax]{}
\define@cmdkey{FloatDefineStyle}{colsep}[\relax]{}
\define@cmdkey{FloatDefineStyle}{valign}[\relax]{}
\define@choicekey*{FloatDefineStyle}{center}[\cmdKV@FloatDefineStyle@center]{true,false,\relax}[\relax]{}% true | false | \relax
\DeclareDocumentCommand{\FloatDefineStyle}{m m}{
	% #1: style name
	% #2: options (key=value list)
	\setkeys{FloatDefineStyle}{style, columns, position, margin, colsep, valign, center}%
	\setkeys{FloatDefineStyle}{#2}%
	%
	\pgfglobalkeys{\Float@Data@Prefix/style/#1/.cd,
		style/.initial/.expand once={\cmdKV@FloatDefineStyle@style}, 
		columns/.initial/.expand once={\cmdKV@FloatDefineStyle@columns}, 
		position/.initial/.expanded={\cmdKV@FloatDefineStyle@position},
		margin/.initial/.expand once={\cmdKV@FloatDefineStyle@margin}, 
		colsep/.initial/.expand once={\cmdKV@FloatDefineStyle@colsep},
		valign/.initial/.expand once={\cmdKV@FloatDefineStyle@valign},
		center/.initial/.expand once={\cmdKV@FloatDefineStyle@center}
	}%
}

%\def\Float@Default@Positions{tbp}%
\ifundef{\fps@figure}{%
	\def\fps@figure{tbp}%
}{}%

\FloatDefineStyle{default}{style={}, columns=1, 
	position=\fps@figure, margin=30pt, colsep=20pt, valign=c, center=true}
\FloatDefineStyle{2columns}{style=default, columns=2}
\FloatDefineStyle{3columns}{style=default, columns=3}
\FloatDefineStyle{4columns}{style=default, columns=4}

% Counters and length for current float (accessible to subfloats)
\newlength{\FloatMargin}
\newlength{\SubfloatColSep}
\newlength{\SubfloatWidth}
\newcounter{SubfloatCountInRow}

\define@cmdkey{Float}{type}{}
\define@cmdkey{Float}{style}[default]{}
\define@cmdkey{Float}{columns}[\relax]{}
\define@cmdkey{Float}{position}[\relax]{}
\define@cmdkey{Float}{margin}[\relax]{}
\define@cmdkey{Float}{colsep}[\relax]{}
\define@cmdkey{Float}{valign}[\relax]{}
\define@choicekey*{Float}{center}[\cmdKV@Float@center]{true,false,\relax}[\relax]{}% true | false | \relax

\newtoggle{Float@Center}%
\DeclareDocumentEnvironment{@Float}{s O{}}
	{% begin
		%
		% Redefine command \newpage inside Float environment
		%\let\newpage\Float@New@Page%
		%
		% Process options #2
		\setkeys{Float}{style, columns, position, margin, colsep, valign, center}%
		\@expandtwoargs\setkeys{Float}{style=default, #2}%
		%
		\Debug@Out@Float[Float]{Style = [\cmdKV@Float@style]}%
		%
		\Float@get@style@options{\cmdKV@Float@style}%
		% sets vars \Float@columns, \Float@position, \Float@margin, \Float@colsep, \Float@valign, \Float@center
		%
		% Override options if given
		\ifequals{\cmdKV@Float@columns}{\relax}{}{%
			\Debug@Out@Float[Float]{Overriding columns=\cmdKV@Float@columns}%
			\def\Float@columns{\cmdKV@Float@columns}%
		}%
		\ifequals{\cmdKV@Float@position}{\relax}{}{%
			\Debug@Out@Float[Float]{Overriding position=\cmdKV@Float@position}%
			\edef\Float@position{\cmdKV@Float@position}%
		}%
		\ifequals{\cmdKV@Float@margin}{\relax}{}{%
			\Debug@Out@Float[Float]{Overriding margin=\cmdKV@Float@margin}%
			\def\Float@margin{\cmdKV@Float@margin}%
		}%
		\ifequals{\cmdKV@Float@colsep}{\relax}{}{%
			\Debug@Out@Float[Float]{Overriding colsep=\cmdKV@Float@colsep}%
			\def\Float@colsep{\cmdKV@Float@colsep}%
		}%
		\ifequals{\cmdKV@Float@valign}{\relax}{}{%
			\Debug@Out@Float[Float]{Overriding valign=\cmdKV@Float@valign}%
			\def\Float@valign{\cmdKV@Float@valign}%
		}%
		\ifequals{\cmdKV@Float@center}{\relax}{}{%
			\Debug@Out@Float[Float]{Overriding center=\cmdKV@Float@center}%
			\def\Float@center{\cmdKV@Float@center}%
		}%
		\let\Float@type\cmdKV@Float@type%
		\settoggle{Float@Center}{\Float@center}%
		%
		\Debug@Out@Float[Float]{Final values for options:}%
		\Debug@Out@Float[Float]{  - type: [\Float@type]}%
		\Debug@Out@Float[Float]{  - columns: [\Float@columns]}%
		\Debug@Out@Float[Float]{  - position: [\Float@position]}%
		\Debug@Out@Float[Float]{  - margin: [\Float@margin]}%
		\Debug@Out@Float[Float]{  - colsep: [\Float@colsep]}%
		\Debug@Out@Float[Float]{  - valign: [\Float@valign]}%
		\Debug@Out@Float[Float]{  - center: [\Float@center]}%
		%
		\begingroup%
		% Define float environment (float or float*)
		\edef\tmpFloatEnv{\Float@type}%
		\IfBooleanT{#1}{%
			\edef\tmpFloatEnv{\Float@type*}%
		}%
		%
		\setlength{\FloatMargin}{\Float@margin}%
		\setlength{\SubfloatColSep}{\Float@colsep}%
		% Define width of each subfloat:
		%  (\textwidth - 2*margin - (columns-1)*colsep) / columns
		% // \textwidth = with of text (and works also with Float* in two column mode)
		\setlength{\SubfloatWidth}{%
			(\textwidth - 
				(\FloatMargin * 2) 
				- 
				(\SubfloatColSep * 
					((\Float@columns) - 1)
				)
			) / (\Float@columns)
		}%
		%
		% \begin{float}, \begin{float*}, \begin{float}[...], \begin{float*}[...]
		\Float@begin@float%
	}
	{% end
		\Float@end@float%		
		\endgroup%
		\undef\Float@type%
	}

\newcommand{\Float@begin@float}{%
	\Debug@Out@Float[Begin@Float]{start}%
	\ifequals{\Float@position}{}{%
		\Debug@Out@Float[Begin@Float]{ - No explicit positioning}%
		\expandafter\csuse\expandafter{\expandafter\tmpFloatEnv\expandafter}%
	}{%
		\Debug@Out@Float[Begin@Float]{ - Explicit positioning [\Float@position]}%
		\expandafter\csuse\expandafter{\expandafter\tmpFloatEnv\expandafter}%
			\expandafter[\Float@position]%
	}%
	%
	\Debug@Out@Float[Begin@Float]{ - Checking whether centering is requested}%
	\iftoggle{Float@Center}{%
		\begin{center}%
		\Debug@Out@Float[Begin@Float]{ - Applying centering}%
	}{%
		\Debug@Out@Float[Begin@Float]{ - NOT applying centering}%
	}%
		% position = [\Float@position]
		% float command: [\tmpFloatEnv]		
		% \par
		% columns = [\cmdKV@Float@columns]
		% \par
		% colsep = [\cmdKV@Float@colsep]
		% \par
		% margin = [\cmdKV@Float@margin]
		% \par
		% width of page: [\the\linewidth]
		% \par
		% width of each subfloat: [\the\SubfloatWidth]
		% \par
		\global\setcounter{SubfloatCountInRow}{1}%
		\IgnoreFollowingSpacesAndPars%
}
\newcommand{\Float@end@float}{%
	\iftoggle{Float@Center}{%
		\end{center}%
		\Debug@Out@Float[Begin@Float]{ - Stopping centering}%
	}{}%
	\csuse{end\tmpFloatEnv}%
}


\newcommand{\FloatNewPage}{%
	\Float@end@float%
	\par%
	\Float@begin@float\ContinuedFloat%
}

\DeclareCaptionLabelFormat{continued}{#1~#2 (continued)}
\captionsetup[ContinuedFloat]{labelformat=continued}


\newlength{\thisSubfloatWidth}
\define@cmdkey{Subfloat}{valign}[\relax]{}
\define@cmdkey{Subfloat}{columns}[1]{}
\newtoggle{Subfloat@Center}
\define@choicekey*{Subfloat}{center}[\cmdKV@Subfloat@center]{true,false,\relax}[\relax]{}% true | false | \relax
\DeclareDocumentEnvironment{@Subfloat}{O{}}
	{% begin
		%
		% Process options #1
		\setkeys{Subfloat}{columns, valign, center}%
		\setkeys{Subfloat}{#1}%
		%
		\ifequals{\cmdKV@Subfloat@valign}{\relax}{%
			\edef\cmdKV@Subfloat@valign{\Float@valign}%
			\Debug@Out@Float[Subfloat]{Inheriting property from including Float: valign=\cmdKV@Subfloat@valign{}}%
		}{%
			\Debug@Out@Float[Subfloat]{Overriding: valign=\cmdKV@Subfloat@valign{} in subfloat}%
		}%
		\ifequals{\cmdKV@Subfloat@center}{\relax}{%
			\edef\cmdKV@Subfloat@center{\Float@center}%
			\Debug@Out@Float[Subfloat]{Inheriting property from including Float: center=\cmdKV@Subfloat@center{}}%
		}{%
			\Debug@Out@Float[Subfloat]{Overriding: center=\cmdKV@Subfloat@center{} in subfloat}%
		}%
		%
		\setlength{\thisSubfloatWidth}{%
			(\SubfloatWidth * \cmdKV@Subfloat@columns) + 
			(
				(\SubfloatColSep) * 
					(\cmdKV@Subfloat@columns-1)
			)
		}%
		%
		% Check if we need to add a hspace or \par
		\ifnumcomp{\Float@columns}{<}{\theSubfloatCountInRow + \cmdKV@Subfloat@columns - 1}%
			{%	subfloat will not fit in current row
        		\global\setcounter{SubfloatCountInRow}{1}%
        		\par%
      		}{}%
      	% invariant: subfloat will fit in current row
      	\ifnumcomp{\theSubfloatCountInRow}{=}{1}{% 
      		% this is first subfig in row, nothing to do
      	}{%
      		% this is not the first subfig in current row -> add colsep space
  	      	\noindent\hspace{\SubfloatColSep}%
  	      	%|
        	%\the\SubfloatColSep%
        }%
      	% 
		%
		\settoggle{Subfloat@Center}{\cmdKV@Subfloat@center}%
		\csuse{sub\Float@type}[\cmdKV@Subfloat@valign]{\thisSubfloatWidth}%
		\iftoggle{Subfloat@Center}{%
			\begin{center}%
			\Debug@Out@Float[@Subfloat]{ - Applying centering}%
		}{%
			\Debug@Out@Float[@Subfloat]{ - NOT applying centering}%
		}%
		%\subcaptionbox{my caption}[\thisSubfloatWidth][c]\begingroup%
			%[\cmdKV@Subfloat@valign]
			%\noindent[startcol=\theSubfloatCountInRow; width=\the\thisSubfloatWidth]%
	}%
	{% end
		%\endgroup%
		\iftoggle{Subfloat@Center}{%
			\end{center}%
			\Debug@Out@Float[@Subfloat]{ - Stop centering}%
		}{}%
		\csuse{endsub\Float@type}%		
        % increment counter to col of next subfig
        \global\addtocounter{SubfloatCountInRow}{\cmdKV@Subfloat@columns}%
      	\IgnoreFollowingSpacesAndPars%
	}


% sets vars \Float@columns, \Float@position, \Float@margin, \Float@colsep, \Float@valign, \Float@center traversing styles hierarchy bottom-up
\newcommand{\Float@get@style@options}[1]{ % #1: style name
	\begingroup%
	\edef\this@style{#1}%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/style/.get=\Float@base@style}%
	\ifequals{\Float@base@style}{}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Base style = empty [\Float@base@style]}%
	}{%
		% base style available: recursive call
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Base style=[\Float@base@style] not empty -> recursive call}%
		%
		\Float@get@style@options{\Float@base@style}%
	}%
	%
	% override given options
	\Debug@Out@Float[Float@get@style@options(\this@style)]{Check whether style specifies 'columns'}%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/columns/.get=\Float@columns@override}%
	\ifequals{\Float@columns@override}{\relax}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{   - no 'columns'}%
	}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{   - overriding columns, now [\Float@columns@override]}%
		\protected@xdef\Float@columns{\Float@columns@override}%
	}%
	%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/position/.get=\Float@position@override}%
	\ifequals{\Float@position@override}{\relax}{}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Overriding position=\Float@position@override}%
		\protected@xdef\Float@position{\Float@position@override}%
	}%
	%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/margin/.get=\Float@margin@override}%
	\ifequals{\Float@margin@override}{\relax}{}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Overriding margin=\Float@margin@override}%
		\protected@xdef\Float@margin{\Float@margin@override}%
	}%
	%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/colsep/.get=\Float@colsep@override}%
	\ifequals{\Float@colsep@override}{\relax}{}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Overriding colsep=\Float@colsep@override}%
		\protected@xdef\Float@colsep{\Float@colsep@override}%
	}%
	%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/valign/.get=\Float@valign@override}%
	\ifequals{\Float@valign@override}{\relax}{}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Overriding valign=\Float@valign@override}%
		\protected@xdef\Float@valign{\Float@valign@override}%
	}%
	\pgfglobalkeys{\Float@Data@Prefix/style/\this@style/center/.get=\Float@center@override}%
	\ifequals{\Float@center@override}{\relax}{}{%
		\Debug@Out@Float[Float@get@style@options(\this@style)]{Overriding center=\Float@center@override}%
		\protected@xdef\Float@center{\Float@center@override}%
	}%
	\endgroup
}



%%%% Public API: Figure, Table

\DeclareDocumentCommand{\FloatNewType}{m m}{% 
	% #1: new environment name, e.g., Figure, Table, etc. 
	% #2: environment to use, e.g., figure, table, etc.
	%
	\DeclareDocumentEnvironment{#1}{s O{}}{%
		\IfBooleanTF{##1}{%
			\def\FloatNewType@begin@cmd{\@Float*[type=#2, ##2]}%
		}{%
			\def\FloatNewType@begin@cmd{\@Float[type=#2, ##2]}
		}%
		\FloatNewType@begin@cmd%
		\cslet{Sub#1}{\@Subfloat}%
		\cslet{endSub#1}{\end@Subfloat}%
	}{%
		\end@Float%
	}%
}

% Standard Float types
\FloatNewType{Figure}{figure}
\FloatNewType{Table}{table}

% Fake Algorithm environment
%\let\Algorithm\algorithm%
%\let\endAlgorithm\endalgorithm



==> MCLabPaper_Glossary_2.tex <==
\MCLabPaper@RequirePackage{datatool}

\MCLabPaper@Set@Tutorial@Section{Glossary}{sec:glossary}


\DeclareDocumentCommand{\Debug@Out@Gloss}{o m}{%
	\Debug@Out{Glossary}[#1]{#2}%
}

\addto\captionsenglish{%
  \def\MCLabPaper@glossaryname{Glossary}%
  \def\MCLabPaper@Glossary@plural@postfix{s}%
}

\addto\captionsitalian{%
  \def\MCLabPaper@glossaryname{Glossario}%  
  \def\MCLabPaper@Glossary@plural@postfix{}%
}
\newcommand{\GlossaryMark}[1]{}% % macro invoked when Glossary (list) is printed

\xdef\GlossPrefix{\pgfkeysPrefix/Glossary}%

%\CommaSepListNew{@List}% contains short versions of acronyms, not acronyms
%\define@cmdkey{NewAcronym}{shortplural}[]{}%
%\define@cmdkey{NewAcronym}{longplural}[]{}%
% \DeclareDocumentCommand{\GlossaryNew}{D(){} m}{%
% 	% #1: (options) currently none
% 	% #2: glossary name
% 	\pgfglobalkeysifdefined{\GlossPrefix/#2}{%
% 		\DiagError{Glossary}{Glossary '#2' already defined}%
% 	}{}%
% }

\ArrayNew{GlossaryDefinition}
\ArrayPush{GlossaryDefinition}{unnamed glossary}%

\DeclareDocumentEnvironment{Glossary}{D(){} m}{%
	% #1: (options) currently none
	% #2: glossary name
	\GlossaryPush{#2}%	
}{%
	\GlossaryPop%	
}

\DeclareDocumentCommand{\GlossaryPush}{m}{%
	\ArrayPush{GlossaryDefinition}{#1}%
	\Debug@Out@Gloss[GlossaryPush]%
			{Pushed glossary name '#1' in array}%
}
\DeclareDocumentCommand{\GlossaryPop}{}{%
	\ArrayPop{GlossaryDefinition}%
	\Debug@Out@Gloss[GlossaryPop]%
			{Popped glossary from array}%
}

\DeclareDocumentCommand{\Glossary@Get@Name}{m m}{%
	% #1: \result
	% #2: user-given name, possibly \NoValue
	\IfValueTF{#2}{% Glossary name given
		\edef@macro{#1}{#2}%
	}{%
		\ArrayTop[\Glossary@Get@Name@glossary]{GlossaryDefinition}%
		\edef@macro{#1}{\Glossary@Get@Name@glossary}%
	}%
}

\define@cmdkey{GlossaryNewTerm}{plural}[]{}
\DeclareDocumentCommand{\GlossaryNewTerm}{D(){} o m o +m O{}}{%
	% #1: (options) currently none
	% #2: [glossary]
	% #3: id	
	% #4: [Term]
	% #5: Definition
	% [#6]: Variants
	%
	\setkeys{GlossaryNewTerm}{plural}%
	\setkeys{GlossaryNewTerm}{#6}%
	%
	\Glossary@Get@Name{\Glossary@NewTerm@glossary}{#2}%
	%
	\def\Glossary@NewTerm@id{#3}%
	\IfValueTF{#4}{% Glossary term given
		\def\Glossary@NewTerm@term{#4}%
	}{%
		\def\Glossary@NewTerm@term{#3}%
	}%
	\long\def\Glossary@NewTerm@def{#5}%
	%
	% Process variants
	\ifequals{\cmdKV@GlossaryNewTerm@plural}{}{%
		\def\Glossary@NewTerm@term@plural{\Glossary@NewTerm@term\MCLabPaper@Glossary@plural@postfix}%
	}{%
		\let\Glossary@NewTerm@term@plural\cmdKV@GlossaryNewTerm@plural%
	}%
	\pgfglobalkeys{\GlossPrefix/\Glossary@NewTerm@glossary/.cd,		
		terms/\Glossary@NewTerm@id/name/.initial/.expanded = {\Glossary@NewTerm@term},
		terms/\Glossary@NewTerm@id/name/plural/.initial/.expanded = {\Glossary@NewTerm@term@plural},
		terms/\Glossary@NewTerm@id/id/.initial/.expanded = {\Glossary@NewTerm@id},
		terms/\Glossary@NewTerm@id/definition/.initial/.expanded = {\Glossary@NewTerm@def},
		list of terms/.append to list/.expanded = {\Glossary@NewTerm@id},%
		%number of terms/.add to int = 1%
	}%
	\Debug@Out@Gloss[{GlossaryNewTerm(#1)[\Glossary@NewTerm@glossary]{\Glossary@NewTerm@id}{\Glossary@NewTerm@term}{\Glossary@NewTerm@def}}]{Done}%
}%

\newcommand{\Glossary@Label}[2]{%
	% #1: glossary name
	% #2: term id
	MCLabPaper:Glossary:#1:#2%
}




% Use glossary term
\DeclareDocumentCommand{\GlossaryTermp}{t^ o m o}{%
	\IfBooleanTF{#1}{%
		\GlossaryTerm+^[#2]{#3}[#4]%
	}{%
		\GlossaryTerm+[#2]{#3}[#4]%
	}%
}
\DeclareDocumentCommand{\GlossaryTerm}{t+ t^ o m o}{%
	% #1: optional + (plural)
	% #2: optional ^ (capitalise term)
	% #3: [glossary name]
	% #4: term id
	% #5: [shown term] (=term name if not given)
	\def\Glossary@Term@id{#4}%
	\Debug@Out@Gloss[{GlossaryTerm[...]{\Glossary@Term@id}[...]}]%
		{Start}%
	\Glossary@Get@Name{\Glossary@Term@glossary}{#3}%
	\Debug@Out@Gloss[{GlossaryTerm[...]{\Glossary@Term@id}[...]}]%
			{Glossary name: '\Glossary@Term@glossary'}%
	%
	\pgfglobalkeysifdefined{\GlossPrefix/\Glossary@Term@glossary/terms/%
			\Glossary@Term@id/id}{%
		% term exists
		\IfValueTF{#5}{%
			% user has decided how to show the term
			\def\Glossary@Term@term{#5}%	
		}{%
			% get term name to be shown
			\IfBooleanTF{#1}{%
				% plural
				\pgfglobalkeys{%
					\GlossPrefix/\Glossary@Term@glossary/terms/%
						\Glossary@Term@id/name/plural/.get = \Glossary@Term@term%
				}%
			}{% singular
				\pgfglobalkeys{%
					\GlossPrefix/\Glossary@Term@glossary/terms/%
						\Glossary@Term@id/name/.get = \Glossary@Term@term%
				}%
			}%
			%
			% Capitalise, if requested
			\IfBooleanT{#2}{%
				\CapitaliseFirst[\Glossary@Term@term]{\Glossary@Term@term}%
			}%
		}%
		%
		%
		\expandafter\hyperlink\expandafter{%
			\Glossary@Label{\Glossary@Term@glossary}{\Glossary@Term@id}%
		}{\Glossary@Term@term}\xspace%
		% Disable link:
		%\Glossary@Term@term\xspace%
	}{%
		\DiagError{Glossary}{Term id='\Glossary@Term@id' does not exist in glossary '\Glossary@Term@glossary'}%
	}%
}

\newlist{glossarytermslist}{description}{10}


\define@cmdkey{GlossaryList}{enumitemoptions}[style=nextline]{}
\DeclareDocumentCommand{\GlossaryList}{D(){} o}{%
	% #1: (options) currently none
	% [#2]: glossary
	%
	% Set default values for options having a default
	\setkeys{GlossaryList}{enumitemoptions}%
	\Glossary@Get@Name{\GlossaryList@glossary}{#2}%
	%
	\Debug@Out@Gloss[GlossaryList(enumitemoptions=%
		'...')%
		{'\GlossaryList@glossary'}]{Start. Default value for enumitemoptions = '\cmdKV@GlossaryList@enumitemoptions'}%
	\@expandtwoargs\setkeys{GlossaryList}{#1}%	
	\Debug@Out@Gloss[GlossaryList(enumitemoptions=%
		'\cmdKV@GlossaryList@enumitemoptions')%
		{'\GlossaryList@glossary'}]{Start}%
	%
	\pgfglobalkeysifdefined{\GlossPrefix/\GlossaryList@glossary/list of terms}{%
		\pgfglobalkeys{%
			\GlossPrefix/\GlossaryList@glossary/list of terms/.get = %
				\Glossary@List@terms%
		}%
		\Debug@Out@Gloss[GlossaryList(enumitemoptions='\cmdKV@GlossaryList@enumitemoptions', #2)]{List of terms: '\Glossary@List@terms'}%
		\ifdef{\dtlsortlist}{%
			\dtlsortlist{\Glossary@List@terms}{\dtlcompare}%
		}{%
			\PackageWarning{MCLabPaper}{You have an old version of the datatool package (older than 2016-07-28). Please, update your Latex Platform. As a result, glossary '\GlossaryList@glossary' is not sorted.}%
			\DraftWarning[MCLabPaper]{You have an old version of the datatool package (older than 2016-07-28). Please, update your Latex Platform.\\ As a result, glossary '\GlossaryList@glossary' is not sorted.}%
		}%
		%
		\begin{Section}*{\MCLabPaper@glossaryname}%	
		\GlossaryMark{\MCLabPaper@glossaryname}%
 		\def\GlossaryList@tmp@cmd##1{\glossarytermslist[##1]}% 
 		\expandafter\GlossaryList@tmp@cmd\expandafter{\cmdKV@GlossaryList@enumitemoptions}%
 			%
 			\xintFor ##1 in {\Glossary@List@terms} \do{%	
				\pgfglobalkeys{\GlossPrefix/\GlossaryList@glossary/terms/.cd,
					##1/name/.get = \Glossary@List@name,
					##1/definition/.get = \Glossary@List@definition
				}%
				\Debug@Out@Gloss[GlossaryList(enumitemoptions='\cmdKV@GlossaryList@enumitemoptions')%
					{'\GlossaryList@glossary'}]{Showing: term='##1', name='\Glossary@List@name', def='\Glossary@List@definition'}%
				%
				\item[\CapitaliseFirst{\Glossary@List@name}] % (id=##1)%  
					\expandafter\hypertarget\expandafter{\Glossary@Label{\GlossaryList@glossary}{##1}}{}% 
					\Glossary@List@definition%
				\IfEndWith{\Glossary@List@definition}{.}{}{.}%
				\par%
 			}%
 		\endglossarytermslist%
 		\end{Section}
		\par%
	}{}% no glossary or no terms in glossary
	\Debug@Out@Gloss[GlossaryList%
		(enumitemoptions='\cmdKV@GlossaryList@enumitemoptions')%
		{'\GlossaryList@glossary'}]{End}%
}%



==> MCLabPaper_Guideline_2.tex <==

\DeclareDocumentCommand{\Debug@Out@Guideline}{o m}{%
	\Debug@Out{Guideline}[#1]{#2}%
}




==> MCLabPaper_Input_2.tex <==
\RequirePackage{pdfpages}

\MCLabPaper@Set@Tutorial@Section{Input}{sec:input}

\DeclareDocumentCommand{\Debug@Out@Input}{o m}{%
	\Debug@Out{Input}[#1]{#2}%
}

\DiagDefineMsgType{missingfile}{
	title={Missing file},
	backgroundcolor={red!30},
	linecolor={black!50}, 
	icon=\Diag@Image@Warning,
	die=false, 
	showinpdf=true, 
	showtutorialbutton=true, 
	showinlog=true
}

\DeclareDocumentCommand{\Input@Diag@Missing@File}{m}{%
	% Call \Diag@Message:
	%  - arg1: \BooleanTrue -> inline, \BooleanFalse -> banner
	%  - (arg2): options
	%  - arg3: module name
	%  - arg4: message to PDF
	%  - arg5: message to log
	\Diag@Message%
		{\BooleanFalse}% \BooleanTrue -> inline
		{missingfile}%	message type
		()%		options
		{Input}%		module name
		{File \RenderFileName{#1} does not exist.}%		message to PDF
		[File '#1' does not exist.]% 	message to log (empty: use msg to PDF)
}


%%% WARNING: Remember to add trailing / to all dirs pushed in stack

\ArrayNew{Directory@Stack}
\ArrayPush{Directory@Stack}{./}
\DeclareDocumentCommand{\GetCurrentDir}{o}{%
	\ArrayTop[\@value]{Directory@Stack}%
	\IfValueTF{#1}{%
		\xdef#1{\@value}%
	}{\@value}%
}

% Array with full filepaths of \Input'ed files. Top is full path to current file.
\ArrayNew{FilePath@Stack}
\ArrayPush{FilePath@Stack}{\jobname.tex}

\DeclareDocumentCommand{\InputCurrentFilePath}{o}{%
	\ArrayTop[\@value]{FilePath@Stack}%
	\IfValueTF{#1}{%
		\xdef#1{\@value}%
	}{%
		\RenderFileName{\@value}%
	}%
}

\define@boolkey{Input}{absolute}[false]{}
\define@boolkey{Input}{sysnotes}[true]{}
%\define@boolkey{Input}{die}[]{}
\DeclareDocumentCommand{\Input}{D(){} O{} m}{%
	% #1: options: absolute=true|false, die=true
	% #2: file path extension wrt. to caller file
	% #3: list of file-paths relative to #2
	%
	% Store value of 'die' option to 
	%   \XKV@KV@Input@die@value for later use
	%\savekeys{Input}{die}%
	\setkeys{Input}{absolute, sysnotes}%, die}%	
	\setkeys{Input}{#1}%	
	%
	%\Debug@Out@Input[Input]{Saved keys: '\XKV@KV@Input@save'}%
	%\Debug@Out@Input[Input]{Value for die='\XKV@KV@Input@die@value'}%
	\edef\Input@base@relpath{#2}%
	\edef\Input@file@list{#3}%
	\ifequals{\Input@base@relpath}{}{}{%
		\IfEndWith{\Input@base@relpath}{/}{}{%
			\edef\Input@base@relpath{\Input@base@relpath/}%
		}% % if non-empty, relpath has now trainling '/'
	}%
	\Debug@Out@Input[{Input(#1)[\Input@base@relpath]{\Input@file@list}}]{Start}%
	\ifKV@Input@absolute%
		\def\current@directory{./}%
		\Debug@Out@Input[Input]{absolute=true -> base directory = [\current@directory]}%
	\else%
		\GetCurrentDir[\current@directory]%
		\Debug@Out@Input[Input]{Current directory: [\current@directory]}%
	\fi%
	%
	\ArrayPush{Directory@Stack}{\current@directory\Input@base@relpath}%
	%
	\xintFor ##1 in {\Input@file@list} \do{%
		\GetCurrentDir[\current@directory]%
		\Debug@Out@Input[Input]{Current directory: [\current@directory]}%
		\Debug@Out@Input[Input]{ - File: [##1]}%	
		\filename@parse{##1}%
		\ArrayPush{Directory@Stack}{\current@directory\filename@area}%
		\GetCurrentDir[\current@directory]%
		\Debug@Out@Input[Input]{Current directory: [\current@directory]}%
		\edef\full@file@path{\current@directory\filename@base.\filename@ext}%
		%
		\ifKV@Input@sysnotes%
			\Draft@SystemNote{Start of file \RenderFileName{\full@file@path}}%
		\fi%
		%
		\Debug@Out@Input[Input]{Including file (fullpath): [\full@file@path]}%
		\IfFileExists{\full@file@path}{%
			\ArrayPush{FilePath@Stack}{\full@file@path}%
			%
			%\IfPreambleTF{}{y}%			
			\input{\full@file@path}%
			%\IfPreambleTF{}{z}%
			\ArrayPop{FilePath@Stack}%
			%\MCLabPaper@Flattening@Append{\input{\full@file@path}}%
		}{%			
			%\DiagError(die=\XKV@KV@Input@die@value){Input}{File \RenderFileName{\full@file@path} does not exist}%
			%	[File \full@file@path\space does not exist]%
			\Input@Diag@Missing@File{\full@file@path}%
		}%
		%\IfPreambleTF{}{a}%
		%
		\ifKV@Input@sysnotes%
			\Draft@SystemNote{End of file \RenderFileName{\full@file@path}}%
		\fi%
		\ArrayPop{Directory@Stack}%
		\GetCurrentDir[\current@directory]%
		\Debug@Out@Input[Input]{Current directory: '\current@directory'}%
		\Debug@Out@Input[Input]{End including file: '##1'}%
		%\IfPreambleTF{}{b}%
	}%
	%
	%\IfValueT{#1}{%
	\ArrayPop{Directory@Stack}%
	%}%
	%\IfPreambleTF{}{c}%
	\GetCurrentDir[\current@directory]%
	\Debug@Out@Input[{Input(#1)[\Input@base@relpath]{\Input@file@list}}]{Current directory: [\current@directory]}%
	\Debug@Out@Input[{Input(#1)[\Input@base@relpath]{\Input@file@list}}]{End}%
	%\IfPreambleTF{}{d}%
}

\define@boolkey{IncludeGraphics}{absolute}[false]{}
\define@boolkey{IncludeGraphics}{center}[true]{}
\ProvideDocumentCommand{\IncludeGraphics}{s O{} m o}{%
	%#1: if star, then no centering (deprecated)
	%#2: width, height, ...
	%#3: local/path/to/image/file
	%#4: overpic optional commands
	%
	% Process options [#2]
	\setkeys{IncludeGraphics}{absolute, center}%
	\setkeys*{IncludeGraphics}{#2}% star: appends undefined keys to \XKV@rm (which can be sent to other commands)
	%
	\Debug@Out@Input[IncludeGraphics[#2]{#3}]{Options to be sent to includegraphics: '\XKV@rm'}%
	\IfBooleanT{#1}{%
		\KV@IncludeGraphics@centerfalse%
		\DiagDeprecation{Input}{Starred command \DiagLatexCmd{IncludeGraphics*} is deprecated. 
		Use \DiagLatexCmd{IncludeGraphics[..., center=false, ...]{...}} instead.}[Starred command \ IncludeGraphics* is deprecated. Use \ IncludeGraphics[.., center=false, ...]{...} instead]%
	}%
	%
	\ifKV@IncludeGraphics@center%
		\begin{center}%
	\fi%
	%
	%
	\ifKV@IncludeGraphics@absolute%
		\edef\current@directory{}%
	\else%
		\GetCurrentDir[\current@directory]%
		\edef\current@directory{\current@directory/}%
	\fi%
	\Debug@Out@Input[IncludeGraphics[#2]{#3}]{Current directory = '\current@directory'}%
	%
	\begingroup%
	\catcode`\_=12%
	\edef\ig@file@path{\current@directory#3}
	\Debug@Out@Input[IncludeGraphics[#2]{#3}]{Input filepath = '\ig@file@path'}%
	\IfFileExists{\ig@file@path}{%
		\iftoggle{@MCLabPaper@draft@show@images}{%
			\Debug@Out@Input[IncludeGraphics[#2]{#3}]{Invoking begin{overpic}[\XKV@rm]{\ig@file@path'}}%
			\expandafter\overpic\expandafter[\XKV@rm]{\ig@file@path}%
			%
			\IfValueT{#4}{%
				#4%
			}%
			\endoverpic%
		}{%
			\Draft@Image@Placeholder{#3}
		}%
	}{%
		\Input@Diag@Missing@File{\ig@file@path}%
	}
	\endgroup%
	\ifKV@IncludeGraphics@center%
		\end{center}%
	\fi%
}


\define@boolkey{InputPDF}{absolute}[false]{}
\ProvideDocumentCommand{\InputPDF}{O{} m}{%
	%#1: absolute + pdfpages options...
	%#2: local/path/to/image/file
	%
	% Process options [#1]
	\setkeys{InputPDF}{absolute}%
	\setkeys*{InputPDF}{pages=-, #1}% star: appends undefined keys to \XKV@rm (which can be sent to other commands)
	%
	\Debug@Out@Input[InputPDF[#1]{#2}]{Options to be sent to includepdf: '\XKV@rm'}%
	%
	\ifKV@InputPDF@absolute%
		\edef\current@directory{}%
	\else%
		\GetCurrentDir[\current@directory]%
		\edef\current@directory{\current@directory/}%
	\fi%
	\Debug@Out@Input[InputPDF[#1]{#2}]{Current directory = '\current@directory'}%
	%
	\begingroup%
	\catcode`\_=12%
	\edef\ig@file@path{\current@directory#2}
	\Debug@Out@Input[InputPDF[#1]{#2}]{Input filepath = '\ig@file@path'}%
	\IfFileExists{\ig@file@path}{%
		\Debug@Out@Input[InputPDF[#1]{#2}]{Input PDF file exists: '\ig@file@path'}%
		\expandafter\includepdf\expandafter[\XKV@rm]{\ig@file@path}%
	}{%
		\Input@Diag@Missing@File{\ig@file@path}%
	}%
	\endgroup%
}



\DeclareDocumentCommand{\IfFileExistsRelTF}{m +m +m}{%
	% #1: relative file path
	% #2: true branch
	% #3: else branch
	\GetCurrentDir[\current@directory]%
	\IfFileExists{\current@directory/#1}{#2}{#3}%
}

\newcounter{InputAllNumberedSubfoldersSubfolder}
\define@cmdkey{InputAllNumberedSubfolders}{padtodigits}[1]{}
\define@cmdkey{InputAllNumberedSubfolders}{file}[content.tex]{}
\define@cmdkey{InputAllNumberedSubfolders}{inbetween}[\cleardoublepage]{}
\DeclareDocumentCommand{\InputAllNumberedSubfolders}{O{} D<>{.}}{%
	% [#1]: options
	% <#2>: path prefix
	\setkeys{InputAllNumberedSubfolders}{padtodigits, file, inbetween}%
	\setkeys{InputAllNumberedSubfolders}{#1}%
	%	
	\setcounter{InputAllNumberedSubfoldersSubfolder}{1}
	\providetoggle{InputAllNumberedSubfoldersDone}
	\settoggle{InputAllNumberedSubfoldersDone}{false}%
	%
	\whileboolexpr{%
		not togl {InputAllNumberedSubfoldersDone}%
	}{%
		\Util@Pad@To@Digits%
		 	{\InputAllNumberedSubfolders@subfolder}%
		 	{\theInputAllNumberedSubfoldersSubfolder}%
		 	{\cmdKV@InputAllNumberedSubfolders@padtodigits}%
		%
		%
		% \InputAllNumberedSubfolders@subfolder now
		% contains subfolder expected name
		\Debug@Out@Input[InputAllNumberedSubfolders[#1]<#2>]{%
			Checking where file '#2/\InputAllNumberedSubfolders@subfolder/\cmdKV@InputAllNumberedSubfolders@file' exists%
		}%
		\IfFileExistsRelTF{#2/\InputAllNumberedSubfolders@subfolder/\cmdKV@InputAllNumberedSubfolders@file}{%
			\Debug@Out@Input[InputAllNumberedSubfolders[#1]<#2>]{%
					--> yes}%
			\ifequals{\theInputAllNumberedSubfoldersSubfolder}{1}{}{%
				\cmdKV@InputAllNumberedSubfolders@inbetween%
			}%
			%
			\Debug@Out@Input[InputAllNumberedSubfolders[#1]<#2>]{%
					--> input '#2/\InputAllNumberedSubfolders@subfolder/\cmdKV@InputAllNumberedSubfolders@file'}%
			\Input{#2/\InputAllNumberedSubfolders@subfolder/\cmdKV@InputAllNumberedSubfolders@file}%	
		}{%
			\Debug@Out@Input[InputAllNumberedSubfolders[#1]<#2>]{%
				--> no, stopping}%
			\settoggle{InputAllNumberedSubfoldersDone}{true}%
		}%
		\stepcounter{InputAllNumberedSubfoldersSubfolder}%
	}%
}


%  \newcommand{\InputAllNumberedSubfolders@Pad@To@Digits}[3]{%
%  	% #1: result
%  	% #2: integer
%  	% #3: final length of padded result
%  	%\edef@macro{#1}{#2}%
%  	\StrLen{#2}[\IANSPTD@len]%
%  	\MathEval[\IANSPTD@start]{trunc(\IANSPTD@len+1 :0)}%
%  	\edef\IANSPTD@prefix{}%
%  	\xintFor* ##1 in {\xintSeq[1]{\IANSPTD@start}{#3}} \do{
%  		\edef\IANSPTD@prefix{\IANSPTD@prefix 0}%
%  	}%
%  	\edef@macro{#1}{\IANSPTD@prefix #2}%
% }

\endinput


%%% WRAP commands for the 'import' package
%%% NOT NEEDED (????)
%\DeclareDocumentCommand{\InputAbsolutePath}{ s O{./} m}{
%	% #1: star (no draft note even if in Draft mode)
%	% #2: absolute file path extension with trailing '/'
%	% #3: file name
%	\IfBooleanTF{#1}{}{\@SystemNote{Start of file #2/#3}}
%	\import{#2/}{#3}
%	\IfBooleanTF{#1}{}{\@SystemNote{End of file #2/#3}}
%}	

%\DeclareDocumentCommand{\Input}{ s O{./} m}{
%	% #1: star (no draft note even if in Draft mode)
%	% #2: file path extension wrt. to caller file, default ./
%	% #3: file name
%	\IfBooleanTF{#1}{}{\@SystemNote{Start of file #2/#3}}
%	\subimport{#2/}{#3}
%	\IfBooleanTF{#1}{}{\@SystemNote{End of file #2/#3}}
%}
%New implementation

==> MCLabPaper_Label_2.tex <==

\MCLabPaper@Set@Tutorial@Section{Label}{sec:label}

\DeclareDocumentCommand{\Debug@Out@Label}{o m}{%
	\Debug@Out{Label}[#1]{#2}%
}


%%% IMPLEMENTATION USING CLEVEREF

\MCLabPaper@RequirePackage[italian, english, noabbrev, capitalize, nameinlink]{cleveref}
\crefname{equation}{}{}
\addto\captionsenglish{%
	\crefname{algocf}{\algorithmcfname}{\algorithmcfname s}	
	% \crefname{subsection}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	% \crefname{subsubsection}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	\crefname{paragraph}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	\crefname{subparagraph}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	\crefname{enumi}{item}{items}	
	\crefname{page}{page}{pages}% enforce lower case
	\Crefname{page}{Page}{Pages}
}	

\addto\captionsitalian{%
	\crefname{algocf}{\algorithmcfname}{Algoritmi}
	% \crefname{subsection}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	% \crefname{subsubsection}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	\crefname{paragraph}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	\crefname{subparagraph}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
	\crefname{enumi}{voce}{voci}
	\crefname{page}{pagina}{pagine}% enforce lower case
	\Crefname{page}{Pagina}{Pagine}
}

\let\namecref\lcnamecref


%%%%% DEPRECATED COMMANDS %%%%%%%%%%%%%%%

\preto\secref{%
	\DiagDeprecationSimple{Label}{secref}{cref}%
}

\preto\figref{%
	\DiagDeprecationSimple{Label}{figref}{cref}%
}
\preto\tabref{%
	\DiagDeprecationSimple{Label}{tabref}{cref}%
}

% To be done at begin document, as other packages may otherwise change them.
\AtBeginDocument{%
	\preto\ref{%
		\DiagDeprecationSimple{Label}{ref}{cref}%	
	}%
	\preto\bf{%
		\DiagDeprecationSimple{Label}{bf}{textbf}%
	}%
}


\endinput








%%%%%%%%%% MY OWN IMPLEMENTATION

\newcommand{\MCLabPaper@sectionname}{Section}
\addto\captionsenglish{%
  \def\MCLabPaper@sectionname{Section}%
  \def\MCLabPaper@sectionname@plural{\MCLabPaper@sectionname s}%  
  \def\MCLabPaper@partname@plural{\partname s}%    
  \def\MCLabPaper@chaptername@plural{\chaptername s}%      
  \def\MCLabPaper@figurename@plural{\figurename s}%
  \def\MCLabPaper@tablename@plural{\tablename s}%  
  \def\MCLabPaper@algoname@plural{\algorithmcfname s}%    
}
\addto\captionsitalian{%
  \def\MCLabPaper@sectionname{Sezione}%    
  \def\MCLabPaper@sectionname@plural{Sezioni}%    
  \def\MCLabPaper@partname@plural{Parti}%    
  \def\MCLabPaper@chaptername@plural{Capitoli}%  
  \def\MCLabPaper@figurename@plural{Figure}%
  \def\MCLabPaper@tablename@plural{Tabelle}%    
  \def\MCLabPaper@algoname@plural{Algoritmi}%
}


\def\@LabelType@Postfix{:LabelType}
\edef\Label@Current@Label@Type{}
\DeclareDocumentCommand{\Label}{o m}{%
	% #1: type
	% #2: label
	\IfValueTF{#1}{
		\edef\Label@Type{#1}%
	}{%
		\edef\Label@Type{\Label@Current@Label@Type}%
	}%
	\immediate\write\@mainaux{%
		\noexpand\csxdef{#2\@LabelType@Postfix}{\Label@Type}%
	}%
	\label{#2}%
}%

\DeclareDocumentCommand{\Ref}{m}{% #1: label
	\pgfkeys{% % reload at every call to \Ref (so use can change language within document)
		\pgfkeysPrefix/Smart Labels/types/.cd,
			part/singular/.initial = \partname,%
			part/plural/.initial = \MCLabPaper@partname@plural,%
			part/ref command/.initial = ref,
			chapter/singular/.initial = \chaptername,%			
			chapter/plural/.initial = \MCLabPaper@chaptername@plural,%
			chapter/ref command/.initial = ref,%
			section/singular/.initial = \MCLabPaper@sectionname,%
			section/plural/.initial = \MCLabPaper@sectionname@plural,%
			section/ref command/.initial = ref,%
			figure/singular/.initial = \figurename,%
			figure/plural/.initial = \MCLabPaper@figurename@plural,%
			figure/ref command/.initial = ref,
			table/singular/.initial = \tablename,%
			table/plural/.initial = \MCLabPaper@tablename@plural,%			
			table/ref command/.initial = ref,%
			algorithm/singular/.initial = \algorithmcfname,%
			algorithm/plural/.initial = \MCLabPaper@algoname@plural,%
			algorithm/ref command/.initial = ref,%
			equation/singular/.initial={},%
			equation/plural/.initial={},%
			equation/ref command/.initial=eqref,
	}%
	%
	%
	\pgfkeys{\pgfkeysPrefix/Smart Labels/this/out list/.initial={}}% the output list of "{XXX~\ref{...}, ... and \ref{...}}" elements
	\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.initial={}}% the current sublist of "\ref{...}" elements
	\edef\Ref@sublist@type{}% % the label-type of the current sublist
	%
	\Debug@Out@Label{Processing \show{\Ref{#1}}}%
	\provideboolean{reflast}\setboolean{reflast}{false}%
	\xintFor ##9 in {#1, {}} \do{% for each label... + {}
		%
		\edef\Ref@label@to@add{##9}%
		\xintifForLast{%
			\Debug@Out@Label{ - processing last sublist and terminating}%
			\setboolean{reflast}{true}%
		}{%
			\Debug@Out@Label{ - Processing label '##9'}%
		}%		
		% get label type into \Ref@this@label@type
		\ifcsdef{##9\@LabelType@Postfix}{%
			% This label type is known
			\edef\Ref@this@label@type{\csuse{##9\@LabelType@Postfix}}%
			% get ref command for type
			\pgfkeys{\pgfkeysPrefix/Smart Labels/types/\Ref@this@label@type/ref command/.get=
				\Ref@this@label@refcommand@string%
			}%				
			\Debug@Out@Label{               --> ref command name '\Ref@this@label@refcommand@string'}%			
		}{%
			% This label type is unknown
			\edef\Ref@this@label@type{}%
			\edef\Ref@this@label@refcommand@string{ref}%
		}%
		%
		\Debug@Out@Label{  - type: '\Ref@this@label@type'}%
		\ifthenelse{ \boolean{reflast}  \OR  \( \NOT \equal{\Ref@sublist@type}{\Ref@this@label@type} \)  }{%
			%
			% I'm done or label is of different type than previous ones: current sublist will be processed and a new sublist will start
			%
			\Debug@Out@Label{   --> different from previous label}%
			%
			% 1) get prev. sublist label type name (singular or plural)
			\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.get=\Ref@curr@sublist}%
			\Debug@Out@Label{          - retrieving text for label type of prev. ref sublist (sublist: \Ref@curr@sublist) (type: \Ref@sublist@type)}%
			\edef\Ref@sublist@type@string{}%
			\ifequals{\Ref@sublist@type}{}{%
				% type unknown --> do nothing
			}{%
				\CommaSepListSize[\Ref@curr@sublist@size]{\Ref@curr@sublist}%
				\ifthenelse{\Ref@curr@sublist@size = 1}{%
					\def\Ref@sublist@type@singular@plural{singular}%
				}{%
					\def\Ref@sublist@type@singular@plural{plural}%
				}%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/types/\Ref@sublist@type/\Ref@sublist@type@singular@plural/.get=
						\Ref@sublist@type@string%
				}%
				\ifequals{\Ref@sublist@type@string}{}{}{%
					\eappto{\Ref@sublist@type@string}{~}%
				}%
				%
			}%
			% \Ref@sublist@type@string contains full label type string (singular/plural + ~ or "")
			\Debug@Out@Label{               --> '\Ref@sublist@type@string'}%
			%
			% 2) ship-out labels in prev. sublist (if non-empty)
			\ifequals{\Ref@curr@sublist}{}{%
				\Debug@Out@Label{          - prev. sublist is empty: skipping}%
			}{%
				\Debug@Out@Label{          - computing prose from sublist}%
				\CommaSepListToProse[\Ref@curr@sublist@prose]{\Ref@curr@sublist}%
				\Debug@Out@Label{            --> '\Ref@curr@sublist@prose'}%
				\Debug@Out@Label{          - appending prose to out list}%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/out list/.get=\Ref@out@list}%
				\ifequals{\Ref@out@list}{}{%
					\Debug@Out@Label{             --> out list is empty}%
					\protected@edef\Ref@sublist@out{\Ref@sublist@type@string\Ref@curr@sublist@prose}%
				}{%
					\Debug@Out@Label{             --> out list is not empty}%
					\protected@edef\Ref@sublist@out{, {\Ref@sublist@type@string\Ref@curr@sublist@prose}}%
				}%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/out list/.append/.expand once=\Ref@sublist@out}%
				%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/out list/.get=\Ref@out@list}%
				\Debug@Out@Label{           --> now out list is '\Ref@out@list'}%
			}%
			%
			% 3) if not 'done', reset current sublist to \refcommand{##9}
			\ifthenelse{\boolean{reflast}}{}{%	
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.expanded=%
					{\noexpand\csname\Ref@this@label@refcommand@string\endcsname{\Ref@label@to@add}}}%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.get=\Ref@curr@sublist}%
				\Debug@Out@Label{          - current refs sublist reset. Now: '\Ref@curr@sublist'}%
				% 4) set type of current sublist to \Ref@this@label@type
				\edef\Ref@sublist@type{\Ref@this@label@type}%
				\Debug@Out@Label{          - current refs sublist type is now: '\Ref@sublist@type'}%
			}%
		}{%
			%
			%
			\Debug@Out@Label{   --> as previous label}%
			% another label of same type of previous one --> append \ref{##9} to current sublist
			\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.get=\Ref@curr@sublist}%
			\ifequals{\Ref@curr@sublist}{}{%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.append/.expanded=%
					{\noexpand\csname\Ref@this@label@refcommand@string\endcsname{\Ref@label@to@add}}}%
			}{%
				\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.append/.expanded=%
					{, {\noexpand\csname\Ref@this@label@refcommand@string\endcsname{\Ref@label@to@add}}}}%
			}%
			\pgfkeys{\pgfkeysPrefix/Smart Labels/this/current sublist/refs/.get=\Ref@curr@sublist}%
			\Debug@Out@Label{        --> now sublist of refs (type: '\Ref@sublist@type') is '\Ref@curr@sublist'}%
		}%
	}% for each label
	%
	%
	% Shipout out list	
	\pgfkeys{\pgfkeysPrefix/Smart Labels/this/out list/.get=\Ref@out@list}%
	\Debug@Out@Label{  - all done: shipping out list '\Ref@out@list'}%
	\CommaSepListToProse{\Ref@out@list}%
	%\Ref@out@list%
}


\AtBeginEnvironment{table}{\edef\Label@Current@Label@Type{table}}
\AtBeginEnvironment{figure}{\edef\Label@Current@Label@Type{figure}}
\AtBeginEnvironment{equation}{\edef\Label@Current@Label@Type{equation}}
\AtBeginEnvironment{align}{\edef\Label@Current@Label@Type{equation}}
\AtBeginEnvironment{algorithm}{\edef\Label@Current@Label@Type{algorithm}}



%%% MY IMPLEMENTATION OF DEPRECATED COMMENTS
\newcommand{\secref@section@type@name}[1]{%
	\edef\secref@cmd{\csname seccmd:#1\endcsname}%
	\ifthenelse{\equal{\secref@cmd}{part}}{%
		%Part%
		\partname%
	}{%
		\ifthenelse{\equal{\secref@cmd}{chapter}}{%
			%Chapter%
			\chaptername%
		}{%
			%Section%
			\MCLabPaper@sectionname%
		}%
	}%	
}

\DeclareDocumentCommand{\smart@refs}{o m}{%
	\Deprecated@Notice{Usage of \noexpand\secref, \noexpand\figref, \noexpand\tabref is deprecated. Use \noexpand \Ref}%
	\edef\smart@refs@list{#2}%
	\CommaSepListSize[\secref@size]{\smart@refs@list}%
	%[size=\secref@size]
	\ifnum\secref@size=1%
		\IfValueTF{#1}{%
			#1%
		}{%
			\secref@section@type@name{\smart@refs@list}%
		}~\ref{#2}%
	\else%
		\foreach \@label [count=\secref@cnt] in \smart@refs@list {%
			%[processing label '\@label'] 
			\ifnum\secref@cnt=1%
				\IfValueTF{#1}{%
					#1%
				}{%
					\secref@section@type@name{\@label}%
				}%
				s~%
			\else%
				\ifnum\secref@cnt=\secref@size%
					{} and~%
				\else%
					,~%
				\fi%
			\fi%
			%
			%\edef\@elabel{\@label}%
			\ref{\@label}%
			%\DraftNote*{[\@elabel]}%
		}%
	\fi%
	\xspace%
}%


\DeclareDocumentCommand{\secref}{m}{%
	\smart@refs{#1}%
}


\DeclareDocumentCommand{\figref}{m}{%
	\smart@refs[\figurename]{#1}%
}
\DeclareDocumentCommand{\tabref}{m}{%
	\smart@refs[\tablename]{#1}%
}



==> MCLabPaper_Language_2.tex <==
\PackageInfo{MCLabPaper}{Loading Language.tex}%

\let\BabelSelectLanguage\selectlanguage

\MCLabPaper@Set@Tutorial@Section{Lanbuage}{sec:language}

\renewcommand{\selectlanguage}[1]{%
	\iftoggle{InPreamble}{%
		\AtBeginDocument{\BabelSelectLanguage{#1}}%
	}{%
		\BabelSelectLanguage{#1}%
	}%
}

\selectlanguage{english}

\PackageInfo{MCLabPaper}{Loading Language.tex done}%

==> MCLabPaper_List_2.tex <==
\MCLabPaper@RequirePackage[inline, shortlabels]{enumitem}
\def\List@Max@Depth{50}
\setlistdepth{\List@Max@Depth}

\MCLabPaper@Set@Tutorial@Section{List}{sec:list}

%\newlist{nestedenum}{enumerate}{10}
%\setlist[nestedenum]{label*=\arabic*.}

\SetEnumitemKey{nested}{label*=\arabic*.}

\SetEnumitemKey{compact}{noitemsep}

\SetEnumitemKey{supercompact}{nosep}

\SetEnumitemKey{2columns}{
	%itemsep=1\itemsep,
	%parsep=1\parsep,
	before=\raggedcolumns\begin{multicols}{2},
	after=\end{multicols}
}
\SetEnumitemKey{3columns}{
	%itemsep=1\itemsep,
	%parsep=1\parsep,
	before=\raggedcolumns\begin{multicols}{3},
	after=\end{multicols}
}
\SetEnumitemKey{4columns}{
	%itemsep=1\itemsep,
	%parsep=1\parsep,
	before=\raggedcolumns\begin{multicols}{4},
	after=\end{multicols}
}



%\newlist{asparaenum}{enumerate}{1}
%\setlist[asparaenum]{label=\arabic*., wide}
%
%\newlist{asparaitem}{itemize}{1}
%\setlist[asparaitem]{label=\textbullet, wide}

==> MCLabPaper_Listing_2.tex <==
\MCLabPaper@RequirePackage{listingsutf8}

\MCLabPaper@Set@Tutorial@Section{Listing}{sec:listing}

\definecolor{MCLabPaper_KeywordColor}{rgb}{0.33, 0.41, 0.47}


\lstdefinelanguage{Murphi}[]{Pascal} { 
	morekeywords={ruleset, rule, invariant, startstate, return, endif, endfor, endswitch, forall, endforall, exists, endexists, finalstate}, 
	mathescape=true, 
	morestring=[b]",
	morestring=[b]', 
	morecomment=[s]{/*}{*/} ,
	morecomment=[l]{--}
}


\lstdefinestyle{Murphi}{
	language=Murphi,
	basicstyle=\normalsize,%\ttfamily,%\small, 
	tabsize=1,
	showlines=false,
	emptylines=*1,
	breaklines=true,
	breakindent=5pt,
	keywordstyle=\bfseries,%\ttfamily\bfseries,%\normalsize, 
	commentstyle=\color{MCLabPaper_CommentColor}\itshape, 
	columns=fullflexible,
	showspaces=false, 
	showstringspaces=false, 
	showtabs=false,
	escapechar=\%
}

%\definecolor{lightgrey}{rgb}{0.9,0.9,0.9}
%\definecolor{darkgreen}{rgb}{0,0.6,0}

\edef\LatexColor{Brown!80}
\lstdefinestyle{LaTeX}{
	language=[LaTeX]TeX,
	basicstyle={\color{\LatexColor}\normalfont},
	tabsize=1,
	showlines=false,
	emptylines=*1,
	breaklines=true,
	breakindent=5pt,
	keywordstyle=\bfseries,
	commentstyle=\color{MCLabPaper_CommentColor}\itshape, 
	columns=fullflexible,
	showspaces=false, 
	showstringspaces=false, 
	showtabs=false,
	escapechar=!
	%otherkeywords={Comment, Input, InputSection, IncludeGraphics, GetCurrentDir}, 
}


\lstdefinestyle{C}{
	language=[ANSI]C,
	basicstyle=\normalsize,%\small, 
	tabsize=3,
	showlines=false,
	emptylines=*1,
	breaklines=true,
	breakindent=5pt,
	keywordstyle=\color{MCLabPaper_KeywordColor}\normalfont\bfseries,%\normalsize, 
	commentstyle=\color{MCLabPaper_CommentColor}\itshape, 
	columns=fullflexible,
	showspaces=false, 
	showstringspaces=false, 
	showtabs=false,
	escapechar=%
}

\lstdefinelanguage{Text}[]{}{
	extendedchars=true,
	inputencoding=utf8/latin1
}


\lstdefinestyle{Text}{
	language=Text,
	basicstyle=\normalsize\normalfont,%\ttfamily,%\small, 
	tabsize=4,
	showlines=false,
	emptylines=*1,
	breaklines=true,
	breakindent=5pt,
	columns=fixed, %fullflexible,
	showspaces=false, 
	showstringspaces=false, 
	showtabs=false,
}

\colorlet{JSONpunct}{red!60!black}
\definecolor{JSONbackground}{HTML}{EEEEEE}
\definecolor{JSONdelim}{RGB}{20,105,176}
\colorlet{JSONnumb}{magenta!60!black}

\lstdefinelanguage{Json}{
    basicstyle=\normalfont\ttfamily,
    numbers=left,
    numberstyle=\scriptsize,
    escapeinside={!*}{*!},
    stepnumber=1,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    %frame=lines,
    %backgroundcolor=\color{background},
    literate=
     *{0}{{{\color{JSONnumb}0}}}{1}
      {1}{{{\color{JSONnumb}1}}}{1}
      {2}{{{\color{JSONnumb}2}}}{1}
      {3}{{{\color{JSONnumb}3}}}{1}
      {4}{{{\color{JSONnumb}4}}}{1}
      {5}{{{\color{JSONnumb}5}}}{1}
      {6}{{{\color{JSONnumb}6}}}{1}
      {7}{{{\color{JSONnumb}7}}}{1}
      {8}{{{\color{JSONnumb}8}}}{1}
      {9}{{{\color{JSONnumb}9}}}{1}
      {:}{{{\color{JSONpunct}{:}}}}{1}
      {,}{{{\color{JSONpunct}{,}}}}{1}
      {\{}{{{\color{JSONdelim}{\{}}}}{1}
      {\}}{{{\color{JSONdelim}{\}}}}}{1}
      {[}{{{\color{JSONdelim}{[}}}}{1}
      {]}{{{\color{JSONdelim}{]}}}}{1},
}
\lstnewenvironment{json}
	{\lstset{language=Json}}
	{}
\newcommand{\jsoninline}[1]{\lstinline[language=Json]{#1}}


\lstset{language=SQL,
	basicstyle=\small,
	keywordstyle=\color{BlueViolet}\bfseries,
	stringstyle=\color{Brown},
	commentstyle=\color{javagreen},
	morecomment=[s][\color{javadocblue}]{/**}{*/},
	%numbers=left,
	numberstyle=\tiny\color{black},
	stepnumber=2,
	numbersep=10pt,
	tabsize=4,
	escapeinside=``,
	%showspaces=true,
	%showtabs=true,
	showstringspaces=false,
	breaklines=true
}

\lstnewenvironment{sql}
	{\lstset{language=SQL}}
	{}
\newcommand{\sqlinline}[1]{\lstinline[language=SQL]{#1}}




\newcommand{\DataListings@encoding@text}{\catcode`_=12\catcode`\\=12\catcode`\{=12\catcode`\}=12}
\newcommand{\LatexInline}{\lstinline[style=LaTeX]}%



==> MCLabPaper_Math_2.tex <==
% Math-related packages
\MCLabPaper@RequirePackage{amsmath}
\MCLabPaper@RequirePackage{amssymb} % amssymb loads amsfonts
\MCLabPaper@RequirePackage{mathtools}

\MCLabPaper@Set@Tutorial@Section{Math}{sec:math}


\DeclareDocumentCommand{\Debug@Out@Math}{o m}{%
	\Debug@Out{Math}[#1]{#2}%
}




\newcommand{\mathup}[1]{\text{\textup{#1}}}

\newcommand{\Reals}{\ensuremath{\mathbb{R}}\xspace} % Reals
\newcommand{\RealsGEZ}{\ensuremath{{\Reals^{\geq 0}}}\xspace} % Reals >= 0
\newcommand{\RealsGZ}{\ensuremath{\Reals^{+}}\xspace} % Reals > 0

\newcommand{\IntegersGZ}{\ensuremath{{\mathbb{N}^+}}\xspace} % Naturals
\newcommand{\IntegersGEZ}{\ensuremath{\mathbb{N}}\xspace} % Naturals union {0}
\let\Naturals\IntegersGEZ%

\newcommand{\Integers}{\ensuremath{\mathbb{Z}}\xspace} % Integers

\newcommand{\Rationals}{\ensuremath{\mathbb{Q}}\xspace} % Rationals
\newcommand{\Bool}{\ensuremath{\textrm{Bool}}\xspace} % Booleans

\newcommand{\Fail}{\textsl{FAIL}\xspace} % FAIL
\newcommand{\Pass}{\textsl{PASS}\xspace} % PASS

\newcommand{\Fun}[1]{{\textup{#1}}} %% functions
\newcommand{\fun}[1]{%
	\Deprecated@Notice{Use of \noexpand\fun is deprecated. Use \noexpand\Fun.}%
	\Fun{#1}%
}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\Abs}[1]{\left|#1\right|}%


%% Sets
\newcommand{\Set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\SetCardinality}[1]{\ensuremath{\left|#1\right|}}%


\xdef\MathStructPrefix{Math/Structs}

\DeclareDocumentCommand{\MathDefineStruct}{m m D(){=} o}{%
	% #1: struct id
	% #2: struct name
	% (#3): =, :, etc.
	% [#4]: struct definitiion
%	\pgfglobalkeys{\MathStructPrefix/#1/.cd,
%		id/.initial = {#1},
%		name/.initial = {#2},
%		def sign/.initial = {#3}
%	}%
	\DataPut{\MathStructPrefix/#1/id = #1}%
	\DataPut{\MathStructPrefix/#1/name = #2}%
	\DataPut{\MathStructPrefix/#1/def sign = #3}%	
	%
	\IfValueT{#4}{%
%		\pgfglobalkeys{\MathStructPrefix/#1/def/.initial = {#4}}%
		\DataPut{\MathStructPrefix/#1/def = #4}%
		\typeout{[MathDefineStruct] Struct [#1]: def --> [#4]}%
	}%
}
\DeclareDocumentCommand{\Math@StructField}{O{} m m}{% [#1]: output macro, #2: struct id, #3: field name	
	\typeout{[Math@StructField] Checking whether struct '#2' is defined...}%
	%\pgfglobalkeysifdefined{\MathStructPrefix/#2/id}{%
	\DataIfKeyDefinedTF{\MathStructPrefix/#2/id}{%
		\typeout{[Math@StructField] Struct '#2' defined}%
		%	
		%\pgfglobalkeysifdefined{\MathStructPrefix/#2/#3}{%
		\DataIfKeyDefinedTF{\MathStructPrefix/#2/#3}{%
			%\pgfglobalkeys{\MathStructPrefix/#2/#3/.get=\@MathStructDef@result}%
			%\typeout{[Math@StructField] getting value of field '#3'}%
			%
			\DataGet[\@MathStructDef@result]{\MathStructPrefix/#2/#3}%
			%\typeout{done}%
			\typeout{[Math@StructField] value of field '#3': '\@MathStructDef@result'}%
			\IfStringEmptyTF{#1}{%
				\ensuremath{\@MathStructDef@result}\xspace%
			}{%
				\edef@macro{#1}{\expandonce{\@MathStructDef@result}}%
			}%
		}{}%
	}{%
		\PackageError{MCLabPaper_Math}{MathStruct having id '#2' is NOT defined}%		
	}%
	%
}

\DeclareDocumentCommand{\MathStructName}{O{} m}{% [#1]: output macro, #2: struct id
	\Math@StructField[#1]{#2}{name}%
}	
\DeclareDocumentCommand{\MathStructDef}{O{} m}{% [#1]: output macro, #2: struct id
	\Math@StructField[#1]{#2}{def}%
}	

\DeclareDocumentCommand{\MathStructFull}{m}{% #1: struct id
	\bgroup%
	\ensuremath{%
		\MathStructName{#1}%
		\def\@MathStructDef@result@def{}%
		\MathStructDef[\@MathStructDef@result@def]{#1}%
		\typeout{[MathStructFull] struct id: [#1] --> def: [\@MathStructDef@result@def]}%
		\ifequals{\@MathStructDef@result@def}{}{}{%
			%\pgfglobalkeys{\MathStructPrefix/#1/def sign/.get=\@MathStructDef@def@sign}%
			\DataGet[\@MathStructDef@def@sign]{\MathStructPrefix/#1/def sign}%
			\@MathStructDef@def@sign \@MathStructDef@result@def%
		}%
	}%
	\egroup%
}



% MATH COMPUTATIONS, wrapping the 'fp' package (pgfmath seems not to not handle large numbers)
\MCLabPaper@RequirePackage{fp}
\MCLabPaper@RequirePackage{fp-eval}



% \edef\Math@Frozen@FileName{\jobname.math}
% \newif\if@Math@Frozen
% \@Math@Frozenfalse
% \newcommand{\MathFrozen}{%
% 	\@Math@Frozentrue%
% 	\IfFileExists{\Math@Frozen@FileName}{%
% 		\input{\Math@Frozen@FileName}%
% 	}{}%
% }

% \newwrite\@Math@Frozen@File@Handler
% \newtoggle{MathFrozen File Open}
% \settoggle{MathFrozen File Open}{false}
% \newcommand{\Add@To@Math@Frozen@File}[1]{%
% 	\iftoggle{MathFrozen File Open}{}{%
% 		\immediate\openout\@Math@Frozen@File@Handler=\Math@Frozen@FileName%
% 		\settoggle{MathFrozen File Open}{true}%
% 	}%
% 	\write\@Math@Frozen@File@Handler{#1}%
% }

% \DeclareDocumentCommand{\Math@Next@csname}{o m}{%
% 	% [#1]: \result
% 	% #2: prefix, e.g., command name, as MathEval
% 	\InputCurrentFilePath[\Math@infile]%
% 	\FileModTimeStamp[\Math@timestamp]{\Math@infile}%
% 	\xdef\Math@Next@csname@result{#2:\Math@infile:\csuse{the#2Cnt}:\Math@timestamp}%
% 	\stepcounter{#2Cnt}%
% 	\IfValueTF{#1}{%
% 		\xdef@macro{#1}{\Math@Next@csname@result}%
% 	}{\Math@Next@csname@result}%
% }



%\RequirePackage{pgfmath}\usepgflibrary{fpu}
\DeclareDocumentCommand{\MathEval}{o m O{}}{%
%	#1: output macro
%	#2: math expression
%	#3: \Pretty options
	\FPeval{\MathEval@result}{#2}%
	%\pgfkeys{/pgf/fpu=true}%
	%\pgfmathparse{#2}%
	\ifMathEval@Show@Computations%
		\IfPreambleTF{}{%
			\Draft@Math{$#2 = \MathEval@result$; }%
		}%
	\fi%
	%
	\IfValueTF{#1}{%
		% Store to output macro
		\xdef@macro{#1}{\MathEval@result}%
		%\pgfmathresult		
	}{%
		\Draft@Math{\Pretty[#3]{\MathEval@result}}%\pgfmathresult%
	}%
	%
	%
}
	

%\newcommand{\MathSavingPercentage}[2]{%	RETURNS ((#1-#2)/#1)*100 \%
%	\FPeval{@perc}{(#1 - #2)*100/#1}%	
%	\FPround{\@perc}{\@perc}{2}%
%	\@perc\%%
%}
\DeclareDocumentCommand{\MathAddSign}{o m}{%
	\edef\@x{#1}%
	\FPifpos{\@x}{+\@x}\else{\@x}\fi%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\@x}%
	}{%
		\Draft@Math{\@x}%
	}%	
}

%\newcommand{\MathOverheadPercentage}[2]{%	RETURNS +/- ((#2-#1)/#1)*100 \%
%	\FPeval{@result}{(#2 - #1)*100/#1}%	
%	\FPround{\@result}{\@result}{2}%	
%	\ensuremath{\MathAddSign{\@result}}%
%	%\FPifpos{\@result}{+\@result}\else{\@result}\fi\%}%
%}


\DeclareDocumentCommand{\MathMin}{o m O{}}{% #1: out macro, #2: comma sep. list of values	, #3: pretty-options
	\edef\Math@min@list{#2}%
	\Debug@Out@Math[MathMin(#2)]{Start}%
	\foreach \@v [count=\@idx] in \Math@min@list {%
		\Debug@Out@Math[MathMin(#2)]{ - read \@idx-th value '\@v' from list}%
		\ifnum\@idx=1%
			\xdef\Math@Min@result{\@v}%
			\Debug@Out@Math[MathMin(#2)]{       --> It is first element. Min is now \Math@Min@result}%
		\else%
			\FPmin{\@m}{\@v}{\Math@Min@result}%
			\xdef\Math@Min@result{\@m}%		
			\Debug@Out@Math[MathMin(#2)]{       --> Min is now \Math@Min@result}%
		\fi%
	}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\Math@Min@result}%
	}{%
		\Draft@Math{\Pretty[#3]{\Math@Min@result}}%
	}%
	\Debug@Out@Math[MathMin(#2)]{End}%
}


\DeclareDocumentCommand{\MathMax}{o m O{}}{% #1: out macro, #2: comma sep. list of values	, #3: pretty-options
	\edef\Math@max@list{#2}%
	\Debug@Out@Math[MathMax(#2)]{Start}%
	\foreach \@v [count=\@idx] in \Math@max@list {%
		\Debug@Out@Math{ - read \@idx-th value '\@v' from list}%
		\ifnum\@idx=1%
			\xdef\Math@Max@result{\@v}%
			\Debug@Out@Math[MathMax(#2)]{       --> It is first element. Max is now \Math@Max@result}%
		\else%
			\FPmax{\@m}{\@v}{\Math@Max@result}%
			\xdef\Math@Max@result{\@m}%		
			\Debug@Out@Math[MathMax(#2)]{       --> Max is now \Math@Max@result}%
		\fi%
	}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\Math@Max@result}%
	}{%
		\Draft@Math{\Pretty[#3]{\Math@Max@result}}%
	}%
	\Debug@Out@Math[MathMax(#2)]{End}%
}

\DeclareDocumentCommand{\MathSum}{o D<>{6} m O{}}{% #1: out macro, #2: comma sep. list of values	, #3: pretty-options
	\edef\Math@Sum@list{#3}%
	\Debug@Out@Math[MathSum(#3)]{Start}%
	\edef\Math@Sum@result{0}%
	\xintFor ##1 in {\Math@Sum@list} \do{%
		\Debug@Out@Math[MathSum(#3)]{ - Adding '##1': '\Math@Sum@result' + '##1' = }%
		\MathEval[\Math@Sum@result]{round(\Math@Sum@result + (##1) : #2)}%
		\Debug@Out@Math[MathSum(#3)]{   --> '\Math@Sum@result'}%
	}%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\Math@Sum@result}%
	}{%
		\Draft@Math{\Pretty[#4]{\Math@Sum@result}}%
	}%
	\Debug@Out@Math[MathSum(#3)]{End}%
}

\DeclareDocumentCommand{\MathAvg}{o D<>{6} m O{}}{% #1: out macro, #2: comma sep. list of values	, #3: pretty-options
	\Debug@Out@Math[MathAvg(#3)]{Start}%
	\MathSum[\Math@Avg@result]<#2>{#3}%
	\Debug@Out@Math[MathAvg(#3)]{Sum = `\Math@Avg@result'}%
	\Comma@Sep@List@Size@raw[\Math@Avg@len]{#3}%
	\Debug@Out@Math[MathAvg(#3)]{Len = `\Math@Avg@len'}%
	\MathEval[\Math@Avg@result]{round(\Math@Avg@result / \Math@Avg@len : #2)}%
	\Debug@Out@Math[MathAvg(#3)]{Result = `\Math@Avg@result'}%
	\IfValueTF{#1}{%
	 	\edef@macro{#1}{\Math@Avg@result}%
	}{%
	 	\Draft@Math{\Pretty[#4]{\Math@Avg@result}}%
	}%
	\Debug@Out@Math[MathAvg(#3)]{End}%
}


\DeclareDocumentCommand{\MathCeil}{o m O{}}{% #1: out macro, #2: value, #3: pretty
	\Debug@Out@Math[MathCeil{#2}]{Start}%
	\MathEval[\Math@Ceil@value]{#2}%
	\Debug@Out@Math[MathCeil{#2}]{ - arg evaluates to '\Math@Ceil@value'}%
	\IfInteger{\Math@Ceil@value}{%
		% integer number --> ceiling is the number itself === trunc(arg)	
		\MathEval[\Math@Ceil@result]{trunc(\Math@Ceil@value:0)}%
		\Debug@Out@Math[MathCeil{#2}]{ - arg is integer -> ceil(arg) = arg = '\Math@Ceil@result'}%		
	}{%
		\FPifneg{\Math@Ceil@value}%
			% negative (non-integer) number --> ceiling = truncation
			\MathEval[\Math@Ceil@result]{trunc(\Math@Ceil@value:0)}%
			\Debug@Out@Math[MathCeil{#2}]{ - arg < 0 and non-integer -> ceil(arg) = trunc(arg) = '\Math@Ceil@result'}%
		\else%
			% non-negative (non-integer) number --> ceiling = trunc + 1
			\MathEval[\Math@Ceil@result]{trunc(\Math@Ceil@value + 1:0)}%
			\Debug@Out@Math[MathCeil{#2}]{ - arg >= 0 and non-integer -> ceil(arg) = trunc(arg) + 1 = '\Math@Ceil@result'}%
		\fi%
	}%
	%
	%
	% \MathEval[\Ceil@trunc]{trunc((\Math@Ceil@value) : 0)}%
	% \Debug@Out@Math{MathCeil{#2}: - trunc(arg) = '\Ceil@trunc'}%
	% \MathEval[\Ceil@diff]{(\Math@Ceil@value) - \Ceil@trunc}%
	% \Debug@Out@Math{MathCeil{#2}: - decimal part of arg (=arg - trunc(arg)) is '\Ceil@diff'}%
	% %
	% \FPifgt{\Ceil@diff}{0}%	
	% 	\MathEval[\Math@Ceil@result]{round( \Ceil@trunc + 1 : 0)}%		
	% 	\Debug@Out@Math{MathCeil{#2}: - decimal part of arg > 0}%
	% \else%
	% 	\MathEval[\Math@Ceil@result]{\Ceil@trunc}%		
	% 	\Debug@Out@Math{MathCeil{#2}: - decimal part of arg = 0}%
	% \fi%
	%
	\Debug@Out@Math[MathCeil{#2}]{Result = ceil(arg) = '\Math@Ceil@result'}%
	%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\Math@Ceil@result}%
	}{%
		\Draft@Math{\Pretty[#3]{\Math@Ceil@result}}%
	}%
	\Debug@Out@Math[MathCeil{#2}]{End}%
}





\DeclareDocumentCommand{\MathMod}{o m m O{}}{% 
	%#1: out macro, 
	% #2: dividend, 
	% #3: divisor
	% [#4]: pretty
	\Debug@Out@Math[MathMod(#2)(#3)]{Start}%
	\MathEval[\Math@Mod@dividend]{#2}%
	\MathEval[\Math@Mod@divisor]{#3}%
	\Debug@Out@Math[MathMod{#2}]{ - dividend evaluates to '\Math@Mod@dividend'}%
	\Debug@Out@Math[MathMod{#2}]{ - divisor evaluates to '\Math@Mod@divisor'}%
	%
	\FPeval{\Math@Mod@result}{%
		trunc(\Math@Mod@dividend-(\Math@Mod@divisor*trunc(\Math@Mod@dividend/\Math@Mod@divisor,0)),0)}%
	%
	\Debug@Out@Math[MathMod(#2)(#3)]{Result = \Math@Mod@dividend\space mod \Math@Mod@divisor\space = '\Math@Mod@result'}%
	%
	\IfValueTF{#1}{%
		\edef@macro{#1}{\Math@Mod@result}%
	}{%
		\Draft@Math{\Pretty[#4]{\Math@Mod@result}}%
	}%
	\Debug@Out@Math[MathMod(#2)(#3)]{End}%
}


\DeclareDocumentCommand{\MathStripLeadingZeroes}{m m}{%
	% #1: \result
	% #2: value
	\edef@macro{#1}{%
		\number#2%
	}%
}%


==> MCLabPaper_Modules_2.tex <==
\PackageInfo{MCLabPaper}{Loading Modules.tex}%

\def\MCLabPaper@Modules@Prefix{MCLabPaper/modules}
\pgfglobalkeys{%
	\MCLabPaper@Modules@Prefix/.list/.initial=%
}


\DeclareDocumentCommand{\Debug@Out@Modules}{o m}{%
	\PackageInfo{MCLabPaper.Modules}{#1: #2}%
}


\DeclareDocumentCommand{\MCLabPaper@Define@Module}{m O{}}{%
	% #1: module name
	% #2: needs modules
	%\input{MCLabPaper_#1.tex}
	%
	\pgfglobalkeys{%
		\MCLabPaper@Modules@Prefix/#1/name/.initial = #1,
		\MCLabPaper@Modules@Prefix/#1/depends on/.initial = {#2},
		\MCLabPaper@Modules@Prefix/.list/.get = \MCLabPaper@Define@Module@list
	}%
	\ifequals{\MCLabPaper@Define@Module@list}{}{%
		\edef\MCLabPaper@Define@Module@list{#1}%
	}{%
		\edef\MCLabPaper@Define@Module@list{%
			\MCLabPaper@Define@Module@list, #1}%
	}%
	\pgfglobalkeys{%
		\MCLabPaper@Modules@Prefix/.list/.expanded = \MCLabPaper@Define@Module@list
	}%
	\pgfglobalkeys{%
		\MCLabPaper@Modules@Prefix/.list/.get = \MCLabPaper@Define@Module@list@again
	}%
	\providebool{Debug@State@#1}%	
	%
	%\PackageWarning{MCLabPaper}{Now list of modules is [\MCLabPaper@Define@Module@list@again]}%
}

\newtoggle{MCLabPaper@load@module}
\newcommand{\MCLabPaper@Load@All@Modules}{%
	\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{Start}%
	\pgfglobalkeys{%
		\MCLabPaper@Modules@Prefix/.list/.get = \MCLabPaper@Define@Module@list
	}%
	\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{Modules defined are: [\MCLabPaper@Define@Module@list]}%
	%
	\ifequals{\MCLabPaper@Define@Module@list}{}{}{%
		\xintFor ##1 in \MCLabPaper@Define@Module@list \do{%
			\toggletrue{MCLabPaper@load@module}%
			\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{Checking whether module ##1 must be loaded}%
			\pgfglobalkeys{%
				\MCLabPaper@Modules@Prefix/##1/depends on/.get=\MCLabPaper@module@depends
			}%
			%
			\IfPackageOrModuleSkippedTF{##1}{%
				\togglefalse{MCLabPaper@load@module}%
				\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{--> skipping ##1 as explicitly required by user}%
			}{%
				\ifequals{\MCLabPaper@module@depends}{}{}{%
					\xintFor ##2 in \MCLabPaper@module@depends \do{%
						%\typeout{\iftoggle{MCLabPaper@load@module}{now toggle is TRUE}{now toggle is FALSE}}
						\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{Module ##1 depends on '##2'...}%
						\IfPackageOrModuleSkippedTF{##2}{%
							\togglefalse{MCLabPaper@load@module}%
							\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{--> skipping ##1, because ##2 has been skipped}%
						}{%
							\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{--> ##2 is/will be loaded... OK.}%
						}%
						%\typeout{\iftoggle{MCLabPaper@load@module}{now toggle is TRUE}{now toggle is FALSE}}
					}%
				}%	
			}%
			\iftoggle{MCLabPaper@load@module}{%
				\Debug@Out@Modules[MCLabPaper@Load@All@Modules]{Loading module ##1}%
				\input{MCLabPaper_##1_\MCLabPaper@file@suffix.tex}%
				\csletcs{Debug@Out@##1@On}{Debug@Out@##1}%
			}{%
				\PackageWarning{MCLabPaper}{Module ##1 skipped, as it depends on a skipped package/module}%
			}%
		}%
	}%
}

\PackageInfo{MCLabPaper}{Loading Modules.tex done}%

==> MCLabPaper_Options_2.tex <==
\PackageInfo{MCLabPaper}{Loading Options.tex}%

\RequirePackage{xkeyval}

\def\MCLabPaper@skipped{} % packages or Modules that user wants to skip
\DeclareOptionX{skip}{
	\def\MCLabPaper@skipped{#1}
}

\newbool{MCLabPaper@Debug}\boolfalse{MCLabPaper@Debug}
\edef\MCLabPaper@debug@modules{}%
\DeclareOptionX{debug}{%
	\booltrue{MCLabPaper@Debug}%
	\edef\MCLabPaper@debug@modules{#1}%
}


\ExecuteOptionsX{}
%NoListOfAcronyms, ResetAcronymsAtEachSection, NoDraft, NoCompact, StartWithSection

\ProcessOptionsX\relax

%\PackageWarning{MCLabPaper}{Skipped modules: \MCLabPaper@modules@skipped}

\def\MCLabPaper@Skipped@Prefix{MCLabPaper/Skipped}%
\foreach \@skipped in \MCLabPaper@skipped {%
	\PackageInfo{MCLabPaper}{User wants to skip package or MCLabPaper module: \@skipped}%
	\pgfglobalkeys{\MCLabPaper@Skipped@Prefix/\@skipped/.initial=skipped}%
}

\DeclareDocumentCommand{\IfPackageOrModuleSkippedTF}{m +m +m}{%
	\pgfglobalkeysifdefined{\MCLabPaper@Skipped@Prefix/#1}{#2}{#3}%
}

\PackageInfo{MCLabPaper}{Loading Options.tex done}%

==> MCLabPaper_Packages_2.tex <==
\PackageInfo{MCLabPaper}{Loading Packages.tex}%

\MCLabPaper@RequirePackage[utf8]{inputenc} %latin1
\MCLabPaper@RequirePackage[T1]{fontenc}

\MCLabPaper@RequirePackage{expl3}
\MCLabPaper@RequirePackage{xspace}

\MCLabPaper@RequirePackage[table,usenames,dvipsnames]{xcolor}

\MCLabPaper@RequirePackage{ifthen}	
\MCLabPaper@RequirePackage{graphicx}
\MCLabPaper@RequirePackage{booktabs}

\MCLabPaper@RequirePackage{etoolbox}
\MCLabPaper@RequirePackage{tikz}
\MCLabPaper@RequirePackage{pgffor}
\MCLabPaper@RequirePackage{xinttools}

\MCLabPaper@RequirePackage{calc}
\MCLabPaper@RequirePackage{float}
% Subfigures
\MCLabPaper@RequirePackage{caption}
\MCLabPaper@RequirePackage{subcaption}

% Number formatting: use \num{...} to format a number with separators
\MCLabPaper@RequirePackage{siunitx} 
\@ifpackageloaded{siunitx}{%
	\sisetup{detect-all}%
}{}

\MCLabPaper@RequirePackage{lipsum}

\MCLabPaper@RequirePackage[percent]{overpic} % put latex text over pictures


\MCLabPaper@RequirePackage{iflang} % offers: \IfLanguageName{lang_name}{true}{false}

\MCLabPaper@RequirePackage[english,italian]{babel} % Quotes won't work without babel

\MCLabPaper@RequirePackage{etex} % to enable pdflatex

\MCLabPaper@RequirePackage{textcomp} % lots of symbols

\MCLabPaper@RequirePackage{xr} % eXternal References (cross-references to external documents}

\MCLabPaper@RequirePackage{multicol}

\MCLabPaper@RequirePackage{rotating}

\DeclareDocumentCommand{\ListMCLabPaperLoadedPackages}{O{supercompact, 2columns}}{%
%
	\dtlsortlist{\MCLabPaper@LoadedPackages}{\dtlcompare}%
	\PackageInfo{MCLabPaper}{List of loaded packages: [\MCLabPaper@LoadedPackages]}%
	\begin{itemize}[#1]
	\xintFor ##1 in \MCLabPaper@LoadedPackages \do{
		\item \RenderFileName{##1}
	}
	\end{itemize}
}

\PackageInfo{MCLabPaper}{Loading Packages.tex done}%

==> MCLabPaper_Partial_2.tex <==
\MCLabPaper@Set@Tutorial@Section{Partial}{sec:partial}

\DeclareDocumentCommand{\Debug@Out@Partial}{o m}{%
	\Debug@Out{Partial}[#1]{#2}%
}


\def\Partial@maxdepth{50}%
\def\Partial@preamble{preamble.tex}

\newcounter{Partial@cnt}
\DeclareDocumentCommand{\PartialDoc}{+O{\Input{content.tex}}}{%
	% [#1] code within \begin{document} and \end{document}
	\Debug@Out@Partial[PartialDoc]{Start}%
	\edef\Partial@root@dir{.}%	
	\setcounter{Partial@cnt}{0}%
	\xintloop%
		\Debug@Out@Partial[PartialDoc]{Does \Partial@root@dir/\Partial@preamble\space exist?}%
		\IfFileExists{\Partial@root@dir/\Partial@preamble}{%
			% 
			\Debug@Out@Partial[PartialDoc]{yes!}%
			% \Partial@root@dir is root dir
			\xintbreakloop%
		}{%
			\Debug@Out@Partial[PartialDoc]{no}%
			\ifnumcomp{\Partial@maxdepth}{<}{\value{Partial@cnt}}{%
				%
				% Too deep! Exit				
				\DiagError{Partial}
					{Cannot find \RenderFileName{\Partial@preamble} in the previous \Partial@maxdepth\space levels of the file system}
					[Cannot find \Partial@preamble\space in the previous \Partial@maxdepth\space levels of the file system]%
				\xintbreakloop% % useless...
			}{%
				% go up one level
				\edef\Partial@root@dir{\Partial@root@dir/..}%
				\stepcounter{Partial@cnt}%
				\Debug@Out@Partial[PartialDoc]{going up one level}%
			}%
		}%
	\iftrue\repeat%		
	%
	% \Partial@root@dir is root dir and contains \Partial@preamble
	\Debug@Out@Partial[PartialDoc]{Input preamble from '\Partial@root@dir/\Partial@preamble'}%
	\Input[\Partial@root@dir]{\Partial@preamble}%
	%
	% Fix Section start level if this is really a partial doc
	\Debug@Out@Partial[PartialDoc]{fixing section level}%
	\ifnumcomp{\value{Partial@cnt}}{>}{0}{%
		\xintFor* ##1 in {\xintSeq[1]{1}{\value{Partial@cnt}}} \do{%
			\SectionSetStart@Incr
			\Debug@Out@Partial[PartialDoc]{- incrementing section level}%
		}%
	}{}%
	%
	\Debug@Out@Partial[PartialDoc]{Outputting begin document}%
	\begin{document}%
	 	#1%
	 	\Debug@Out@Partial[PartialDoc]{Outputting end document}%
	\end{document}%
	%\Debug@Out@Partial[PartialDoc]{Done}%
}

==> MCLabPaper_PgfGlobalKeys_2.tex <==
\PackageInfo{MCLabPaper}{Loading PgfGlobalKeys.tex}%
% enables level-0 pgfkeys
\def\pgfglobalkeys#1{\begingroup \ifnum\the\globaldefs>0\relax \else \globaldefs=1\fi \pgfkeys{#1}\endgroup}




%\def\pgfglobalkeysifdefined#1#2#3{\begingroup \ifnum\the\globaldefs>0\relax \else \globaldefs=1\fi \pgfkeysifdefined{#1}{#2}{#3}\endgroup}

\newcommand{\pgfglobalkeysifdefined}[3]{%
	\pgfglobalkeys{#1/.get=\pgfglobalkeysifdefined@value}%
	\ifx\pgfglobalkeysifdefined@value\relax%
		#3%
	\else%
		#2%
	\fi%
}


\xdef\pgfkeysPrefix{MCLabPaper}

\PackageInfo{MCLabPaper}{Loading PgfGlobalKeys.tex done}%

==> MCLabPaper_PgfGlobalKeys_Handlers_2.tex <==
\DeclareDocumentCommand{\Debug@Out@PgfHandlers}{o m}{%
	\Debug@Out{PgfHandlers}[#1]{#2}%
}


\pgfkeysdef{/handlers/.append to list}{%
	\pgfkeysifdefined{\pgfkeyscurrentpath}{%
		\pgfkeys{\pgfkeyscurrentpath/.get=\tmp}%
		\IfStrEq{\tmp}{}{%
			\pgfkeys{\pgfkeyscurrentpath/.append={#1}}%
		}{%
			\pgfkeys{\pgfkeyscurrentpath/.append={, #1}}%
		}%
	}{%
		\pgfkeys{\pgfkeyscurrentpath/.append={#1}}%
	}%
}

\newcounter{PgfAddToIntCnt}
\pgfkeysdef{/handlers/.add to int}{%
	\pgfkeysifdefined{\pgfkeyscurrentpath}{%
		% if key is defined
		%\Debug@Out@PgfHandlers{.add to int: key '\pgfkeyscurrentpath' is defined}%
		\pgfkeys{\pgfkeyscurrentpath/.get=\add@to@int@tmp}%
		%\Debug@Out@PgfHandlers{.add to int: current value = '\add@to@int@tmp'}%
		\IfStrEq{\add@to@int@tmp}{}{%
			\edef\add@to@int@tmp{0}%
		}{}%
	}{%
		% key is not defined
		%\Debug@Out@PgfHandlers{.add to int: key '\pgfkeyscurrentpath' is NOT defined}%
		\edef\add@to@int@tmp{0}%
	}%
	%\Debug@Out@PgfHandlers{.add to int: current value after possible adjustment = '\add@to@int@tmp'}%
	\setcounter{PgfAddToIntCnt}{\add@to@int@tmp}%
	%\Debug@Out@PgfHandlers{.add to int: counter set to curr value: '\thePgfAddToIntCnt'}%
	\addtocounter{PgfAddToIntCnt}{#1}%
	%\Debug@Out@PgfHandlers{.add to int: counter incremented to final value: '\thePgfAddToIntCnt'}%
	\pgfkeys{\pgfkeyscurrentpath/.expanded = {\thePgfAddToIntCnt}}%
	%\pgfkeys{\pgfkeyscurrentpath/.get=\add@to@int@tmp@final}%
	%\Debug@Out@PgfHandlers{.add to int: new value for key '\pgfkeyscurrentpath' stored: '\add@to@int@tmp@final'}%
}

\pgfkeysdef{/handlers/.replace if larger}{%
	\PgfKeys@Replace@If{#1}{>}%
}	
\pgfkeysdef{/handlers/.replace if smaller}{%
	\PgfKeys@Replace@If{#1}{<}%
}	


\newcommand{\PgfKeys@Replace@If}[2]{% 
	% #1: possible new value
	% >|<  : #1 will replace current value if >|< it
	\pgfkeysifdefined{\pgfkeyscurrentpath}{%
		% if key is defined
		\pgfkeys{\pgfkeyscurrentpath/.get=\replace@if@larger@tmp}%
		\IfStrEq{\replace@if@larger@tmp}{}{%
			\edef\replace@if@larger@tmp{0}%
		}{}%
	}{%
		% key is not defined
		\edef\replace@if@larger@tmp{0}%
	}%
	\ifnumcomp{#1}{#2}{\replace@if@larger@tmp}{%		
		\pgfkeys{\pgfkeyscurrentpath/.expanded = {#1}}%
	}{}%
}




%% WHY THIS DOES NOT WORK?!!!
%% Weird compilation errors and & in PgfHandlerss are displayed as '&' !
% \usetikzlibrary{fpu}
% \pgfkeysdef{/handlers/.add to float}{%
% 	\pgfkeysifdefined{\pgfkeyscurrentpath}{%
% 		% if key is defined
% 		%\typeout{.add to int: key is defined}%
% 		\pgfkeys{\pgfkeyscurrentpath/.get=\tmp@Initial}%
% 		\IfStrEq{\tmp@Initial}{}{%
% 			\edef\tmp@Initial{0}%
% 		}{}%
% 	}{%
% 		% key is not defined
% 		\edef\tmp@Initial{0}%
% 	}%
% 	%\typeout{add to float: starting value: [\tmp@Initial] -- increment: [#1]}%	
% 	\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}
% 	\pgfmathparse{50 + 3}%{\tmp@Initial + #1}%
% 	%\typeout{add to float: result is \pgfmathresult}%
% 	\pgfkeys{\pgfkeyscurrentpath/.expanded = \pgfmathresult}%
% 	\pgfkeys{/pgf/fpu=false}%
% }

==> MCLabPaper_Pretty_2.tex <==
\MCLabPaper@Set@Tutorial@Section{Pretty}{sec:pretty}

\DeclareDocumentCommand{\Debug@Out@Pretty}{o m}{%
	\Debug@Out{Pretty}[#1]{#2}%
}

\def\Pretty@Eur{Eur}

%% STYLES
\def\Pretty@Data@Prefix{MCLabPaper/Pretty}


\define@cmdkey{PrettyNewStyle}{decimaldigits}[]{}
\define@cmdkey{PrettyNewStyle}{unit}[]{}
\define@cmdkey{PrettyNewStyle}{unitpos}[after]{}
\define@cmdkey{PrettyNewStyle}{unitsep}[\nobreakspace]{}
\define@cmdkey{PrettyNewStyle}{convert}[\Pretty@Convert@nop]{}
\define@cmdkey{PrettyNewStyle}{output}[\num]{}

\DeclareDocumentCommand{\PrettyDefineStyle}{m m}{
	% #1: style name
	% #2: options (key=value list)
	\setkeys{PrettyNewStyle}{decimaldigits, unit, unitpos, unitsep, convert, output}%
	\setkeys{PrettyNewStyle}{#2}%
	%
	\pgfglobalkeys{\Pretty@Data@Prefix/style/#1/.cd,
		unit/.initial/.expand once={\cmdKV@PrettyNewStyle@unit}, 
		unitpos/.initial/.expand once={\cmdKV@PrettyNewStyle@unitpos}, 
		unitsep/.initial/.expand once={\cmdKV@PrettyNewStyle@unitsep},
		decimaldigits/.initial/.expand once={\cmdKV@PrettyNewStyle@decimaldigits}, 
		convert/.initial/.expand once={\cmdKV@PrettyNewStyle@convert}, 
		output/.initial/.expand once={\cmdKV@PrettyNewStyle@output}, 
	}%
}

\DeclareDocumentCommand{\PrettyStyleUnit}{m}{% #1 = style
	\pgfglobalkeys{\Pretty@Data@Prefix/style/#1/unit}%
}

\PrettyDefineStyle{default}{}
\PrettyDefineStyle{eur}{unit=\Pretty@Eur, unitpos=before, decimaldigits=2}
\PrettyDefineStyle{keur}{unit=k\Pretty@Eur, unitpos=after, decimaldigits=0, convert=\Pretty@Convert@k}
\PrettyDefineStyle{meur}{unit=M\Pretty@Eur, unitpos=after, decimaldigits=0, convert=\Pretty@Convert@m}

%\pgfglobalkeys{\Pretty@Data@Prefix/style/keur/.cd,
%	unit/.initial={k\Pretty@Eur}, 
%	unitpos/.initial=after, 
%	unitsep/.initial={\nobreakspace}, 
%	decimaldigits/.initial=0,
%	convert/.initial={\Pretty@Convert@k},
%	output/.initial={\num}	
%}
%% Style 'meur'
%\pgfglobalkeys{\Pretty@Data@Prefix/style/meur/.cd,
%	unit/.initial={M\Pretty@Eur}, 
%	unitpos/.initial=after, 
%	unitsep/.initial={\nobreakspace}, 
%	decimaldigits/.initial=0,
%	convert/.initial={\Pretty@Convert@m},
%	output/.initial={\num}	
%}



%% Style 'percentage'
\PrettyDefineStyle{percentage}{unit=\%, unitpos=after, unitsep={}, decimaldigits=2, convert=\Pretty@Convert@percentage}
%\pgfglobalkeys{\Pretty@Data@Prefix/style/percentage/.cd,
%	unit/.initial={\%}, 
%	unitpos/.initial=after, 
%	unitsep/.initial={}, 
%	decimaldigits/.initial=2,
%	convert/.initial={\Pretty@Convert@percentage},
%	output/.initial={\num}	
%}

%% Style 'hms'
\PrettyDefineStyle{hms}{unit=(h:m:s), unitpos=after, decimaldigits={}, convert=\Pretty@Convert@hms, output=\Pretty@Output@nop}
%\pgfglobalkeys{\Pretty@Data@Prefix/style/hms/.cd,
%	unit/.initial={(h:m:s)}, 
%	unitpos/.initial=after, 
%	unitsep/.initial={\nobreakspace}, 
%	decimaldigits/.initial={},
%	convert/.initial={\Pretty@Convert@hms},
%	output/.initial={\Pretty@Output@nop}	
%}
%% Style 'timeprose'
\PrettyDefineStyle{timeprose}{unit={}, unitpos=after, unitsep={}, decimaldigits={}, convert=\Pretty@Convert@timeprose, output=\CommaSepListToProse}

%\pgfglobalkeys{\Pretty@Data@Prefix/style/timeprose/.cd,
%	unit/.initial={}, 
%	unitpos/.initial=after, 
%	unitsep/.initial={}, 
%	decimaldigits/.initial={},
%	convert/.initial={\Pretty@Convert@timeprose},
%	output/.initial={\CommaSepListToProse}
%}
%% Style 'list'
%\pgfglobalkeys{\Pretty@Data@Prefix/style/list/.cd,
%	unit/.initial={}, 
%	unitpos/.initial=after, 
%	unitsep/.initial={}, 
%	decimaldigits/.initial={},
%	convert/.initial={Pretty@Convert@timeprose}
%}

\def\Pretty@max@decimals@in@conversion{5}

\def\Pretty@Output@nop#1{#1}%
\def\Pretty@Convert@nop#1#2{\let#1#2}%
\def\Pretty@Convert@percentage#1#2{%
	\MathEval[#1]{%
		round( (#2)*100 : \Pretty@max@decimals@in@conversion)%
	}%
} % note (#2) to handle negative values!
\def\Pretty@Convert@k#1#2{\MathEval[#1]{round(#2/1000 : \Pretty@max@decimals@in@conversion)}}
\def\Pretty@Convert@m#1#2{\MathEval[#1]{round( #2/1000000 : \Pretty@max@decimals@in@conversion)}}

\def\Pretty@Convert@hms#1#2{%	
	%RETURNS #2 seconds converted to H:M:S
	%\def\@value{#2}%
	\Debug@Out@Pretty[Convert@hms(#2)]{Start}%
	\IfDecimal{#2}{%
		\Debug@Out@Pretty[Convert@hms(#2)]{arg is decimal}%
		\edef\@value{\number\integerpart}%
		\Debug@Out@Pretty[Convert@hms(#2)]{  - int part = '\@value'}%
		\edef\@value@decimal{\number\decimalpart}%
		\Debug@Out@Pretty[Convert@hms(#2)]{  - decimal part = '\@value@decimal'}%
		\IfInteger{#2}{%
			\edef\@value@decimal{}% %empty, as used did not request to show fraction
		}{}%
		%
		\Debug@Out@Pretty[Convert@hms(#2)]{integer part = '\@value', decimal part = '\@value@decimal'}%
		\xdef\@sign{}%
		\FPifneg{\@value}%
			\xdef\@sign{-}%
			%\typeout{argument is negative}
			\FPeval{\@value}{0-\@value}%
			%\typeout{MathSecondsToHMS: value < 0. Now \@value}
		\fi%
		\FPeval{@hours}{\@value / (60*60)}%
		\FPtrunc{\@hours}{\@hours}{0}%
		\FPeval{@rest}{\@value - (\@hours*60*60)}%
		\FPeval{@minutes}{\@rest/60}%	
		\FPtrunc{\@minutes}{\@minutes}{0}%	
		\FPeval{@seconds}{\@rest - (\@minutes*60)}%	
		\FPtrunc{\@seconds}{\@seconds}{0}%		
		\edef\TimeSecondsToHMS@result{\@sign\@hours:\@minutes:\@seconds}%
		\ifequals{\@value@decimal}{}{}{%
			\edef\TimeSecondsToHMS@result{\TimeSecondsToHMS@result.\@value@decimal}%
		}%
		\edef@macro{#1}{\TimeSecondsToHMS@result}%
	}{%
		\DiagWarning{Pretty}{Cannot convert `#2' to h:m:s because argument is not a decimal number}%
	}%
	\Debug@Out@Pretty[Convert@hms(#2)]{End}%
}

\def\Pretty@Convert@ordinal@english#1#2{%
	\Debug@Out@Pretty[Convert@ordinal(#2)]{Start}%
	\IfInteger{#2}{}{%
		\DiagError{Pretty}{\DiagLatexCmd{Pretty[style=ordinal...]\{#2\}}: Value must be an integer}[\ Pretty[style=ordinal...]{#2}: Value must be an integer]%
	}%
	%
	\ifnumcomp{#2}{<}{0}{%
		\DiagError{Pretty}{\DiagLatexCmd{Pretty[style=ordinal...]\{#2\}}: Number must be >= 0}[\ Pretty[style=ordinal...]{#2}: Number must be >= 0]%
	}{}%
	%
	\StrRight{#2}{1}[\Pretty@Convert@ordinal@last]%
	%
	\def\Pretty@Convert@ordinal@suffix{th}%
	%
	\ifcase\Pretty@Convert@ordinal@last% 0
		\or% 1
			\def\Pretty@Convert@ordinal@suffix{st}%
		\or% 2
			\def\Pretty@Convert@ordinal@suffix{nd}%
		\or% 3
			\def\Pretty@Convert@ordinal@suffix{rd}%
	  	\else% >2
 	\fi
 	%
	\edef@macro{#1}{#2\Pretty@Convert@ordinal@suffix}%
	\Debug@Out@Pretty[Convert@ordinal(#2)]{Result = '#1'}%
	\Debug@Out@Pretty[Convert@ordinal(#2)]{End}%
}




\addto\captionsenglish{%
  \def\MCLabPaper@hour{hour}%
  \def\MCLabPaper@hours{hours}%  
  \def\MCLabPaper@minute{minute}%  
  \def\MCLabPaper@minutes{minutes}%
  \def\MCLabPaper@second{second}%  
  \def\MCLabPaper@seconds{seconds}% 
  \PrettyDefineStyle{ordinal}{unit={}, unitpos=after, decimaldigits=0, convert=\Pretty@Convert@ordinal@english}
}
\addto\captionsitalian{%
  \def\MCLabPaper@hour{ora}%
  \def\MCLabPaper@hours{ore}%  
  \def\MCLabPaper@minute{minuto}%  
  \def\MCLabPaper@minutes{minuti}%
  \def\MCLabPaper@second{secondo}%  
  \def\MCLabPaper@seconds{secondi}% 
  \PrettyDefineStyle{ordinal}{unit={\ensuremath{{}^{\circ}}}, unitpos=after, unitsep={}, decimaldigits=0, convert=\Pretty@Convert@nop}
}

\def\Pretty@Convert@timeprose#1#2{%
	\Debug@Out@Pretty[Convert@timeprose(#2)]{Start}%
	\IfDecimal{#2}{%
		\Debug@Out@Pretty[Convert@timeprose(#2)]{arg is decimal}%
		\edef\@value{\number\integerpart}%
		\Debug@Out@Pretty[Convert@timeprose(#2)]{  - int part = '\@value'}%
		\edef\@value@decimal{\number\decimalpart}%
		\Debug@Out@Pretty[Convert@timeprose(#2)]{  - decimal part = '\@value@decimal'}%
		\IfInteger{#2}{%
			\edef\@value@decimal{}% %empty, as used did not request to show fraction
		}{}%
		\FPeval{@hours}{\@value / (60*60)}%
		\FPtrunc{\@hours}{\@hours}{0}%
		%\typeout{\@value -> hours (trunc): [\@hours]}%	
		\FPeval{@rest}{\@value - (\@hours*60*60)}%
		%\typeout{\@value -> rest: [\@rest]}%		
		\FPeval{@minutes}{\@rest/60}%
		\FPtrunc{\@minutes}{\@minutes}{0}%	
		%\typeout{\@value -> minutes (trunc): [\@minutes]}%	
		\FPeval{@seconds}{\@rest - (\@minutes*60)}%	
		\FPtrunc{\@seconds}{\@seconds}{0}%
		%\typeout{\@value -> seconds (trunc): [\@seconds]}%		
		%
		\CommaSepListNew{TimeSecondsToHMSProse@result}%
		%
		\Debug@Out@Pretty[Convert@timeprose(#2)]{Converting into time-prose: \@hours:\@minutes:\@seconds}%
		\ifthenelse{\@hours = 0}{}{%
			\edef\@hours@prose{\@hours\space}%
			\ifthenelse{\@hours > 1}{%
				\edef\@hours@prose{\@hours@prose\MCLabPaper@hours}%
			}{%
				\edef\@hours@prose{\@hours@prose\MCLabPaper@hour}%
			}%
			\CommaSepListAppend{TimeSecondsToHMSProse@result}[/.expanded]{\@hours@prose}%
		}%
		\ifthenelse{\@minutes = 0}{}{%
			\edef\@minutes@prose{\@minutes\space}%
			\ifthenelse{\@minutes > 1}{%
				\edef\@minutes@prose{\@minutes@prose\MCLabPaper@minutes}%
			}{%
				\edef\@minutes@prose{\@minutes@prose\MCLabPaper@minute}%
			}%
			\CommaSepListAppend{TimeSecondsToHMSProse@result}[/.expanded]{\@minutes@prose}%		
		}%
		\Debug@Out@Pretty[Convert@timeprose(#2)]{ - processing seconds: '\@seconds'}%
		\ifthenelse{ \equal{\@seconds}{0} \AND \(\equal{\@value@decimal}{} \OR \equal{\@value@decimal}{0}\)}{%
			\Debug@Out@Pretty[Convert@timeprose(#2)]{   --> seconds is zero}%
		}{%
			\Debug@Out@Pretty[Convert@timeprose(#2)]{   --> seconds is not zero}%
			\ifequals{\@value@decimal}{}{}{%
				\edef\@seconds{\@seconds.\@value@decimal}%
			}%
			%
			\edef\@seconds@prose{\@seconds\space}%
			\Debug@Out@Pretty[Convert@timeprose(#2)]{   --> seconds-prose (step 1) is '\@seconds@prose'}%
			\ifthenelse{\equal{\@seconds}{1}}{% % can be decimal
				\edef\@seconds@prose{\@seconds@prose\MCLabPaper@second.}%
			}{%
				\edef\@seconds@prose{\@seconds@prose\MCLabPaper@seconds}%
			}%
			\Debug@Out@Pretty[Convert@timeprose(#2)]{   --> final seconds-prose is '\@seconds@prose'}%
			\CommaSepListAppend{TimeSecondsToHMSProse@result}[/.expanded]{\@seconds@prose}%
		}%
		%
		%\CommaSepListToProse[\TimeSecondsToHMSProse@result]%
			%{TimeSecondsToHMSProse@result}			
		%\Debug@Out@Pretty[Convert@timeprose(#2)]{ --> final prose: [\TimeSecondsToHMSProse@result]}%
		%\edef@macro{#1}{\TimeSecondsToHMSProse@result}%	
		\CommaSepList{TimeSecondsToHMSProse@result}{#1}%	
	}{%
		\DiagWarning{Pretty}{Cannot convert `#2' to timeprose because argument is not a decimal number}%
	}%
	\Debug@Out@Pretty[Convert@timeprose(#2)]{End}%
}



\define@cmdkey{Pretty}{style}[default]{}
\define@cmdkey{Pretty}{decimaldigits}[\relax]{}
\define@cmdkey{Pretty}{unit}[\relax]{}
\define@cmdkey{Pretty}{unitpos}[\relax]{}
\define@cmdkey{Pretty}{unitsep}[\relax]{}

\DeclareDocumentCommand{\Pretty}{O{} m}{%
	% Pretty prints numbers
	% [#1]: style hints
	% #2: a comma sep. list of values
	\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Start}%
	\setkeys{Pretty}{style, decimaldigits, unit, unitpos, unitsep}%
	\@expandtwoargs\setkeys{Pretty}{style=default, #1}%
	%
	\ifequals{\cmdKV@Pretty@style}{none}{#2}{%
		%
		% Get options from style
		\pgfglobalkeys{\Pretty@Data@Prefix/style/\cmdKV@Pretty@style/.cd,
			unit/.get=\Pretty@unit,
			unitpos/.get=\Pretty@unitpos, 
			unitsep/.get=\Pretty@unitsep, 
			decimaldigits/.get=\Pretty@decimaldigits,
		}%
		% Override options if given
		\ifequals{\cmdKV@Pretty@decimaldigits}{\relax}{}{%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Overriding: decimaldigits=\cmdKV@Pretty@decimaldigits}%
			\def\Pretty@decimaldigits{\cmdKV@Pretty@decimaldigits}%
		}%
		\ifequals{\cmdKV@Pretty@unit}{\relax}{}{%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Overriding: unit=\cmdKV@Pretty@unit}%	
			\def\Pretty@unit{\cmdKV@Pretty@unit}%
		}%
		\ifequals{\cmdKV@Pretty@unitpos}{\relax}{}{%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Overriding: unitpos=\cmdKV@Pretty@unitpos}%	
			\def\Pretty@unitpos{\cmdKV@Pretty@unitpos}%
		}%
		\ifequals{\cmdKV@Pretty@unitsep}{\relax}{}{%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Overriding: unitsep=\cmdKV@Pretty@unitsep}%	
			\def\Pretty@unitsep{\cmdKV@Pretty@unitsep}%
		}%
		%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Pretty-printing (possibly) list of values: [#2]}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{After having read style and overridden options:}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ - style:  [\cmdKV@Pretty@style]}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ - unit: [\Pretty@unit]}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ - unitpos: [\Pretty@unitpos]}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ - unitsep: [\Pretty@unitsep]}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ - decimaldigits: [\Pretty@decimaldigits]}%
		%
		%
		\CommaSepListNew{Pretty@output@list}%
		\xintFor ##3 in {#2} \do{%
			\def\Pretty@user@value{##3}%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{}%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Pretty printing single user value: [\Pretty@user@value]}%
			%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Applying conversion to [\Pretty@user@value]...}%		
			\pgfglobalkeys{\Pretty@Data@Prefix/style/\cmdKV@Pretty@style/%
				convert/.get=\Pretty@convert@cmd}%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ - conversion function is \expandonce\Pretty@convert@cmd}%
			\Pretty@convert@cmd{\Pretty@value}{\Pretty@user@value}%
			%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ --> actual value to be pretty-printed is [\Pretty@value]}%
			%
			%
			\saveexpandmode%
			\expandarg%
			\IfDecimal{\Pretty@value}{%		
				\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Value [\Pretty@value] is a number}%
				%				
				%
				\ifequals{\Pretty@decimaldigits}{}{}{%
					\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Rounding to [\Pretty@decimaldigits] decimal digits}%
					\MathEval[\Pretty@value]{round(\Pretty@value : \Pretty@decimaldigits)}%
					\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ --> value is now [\Pretty@value]}%
				}%
				%
				% Pretty printing value
				\pgfglobalkeys{\Pretty@Data@Prefix/style/\cmdKV@Pretty@style/%
					output/.get=\Pretty@output@cmd}%
				%
				\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ --> applying output function to value [\Pretty@value]}%
				\edef\Pretty@value{\Pretty@output@cmd{\Pretty@value}}%
				\Debug@Out@Pretty[{Pretty[#1]{#2}}]{ --> output value is [\Pretty@value]}%
				%
				% Adding unit, if given
				\ifequals{\Pretty@unit}{}{}{%
					% Unit given
					\ifequals{\Pretty@unitpos}{before}{%
						\edef\Pretty@value{\Pretty@unit\Pretty@unitsep\Pretty@value}%
					}{%
						\edef\Pretty@value{\Pretty@value\Pretty@unitsep\Pretty@unit}%
					}%
				}%
			}{%
				\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Pretty: value is NOT a number. Doing nothing (except conversion from user-value: [\Pretty@user@value] -> [\Pretty@value])}%
			}%
			%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{  --> adding [\Pretty@value] to output list}%
			%
			\CommaSepListAppend{Pretty@output@list}[/.expand once]{{\Pretty@value}}%
			%
			\CommaSepListSize[\tmpNbElems]{Pretty@output@list}%
			\Debug@Out@Pretty[{Pretty[#1]{#2}}]{  --> now output list contains \tmpNbElems\space elements}%
			\restoreexpandmode%
		}% end xintFor
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{All items done.}%
		\CommaSepList{Pretty@output@list}{\Pretty@output@list@content}%
		\Debug@Out@Pretty[{Pretty[#1]{#2}}]{Output list (to be printed as prose) is [\Pretty@output@list@content].}%
		\CommaSepListToProse[\Pretty@final@prose]{Pretty@output@list}%
		\Pretty@final@prose%
	}%
}










\endinput



\define@cmdkey{Pretty}{decimaldigits}[-1]{}
\define@cmdkey{Pretty}{unit}[]{}

\pgfglobalkeys{\pgfkeysPrefix/Pretty/auto/.cd,
	unit/EUR/.initial={decimaldigits=2},
	unit/Eur/.initial={decimaldigits=2},
}

\DeclareDocumentCommand{\Pretty}{O{} m}{%
	% Pretty prints numbers
	% [#1]: style hints
	% #2: value
	\setkeys{Pretty}{style, decimaldigits, unit}%	
	\@expandtwoargs\setkeys{Pretty}{#1}%
	%
%	\ifthenelse{\equal{\cmdKV@Pretty@style}{auto}}{% % auto style
%		\pgfglobalkeys{\pgfkeysPrefix/Pretty/auto/unit/\cmdKV@Pretty@unit/.get=\Pretty@auto@options}%
%		\Debug@Out@Pretty{Pretty: setting autooptions [\Pretty@auto@options]...}%
%		\setkeys{Pretty}\Pretty@auto@options@exp	% % set auto options
%		\Debug@Out@Pretty{Pretty: setting autooptions [\Pretty@auto@options] done}%
%		\setkeys{Pretty}{#1}% re-set given options to override auto optiokns
%	}{}%
	%
	\Debug@Out@Pretty{style:  [\cmdKV@Pretty@style]}%
	\Debug@Out@Pretty{unit: [\cmdKV@Pretty@unit]}%
	\Debug@Out@Pretty{decimaldigits: [\cmdKV@Pretty@decimaldigits]}%	
	\edef\Pretty@value{#2}%
	\Debug@Out@Pretty{Pretty: expanded value: [\Pretty@value]}%
	\IfDecimal{\Pretty@value}{%		
		\Debug@Out@Pretty{Pretty: value is a number}%
		%
		% Processing style=percentage option
		%
		\ifthenelse{\equal{\cmdKV@Pretty@style}{percentage}}{%
			\MathEval[\Pretty@value]{\Pretty@value * 100}%
			\setkeys{Pretty}{unit=\%}%
		}{}%
		% Processing decimaldigits=N option
		\ifnumgreater{\cmdKV@Pretty@decimaldigits}{-1}{%
			\Debug@Out@Pretty{Pretty: rounding to [\cmdKV@Pretty@decimaldigits] decimal digits}%
			\MathEval[\Pretty@value]{round(\Pretty@value : \cmdKV@Pretty@decimaldigits)}%
		}%
		%
		\expandafter\num{\Pretty@value}%
	}{%
		\Debug@Out@Pretty{Pretty: value is NOT a number}%
		% style=list
		\ifthenelse{\equal{\cmdKV@Pretty@style}{list}}{%
			\edef\Pretty@value{\CommaSepListToProse{\Pretty@value}}%
		}{}%	
		\Pretty@value%
	}%
	\ifthenelse{\equal{\cmdKV@Pretty@unit}{}}{}{%
		\ifthenelse{\equal{\cmdKV@Pretty@unit}{\%}}{}{%
			\edef\cmdKV@Pretty@unit{ \cmdKV@Pretty@unit}%
		}%
		\cmdKV@Pretty@unit%
	}%
}
%\ExplSyntaxOff

==> MCLabPaper_Section_2.tex <==

\MCLabPaper@Set@Tutorial@Section{Section}{sec:section}

\DeclareDocumentCommand{\Debug@Out@Section}{o m}{%
	\Debug@Out{Section}[#1]{#2}%
}




\addto\captionsenglish{%
	\def\MCLabPaper@sectionname{Section}%
	\def\MCLabPaper@sectionname@plural{Sections}%
}
\addto\captionsitalian{%
	\def\MCLabPaper@sectionname{Sezione}%
	\def\MCLabPaper@sectionname@plural{Sezioni}%
}



\ArrayNew{Sectioning}
\ArrayAdd{Sectioning}{part}
\ArrayAdd{Sectioning}{chapter}
\ArrayAdd{Sectioning}{section}
\ArrayAdd{Sectioning}{subsection}
\ArrayAdd{Sectioning}{subsubsection}
\ArrayAdd{Sectioning}{paragraph}
\ArrayAdd{Sectioning}{subparagraph}


\newcounter{Section@AddLevel@curr@depth}

\DeclareDocumentCommand{\SectionAddLevel}{}{%
	\Debug@Out@Section[SectionAddLevel]{Start}%
	\ArrayLastIndex[\Section@max@depth]{Sectioning}%
	\Debug@Out@Section[SectionAddLevel]{Max depth = \Section@max@depth}%
	\setcounter{Section@AddLevel@curr@depth}{\Section@max@depth}%
	\stepcounter{Section@AddLevel@curr@depth}%
	%\MathEval[\Section@AddLevel@curr@depth]{round(\Section@max@depth + 1 :0)}%
	%
	%\Debug@Out@Section{MCLabPaper_Section: SectionAddLevel: curr depth = \theSection@AddLevel@curr@depth}%
	\Debug@Out@Section[SectionAddLevel]{Creating section commands from depth `\theSection@AddLevel@curr@depth'}%
		%
		% Command at previous depth
		\ArrayGet[\Section@prev@section@cmd@name]{Sectioning}{\Section@max@depth}%
		%
		% New section command name
		\edef\Section@curr@cmd@name{SectionLevel\theSection@AddLevel@curr@depth}
		\Debug@Out@Section[SectionAddLevel]{Creating counter `\Section@curr@cmd@name' based on `\Section@prev@section@cmd@name'}%
		\newcounter{\Section@curr@cmd@name}[\Section@prev@section@cmd@name]%
		\Debug@Out@Section[SectionAddLevel]{ --> done}%
		\csgdef{the\Section@curr@cmd@name}{%
			\csuse{the\Section@prev@section@cmd@name}.\@arabic\csuse{c@\Section@curr@cmd@name}%
		}%
		\Debug@Out@Section[SectionAddLevel]{Command the\Section@curr@cmd@name\space defined}%
		\csgdef{\Section@curr@cmd@name}{%
			\@startsection{\Section@curr@cmd@name}% counter
			{\theSection@AddLevel@curr@depth}% level
			{0pt}%{\parindent}% indent
			{3.25ex \@plus 1ex \@minus .2ex}% beforeskip
			{-1em}% afterskip
			{\normalfont\normalsize\bfseries}%
		}%
		\crefname{\Section@curr@cmd@name}{\MCLabPaper@sectionname}{\MCLabPaper@sectionname@plural}
		\Debug@Out@Section[SectionAddLevel]{Command \Section@curr@cmd@name\space  defined}%
		\csgdef{l@\Section@curr@cmd@name}{\@dottedtocline{6}{10em}{5em}}%
		\Debug@Out@Section[SectionAddLevel]{Command l@\Section@curr@cmd@name\space  defined}%
		\csgdef{\Section@curr@cmd@name mark}##1{}%
		\Debug@Out@Section[SectionAddLevel]{Command \Section@curr@cmd@name mark\space  defined}%
		\Debug@Out@Section[SectionAddLevel]{Adding command \Section@curr@cmd@name\space  to Sectioning Array...}%
		%
		\ArrayAdd{Sectioning}{\Section@curr@cmd@name}%
		\ArrayLastIndex[\Section@max@depth]{Sectioning}%
		\Debug@Out@Section[SectionAddLevel]{End. Now Sectioning Array has \Section@max@depth\space elements.}%
}


%% CREATE HOOKS 
\DeclareDocumentCommand{\MCLabPaper@Sectioning@Hook@Name}{m m}{%
	% #1: output macro, #2: section command
	\edef@macro{#1}{MCLabPaper@Sectioning@hook@#2}%	
}

\DeclareDocumentCommand{\Section@Create@Hooks}{}{%
	\Debug@Out@Section[Create@Hooks]{Start}%
	\ArrayLastIndex[\tmp@sectioning@maxlevel]{Sectioning}	
	\Debug@Out@Section[Create@Hooks]{ - max defined depth is '\tmp@sectioning@maxlevel'}
	\xintFor* ##1 in {\xintSeq [1]{0}{\tmp@sectioning@maxlevel}} \do{%
		%\Debug@Out@Section{ - command at depth #1 is...}%
		\ArrayGet[\tmp@sectioning@section@command]{Sectioning}{##1}%
		%\Debug@Out@Section{ ---> '\tmp@sectioning@section@command'}%
		\Debug@Out@Section[Create@Hooks]{Creating hook for section level '##1' (\tmp@sectioning@section@command)}		
		\MCLabPaper@Sectioning@Hook@Name%
			{\tmp@sectioning@hook@name}{\tmp@sectioning@section@command}%
		%
		\Debug@Out@Section[Create@Hooks]{ --> Hook function name is \tmp@sectioning@hook@name}
		%\@expandtwoargs
		\csdef{\tmp@sectioning@hook@name}{}%test hook \tmp@sectioning@section@command}%
	}%
	\Debug@Out@Section[Create@Hooks]{End}%
}

\AtBeginDocument{%
	\Section@Create@Hooks%
}



\newcounter{Sections@current@depth}
\setcounter{Sections@current@depth}{0} %{\Sections@min@depth}
\gdef\Sections@min@depth{0}

\newcommand{\SectionSetStart@by@number}[1]{%
	\def\SectionSetStart@by@number@depth{#1}%
	\Debug@Out@Section[SectionSetStart@by@number{#1}]{Requested top-level is '\SectionSetStart@by@number@depth'}%
 	\ifnumcomp{\SectionSetStart@by@number@depth}{<}{0}{%
 		\DiagError{SectionSetStart}{Wrong argument '#1'}%
 	}{}%
 	\setcounter{Sections@current@depth}{\SectionSetStart@by@number@depth}%
 	\xdef\Sections@min@depth{\SectionSetStart@by@number@depth}%
 	\Debug@Out@Section[SectionSetStart@by@number{#1}]{Section depth set to (\theSections@current@depth)}%
}
\DeclareDocumentCommand{\SetSectionStart}{m}{%
	\DiagDeprecationSimple{Section}{SetSectionStart}{SectionSetStart}%
	\SectionSetStart{#1}%
}

\newcommand{\SectionSetStart}[1]{%
	\Debug@Out@Section[SectionSetStart{#1}]{Requested top-level name is '#1'}%
	\ArrayPos[\SectionSetStart@depth]{Sectioning}{#1}%
	\SectionSetStart@by@number{\SectionSetStart@depth}%
}

\newcommand{\SectionSetStart@Incr}{%
	\MathEval[\SectionSetStart@Incr@depth]{round(\theSections@current@depth + 1 :0)}%
	\SectionSetStart@by@number{\SectionSetStart@Incr@depth}%
}



\DeclareDocumentCommand{\Fake@Section}{s m}{%
	% #1: star
	% #2: section title
	\par%
	\medskip%
	\noindent%
	\textbf{#2}~%
}

		
	
\DeclareDocumentEnvironment{Section}{ s o m }{
	% #1: star
	% #2: label
	% #3: section title
	\Debug@Out@Section[Section{#3}]{Start}%
	\ArrayLastIndex[\Section@max@depth]{Sectioning}%
	\Debug@Out@Section[Section{#3}]{Section max depth is '\Section@max@depth'}%
	\ifnum \theSections@current@depth > \Section@max@depth%
		\PackageWarning{MCLabPaper}{Too much nesting in Section environments. If you want deeper nesting, use a different class file (e.g., report) supporting chapters/parts and the SectionSetStart command. I'm flattening this subtree, layout could be ugly.}{}%
		\def\section@cmd{Fake@Section}%
	\else%
		\ArrayGet[\section@cmd]{Sectioning}{\theSections@current@depth}%%
	\fi%
		%
	\Debug@Out@Section[Section{#3}]{Starting Section: depth=\theSections@current@depth --> sec cmd = \section@cmd, title = '#3'}%		
	%\MCLabPaper@Flattening@Append{}%
	\IfBooleanTF{#1}%
		{%
			\csname\section@cmd\endcsname*{#3}%
				%\MCLabPaper@Flattening@Append{%
				%	\csuse{\section@cmd*}{#3}%
				%}%								
		}%
		{%
			\csname\section@cmd\endcsname{#3}%
				%\MCLabPaper@Flattening@Append{%
				%	\csuse{\section@cmd}{#3}%
				%}%				
		}%
	%
	\Debug@Out@Section[Section{#3}]{ - \section@cmd\space command called}%
	\MCLabPaper@Sectioning@Hook@Name{\section@hook}{\section@cmd}%		
	\csuse{\section@hook}%
		%\MCLabPaper@Flattening@Append{\csuse{\section@hook}}%
	\Debug@Out@Section[Section{#3}]{ - \section@cmd\space hooked}%
	\IfValueT{#2}{% #2 = label
		\edef\Section@label@type{section}%
		\ifequals{\section@cmd}{chapter}{%
			\edef\Section@label@type{chapter}%
		}{}%
		\ifequals{\section@cmd}{part}{%
			\edef\Section@label@type{part}%
		}{}%		
		%\Label[\Section@label@type]{#2}%
		\label{#2}%
		\Debug@Out@Section[Section{#3}]{ - \section@cmd labelled}%
			%\MCLabPaper@Flattening@Append{\Label[\Section@label@type]{#2}}%
		\immediate\write\@mainaux{%
			\noexpand\expandafter\gdef\noexpand\csname seccmd:#2%
				\noexpand\endcsname{\section@cmd}%
		}%
		\Debug@Out@Section[Section{#3}]{ - \section@cmd label info stored in aux file}%
		%
		\Draft@SystemNote{Label: \RenderLabel{#2}}%  
	}%
	\addtocounter{Sections@current@depth}{1}%	
	%
	%
}{%
	\addtocounter{Sections@current@depth}{-1}%
	\ifnum \theSections@current@depth < \Sections@min@depth%
		\PackageError{MCLabPaper}{Bad nesting of Section environments!}{}%
	\fi%
	\par%
}


\DeclareDocumentCommand{\SectionInput}{ s t- o m O{} m}{%
	% #1: star
	% #2: - (optional): skips content in draft mode
	% #3: label
	% #4: section title
	% #5: base relative path
	% #6: file relpath names (comma separated)
	\Debug@Out@Section[SectionInput{#4}[#5]{#6}]{Start}%
	\IfBooleanTF{#1}%
		{ \begin{Section}*[#3]{#4} }%
		{ \begin{Section}[#3]{#4} }%
	\IfDraftTF{%
		\IfBooleanTF{#2}{%
			\DraftWarning{Body of section `#4' skipped in draft mode}
		}{%
			\Input[#5]{#6}%
		}%
	}{
		\Input[#5]{#6}%
	}
	\end{Section}%
	\Debug@Out@Section[SectionInput{#4}[#5]{#6}]{End}%
}
\let\InputSection\SectionInput



==> MCLabPaper_Statement_2.tex <==
\MCLabPaper@RequirePackage{newenviron}
\MCLabPaper@RequirePackage{amsthm}

\MCLabPaper@Set@Tutorial@Section{Statement}{sec:stmt}

\DeclareDocumentCommand{\Debug@Out@Stmt}{o m}{%
	\Debug@Out{Statement}[#1]{#2}%
}




\let\StmtOldProof\proof
\let\endStmtOldProof\endproof


\def\stmt@appendToPgfglobalkeyList#1#2{%
	% #1: elem, #2: a pgfkey of type 'list'.  Appends #1 to the list in pgfkey #2
	\pgfglobalkeysifdefined{#2}{}{%
		% define #2 as empty list
		%\outdebug{key undefined, set to the empty list}%
		\pgfglobalkeys{#2/.initial={}}%
	}%
	%
	\pgfglobalkeys{#2/.get=\ToniLists@list}%
	%
	\ifthenelse{ \equal{\ToniLists@list}{} }{}{%
		\pgfglobalkeys{#2/.append={, }}%
	}
	\pgfglobalkeys{#2/.append/.expanded={#1}}%
	%
	%\pgfglobalkeys{#2/.get=\ToniLists@list}
}


\pgfglobalkeys{/statements/config/ShowAlwaysProofs/.initial=0}



%\DeclareDocumentCommand{\stmt@debug}{o m}{%
%	\ifthenelse{\stmt@DEBUG = 0}{}{
%	        	\def\stmt@short@msg{#1}
%     		\def\stmt@long@msg{#2}
%	        	\IfValueF{#1}{%
%        			% no short msg
%        			\def\stmt@short@msg{\stmt@long@msg}
%	        	}
%        		\typeout{\stmt@short@msg}
%        		\par
%	        	\todo[inline]{\stmt@long@msg}	
%     		\par
%	}
%}



\DeclareDocumentCommand{\qed}{}{%
	\ensuremath{\hfill\square}
}


\newenviron{Statements@SkipContentEnv}{}


\gdef\stmt@at@end@body{\relax}
\newenviron{Statements@ShowProof}[2]{%
	% #1: label
	% #2: boolean (1 = show proof, 0 = don't show proof)
	\edef\proof@label{#1}
	\edef\proof@show{#2}
	%
	%
	\stmt@at@end@body{}
	%
	\ifthenelse{\proof@show = 0}{
		% don't show proof		
	}{ % show proof		
		%
		\edef\proof@current@eqcounter{\theequation}
		%
	        	\pgfglobalkeys{%
        			/statements/\proof@label/proof/nbshown/.get=\proof@nbshown
	        	}
	        	\ifthenelse{\proof@nbshown > 0}{%
        			%
        			\pgfglobalkeys{%
        				/statements/\proof@label/proof/eqcounter/.get=\proof@eqcounter
	        		}
			% temporarily set equation counter
	        		\setcounter{equation}{\proof@eqcounter}
        			\Debug@Out@Stmt[ShowProof(\proof@label)]{@proof@nbshown = \proof@nbshown (non-zero):
        				theequation set now to [\theequation]}
	        	}{%
			% first time proof is shown
        			\pgfglobalkeys{%
        				/statements/\proof@label/proof/eqcounter/.initial/.expanded=\theequation
	        		}
        			\Debug@Out@Stmt[@ShowProof(\proof@label)]{@proof@nbshown = \proof@nbshown (zero): 
        				setting eqcounter proof to theequation = \theequation}
	        	}
		%
        		\StmtOldProof
		\envbody
		\endStmtOldProof
		%
		%
		\ifthenelse{\proof@nbshown > 0}{
			% reset eqcounter to global counter
			\setcounter{equation}{\proof@current@eqcounter}
		}{}
		%
		% increment @nbshown@proof
		\FPeval{\proof@nbshown@new}{round(proof@nbshown+1:0)}	%
		\pgfglobalkeys{%
			/statements/\proof@label/proof/nbshown/.expanded=\proof@nbshown@new
		}%
		%
		%
		\Debug@Out@Stmt[@ShowProof(\proof@label)]{Proof shown. Now theequation is [\theequation]}%
		\Debug@Out@Stmt[@ShowProof(\proof@label)]{End}%
	}%end \ifthenelse
}


\DeclareDocumentCommand{\Statement@outStats}{m}{
	% #1: label
	\edef\stats@label{#1}
	\pgfglobalkeys{%
		/statements/\stats@label/counter/.get=\stats@counter,	
		/statements/\stats@label/type/.get=\stats@type,
		/statements/\stats@label/title/.get=\stats@title,
		/statements/\stats@label/body/nbshown/.get=\stats@nbshown@body,
		/statements/\stats@label/body/eqcounter/.get=\stats@eqcounter@body,				
		/statements/\stats@label/proof/nbshown/.get=\stats@nbshown@proof,	
		/statements/\stats@label/proof/eqcounter/.get=\stats@eqcounter@proof,	
	}%
	\par
	=== STATEMENT \stats@label ===:
	\begin{itemize}
	\item counter: [\stats@counter]  (prev number of this stmt counter)	
	\item type: [\stats@type]
	\item title: [\stats@title]
	\item body/nbshown: [\stats@nbshown@body]
	\item body/eqcounter: [\stats@eqcounter@body] (prev number of the first equation in the body of this stmt)	
	\item proof/nbshown: [\stats@nbshown@proof]	
	\item proof/eqcounter: [\stats@eqcounter@proof] (prev number of the first equation in the proof of this stmt)	
	\end{itemize}
	=======================
	\par
}


\newenviron{Statement@Define}[3]%
	% #1: type
	% #2: title (possibly {})
	% #3: label
	{%
		\edef\define@label{#3}
		%\stepcounter{#1}	
		%\def\@counter{\csname the#1\endcsname}
		%\def\@eqcounter{\theequation}		
		\pgfglobalkeys{%
			/statements/\define@label/type/.initial=#1,
			/statements/\define@label/title/.initial={#2},
			/statements/\define@label/body/nbshown/.initial=0,
			/statements/\define@label/proof/nbshown/.initial=0,			
			/statements/\define@label/body/.initial/.expand once={\envbody},
		}%
		\stmt@appendToPgfglobalkeyList{\define@label}{/statements/list of defined statements}
		%[Definition of statement \define@label done]
		\Debug@Out@Stmt[@Define]{\Statement@outStats{#3}}
	}	
	
	%{%
		%\endStatementsBodyEnv%   % stops collecting environment body and stores it into pgfkeys
%		\def\statement@end{\qed}
%		\pgfglobalkeysifdefined{/statements/config/#1/qed}{%
%			\pgfglobalkeys{/statements/config/#1/qed/.get=\statement@end}
%		}{}
%		\statement@end
		%
		%\gdef\Statements@currentStatementLabel{}%		
	%}%


\gdef\Statements@currentStatementLabel{}
\DeclareDocumentEnvironment{Statement}{m s O{} m}
	% #1: type (e.g., theorem, definition)
	% #2: star (don't show proof now)
	% [#3]: title
	% #4: label
	{%
		\Statement@Define{#1}{#3}{#4}
		%\def\stmt@title{#3}
		%\IfNoValueT{#3}{\edef\stmt@title{}}
		%\Statement@Define{#1}{\stmt@title}{#4}
	}%
	{%
		\endStatement@Define
		\Statement@Show{#2}{#4}
	}
	
	



\DeclareDocumentCommand{\Statement@Show}{m m}
	% #1: boolean (no proof now)
	% #2: label
	{
		\edef\show@label{#2}
		%
		\edef\show@showProof{1}
		%
		\IfBooleanTF{#1}{
			\edef\show@showProof{0}			
		}%
		\par			
		\pgfglobalkeys{%
			/statements/config/ShowAlwaysProofs/.get=\show@always@proofs
		}%
		\ifthenelse{\show@always@proofs > 0}{%
			\edef\show@showProof{1}%
		}{}%
		\par
		\Debug@Out@Stmt[@Show(\show@label)]{Showing proof? [\show@showProof]}%
		%
		%
		%
		\pgfglobalkeys{%
			/statements/\show@label/type/.get=\show@type,
			/statements/\show@label/title/.get=\show@title,
			/statements/\show@label/body/nbshown/.get=\show@body@nbshown,
			/statements/\show@label/body/.get=\show@body
		}%		
		\Debug@Out@Stmt[@Show(\show@label)]{@type is [\show@type]}
		%
		\Debug@Out@Stmt[@Show(\show@label)]{backing-up counters:}%
		%\Debug@Out@Stmt[@Show(\show@label)]{  - stmt counter: \csuse{the\show@type}}%		
		\edef\show@current@counter{\csuse{the\show@type}} % <--------------------------------------------{\csuse{the\show@type}}
		%\Debug@Out@Stmt[@Show(\show@label)]{  - eq counter: \theequation}}%
		\edef\show@current@eqcounter{\theequation}%{\theequation}  %% <<----------------------------------------------
		%
		%
		\Debug@Out@Stmt[@Show(\show@label)]{counters backed-up}%
		%
		%
		\ifthenelse{\show@body@nbshown = 0}{%
			% first time that body stmt is shown
			\Debug@Out@Stmt[@Show(\show@label)]{show@body@nbshown = \show@body@nbshown\space (zero):  
				this is the first time the body of this stmt is shown}
			%
			\pgfglobalkeys{/statements/\show@label/counter/.initial/.expanded=\show@current@counter}
			\Debug@Out@Stmt[@Show(\show@label)]{stmt/counter set to [\show@current@counter]}
			%
			\pgfglobalkeys{/statements/\show@label/body/eqcounter/.initial/.expanded=\show@current@eqcounter}
		
			\Debug@Out@Stmt[@Show(\show@label)]{body/eqcounter set to [\show@current@eqcounter]}
			%
			% [running outStats(\show@label)]
			\Debug@Out@Stmt[@Show(\show@label)]{\Statement@outStats{\show@label}}
		}{%
			\Debug@Out@Stmt[@Show(\show@label)]{retrieving stmt counter values}
			% repeated stmt
			%			
			% retrieve stmt counter and eq counter values
			\pgfglobalkeys{%
				/statements/\show@label/counter/.get=\show@counter,
				/statements/\show@label/body/eqcounter/.get=\show@eqcounter
			}
			%[@Show(\show@label): @nbshown@body = \show@body@nbshown]
			\Debug@Out@Stmt[@Show(\show@label)]{show@body@nbshown = \show@body@nbshown\space (non-zero): 
				the body of this stmt has already been shown: \Statement@outStats(\show@label)
			}
			%
			\Debug@Out@Stmt[@Show(\show@label)]{@type is [\show@type]}
			%
			\setcounter{\show@type}{\show@counter}
			\Debug@Out@Stmt[@Show(\show@label)]{Stmt counter set to [\csname the\show@type\endcsname]}
			%
			% temporarily set equation counter
			\setcounter{equation}{\show@eqcounter}
			\Debug@Out@Stmt[@Show(\show@label)]{Equation counter set to [\show@eqcounter]}
			%
			\gdef\stmt@at@end@body{%
				% restore global eqcounter
				\setcounter{equation}{\show@current@eqcounter}
				\Debug@Out@Stmt[@Show(\show@label)]{body terminated, 
					setting theequation to global value [\theequation]}
			}			
		}%
		%
		%
		%		
		%
		\ifthenelse{\equal{\show@title}{}}{%
			\begin{\show@type}%
		}{%
			\begin{\show@type}[\show@title]%
		}%
		\ifthenelse{\show@body@nbshown = 0}{%
			\label{\show@label}
		}{}%
		%
		%				
		\def\LabelWithin##1{\Statement@LabelWithin{\show@body@nbshown}{##1}}		
		\def\EqrefWithin##1{\Statement@EqrefWithin{\show@body@nbshown}{##1}}				
		\def\RefWithin##1{\Statement@RefWithin{\show@body@nbshown}{##1}}		
		%
		%
		%
		\def\proof{\Statements@ShowProof{\show@label}{\show@showProof}}
		\def\endproof{\endStatements@ShowProof}		
		%	
		\show@body%
		%
		% show QED, if defined
		%
		\xdef\show@qed{}%
		\pgfglobalkeysifdefined{/statements/config/\show@type/qed}{%
			\pgfglobalkeys{/statements/config/\show@type/qed/.get=\@qed}%
			\xdef\show@qed{\@qed}%
		}{}%
		\show@qed%
		%
		\gdef\stmt@at@end@body{\relax}
		%		
		%
		\end{\show@type}%
		%
		\Debug@Out@Stmt[@Show(\show@label)]{stmt terminated}
		%
		\ifthenelse{\show@body@nbshown > 0}{%
			% repeated stmt: set counter and eqcounter back to old values
			\Debug@Out@Stmt[@Show(\show@label)]{show@body@nbshown = \show@body@nbshown (non-zero): 
				resetting old counter and old eq counter}
			\setcounter{\show@type}{\show@current@counter}
			\Debug@Out@Stmt[@Show(\show@label)]{counter [\show@type] set to [\show@current@counter]}
			%\setcounter{equation}{\show@current@eqcounter}
			%\Debug@Out@Stmt[@Show(\show@label)]{equation counter set to [\theequation]}
		}{}%
		%
		%Increment @nbshown@body
		\FPeval{\show@body@nbshown@new}{round(show@body@nbshown+1:0)}	%
		\pgfglobalkeys{%
			/statements/\show@label/body/nbshown/.expanded=\show@body@nbshown@new
		}%
		\Debug@Out@Stmt[@Show(\show@label)]{show@body@nbshown incremented to [\show@body@nbshown@new]}
		%
		%
		\def\LabelWithin##1{\relax}		
		\def\EqrefWithin##1{\relax}				
		\def\RefWithin##1{\relax}		
		%
		% [@Show(\show@label) all done]
		\Debug@Out@Stmt{\Statement@outStats{\show@label}}
	}		


\DeclareDocumentCommand{\Statement@LabelWithin}{m m}{%
	% #1: nbshown
	% #2 label
	\ifthenelse{#1 = 0}{%
		\label{#2}%[#2]%
	}{%
		\label{::stmt:#1:#2}%[::stmt:#1:#2]%
	}%
}

\DeclareDocumentCommand{\Statement@EqrefWithin}{m m}{%
	% #1: nbshown 
	% #2 label
	\ifthenelse{#1 = 0}{%
		\eqref{#2}%[#2]%
	}{%
		\eqref{::stmt:#1:#2}%[::stmt:#1:#2]%
	}%
}

\DeclareDocumentCommand{\Statement@RefWithin}{m m}{%
	% #1: nbshown
	% #2 label
	\ifthenelse{#1 = 0}{%
		\ref{#2}%[#2]%
	}{%
		\ref{::stmt:#1:#2}%[::stmt:#1:#2]%
	}%
}


		
%%% PUBLIC API


\newcommand{\StmtAlwaysShowProofs}{
	\pgfglobalkeys{/statements/config/ShowAlwaysProofs=1}%
}



\DeclareDocumentCommand{\StmtShow}{s m}{%
	\Statement@Show{#1}{#2}%
}


\DeclareDocumentCommand{\StmtSetQED}{m m}{%
	% #1: type (e.g., theorem, definition
	% #2: latex code, e.g., \qed
	\pgfglobalkeysifdefined{/statements/config/#1/qed}{%
		\pgfglobalkeys{/statements/config/#1/qed=#2}%
	}{%
		\pgfglobalkeys{/statements/config/#1/qed/.initial=#2}%
	}
}


\DeclareDocumentCommand{\StmtShowFullStatements}{s o}{%
	% #1: star: all statements (also those whose proof has already been shown
	% #2: [type]: (no value = all types)
	%
	\pgfglobalkeys{/statements/list of defined statements/.get=\stmt@all}%
	%
	\foreach \show@stmt in \stmt@all {
		\pgfglobalkeys{%
			/statements/\show@stmt/type/.get=\show@full@type,
			/statements/\show@stmt/proof/nbshown/.get=\show@full@proof@nbshown
		}%
		\Debug@Out@Stmt[@ShowFull]{Deciding whether stmt [\show@stmt] should be shown: 
			type=[\show@full@type], @proof@nbshown=[\show@full@proof@nbshown]}%
		\def\@show@full@showThis{1}%
		%		
		\IfValueT{#2}{% a type has been given
			\Debug@Out@Stmt[@ShowFull]{User wants only stmts of type [#2]}%
			\ifthenelse{\equal{#2}{\show@full@type}}{}{% 
				% not of the right type
				\Debug@Out@Stmt[@ShowFull]{Not of the right type}%
				\def\@show@full@showThis{0}% 
			}%
		}%
		%	
		\IfBooleanT{#1}{%
			% star given
			\Debug@Out@Stmt[@ShowFull]{User wants only stmts whose proof has never been shown}
			\ifthenelse{\show@full@proof@nbshown > 0}{%
				% already shown
				\Debug@Out@Stmt[@ShowFull]{Stmt proof has already been shown}
				\def\@show@full@showThis{0}% 
			}%
		}%		
		\par	
		\Debug@Out@Stmt[@ShowFull]{Final decision taken: will stmt [\show@stmt] be shown? [\@show@full@showThis]}%
		\ifthenelse{\@show@full@showThis > 0}{%
			\par
			\StmtShow{\show@stmt}%
		}%
	}%
}





	


==> MCLabPaper_Table_2.tex <==
% Tables

\MCLabPaper@Set@Tutorial@Section{Table}{sec:table}

\DeclareDocumentCommand{\Debug@Out@Table}{o m}{%
	\Debug@Out{Table}[#1]{#2}%
}


\MCLabPaper@RequirePackage{longtable}
\MCLabPaper@RequirePackage{array}
\MCLabPaper@RequirePackage{multirow}
\MCLabPaper@RequirePackage{colortbl}
\MCLabPaper@RequirePackage{tabu}%larx}

%\newcolumntype{Y}{>{\raggedright}X}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}} % A tabular column-type to HIDE a column
\newcolumntype{C}{>{\centering\arraybackslash}p} % A tabular column-type to CENTER a paragraph content
\newcolumntype{L}{>{\raggedright\arraybackslash}p} % A tabular column-type to LEFT-ALIGN a paragraph content
\newcolumntype{R}{>{\raggedleft\arraybackslash}p} % A tabular column-type to RIGHT-ALIGN a paragraph content

%\newcolumntype{M}{>{\centering\arraybackslash}m} % CENTER-H/MIDDLE-V aligned paragraph

%\arrayrulewidth=0pt % no vertical lines by default


%%% DEFINING NEW STYLES

\def\Table@Data@Prefix{MCLabPaper/Table}
\undef\Table@Current@Table@Style%

\colorlet{TableFG}{black}
\colorlet{TableBG}{white}

\newcommand{\Table@Apply@Mandatory@Styles}{%
	\RuleNewStyle{norule}[0pt]% 
	\RuleNewStyle{top}[1pt]%
	\RuleNewStyle{middle}[0.5pt]%
	\RuleNewStyle{bottom}[1pt]%
	\RuleNewStyle{section}[0.5pt]%
	\RuleNewStyle{left}[0pt]%
	\RuleNewStyle{right}[0pt]%
}

\DeclareDocumentCommand{\TableNewStyle}{m +m}{% #1:name, #2: code	
	% Defines style function
	\long\csdef{TableStyle@#1}{%
		% Code run when style is applied
		\edef\Table@Current@Table@Style{#1}%
		\Debug@Out@Table[TableNewStyle]{Current table style is now: [\Table@Current@Table@Style]}%		
		%
		%
		% Defines always defined styles
		\Debug@Out@Table[TableNewStyle]{Applying mandatory styles}%
		\Table@Apply@Mandatory@Styles%
		%
		\Debug@Out@Table[TableNewStyle]{done}%
		% User style definition, can override the above
		\Debug@Out@Table[TableNewStyle]{Applying user styles}%
		#2%
		\Debug@Out@Table[TableNewStyle]{done. End.}%
	}% 
}

% Auxiliary commands enabled only within table
\DeclareDocumentCommand{\RuleNewStyle}{m O{}}{%
	\DiagError{Table}{Command \DiagLatexCmd{TableRuleNewStyle} can not be placed here.}%
}
\DeclareDocumentCommand{\Table@Rule@New@Style}{m O{\arrayrulewidth}}{%
	%   #1: rule style name
	% [#2]: rule style spec in the form: 'thickness other specs'
	% rule style spec are according to \newtabulinestyle 
	%			syntax (color, dash type etc.)
	\StrExtractFirstWord{\Table@Rule@New@Style@thickness}{#2}%
	\Debug@Out@Table[@Rule@New@Style]{Defining rule style '#1', spec='#2' (thickness='\Table@Rule@New@Style@thickness')}%
	\expandafter\let\csname tablestyle@\Table@Current@Table@Style @rule@style@thickness@#1\endcsname\relax%
	\expandafter\newlength
		\csname tablestyle@\Table@Current@Table@Style @rule@style@thickness@#1\endcsname%
	\expandafter\setlength
		\csname tablestyle@\Table@Current@Table@Style @rule@style@thickness@#1\endcsname{\Table@Rule@New@Style@thickness}%
	\newtabulinestyle{#1=#2}%
	\Debug@Out@Table[@Rule@New@Style]{Rule style '#1' definition done.}%
}

% Set Table default specs (colors, font, linesep)
\def\Table@Style@Default@EmptyCell{}%

\define@cmdkey{TableDefaults}{emptycell}[]{%
	\def\Table@Style@Default@EmptyCell{#1}%
}
\define@cmdkey{TableDefaults}{text}[\relax]{}
\define@cmdkey{TableDefaults}{rule}[norule]{%
	\def\Table@Style@Default@Rule@Style{#1}%
}
\define@cmdkey{TableDefaults}{bgcolor}[\relax]{}
\define@cmdkey{TableDefaults}{rulecolor}[\relax]{}
\define@cmdkey{TableDefaults}{linesep}[\relax]{}
\define@cmdkey{TableDefaults}{colsep}[\relax]{}

\def\Table@Style@Default@Cell@Style{}%
\define@cmdkey{TableDefaults}{cellstyle}[]{%
	\def\Table@Style@Default@Cell@Style{#1}%
}
\define@cmdkey{TableDefaults}{rulewidth}[0pt]{%
	\arrayrulewidth=#1%
}

\DeclareDocumentCommand{\SetDefaults}{m}{%
	\DiagError{Table}{Command \DiagLatexCmd{TableSetDefaults} can not be placed here.}%
}
\DeclareDocumentCommand{\Table@Set@Defaults}{m}{%
	% #1: specs
	\setkeys{TableDefaults}{text, bgcolor, cellstyle, rule, rulecolor, linesep, rulewidth, colsep}%color, 
	\@expandtwoargs\setkeys{TableDefaults}{#1}%
	%
	\Debug@Out@Table[SetDefaults]{Applying defaults for table style '\Table@Current@Table@Style'}%
	% Apply bgcolor
	\ifequals{\cmdKV@TableDefaults@bgcolor}{\relax}{}{%
		\colorlet{TableBG}{\cmdKV@TableDefaults@bgcolor}%
		\rowcolors{1}{TableBG}{TableBG}% Apply default bgcolor
	}%
	%
	% Apply rulecolor
	\ifequals{\cmdKV@TableDefaults@rulecolor}{\relax}{%
		% if not given, default to (text) color
		\def\cmdKV@TableDefaults@rulecolor{TableFG}%\cmdKV@TableDefaults@color%
	}{}%
	\taburulecolor{\cmdKV@TableDefaults@rulecolor}%
	%
	% Apply linesep
	\ifequals{\cmdKV@TableDefaults@linesep}{\relax}{}{%
		\tabulinesep=\cmdKV@TableDefaults@linesep%
	}%
	% Apply colsep
	\ifequals{\cmdKV@TableDefaults@colsep}{\relax}{}{%
		\tabcolsep=\cmdKV@TableDefaults@colsep%
	}%	
	% Apply text options
	\cmdKV@TableDefaults@text% 
	% 'text' a sequence of latex commands, 
	% e.g., \itseries\color{blue}: just run them.
}

\define@cmdkey{TableCellNewStyle}{text}[]{}
\define@cmdkey{TableCellNewStyle}{vsep}[0pt]{}
\define@cmdkey{TableCellNewStyle}{bgcolor}[TableBG]{}
\define@boolkey{TableCellNewStyle}{allowpagebreaks}[true]{}
\define@cmdkey{TableCellNewStyle}{emptycell}[\Table@Style@Default@EmptyCell]{}

\DeclareDocumentCommand{\CellNewStyle}{m O{}}{%
	\DiagError{Table}{Command \DiagLatexCmd{TableCellNewStyle} can not be placed here.}%
}
\DeclareDocumentCommand{\Table@Cell@New@Style}{m O{}}{%
	% #1: cell style name
	% [#2]: cell specification
	\setkeys{TableCellNewStyle}{text, emptycell, vsep, bgcolor, allowpagebreaks}%
	%\@expandtwoargs # no, as #2 can contain commands like text={\bfseries}
	\setkeys{TableCellNewStyle}{#2}%
	%
	%
	% % Defines style data entry
	\pgfglobalkeys{\Table@Data@Prefix/styles/\Table@Current@Table@Style/cells/#1/.cd,
		iexist/.initial = {},
		%align/.initial/.expand once = \Table@Cell@New@Style@align,
		%color/.initial/.expand once = \cmdKV@TableCellNewStyle@color,
		bgcolor/.initial/.expand once = \cmdKV@TableCellNewStyle@bgcolor,
		text/.initial/.expand once = {\cmdKV@TableCellNewStyle@text},
		emptycell/.initial/.expand once = \cmdKV@TableCellNewStyle@emptycell,
		vsep/.initial/.expand once = \cmdKV@TableCellNewStyle@vsep,
		allowpagebreaks/.initial/.expanded = 
			\ifKV@TableCellNewStyle@allowpagebreaks 1\else 0\fi%
	}%
}	



%% Applies cell style #1 to current cell
\DeclareExpandableDocumentCommand{\Cell}{+O{} +D(){} +m}{%
	\DiagError{Table}{Command \DiagLatexCmd{TableCell} can not be placed here.}%
}

\define@choicekey*{Table@Cell}{allowpagebreaks}%
	[\kw@Table@Cell@allow@page@breaks]{,true,false}[]{}
\DeclareExpandableDocumentCommand{\Table@Cell}{+O{\Table@Style@Default@Cell@Style} +D(){} +m}{%
	%  #1:  style name, can be {}
	%  (#2): options
	%  #3:  content
	%
	\@expandtwoargs\setkeys{Table@Cell}{allowpagebreaks, #2}%
	\def\Table@Cell@allowpagebreaks{1}%	
	\ifequals{#1}{}{%
		% No style given, setting defaults that need to be set on 
		% a per-cell basis
		\let\Table@Cell@emptycell\Table@Style@Default@EmptyCell%
	}{%
		\pgfglobalkeysifdefined{\Table@Data@Prefix/styles/\Table@Current@Table@Style/cells/#1/iexist}{%		
			\pgfglobalkeys{\Table@Data@Prefix/styles/\Table@Current@Table@Style/cells/#1/.cd,
				bgcolor/.get = \Table@Cell@bgcolor,
				text/.get = \Table@Cell@text,
				emptycell/.get = \Table@Cell@emptycell,
				vsep/.get = \Table@Cell@vsep,
				allowpagebreaks/.get = \Table@Cell@allowpagebreaks% 1 or 0
			}%
		}{%
			\DiagError{Table@Cell}{Cell style '#1' undefined}%
		}%
	 	%
	 	% Apply vsep - NOT YET IMPLEMENTED
		%\rule{0pt}{\Table@Cell@vsep}%
		%	
		%
		% Apply bgcolor
	 	\cellcolor{\Table@Cell@bgcolor}%
	 	% 
	 	%
	 	% Apply text properties
	 	\Table@Cell@text%	 	
	}% end style name non-empty
	%
 	% Typeout content 	
 	\ifequals{#3}{}{\Table@Cell@emptycell}{#3}%
 	%
 	%
 	% Handle allowpagebreaks:
 	% 1) Override style option if requested by user
 	\ifequals{\kw@Table@Cell@allow@page@breaks}{}{}{%
 		\ifequals{\kw@Table@Cell@allow@page@breaks}{true}{%
 			\def\Table@Cell@allowpagebreaks{1}%
 		}{%
 			\def\Table@Cell@allowpagebreaks{0}%
 		}%
 	}%
 	% 2) Set option
 	\Table@Remember@AllowPageBreaks{\Table@Cell@allowpagebreaks}%	
}

\DeclareExpandableDocumentCommand{\MultiCell}{+m +m +m +O{} +m}{%
	\DiagError{Table}{Command \DiagLatexCmd{TableMultiCell} can not be placed here.}%
}
\DeclareExpandableDocumentCommand{\Table@Multi@Cell}{+m +m +m +O{} +m}{%
	%  #1: number of rows
	%  #2: number of columns
	%  #3: column spec
	%  [#4]:  style name
	%  #5:  content
	%
	% SOMETIMES \multirow has problems!!! *******************
	%
	% Why do I need to write the *unrolled* code below?!
	\ifnumcomp{#2}{=}{1}{% one column
		\ifnumcomp{#1}{=}{1}{% one row
			% user wants new colspec
			\multicolumn{1}{#3}{\Table@Cell[#4]{#5}}%
		}{% multiple rows
			\multirow{#1}{=}{\Table@Cell[#4]{#5}}%
		}%
	}{% multiple columns
		\ifnumcomp{#1}{=}{1}{% one row
			\multicolumn{#2}{#3}{\Table@Cell[#4]{#5}}%
		}{% multiple rows
			\multicolumn{#2}%
			{#3}%
			{\multirow{#1}{*}{\Table@Cell[#4]{#5}}}%
		}%
	}%
}

%% Set style to use
\DeclareDocumentCommand{\Table@Set@Style}{m}{% #1: style name
	%	
	\ifequals{#1}{}{%
		\let\Table@Set@Style@style\Table@default@Style%
	}{%
		\def\Table@Set@Style@style{#1}%
	}%
	\ifcsdef{TableStyle@\Table@Set@Style@style}{%		
		\Debug@Out@Table[@Set@Style]{Applying table style '\Table@Set@Style@style'}%
		\csuse{TableStyle@\Table@Set@Style@style}%
	}{%
		\DiagError{Table}{TableStyle '\Table@Set@Style@style' unknown}%
	}%
}



% Handle setting of default table style for the whole document
\edef\Table@default@Style{default}%
\DeclareDocumentCommand{\TableSetDefaultStyle}{m}{% #1:style name
	\edef\Table@default@Style{#1}%
}


% Default implementation of default table style
\TableNewStyle{default}{%
	\SetDefaults{%
		linesep=3pt, 
		rule=norule,
		cellstyle = {default}
	}%
	\CellNewStyle{default}	
	\CellNewStyle{header}[
    	text={\centering\bfseries}, 
	    allowpagebreaks=false
  	]
  	\CellNewStyle{footer}[
    	text={\centering\bfseries}, 
	    allowpagebreaks=false
  	]
}




%% DRAWING TABLES

\gdef\Table@No@Break@Line@Code{\noalign{\nobreak}}%
\gdef\Table@Break@Line@Code{}%

\DeclareExpandableDocumentCommand{\Table@Reset@AllowPageBreaks}{}{%
	\gdef\Table@Curr@Line@Break@Line@Code{\Table@Break@Line@Code}%
}%


\DeclareExpandableDocumentCommand{\Table@Remember@AllowPageBreaks}{m}{%
	% #1: 1 (true) or 0 (false)
	\ifnum#1=0%
		\gdef\Table@Curr@Line@Break@Line@Code{\Table@No@Break@Line@Code}%
	\fi%
}

\DeclareDocumentCommand{\Rule}{D(){-} m}{%
	\DiagError{Table}{Command \DiagLatexCmd{Rule} can not be placed here.}%
}
\DeclareExpandableDocumentCommand{\Table@Rule}{D(){-} m}{%
	\tabucline[#2]{#1}%
}
\DeclareDocumentCommand{\NewLine}{s D(){-} O{}}{%	
	\DiagError{Table}{Command \DiagLatexCmd{NewLine} can not be placed here.}%
}
\DeclareDocumentCommand{\Table@NewLine}{s D(){-} O{\Table@Style@Default@Rule@Style}}{%
	% #1: [start] --> no page break
	% (#2): columns
	% [#3]: rule style
	%	
	\tabularnewline%
	\Table@Curr@Line@Break@Line@Code%
	%
	\if-#2\else\noalign{\vskip-\csname tablestyle@\Table@Current@Table@Style @rule@style@thickness@#3\endcsname}\fi%
	\Table@Rule(#2){#3}% (columns){style}
	\Table@Curr@Line@Break@Line@Code%
	%
	% Reset knowledge about allowing page breaks
	\noalign{\Table@Reset@AllowPageBreaks}%	
}%

% \mdfdefinestyle{Table@MDFrameStyle@Perfect@Fit}{%
% 	leftmargin=0pt,
% 	skipabove=0pt,
% 	rightmargin=0pt,
% 	skipbelow=0pt,
% 	innerleftmargin=0pt,
% 	innertopmargin=0pt,
% 	innerrightmargin=0pt,
% 	innerbottommargin=0pt,
% 	roundcorner=0pt,
% 	hidealllines
% }

\DeclareDocumentEnvironment{Tabu}{t+ O{}}{%	
	%	
	\begingroup%		
		% Enable interpretation of commands in \TableNewStyle
		\let\RuleNewStyle\Table@Rule@New@Style%
		\let\SetDefaults\Table@Set@Defaults%
		\let\CellNewStyle\Table@Cell@New@Style%
		%
		\let\Cell\Table@Cell%
		\let\MultiCell\Table@Multi@Cell%
		%
		\let\NewLine\Table@NewLine%
		\let\Rule\Table@Rule%	
		\let\PhantomLine\tabuphantomline%	
	% 	% End
	\Table@Set@Style{#2}%	
	\Table@Reset@AllowPageBreaks%	
	%
	\IfBooleanTF{#1}{%		
		\begin{longtabu}%
	}{%
		\begin{tabu}%
	}%
}{%
	\PhantomLine%
	\IfBooleanTF{#1}{\end{longtabu}}{\end{tabu}}%
	\endgroup%
}



==> MCLabPaper_TagCloud_2.tex <==
\MCLabPaper@RequirePackage{anyfontsize}

\MCLabPaper@Set@Tutorial@Section{TagCloud}{sec:tagcloud}

\DeclareDocumentCommand{\Debug@Out@TagCloud}{o m}{%
	\Debug@Out{TagCloud}[#1]{#2}%
}


\providetoggle{TagCloud@first}%
\define@cmdkey{TagCloud}{width}[\linewidth]{}
\define@cmdkey{TagCloud}{basefontsize}[8]{}
\define@cmdkey{TagCloud}{amplification}[1.5]{}
\DeclareDocumentCommand{\TagCloud}{O{} m}{% #1: optons #2: prefix
	\begingroup%	
	\setkeys{TagCloud}{width, basefontsize, amplification}%
	\@expandtwoargs\setkeys{TagCloud}{#1}%
	\def\TagCloud@field@prefix{#2}%
	\def\TagCloud@field@tag{tag}%
	\def\TagCloud@field@size{size}%
	\def\TagCloud@field@color{color}%
	\def\TagCloud@fontsize@min{\cmdKV@TagCloud@basefontsize}%
	\def\TagCloud@fontsize@aplification{\cmdKV@TagCloud@amplification}%
	\DataChildren[\TagCloud@tags]{\TagCloud@field@prefix/\TagCloud@field@tag}%
	\settoggle{TagCloud@first}{true}%
	\begin{minipage}{\cmdKV@TagCloud@width}\centering%
	\xintFor ##1 in \TagCloud@tags \do{%		
		\DataGet[\TagCloud@tag]<\TagCloud@field@prefix/\TagCloud@field@tag/##1>{\TagCloud@field@tag}%
		\DataGet[\TagCloud@size]<\TagCloud@field@prefix/\TagCloud@field@tag/##1>{\TagCloud@field@size}%
		\DataGet[\TagCloud@color]<\TagCloud@field@prefix/\TagCloud@field@tag/##1>{\TagCloud@field@color}%
		\MathEval[\TagCloud@fontsize]{%
			round(\TagCloud@fontsize@min + (\TagCloud@size*\TagCloud@fontsize@aplification) : 2)}%
		\MathEval[\TagCloud@skip]{round(\TagCloud@fontsize * 1.2 : 2)}%		
		\fontsize{\TagCloud@fontsize}{\TagCloud@skip}\selectfont%
			\iftoggle{TagCloud@first}{%	
				\settoggle{TagCloud@first}{false}%
			}{\space}%
			\textcolor{\TagCloud@color}{\TagCloud@tag}%
		% 		
	}%
	\end{minipage}
	\endgroup%
}

==> MCLabPaper_Time_2.tex <==

\let\MathSecondsToHMS\TimeSecondsToHMS
\DeclareDocumentCommand{\TimeSecondsToHMS}{o m}{%	
	%RETURNS #2 seconds converted to H:M:S
	\def\@value{#2}%
	%\typeout{MathSecondsToHMS(\@value)}%
	\xdef\@sign{}%
	\FPifneg{\@value}%
		\xdef\@sign{-}%
		%\typeout{argument is negative}
		\FPeval{\@value}{0-\@value}%
		%\typeout{MathSecondsToHMS: value < 0. Now \@value}
	\fi%
	\FPeval{@hours}{\@value / (60*60)}%
	\FPtrunc{\@hours}{\@hours}{0}%
	\FPeval{@rest}{\@value - (\@hours*60*60)}%
	\FPeval{@minutes}{\@rest/60}%	
	\FPtrunc{\@minutes}{\@minutes}{0}%	
	\FPeval{@seconds}{\@rest - (\@minutes*60)}%	
	\FPtrunc{\@seconds}{\@seconds}{0}%		
	\edef\TimeSecondsToHMS@result{\@sign\@hours:\@minutes:\@seconds}%	
	\IfValueTF{#1}{%
		\xdef#1{\TimeSecondsToHMS@result}
	}{%
		\TimeSecondsToHMS@result\xspace%
	}%	
}	


\DeclareDocumentCommand{\TimeSecondsToHMSProse}{o m}{%
	\def\@value{#2}%
	\FPeval{@hours}{\@value / (60*60)}%
	\FPtrunc{\@hours}{\@hours}{0}%
	%\typeout{\@value -> hours (trunc): [\@hours]}%	
	\FPeval{@rest}{\@value - (\@hours*60*60)}%
	%\typeout{\@value -> rest: [\@rest]}%		
	\FPeval{@minutes}{\@rest/60}%
	\FPtrunc{\@minutes}{\@minutes}{0}%	
	%\typeout{\@value -> minutes (trunc): [\@minutes]}%	
	\FPeval{@seconds}{\@rest - (\@minutes*60)}%	
	\FPtrunc{\@seconds}{\@seconds}{0}%		
	%\typeout{\@value -> seconds (trunc): [\@seconds]}%		
	%
	\edef\TimeSecondsToHMSProse@result{}%
	%
	\ifthenelse{\@hours = 0}{}{%
		\ifthenelse{\@hours > 1}{\def\@plural{s}}{\def\@plural{}}%
		\edef\TimeSecondsToHMSProse@result{\@hours\space hour\@plural}%
	}%
	\ifthenelse{\@minutes = 0}{}{%
		\ifthenelse{\equal{%
			\TimeSecondsToHMSProse@result}{}%
		}{}{\edef\TimeSecondsToHMSProse@result{\TimeSecondsToHMSProse@result, }}%
		\ifthenelse{\@minutes > 1}{\def\@plural{s}}{\def\@plural{}}%
		\edef\TimeSecondsToHMSProse@result%
			{\TimeSecondsToHMSProse@result\@minutes\space minute\@plural}%
	}%
	\ifthenelse{\@seconds = 0}{}{%	
		\ifthenelse{\equal{%
			\TimeSecondsToHMSProse@result}{}%
		}{}{%
			\edef\TimeSecondsToHMSProse@result{\TimeSecondsToHMSProse@result\space and }%
		}%
		%
		\ifthenelse{\@seconds > 1}{\def\@plural{s}}{\def\@plural{}}%
		\edef\TimeSecondsToHMSProse@result%
			{\TimeSecondsToHMSProse@result\@seconds\space second\@plural}%
	}%
	\IfValueTF{#1}{%
		\xdef#1{\TimeSecondsToHMSProse@result}%
	}{%
		\TimeSecondsToHMSProse@result\xspace%
	}%
}



==> MCLabPaper_Url_2.tex <==

\MCLabPaper@Set@Tutorial@Section{Url}{sec:url}

%\PassOptionsToPackage{hyphens}{url}
\MCLabPaper@RequirePackage[unicode, destlabel=true, pdfpagelabels]{hyperref}
\MCLabPaper@RequirePackage{bookmark}

\providecolor{MidnightBlue}{rgb}{0.1, 0.1, 0.44}
\colorlet{LinksColor}{MidnightBlue}

\hypersetup{
	colorlinks=true,
	allcolors=LinksColor,
	breaklinks=true,
	pageanchor=true,
	%
	%backref=true,
}

\urlstyle{same}

\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
      \do\-\do\/\do\.\do\#}
     

\DeclareDocumentCommand{\RenderUrl}{+m}{%
  %\begingroup%
  %	\catcode`_=12%
  %	#1%
  %\endgroup%
  \expandafter\detokenize\expandafter{#1}%
}


\newcommand{\UrlEmail}[1]{\href{mailto:#1}{\RenderUrl{#1}}}
\newcommand{\UrlHttp}[1]{\href{http://#1}{\RenderUrl{#1}}}

%\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
%      \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
%      \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
%      \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
%      \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
%      \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
%      \do\Y\do\Z}



==> MCLabPaper_Util_2.tex <==
\PackageInfo{MCLabPaper}{Loading Util.tex}%

\MCLabPaper@Set@Tutorial@Section{Util}{sec:util}

\newcommand{\def@macro}[2]{% #1=\macro, #2=value
	\long\expandafter\def\csname\expandafter\@gobble\string#1\endcsname{#2}%
}
\newcommand{\gdef@macro}[2]{% #1=\macro, #2=value
	\long\expandafter\gdef\csname\expandafter\@gobble\string#1\endcsname{#2}%
}

\newcommand{\edef@macro}[2]{% #1=\macro, #2=value
	\long\expandafter\edef\csname\expandafter\@gobble\string#1\endcsname{#2}%
}
\newcommand{\xdef@macro}[2]{% #1=\macro, #2=value
	\long\expandafter\xdef\csname\expandafter\@gobble\string#1\endcsname{#2}%
}

\DeclareDocumentCommand{\UtilGlobalDefinitions}{+m}{%
	% #1: latex code to be executed as if outside any group (i.e., global)
	\begingroup%
		\ifnum\the\globaldefs>0\relax%
		\else%
			\globaldefs=1%
		\fi%
		#1%
	\endgroup%
}


%% Allows PDF rendering of filenames with special chars (i.e., '_')
\DeclareDocumentCommand{\RenderFileName}{+m}{%
  %\begingroup%
  %	\catcode`_=12%
  %	#1%
  %\endgroup%
  \expandafter\detokenize\expandafter{#1}%
}

%% Allows PDF rendering of labels with special chars (i.e., '_')
\DeclareDocumentCommand{\RenderLabel}{+m}{%
  %\begingroup%
  %	\catcode`_=12%
  %	#1%
  %\endgroup%
  \expandafter\detokenize\expandafter{#1}%
}


\DeclareDocumentCommand{\RenderLatex}{+m}{%
  \expandafter\detokenize\expandafter{#1}%
}

\DeclareDocumentCommand{\IfStringEmptyTF}{+m +m +m}{%
	\ifthenelse{\equal{\detokenize{#1}}{}}{%
		#2%
	}{%
		#3%
	}%
}

\DeclareDocumentCommand{\ifequals}{+m +m +m +m}{%
	% #1 expr1
	% #2 expr2
	% #3 then body (expr1 == expr2)
	% #4 else body
	\ifthenelse{\equal{#1}{#2}}{#3}{#4}%
}


\DeclareDocumentCommand{\StrRemoveEndSlash}{o m}{%
	\IfEndWith{#2}{/}{%
		\StrGobbleRight{#2}{1}[#1]%
	}{%
		\StrGobbleRight{#2}{0}[#1]%
	}%
}

\DeclareDocumentCommand{\StrRightTrim}{o m}{%
	\IfEndWith{#2}{ }{%
		\StrGobbleRight{#2}{1}[\StrRightTrim@tmp]%
		\StrRightTrim[#1]{\StrRightTrim@tmp}%
	}{%
		\StrGobbleRight{#2}{0}[#1]%
	}%
}
\DeclareDocumentCommand{\StrLeftTrim}{o m}{%
	\IfBeginWith{#2}{ }{%
		\StrGobbleLeft{#2}{1}[\StrLeftTrim@tmp]%
		\StrLeftTrim[#1]{\StrLeftTrim@tmp}%
	}{%
		\StrGobbleLeft{#2}{0}[#1]%
	}%
}
\DeclareDocumentCommand{\StrTrim}{o m}{%
	\StrLeftTrim[#1]{#2}%
	\StrRightTrim[#1]{#1}%	
}

\newtoggle{InPreamble}
\settoggle{InPreamble}{true}
\AtBeginDocument{\settoggle{InPreamble}{false}}
\DeclareDocumentCommand{\IfPreambleTF}{+m +m}{%
	\iftoggle{InPreamble}{#1}{#2}%
}

\DeclareDocumentCommand{\StrExtractFirstWord}{m m}{%
	% #1: output macro
	% #2: string
 	\StrLeftTrim[#1]{#2}%
 	\StrBefore{#1}{ }[#1]%
 	\ifequals{#1}{}{\edef#1{#2}}{}%
}
\newcommand{\IntToBool}[1]{\ifnum#1=0 false\else true\fi}%

\DeclareDocumentCommand{\StrRemoveSpacesFromCommaSepList}{m m}{%
	% #1: output macro (containg "value1,value2,...")
	% #2: string: "value1, value2, ...."
	\edef\Str@rem@spaces@from@csl{}%
	\xintFor ##9 in {#2} \do{%
		\ifequals{\Str@rem@spaces@from@csl}{}{%
			% first item
			\edef\Str@rem@spaces@from@csl{##9}%
		}{%
			\edef\Str@rem@spaces@from@csl{\Str@rem@spaces@from@csl,##9}%
		}%
	}%
	\edef@macro{#1}{\Str@rem@spaces@from@csl}%
}


% \newcommand{\IgnoreSpacesAndAllPars}{%
%   \begingroup
%   \catcode13=10
%   \@ifnextchar\par
%     {\endgroup\expandafter\IgnoreSpacesAndAllPars\@gobble}%
%     {\endgroup}%
% }

% \newcommand{\IgnoreSpacesAndImplicitePars}{%
%   \begingroup
%   \catcode13=10
%   \@ifnextchar\relax
%     {\endgroup}%
%     {\endgroup}%
% }



\newcommand{\IgnoreFollowingSpacesAndPars}{%
	\ifhmode\unskip\fi%
		\aftergroup\Use@Ignore@Spaces@And@All@Pars%
}

\def\Use@Ignore@Spaces@And@All@Pars#1\ignorespaces\fi{%
#1\fi\Ignore@Spaces@And@All@Pars}

\def\Ignore@Spaces@And@All@Pars{%
  \@ifnextchar\par
    {\expandafter\Ignore@Spaces@And@All@Pars\@gobble}%
    {}%
}



\newcommand{\Util@Pad@To@Digits}[3]{%
 	% #1: result
 	% #2: integer
 	% #3: final length of padded result
 	%\edef@macro{#1}{#2}%
 	\StrLen{#2}[\IANSPTD@len]%
 	\MathEval[\IANSPTD@start]{trunc(\IANSPTD@len+1 :0)}%
 	\edef\IANSPTD@prefix{}%
 	\xintFor* ##1 in {\xintSeq[1]{\IANSPTD@start}{#3}} \do{
 		\edef\IANSPTD@prefix{\IANSPTD@prefix 0}%
 	}%
 	\edef@macro{#1}{\IANSPTD@prefix #2}%
}

\PackageInfo{MCLabPaper}{Loading Util.tex done}%

==> abs.tex <==
% !TEX root =  root.tex
%
By using small computing devices deployed at user premises,
\Ac{ADR} adapts users electricity consumption
to given time-dependent electricity tariffs.
This allows end-users to save on their electricity bill and
\Aclp{DSO} to optimise (through suitable time-dependent tariffs) management of the electric grid by avoiding
\emph{demand peaks}.

Unfortunately, even with \Ac{ADR}, users power consumption may deviate from
the expected (minimum cost) one, \eg because \Ac{ADR} devices fail to correctly forecast energy needs at user premises.
As a result, the \emph{aggregated power demand} may present undesirable peaks.

In this paper we address such a problem by presenting methods and a software tool (\Acs{PPSV})
implementing them,
enabling \Aclp{DSO} to effectively verify that a given time-dependent electricity tariff achieves
the desired goals even when end-users deviate from their expected behaviour.

We show feasibility of the proposed approach through a realistic scenario from a medium voltage Danish distribution network.  


==> ack.tex <==
%!TEX root = ./root.tex
\paragraph*{Acknowledgements}
This work was partially supported by the following research projects/grants: 
%
Italian Ministry of University \& Research (MIUR) grant ``Dipartimenti di Eccellenza 2018--2022'' (Dept.\ Computer Science, Sapienza Univ.\ of Rome); 
EC FP7 project SmartHG (Energy Demand Aware Open Services for Smart Grid Intelligent Automation, 317761);
INdAM ``GNCS Project 2018''.


==> acronyms.tex <==
%!TEX root = ./root.tex
% Acronyms in alphabetical order

\NewAcronym{AA}{Approximation Algorithm}

\NewAcronym{ADR}{Autonomous Demand Response}
\NewAcronym{APD}{Aggregated Power Demand}

\NewAcronym{CPP}{Collaborative Power Profile}

\NewAcronym{DAPP}{Demand-Aware Price Policy}
\NewAcronym{DER}{Distributed Energy Resources}
\NewAcronym{DNO}{Distribution Network Operator}
\NewAcronym{DLC}{Direct Load Control}
\NewAcronym{DR}{Demand Response}
\NewAcronym{DSM}{Demand Side Management}
\NewAcronym{DSO}{Distribution System Operator}
\NewAcronym{DSS}{Decision Support System}[expand=always]


\NewAcronym{EDN}{Electric Distribution Network}
\NewAcronym{EPP}{Expected Power Profile}
\NewAcronym{EVT}{EDN Virtual Tomography}

\NewAcronym{HPC}{High Performance Computing}
\NewAcronym{HEC}{Home Energy Controller} % Better name?!

\NewAcronym{IBR}{Inclining Block Rate}[expand=always]
\NewAcronym{iid}{independent and identically distributed}
\NewAcronym{IaaS}{Infrastructure as a Service}

\NewAcronym{KPI}{Key Performance Indicator}

\NewAcronym{LP}{Linear Programming}

\NewAcronym{MC2}{Monte Carlo Model Checking}
\NewAcronym{MILP}{Mixed Integer Linear Programming}
\NewAcronym{MPI}{Message Passing Interface}

\NewAcronym{PEV}{Plug-in Electric Vehicle}[expand=always]
\NewAcronym{PPSV}[APD-Analyser]{Aggregated Power Demand Analyser} % find a better name!!

\NewAcronym{PV}{Photovoltaic}[expand=always]

\NewAcronym{SRA}{Stopping Rule Algorithm}

\NewAcronym{UDP}{Usage-based Dynamic Pricing}


==> conclusion.tex <==
% !TEX root =  root.tex

In this paper we presented \Ac{PPSV}, a \Ac{HPC}-based software system aimed at supporting \Acp{DSO} in analysing the possible aggregated effects, on an \Ac{EDN} substation, of new envisioned, possibly highly-fluctuating and individualised price policies for electricity end-users. 
%
\Ac{PPSV} uses information about \Ac{DSO}-expected user behaviours under the new policies as well as probabilistic models of user deviations from such expected behaviours, thus acting both as a \emph{\Ac{DSS}} (as it allows \emph{what-if analyses}) and as an \emph{automated verifier} for the \emph{safety} of an envisioned set of price policies.
In particular, \Ac{PPSV} enables safety assessment of the price policies computed through automated methods as part of highly dynamic \Ac{ADR} schemas.

Feasibility and scalability of the system have been assessed by using realistic scenarios taken from an existing medium voltage Danish distribution network.  


\endinput

In this paper we presented \Ac{PPSV}, a decision support system a novel parallel algorithm, along with its distributed multi-core implementation, to compute the probability distribution of the \Ac{APD} on a substation line in an \Ac{EDN}.
The algorithm takes as input the predicted power profiles of all users (as envisioned by the \Ac{DSO}, according to historical data and the price policies offered to the users) and a probabilistic model of user deviations \wrt their predicted power profiles.

Our algorithm combines two different statistical model checking techniques in order to compute an estimation of the \Ac{APD} with arbitrary precision.
This allows stakeholders (e.g., \Acp{DSO}) to check if the probability of violating the substation safety is kept sufficiently low. 



%% In this paper we presented a novel %hierarchical
%% service-based methodology to improve \Ac{EDN} management. Namely, with our approach, all actors involved obtain a gain: residential end users are able to lower down their energy bills, while the energy retailer and the \Ac{DSO} are able to sell as much energy as possible while avoiding \Ac{EDN} overloading (thus preserving \Ac{EDN} safety). Our approach is based on three integrated services: 
%% \begin{inparaenum}[(i)]
%%   \item \Ac{EVT} monitors the whole \Ac{EDN} and detect overloaded subnetworks;
%%   \item given an \Ac{EDN} substation $s$, \Ac{DAPP} proposes {\em individualized price policies} (based on {\em individualized power profiles}) to all end users connected to the substation$s$, so that desired operational constraints on $s$ are met if each user follows the proposed power profile;
%%   \item \Ac{PPSV} proves that operational constraints on substations are met with high probability also when users are allowed to (reasonably) deviate from their proposed power profile.
%% \end{inparaenum}

%% We showed the feasibility of our approach on a medium voltage \Ac{EDN} in a Danish village. %Kalundborg (Denmark). % managed by Danish \Ac{DSO} SEAS-NVE.
%% Namely, in the reference scenario, \Ac{EVT} was able to suggest to \Ac{DSO} operational constraints on each substation in order to improve \Ac{EDN} usage (by avoiding overloads). By focusing on the most critical of such substations $s$, we showed that \Ac{DAPP} was able to motivate user to move their loads in order to (unknowingly) meet the operational constraints on $s$.
%% %% In fact, all end users have a minimum 27\% gain
%% %% in accepting the \Ac{DAPP} individualized price policy, without even trying to follow the proposed power profile.
%% %% This shows that such proposed power profile is easy to follow for users. Furthermore, the
%% %% collaborative user as an average gain on the energy bill of at least 46\% in
%% %% the reference scenario. This shows that our approach enables money saving.
%% Finally, \Ac{PPSV} showed that operational constraints on $s$ in the reference scenario are met even if end users deviate from the proposed power profile for the 60\% of the time.

%% As future work we plan to further improve our services, by refining
%% methods for dealing with bad %noisy???
%% data and missing measurements in the input data (\Ac{EVT}), by investigating price policies that explicitly take into account users energy storage capabilities (\Ac{DAPP}) and by devising parallel verification approaches (\Ac{PPSV}).




==> content.tex <==
%!TEX root = root.tex
\maketitle

\begin{abstract}
	\Input{abs.tex}
\end{abstract}	

\AcronymResetAll

\SectionInput[sec:introduction]{Introduction}{10_introduction/content.tex}

\SectionInput[sec:system]{\Acl{PPSV}}{20_system/content.tex}

%\SectionInput[sec:preliminaries]{Preliminaries}{40_preliminaries/content.tex}
\SectionInput[sec:edApproximation]{Random variable mean \EDApproximation}{30_approximation/content.tex}

\SectionInput[sec:computing]{Monte Carlo--based computation of \Acs{APD} probability \EDApproximation{s}}{40_computing/content.tex}

\SectionInput[sec:parallel]{A parallel algorithm for \Acs{PPSV}}{50_algo/content.tex}

\SectionInput[sec:expres]{Experimental results}{60_expres/content.tex}

\SectionInput[sec:relwork]{Related work}{related_work.tex}

\SectionInput[sec:conclusions]{Conclusions}{conclusion.tex}

\Input{ack.tex}


\Bibliography[style=IEEEtran,verbosity=XS]
%\DraftWarning{Enable Bibliography in content.tex after having added at least one entry in bib DB}

%\newpage
%\AcronymList

%\appendix

%\SectionInput[sec:appendix]{Appendix}{99_appendix/content.tex}

%\SectionInput[sec:ppsv]{\Acl{PPSV}}{ppsv/content.tex}

%\SectionInput[sec:background]{Background}{90_background/content.tex}

%\SectionInput[sec:algo]{OLD: A Parallel Algorithm for \Acs{PPSV}}{30_algo/_old/conf_content.tex}


==> mclab_acronyms.tex <==
\NewAcronym{BMC}[BMC]{Bounded \Acl{MC}}
\NewAcronym{CPS}{Cyber-Physical System}
\NewAcronym{CT}{Continuous Time}[shortplural=CT,longplural=Continuous Time]

\NewAcronym{DFS}{Depth-First Search}
\NewAcronym{DS}{Dynamical System}

\NewAcronym{HILS}{Hardware In the Loop Simulation}

\NewAcronym{IP}{Intellectual Property}

\NewAcronym{MC}{Model Checking}

\NewAcronym{SLFV}{System Level Formal Verification}
\NewAcronym{SMC}[SMC]{Statistical \Acl{MC}}
\NewAcronym{SUV}{System Under Verification}

\NewAcronym{VPH}{Virtual Physiological Human}


==> preamble.tex <==
% !TEX root =  root.tex

\title{
%A Parallel Approach to Formal Verification of Demand Aware Price Policies
Parallel Statistical Model Checking for Safety Verification in Smart Grids%
% \thanks{This paper appears as:
% T. Mancini, F. Mari, I. Melatti, I. Salvo, E. Tronci, J.K. Gruber, B. Hayes, M. Prodanovic, L. Elmegaard.
% \emph{Parallel Statistical Model Checking for Safety Verification in Smart Grids}.
% In proceedings of the 2018 IEEE International Conference on Smart Grid Communications (SmartGridComm 2018). Aalborg, Denmark. 
% Lecture Notes in Computer Science, vol. 11177. IEEE, 2018.
% DOI: 10.1109/SmartGridComm.2018.8587416}
}

\author{%
	\IEEEauthorblockN{%
		Toni Mancini, 
		Federico Mari, 
		Igor Melatti,\\ 
		Ivano Salvo, 
		and Enrico Tronci
	}
	\IEEEauthorblockA{%
		Computer Science Department,\\
		Sapienza University of Rome, Italy %\\ 
%		Roma, Italy
	}
    \and
    \IEEEauthorblockN{%
    	Jorn Klaas Gruber, 
		Barry Hayes,\\
		and Milan Prodanovic}
    \IEEEauthorblockA{Instituto IMDEA Energ\'ia, Spain}
    \and
    \IEEEauthorblockN{Lars Elmegaard}
    \IEEEauthorblockA{SEAS-NVE, Denmark}
}
%% %Email: \texttt{\{tronci,melatti,mari,mancini,salvo\}@di.uniroma1.it}}
%% \and
%% \IEEEauthorblockN{Jorn Klaas Gruber, Barry Hayes,\\and Milan Prodanovic}
%% \IEEEauthorblockA{Instituto IMDEA Energ\'ia, Spain}
%% \and
%% \IEEEauthorblockN{Lars Elmegaard}
%% \IEEEauthorblockA{SEAS-NVE, Denmark
%% %\\Madrid, Spain
%% }
%% %Email: \texttt{\{milan.prodanovic,jorn.gruber\}@imdea.org}}
%% }  %  author


%%% TO BE REMOVED
% \newcommand{\estPrAPD}{\ensuremath{{\tilde{Pr}}}}
% \newcommand{\PrAPD}{\ensuremath{{{Pr}}}}
% \newcommand{\dist}{\ensuremath{\Fun{dist}}}

\let\url\texttt

\AcronymResetAllAtEach{chapter}

\newcommand{\User}{\ensuremath{u}}
\newcommand{\SetUsers}{\ensuremath{\mathcal{U}}}

\newcommand{\TimeSlot}{\ensuremath{t}}
\newcommand{\SetTimeSlots}{\ensuremath{\mathcal{T}}}

\newcommand{\DomainDeviations}[1]{\ensuremath{D_{#1}}}
\newcommand{\Deviation}{\ensuremath{d}}
\newcommand{\DeviationModel}[1]{\ensuremath{\Fun{dev}_{#1}}}

\newcommand{\PowerProfile}{\ensuremath{p}}
\newcommand{\APD}{\PowerProfile}

\newcommand{\EPP}[1]{\ensuremath{\PowerProfile_{#1}}}

\newcommand{\SetKPIs}{\ensuremath{\mathcal{K}}}
\newcommand{\KPI}{\ensuremath{k}}

\newcommand{\Tolerance}{\ensuremath{\varepsilon}}
\newcommand{\Confidence}{\ensuremath{\delta}}
\newcommand{\DiscretisationStep}{\ensuremath{\gamma}}
\newcommand{\EDGApproximation}{($\Tolerance,\Confidence,\DiscretisationStep)$-approximation\xspace}

\newcommand{\EDApproximation}{$(\Tolerance,\Confidence)$-approximation\xspace}


\newcommand{\APDDistribution}{\ensuremath{\Psi}}
\newcommand{\APDDistributionDef}{\ensuremath{\Reals \to [0,1]}}
%\newcommand{\SetAPDDistributions}{\ensuremath{\mathcal{A}}}

\newcommand{\APDDistributionApprox}{\ensuremath{\tilde{\APDDistribution}}}
\newcommand{\SetPowerSlots}{\ensuremath{W}}

\newcommand{\PowerSlot}{\ensuremath{w}}%
\newcommand{\PowerValueMin}{\ensuremath{w_\text{min}}}%
\newcommand{\PowerValueMax}{\ensuremath{w_\text{max}}}%
\DeclareMathOperator*{\minmax}{\star}
\newcommand{\PowerValueMinmax}{\ensuremath{w_{\minmax{}}}}%


\newcommand{\SetPowerSlotsDef}{\ensuremath{%
	\left\{ 
		\left[ j\DiscretisationStep, (j+1)\DiscretisationStep \right)
		~\middle|~ j \in \Integers
	\right\}
}}
\newcommand{\APDDistributionApproxDef}{\ensuremath{\SetPowerSlots \to [0,1]}}


\newcommand{\Probability}[1]{\textup{Pr}\left[#1\right]}

\newcommand{\Substation}{\ensuremath{s}}%
\newcommand{\SubstationProfile}{\ensuremath{\PowerProfile_{\Substation}}}%



\newcommand{\NbSamplesPerCall}{\ensuremath{c}}%
\newcommand{\NbSamplesPerCallDef}{\ensuremath{2 \times 10^4}}
\newcommand{\NullHyp}[1]{\ensuremath{H_0^{#1}}}%


\newcommand{\NbWorkers}{\ensuremath{k}}%

\DeclareDocumentCommand{\DiracDeltaFunction}{d()}{%
	% #1: variable
	\ensuremath{%
		\delta%
		\IfValueT{#1}{\left(#1\right)}%
	}%
}%

\DataPut<exps>{workers/number = 80}
\DataPut<exps>{nodes/number = 81}


\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}

\Input{acronyms.tex}

\crefname{case}{case}{cases}


\PrettyDefineStyle{kw}{unit=kW, decimaldigits=0}
\PrettyDefineStyle{eur0}{unit=Eur, decimaldigits=0}


\endinput

% OLD STUFF, use only if strictly requested



%

%%%% START ALGORITHMS RELATED MACROS %%%%%%
\usepackage[noline,scleft,linesnumbered]{algorithm2e} %add 'noend' to make algos shorter
\SetInd{0.3em}{0.3em}
\def\algoType#1{\textbf{#1}}
\def\algoVar#1{\ensuremath{\fun{#1}}}
\def\algoFun#1{\ensuremath{\fun{#1}}}
\def\algoVarGets#1#2{\ensuremath{\algoVar{#1}\gets} #2}
\def\algoIncrVar#1{\ensuremath{\algoVar{#1}\text{++}}}
\def\algoDecrVar#1{\ensuremath{\algoVar{#1}\text{--}}}
\SetKw{KwFunction}{function}
\long\def\algoFunction#1#2{\noindent\KwFunction{#1}\EndNoBegin{#2}}
\SetKw{KwNew}{new}
\SetKw{KwNil}{nil}
\SetKw{KwBreak}{break}
\SetKw{KwOutput}{output}
\SetKw{KwField}{field}
\SetKw{KwGlobal}{Global:}
\SetKw{KwMethod}{method}
\SetKw{KwParam}{param}
\SetKw{KwAssert}{assert}
\SetKw{KwReturns}{returns}
\SetKw{KwEnd}{end}
\SetKwRepeat{DoWhile}{do}{while}
\SetKwBlock{BeginNoEnd}{begin}{}
\SetKwBlock{EndNoBegin}{}{end}
\SetKwBlock{NoBeginNoEnd}{}{}

\SetKw{KwSend}{send}
\SetKw{KwRecv}{recv}
\SetKw{KwWait}{wait}
%%%% END ALGORITHMS RELATED MACROS %%%%%%



\endinput


























































\usepackage{color}
\usepackage{balance}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{epsfig}
%\usepackage[hang]{subfigure}
\usepackage{subfig}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
%\usepackage[T1]{fontenc}
\usepackage{epic}
\usepackage{eepic}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{stmaryrd}
%\usepackage{amsthm}
\usepackage[all]{xy}
\usepackage{balance}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{multicol}
\usepackage{soul}
%\usepackage{hyperref}
%\usepackage[printonlyused,withpage]{acronym}
\usepackage[nolist]{acronym}
\usepackage{etex}
\usepackage{tikz}
%\usepackage{appendix}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{automata}
\usetikzlibrary{positioning}
\usepackage{paralist}

%smart frac
\usepackage{xfrac}
% \theoremstyle{plain}
%\newdef{definition}{Definition}
%\newdef{notation}{Notation}
%\newdef{example}{Example}
%\newdef{remark}{Remark}
%\newdef{fact}{Fact}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}

% \newtheorem{expfact}{Experimental Fact}{\bfseries}{\itshape}


% algorithmic
\algsetup{linenodelimiter=.} 
\algsetup{indent=3em}
\renewcommand{\algorithmicensure}{\textbf{function}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \numberwithin{algorithm}{chapter}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}


%\input{lstdefinitions.tex}
%\input{oldstuff/listings-def.tex}

% ntheorem stuff
% \theoremstyle{changebreak}
% \theoremsymbol{\ensuremath{\heartsuit}}
% \theoremindent0.5cm
% \theoremnumbering{greek}
% \newtheorem{Lemma}{Lemma}

% \theoremstyle{changebreak}
% \theoremsymbol{\ensuremath{\heartsuit}}
% \theoremindent0.5cm
% \theoremnumbering{greek}
% \newtheorem{lemma}{Lemma}

% \theoremstyle{changebreak}
% \theoremsymbol{\ensuremath{\heartsuit}}
% \theoremindent0.5cm
% \theoremnumbering{greek}
% \newtheorem{proposition}{Proposition}

% \theoremstyle{changebreak}
% \theoremsymbol{\ensuremath{\heartsuit}}
% \theoremindent0.5cm
% \theoremnumbering{greek}
% \newtheorem{Proposition}{Proposition}


% \theoremstyle{marginbreak}
% \theoremheaderfont{\normalfont\bfseries}\theorembodyfont{\slshape}
% \theoremsymbol{\ensuremath{\diamondsuit}}
% \theoremseparator{:}
% \newtheorem{Theorem}{Theorem}

% \theoremstyle{marginbreak}
% \theoremheaderfont{\normalfont\bfseries}\theorembodyfont{\slshape}
% \theoremsymbol{\ensuremath{\diamondsuit}}
% \theoremseparator{:}
% \newtheorem{theorem}{Theorem}


% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{Definition}{Definition}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{definition}{Definition}


% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{remark}{Remark}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{Remark}{Remark}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{notation}{Notation}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{Notation}{Notation}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{Example}{Example}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{example}{Example}


% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{Corollary}{Corollary}

% \theoremstyle{plain}
% \theoremsymbol{\ensuremath{\clubsuit}}
% \theoremseparator{.}
% \theoremprework{\bigskip\hrule}
% \theorempostwork{\hrule\bigskip}
% \newtheorem{corollary}{Corollary}


% \theoremheaderfont{\sc}\theorembodyfont{\upshape}
% \theoremstyle{nonumberplain}
% \theoremseparator{}
% \theoremsymbol{\rule{1ex}{1ex}}
% \newtheorem{Proof}{Proof}

% \theoremheaderfont{\sc}\theorembodyfont{\upshape}
% \theoremstyle{nonumberplain}
% \theoremseparator{}
% \theoremsymbol{\rule{1ex}{1ex}}
% \newtheorem{proof}{Proof}


\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}

\usepackage{listings}
\lstloadlanguages{C++,Pascal}

\lstset{
language=C++,
tabsize=1,
showlines=false,
emptylines=*1,
breaklines=true,
breakindent=20pt,
basicstyle=\ttfamily\small,
keywordstyle=[2]\itshape,
commentstyle=\itshape,
columns=fixed,
showspaces=false,
showstringspaces=false,
showtabs=false
}

\lstdefinelanguage{PseudoC}[ISO]{C++} { 
morekeywords={foreach, and, not, or, is, FIFO_Queue, HashTable, FILE, Cache}, 
%morekeywords=[2]{Enqueue, Dequeue, next, head_queue, tail_queue, swapin_file, swapout_file, head_queue_elements, tail_queue_elements, hash, init_states, swap_in, swap_out, collision_rate, ram_queue_size, Q_ck, Q_unck, deleted_in_cloud, deleted_not_in_cloud, GetDiskCloud, DiskCloud, beta, disk_cloud_size, speedup, slowdown, D, h, M, init_states, deleted_states,  something_not_in_cloud, Calibration_Required, QueryCalibration, Block}, 
morekeywords=[2]{HashInsert, Enqueue, Dequeue, next}, 
mathescape=true,
alsoletter={'},
deletestring=[b]'
}

\lstdefinelanguage{PseudoCWithNumbers}[ISO]{C++} { 
morekeywords={foreach, and, not, or, is, FIFO_Queue, HashTable, FILE, Cache}, 
%morekeywords=[2]{Enqueue, Dequeue, next, head_queue, tail_queue, swapin_file, swapout_file, head_queue_elements, tail_queue_elements, hash, init_states, swap_in, swap_out, collision_rate, ram_queue_size, Q_ck, Q_unck, deleted_in_cloud, deleted_not_in_cloud, GetDiskCloud, DiskCloud, beta, disk_cloud_size, speedup, slowdown, D, h, M, init_states, deleted_states,  something_not_in_cloud, Calibration_Required, QueryCalibration, Block}, 
morekeywords=[2]{HashInsert, Enqueue, Dequeue, next}, 
mathescape=true,
alsoletter={'},
deletestring=[b]'
}

\lstdefinelanguage{Murphi}[]{Pascal} { 
morekeywords={ruleset, rule, invariant, startstate, return, endif, endfor, endswitch, forall, endforall, exists, endexists}, 
mathescape=true, 
morestring=[b]",
morestring=[b]', 
morecomment=[s]{/*}{*/} ,
morecomment=[l]{--}
}

\lstdefinelanguage{PRISM}[ISO]{C++} { 
morekeywords={probabilistic, stochastic, const, rate, module, endmodule, init, P, U},
mathescape=true, 
alsoletter={'},
deletestring=[b]'
}

\lstdefinelanguage{Yacc}[ISO]{C++} { 
morekeywords={token, left}, 
mathescape=false,
alsoletter={'},
deletestring=[b]'
}

\lstdefinestyle{PseudoC}{
language=PseudoC,
basicstyle=\ttfamily,%\small, 
tabsize=1,
showlines=false,
emptylines=*1,
breaklines=true,
breakindent=5pt,
keywordstyle=\rmfamily\bfseries,%\normalsize, 
keywordstyle=[2]\rmfamily,%\normalsize, 
commentstyle=\itshape, 
columns=fixed,
showspaces=false, 
showstringspaces=false, 
showtabs=false, 
escapechar=\%
}

\lstdefinestyle{PseudoCWithNumbers}{
language=PseudoC,
basicstyle=\ttfamily,%\small, 
tabsize=1,
showlines=false,
emptylines=*1,
breaklines=true,
breakindent=5pt,
keywordstyle=\rmfamily\bfseries,%\normalsize, 
keywordstyle=[2]\rmfamily,%\normalsize, 
commentstyle=\itshape, 
columns=fixed,
showspaces=false, 
showstringspaces=false, 
showtabs=false, 
escapechar=\%,
numbersep=5pt,framexleftmargin=15pt,numbers=left,
}

\lstdefinestyle{Murphi}{
language=Murphi,
basicstyle=\ttfamily,%\small, 
tabsize=1,
showlines=false,
emptylines=*1,
breaklines=true,
breakindent=5pt,
keywordstyle=\rmfamily\bfseries,%\normalsize, 
commentstyle=\itshape, 
columns=fixed,
showspaces=false, 
showstringspaces=false, 
showtabs=false,
escapechar=\%}

\lstdefinestyle{PRISM}{
language=PRISM,
basicstyle=\ttfamily,%\small, 
tabsize=1,
showlines=false,
emptylines=*1,
breaklines=true,
breakindent=5pt,
keywordstyle=\rmfamily\bfseries,%\normalsize, 
commentstyle=\itshape, 
columns=fixed,
showspaces=false, 
showstringspaces=false, 
showtabs=false,
escapechar=\%}

\lstdefinestyle{Yacc}{
language=PseudoC,
basicstyle=\ttfamily,%\small, 
tabsize=1,
showlines=false,
emptylines=*1,
breaklines=true,
breakindent=5pt,
keywordstyle=\rmfamily\bfseries,%\normalsize, 
keywordstyle=[2]\rmfamily,%\normalsize, 
commentstyle=\itshape, 
columns=fixed,
showspaces=false, 
showstringspaces=false, 
showtabs=false, 
}

% \newcommand{\complref}[1]{\ref{#1} of page \pageref{#1}}
% \newcommand{\eqref}[1]{(\ref{#1})}
% \renewcommand{\arraystretch}{1.2}

\newcommand{\mybold}[1]{\mbox{\boldmath$#1$}}
\newcommand{\myboldsub}[1]{\mbox{\scriptsize\boldmath$#1$}}

\newcommand{\qks}{\mbox{\sl QKS}}
%\newcommand{\qksinc}{\mbox{QKS}$^\mbox{\sc inc}$}
\newcommand{\qksinc}{\mbox{\sl QKS}$^{\,\sf otf}$}

\newcommand{\coda}[2]{#1\!\!\mid^{#2}}
\newcommand{\pref}[2]{#1\!\!\mid_{#2}}

\definecolor{Blue}{rgb}{0.25,0.33,0.77}
\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0,1,0}
\newcommand{\Blue}[1]{{\color{Blue}{#1}}}
\newcommand{\Red}[1]{{\color{Red}{#1}}}
\newcommand{\Green}[1]{{\color{Green}{#1}}}


\newcommand{\sem}[1]{\mbox{ $[\![\! #1 \!]\!]$}}
\newcommand{\qerelax}[1]{{\mbox{\mbox{\rm Relax}$(#1)$}}}


\newcommand{\overaqe}[1]{\mbox{$\mbox{\rm AQE}^{+}( #1 )$}}
\newcommand{\underaqe}[1]{\mbox{$\mbox{\rm AQE}^{-}( #1 )$}}
\newcommand{\overaprx}[1]{\mbox{$\mbox{\rm APX}^{+}( #1 )$}}
\newcommand{\underaprx}[1]{\mbox{$\mbox{\rm AQE}^{-}( #1 )$}}

%\newcommand{\overaqe}[1]{\mbox{ $\Xi^{+}( #1 )$ }}
%\newcommand{\underaqe}[1]{\mbox{ $\Xi^{-}( #1 )$ }}
%\newcommand{\overaprx}[1]{\mbox{ $\Upsilon^{+}( #1 )$ }}
%\newcommand{\underaprx}[1]{\mbox{ $\Upsilon^{-}( #1 )$ }}

\newcommand{\varseq}[1]{\mybold{#1}}
%\newcommand{\varseq}[1]{\mbox{${\bf #1}$}}
\newcommand{\dths}[1]{\mbox{${\cal #1}$}}
\newcommand{\domain}[1]{\mbox{${{\cal D}_{#1}}$}}
\newcommand{\adm}[1]{\mbox{$\mbox{\rm Adm}(#1)$}}
\newcommand{\dom}[1]{\mbox{$\mbox{\rm Dom}(#1)$}}

\newcommand{\evalform}[3]{\mbox{ $[\![\!\; #1 \;\!]\!]_{#2}^{#3}$}}

\newcommand{\fun}[1]{{\sl #1}}
%\renewcommand{\baselinestretch}{0.963}
\newcommand{\Rpos}{\R^{\geq 0}}



%\newtheorem{case}{Case}
%\newtheorem{subcase}{Case}
%\numberwithin{subcase}{case}


==> related_work.tex <==
% !TEX root =  root.tex

% To be cited:
%
%SYLVER
% * mancini-etal:2013:cav
% * mancini-etal:2017:ipl
% * mancini-etal:2016:micpro
% * mancini-etal:2014:dsd-anytime
% * mancini-etal:2015:sylvaas-pdp
% * (mancini-etal:2014:pdp)  // non fondamentale, ma se riesci non fa male.
%
%SMART GRID
% * hayes-etal:2016:tsg
% * mancini-etal:2014:smartgridcomm
% * mancini-etal:2015:dsd
%
%BIO
% * mancini-etal:2015:iwbbio
% * mancini-etal:2014:fmcad


%Missing: mari-etal:2014:tosem, mari-etal:2012:ictac, alimguzhin-etal:2012:emsoft, alimguzhin-etal:2012:cdc, alimguzhin-etal:2013:onthefly, alimguzhin-etal:2013:mapreduce, mari-etal:2010:cav

\Comment{%%%%%%
The closest paper to our work is~\cite{mancini-etal:2014:smartgridcomm}, where the input and output of \Ac{PPSV} is presented and a preliminary \emph{sequential} algorithm for it is briefly sketched. 
%
With respect to~\cite{mancini-etal:2014:smartgridcomm}, here we present a novel \emph{parallel} algorithm for \Ac{PPSV} together with a \emph{new} distributed multi-core implementation for %(possibly heterogeneous) 
clusters of computers, which provides \Acp{DSO} a \emph{short response-time} way of checking for safety violations. 
%
% The parallel algorithm is not trivial to realise.
Our novel approach is not \emph{embarassingly parallel}, since
\begin{enumerate*}[(i)] 
\item aggregating slaves results is not straightforward (\cref{sec:algo}) and
\item choosing the size of samples for each slave that reduces communication and, at the same time, speeds-up computation is essential for the overall method \emph{efficiency} (\cref{sec:expres}).
\end{enumerate*}

To understand if the designed price policies avoid peaks
(in the context of smart grids predictive maintenance and 
vulnerability assessment), 
a \Ac{DSO} could perform \emph{worst-case scenario} analyses 
(\eg \cite{hayes-etal:2016:tsg,mancini-etal:2015:dsd}).
Unfortunately, such analyses are too skeptical and do not consider the average grid usage.
For these reasons, we focus on \emph{statistical} approaches.
}

\Comment{
The closest paper to our work is~\cite{mancini-etal:2014:smartgridcomm}, where the input and output of \Ac{PPSV} is presented and a sequential algorithm for it is briefly sketched. 
%
Namely, \cite{mancini-etal:2014:smartgridcomm}~introduces a novel methodology based on three integrated services to improve \Ac{EDN} management. 
%
The first service, \Ac{EVT}, computes safety thresholds for all substations in an \Ac{EDN}. 
%
The second service, \Ac{DAPP}, computes suitable price policies and collaborative power profiles for all users connected to a given substation. If all users follow their \Ac{DAPP}-computed collaborative profiles, the substation safety conditions are guaranteed to be met.
%
As, although incentivised by better tariffs, there is no guarantee that users will always behave according to their collaborative profiles, the third service, \Ac{PPSV}, provides \Acp{DSO} with means to determine the probability of safety violations on the substation power thresholds, by computing the \Acf{APD} probability distribution, given the users collaborative profiles (as synthesised by the \Ac{DSO}, e.g., using \Ac{DAPP}) and a probabilistic model of user deviations (\wrt their collaborative profiles) as input.

With respect to~\cite{mancini-etal:2014:smartgridcomm}, here we present a novel \emph{parallel} algorithm for \Ac{PPSV} together with a \emph{new} distributed multi-core implementation for (possibly heterogeneous) clusters of computers, which provides \Acp{DSO} a \emph{short response-time} way of checking for safety violations. 
%, so that it is optimised for the probability distribution computation. Moreover, we make such algorithm parallel, so as to exploit higher computational power of modern clusters of computer. Summing up, \Ac{pPPSV} allows a \Ac{DSO} to obtain more precise results (i.e., to use smaller values of $\delta, \epsilon$) in less time.
}

\Comment{%%%%%
Note that here price policies are an input and we are not interested in how they have been computed.
Computation of suitable price policies for users typically start from system level formal specifications.
Other works on synthesis from system level formal specifications
(focusing on synthesis of controllers for hybrid systems) are
in~\cite{mari-etal:2014:tosem,mari-etal:2012:ictac,alimguzhin-etal:2012:emsoft,alimguzhin-etal:2012:cdc,alimguzhin-etal:2013:onthefly,alimguzhin-etal:2013:mapreduce,mari-etal:2010:cav}.
}%%%%%%




\Comment{
A verification tool closely related to ours is {\sc PVeStA}~\cite{alturki-etal:2011:calco}. 
{\sc PVeStA} is a parallel tool for general-purpose statistical model checking, accepting in input any Markov Chain and any PCTL or CSL formula. 
Differently from {\sc PVeStA}, we do not compute an estimation of the probability of a formula, but an estimation (with arbitrarily high precision) of an entire probability distribution.
%is optimised so as to output a distribution probability, rather than the (single) probability of a formula.  %On the other hand, \Ac{PPSV} and \Ac{pPPSV} are more application-specific, and results to be be more efficient on the problem at hand (i.e., verification of).
%Other parallel tools in model-checking contexts
}

\Input{related_works_dapp.tex}

\Input{related_works_ppsv.tex}



==> related_works_dapp.tex <==
\Comment{
\ac{DSM}~\cite{vlot-etal:2013:tsg} approaches are used to regulate \acp{EDN} by acting, directly or indirectly, on end users.
There are two main approaches to \ac{DSM}, namely
\ac{DLC} and \ac{DR}.
With a \ac{DLC} %(see, e.g.,~\cite{douglass-etal:2013:tsg})
approach the utility (\ac{DSO}) remotely controls energy consumption
by curtailing high-load household appliances.
With a \ac{DR}  approach each user receives %(for example, from the \ac{DSO})
an energy price policy %(for example, hourly based)
for the next few days. 
Users will autonomously manage their loads (e.g., by reducing their consumption at peak hours)
and their generation (say, from \ac{PV} panels) so as to minimize their energy bill.
This, in turn, will optimize \ac{EDN} operations.
In this paper, we assume to be in a \ac{DR} approach, more in detail on
an \acp{IBR} price policy
(e.g., see~\cite{reiss-white:2005:res}).
%% Note that indeed \ac{DAPP} {\em synthesizes} price policies
%% starting from system level formal specifications.
%% Other works on synthesis from system level formal specifications
%% (focusing on synthesis of controllers for hybrid systems) are
%% in~\cite{mari-etal:2014:tosem,alimguzhin-etal:2013:onthefly,alimguzhin-etal:2013:mapreduce}.
%% As for price policies computation, many works are based on distributed algorithms and architectures (e.g., as in~\cite{wang-wang:2013:negotiation}). On the contrary, \ac{DAPP} is
%% based on a centralized algorithm which computes all required price policies. A centralized (Neural Network based) approach similar to the one in \ac{DAPP} is in~\cite{kunwar-etal:2013:tsg}.
%% Differently from~\cite{kunwar-etal:2013:tsg}, \ac{DAPP} assigns a {\em different} price policy to each user in the same area
%% (e.g., connected to the same substation),
%% considers the case where users are producing energy,
%% and
%% uses a \ac{LP}
%% based approach.
%% Finally, we point out that the mechanism used by \ac{DAPP} to encourage users to follow such a suggested 
%% behaviour is pricing, which is decided by the 
%% energy retailer based on
%% economical as well as social considerations, as described, e.g., 
%% in~\cite{thimmapuram-kim:2013:tsg}.
}


==> related_works_ppsv.tex <==
% !TEX root =  root.tex

In statistical model checking approaches (see, \eg \cite{zuliani-etal:2013:fmsd,
mancini-etal:2013:cav,mancini-etal:2017:ipl,mancini-etal:2016:micpro,mancini-etal:2014:dsd-anytime,%
mancini-etal:2016:fundam,%mancini-etal:2015:sylvaas-pdp,%
%mancini-etal:2014:pdp,
sebastio-etal:2013:multivesta,grosu-etal:2005:tacas,dagum-etal:2000:sicomp}), scenarios are sampled until a certain degree of confidence in the estimated probability is achieved. \Ac{PPSV} is based on such techniques, 
and employs a parallel version of
the algorithms in \cite{grosu-etal:2005:tacas,dagum-etal:2000:sicomp}, also adapting them
to the smart grid context.
%
There exist other works adapting statistical model checking techniques to smart grids, see, \eg~\cite{martins-etal:2011:icfem,mancini-etal:2014:smartgridcomm}, which however are based on sequential (non-parallel) algorithms.
%
In a smart grid context, usage of \emph{exhaustive} (instead of statistical) methods for safety analysis has been studied, \eg in~\cite{lemay-gunter:2012:tsg,garlapati-shukla:2012:spin,yuksel-etal:2012:tase}. 
%Namely, \cite{garlapati-shukla:2012:spin}~uses the UPPAAL model checker to formally verify a grid fault protection system. \cite{lemay-gunter:2012:tsg}~uses the model checker MAUDE to formally prove that a microprocessor based implementation of \textit{Cumulative Attestation Kernel} is tolerant to power supply interruptions. Finally, \cite{yuksel-etal:2012:tase}~uses a Markov chain based modelling approach and the PRISM model checker to analyse robustness to failures of a smart grid power transmission line.
All such works are plagued by the %so called 
\emph{state explosion} problem.
Since \Ac{PPSV} aims at evaluating safety of a large system (a substation connecting hundreds of end-users), 
exhaustive or non-massively-parallel approaches \emph{cannot} be used.
%An exhaustive simulation-based approach (applied on verification of satellite procedures) similar to the one used for the standalone \Ac{PPSV} has also been studied in~\cite{verzino-etal:2012:spaceops}.

%{\bf FROM HERE ON: LONG VERSION FROM DELIVERABLES, CURRENTLY UNDER REVIEW}

%% Correct-by-construction approaches to systems are also often based on formal verification techniques.
%% For example, \cite{hackenberg-etal:2012:se4sg} describes how is possible to adapt FOCUS, 
%% a system engineering method featuring formal specification of structure and behaviour as well as step-wise decomposition and refinement, 
%% to the smart grid context.
%% The authors propose the adaptation of existing formal, component-based methods, 
%% focusing on households and their involvement in low voltage nets as a case study.
%% Such an approach, presently, can only handle abstract model of networks where most 
%% electrical elements are abstracted away.

%% Formal verification approaches provide the highest degree of safety assurance one can get. 
%% However they are plagued by the so called \textit{state explosion} problem that limits their application,
%% in our context, to small systems (e,g,. like the controller in \cite{lemay-gunter:2012:tsg}) or to abstract models
%% of the system under verification (as in \cite{garlapati-shukla:2012:spin}, \cite{hackenberg-etal:2012:se4sg}).

%% PPSV, on the contrary, aims at evaluating safety of a large system 
%% using the full scale EDN model where all electrical components are adequately modelled. 
%% For this reason the approaches used in the above papers cannot be used in our context. 


%% \subsubsection{Statistical Methods}

%% Statistical methods aim at computing, with the desired confidence, the probability that a given scenario occurs.
%% In our context statistical methods can be used to show that the probability that an unsafe scenario occurs is, with high probability 
%% (high \textit{statistical confidence}),
%% below a given threshold. 

%% On one side, statistical methods do not suffer of the state explosion problem as formal verification methods,
%% on the other side they are not exhaustive, 
%% thus they cannot give that assurance provided by formal verification methods.
%% We note however that, by using a large number of samples (and thus of computation time),
%% we can make their degree of confidence as close to 1 as we like.

%SO' MICA TANTO SICURO CHE SIA VERO...
%% PPSV uses a statistical approach for its safety analysis.
%% From a methodological point of view the approach closest to PPSV is the one in \cite{grosu-etal:2004:isola} and in \cite{grosu-etal:2005:tacas}
%% where the authors present statistical model checking algorithms (based on the optimal approximation algorithm in \cite{dagum-etal:2000:sicomp})
%% to estimate, with a given degree of confidence, the probability
%% that the system under verification satisfies a given property (safety, liveness, etc).
%% We note however, that the approach in \cite{grosu-etal:2004:isola,grosu-etal:2005:tacas} only applies to finite state systems 
%% (i.e., systems whose state ranges on a finite set of values) 
%% whereas PPSV addresses dynamical systems (EDNs) with an infinite number of states.

%MESSI PIU' SU
%% The work in \cite{martins-etal:2011:icfem} applies to a smart grid context the general purpose
%% Bayesian statistical model checking techniques developed \cite{zuliani-etal:2013:fmsd}. 
%% We note however that the approach in \cite{martins-etal:2011:icfem} can only handle abstract (simplified) models
%% of an EDN whereas PPSV, resting on an EDN simulator, can handle a full scale EDN model.
%% The work in \cite{yuksel-etal:2012:tase} 
%% %Yuksel \textit{et al.} 
%% uses a Markov chain based modelling approach and
%% uses the PRISM model checker to analyse robustness to failures of a smart grid power transmission line.

%% To the best of our knowledge, no statistical safety verification approach has ever been developed to handle 
%% safety verification of user demand control policies using a full scale EDN model, like those that PPSV can handle.

%% \subsubsection{Average Case Analysis Methods}

Monte Carlo--based methods aiming at evaluating the average behaviour of the system under analysis
are widely used in \emph{performance evaluation} where, typically, the average case is the 
most interesting one. However such methods, used in a smart grid context for example in \cite{koutitas-tassiulas:2013:tsg,chang-etal:2013:tsg}, are not very well suited for safety analysis, since they cannot address rare (low probability) events and, most importantly, 
do not provide any lower bound for the statistical confidence achieved.

%% We note however that many works about user demand control policies focus indeed on performance evaluation,
%% rather than on safety verification, of the control policy, and, to that end,
%% rely on an average case analysis based on Monte Carlo method. 
%% Accordingly, for sake of completeness, we include Monte Carlo based methods in our comparison.

%% The work in \cite{koutitas-tassiulas:2013:tsg} 
%% presents control policies defining time shifts on periodic loads
%% in order to provide peak power and energy cost reduction over a
%% limited time horizon. Effectiveness of the proposed control policies is evaluated 
%% using a Monte Carlo based approach where 100 network topologies are generated at random
%% and smart devices in each smart building are generated by following a suitable stochastic model.

%% The work in \cite{chang-etal:2013:tsg} proposes control strategies to improve real-time power balancing with collaborative energy management.
%% %The approach is multi-stage stochastic optimisation problem with customers energy requests random in time. They propose a decentralised stochastic optimisation algorithm, CoHEM, that performs a local computation of scheduling solutions based on domestic user information and message exchange between neighbours. 
%% Effectiveness of the approach is showed by estimating the expected power load using the Monte Carlo method. 
%% %To this end, simulation on 100 randomly generated realizations are executed. Simulation results are averaged, and demonstrate that the proposed CoHEM architecture can  improve real-time power balancing. 

%% While average case analysis approaches aim at evaluating the average behaviour of the system,
%% PPSV, aiming at safety verification, estimates the distribution probability of (aggregated user demand) scenarios and also computes a 
%% statistical confidence for such a distribution. 

%% \subsubsection{Benchmark Based Methods}

Performance evaluation can also be done using suitable benchmarks. This is often quite interesting since it guarantees
that the system is evaluated on relevant case studies (see, \eg~\cite{lee-etal:2013:tsg,lee-hui:2013:tsg}). 
However, this approach cannot be used for safety verification, since it cannot provide an upper bound to the 
probability that a potentially unsafe scenario has not been considered in the analysis.

%% Many control policies in a smart grid context are evaluated using case studies. Accordingly,
%% for sake of completeness, we include benchmark based methods in our comparison.

%% In order to ensure that the load demand follows the power generation the work in \cite{lee-etal:2013:tsg} proposes control policies for electric springs aiming at solving the stability problems arising from the intermittent nature of renewable energy sources. Effectiveness of the approach is shown
%% with an experimental evaluation conducted considering different case studies. 

%% The work in \cite{lee-hui:2013:tsg} %Lee \textit{et al.} give the mathematical proof that the 
%% presents electric spring control strategies to reduce energy storage requirements in power grids. 
%% Effectiveness of the proposed approach is shown by taking measurements on a smart grid setup in laboratory.

%% The works in \cite{guo-etal:2013:tsg}, \cite{atzeni-etal:2013:tsg}, \cite{lou-etal:2013:tsg}, \cite{zhao-etal:2013:tsg}  propose
%% smart grid control policies and show their effectiveness by performing simulation on meaningful case studies.

%% Case study based approaches aim at evaluating performance of the system on scenarios that are known to be meaningful.
%% However, safety analysis has the goal of ruling out existence of an unsafe scenario. 
%% Accordingly, case study based approaches are not well suited for safety verification and are, of course, quite different,
%% from PPSV approach. On the other side we note that effectiveness of PPSV approach itself has been evaluated using a case study
%% (namely, the one from Kalundborg demonstration).





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% {\bf FROM HERE ON: LONG VERSION FROM DELIVERABLES}

%% In this section we compare PPSV approach to safety verification with state of the art approaches
%% to the safety analysis of control strategies in a smart grid context.

%% The DAPP service computes for each user (residential home) a price policy defining, 
%% for each time slot (say one hour) a low price power range and a high price power range.
%% This basically means that the DAPP service proposes, for each time slot, to each user a (low price) 
%% \textit{power profile} that the user is expected to follow

%% Such a power profile is computed by DAPP in so as to ensure that the aggregated demand,
%% in turn, follows a power profile provided by the DNO. 
%% Accordingly, as long as users follow the DAPP proposed power profile,
%% we are sure, by construction, that the aggregated demand will follow the power profile
%% proposed by the DNO thereby satisfying the DNO \textit{safety constraints}.

%% However, of course, users may occasionally deviate from the behaviour proposed by DAPP.
%% In such a case the DAPP design, a priori, does not guarantee safety 
%% (with respect to the DNO requirements) of the power profiles proposed by DAPP to the users.
%% %
%% PPSV goal is exactly to evaluate robustness of the DAPP proposed power profiles
%% with respect to users deviation.

%% The risk associated to an event is the product between the probability of the event and its cost.
%% Safety is concerned with high cost events. As a result, safety analysis needs to
%% consider also low probability events. 
%% For this reason safety assurance cannot be done by simply considering the average behaviour.
%% %In fact, by proposing a power profile to each user, 
%% %the DAPP service tend to coordinate the user behaviour.
%% %As a result, small probability scenarios (many users acting in a similar way at the same time)
%% %may become relevant.

%% Accordingly, PPSV objective is to compute the probability distribution of the 
%% aggregated power demand when each user follows the DAPP proposed profile
%% \textit{most} of the time, but not always.
%% %
%% This is done by using a \textit{statistical model checking} (e.g., see \cite{zuliani-etal:2013:fmsd})
%% approach, where scenarios are sampled until a certain degree of confidence in the estimated distribution is achieved.
%% In the following we compare such an approach with state of the art safety analysis techniques used in a smart grid context.


%% %The main goal of the safety verificaion in the PPSV service is to show robustness of such a power profile
%% %with respect to users deviating from it. We note that 

%% %utilization of smart grid requires to introduce information and communication support to the traditional power grid for monitoring and controlling purposes.
%% %The introduction of new requirements involves the adoption of methods for the verification of control policies or quantitative properties of the system.

%% %Examples of research objectives in the smart grid field are reduction of energy consumption, reduction of energy cost, real-time power balancing, peak power reduction, management of production by means of renewable energy sources, modulation of load demand according to power generation, robustness against failures of power transmission line.

%% %Our goal is to verify the power load on a power line determined by the control scheme on  the demand and offer of energy obtained by means of suitable price policies proposed to customers.
%% %To this end we compute the statistical distribution of the demand along with an upper bound to the probability that such an estimation is wrong- confidence interval. provide a distribution of probability 

%% \subsubsection{Exhaustive Methods}

%% Exhaustive methods (typically referred to as \textit{formal verification})
%% aim at showing absence of unsafe scenarios by using clever algorithms to simulate \textit{all} possible scenarios
%% (\textit{model checking based approaches}) or by
%% using a mathematical approach to prove that no unsafe scenario may ever occur (\textit{theorem proving based approaches}). 
%% Here are a few examples of application of formal verification techniques in a smart grid context.

%% %When the state space of the system under investigation is finite state, model checking may proceed in automatic fashion.
%% %If the system fail to satisfy the formula, a counter-example trace leading the user to the error state is produced.

%% %The model checking technique has been used with different goals in smart grid context in several papers \cite{garlapati-shukla:2012:spin, lemay-gunter:2012:tsg, yuksel-etal:2012:tase}.

%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% %% ADD CITATION TO UPPAAL
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The work in \cite{garlapati-shukla:2012:spin} uses the UPPAAL model checker to formally verify
%% a grid fault protection system having the goal of minimising the impact of a fault as well as the amount
%% of load shed due to the relay induced disconnection of lines. 
%% %Garlapati \textit{et al.} consider the case of protection system with the objective of isolating a fault as soon as possible to minimize the negative impact of the fault on the grid and to minimize the amount of load shed due to the relay induced disconnection of lines. 
%% %They use UPPAAL, a formal verification tool, to formally verify the protection scheme. 
%% %Namely, UPPAAL Timed Computation Tree Logic (TCTL) is used to specify system properties. The properties of the agent based relay supervision scheme that are verified are: Safety Property, Bounded Liveness Property, Model Correctness Properties.

%% Many smart grid devices are indeed \textit{safety critical} systems, it is then not surprising that
%% formal verification techniques have been used to verify such devices.
%% For example,
%% %The aim of LeMay \textit{et al.} 
%% \cite{lemay-gunter:2012:tsg} presents a
%% \textit{Cumulative Attestation Kernel} (CAK) to be used in 
%% \textit{Advanced Metering Infrastructures} (AMI). 
%% The authors use the model checker MAUDE to formally prove
%% that their microprocessor based implementation of CAK is
%% tolerant to power supply interruptions, 
%% a vital requirement for this kind of devices.

%% %is to mitigate the threat of malware intrusions on networked embedded systems by remote attestation assurances.
%% %They propose an architecture for providing remote attestation for advanced meters (Cumulative Remote Attestation of Embedded System Integrity CRAESI), and define the requirements for cumulative attestation kernels and coprocessors for flash microcontroller units to audit application firmware integrity. They provide the formal proof of security and fault-tolerance properties for CRAESI, and the formal proof of system tolerance to power supply interruptions Authors use Maude LTL model checker and realize a prototype.

%% Correct-by-construction approaches to systems are also often based on formal verification techniques.
%% For example, \cite{hackenberg-etal:2012:se4sg} describes how is possible to adapt FOCUS, 
%% a system engineering method featuring formal specification of structure and behaviour as well as step-wise decomposition and refinement, 
%% to the smart grid context.
%% The authors propose the adaptation of existing formal, component-based methods, 
%% focusing on households and their involvement in low voltage nets as a case study.
%% Such an approach, presently, can only handle abstract model of networks where most 
%% electrical elements are abstracted away.

%% %The method need to be further adapted to be able to deal with large system. 
%% %With respect to model analysis, models more precise than the only pyhsical model involve much more parameters with respect to those considered in the simulations. In fact authors provide simulation results for two simple scenarios.
%% %Futhermore, statistical models can be used to reduce modeling effort and increase behavioral coverage.

%% Formal verification approaches provide the highest degree of safety assurance one can get. 
%% However they are plagued by the so called \textit{state explosion} problem that limits their application,
%% in our context, to small systems (e,g,. like the controller in \cite{lemay-gunter:2012:tsg}) or to abstract models
%% of the system under verification (as in \cite{garlapati-shukla:2012:spin}, \cite{hackenberg-etal:2012:se4sg}).

%% PPSV, on the contrary, aims at evaluating safety of a large system 
%% using the full scale EDN model where all electrical components are adequately modelled. 
%% For this reason the approaches used in the above papers cannot be used in our context. 


%% \subsubsection{Statistical Methods}

%% %The model checking approach has been used to tackle the problem of deciding whether or not a property, specified
%% %in temporal logic, holds and it has been used for hardware, software and protocol verification. 
%% %Model checking has its drawbacks, among which the most awkward is the state explosion. This inconvenient can make model checking intractable for many applications of practical interest. Over the past two decades, several techniques have been developed to tackle the state explosion problem: symbolic model checking, partial-order reduction, symmetry reduction, bounded model checking, and statistical model checking.
%% %Previous work has shown that statistical model checking is an adeguate approach for the verification of probabilistic systems. 

%% Statistical methods aim at computing, with the desired confidence, the probability that a given scenario occurs.
%% In our context statistical methods can be used to show that the probability that an unsafe scenario occurs is, with high probability 
%% (high \textit{statistical confidence}),
%% below a given threshold. 

%% On one side, statistical methods do not suffer of the state explosion problem as formal verification methods,
%% on the other side they are not exhaustive, 
%% thus they cannot give that assurance provided by formal verification methods.
%% We note however that, by using a large number of samples (and thus of computation time),
%% we can make their degree of confidence as close to 1 as we like.

%% PPSV uses a statistical approach for its safety analysis.
%% From a methodological point of view the approach closest to PPSV is the one in \cite{grosu-etal:2004:isola} and in \cite{grosu-etal:2005:tacas}
%% where the authors present statistical model checking algorithms (based on the optimal approximation algorithm in \cite{dagum-etal:2000:sicomp})
%% to estimate, with a given degree of confidence, the probability
%% that the system under verification satisfies a given property (safety, liveness, etc).
%% We note however, that the approach in \cite{grosu-etal:2004:isola,grosu-etal:2005:tacas} only applies to finite state systems 
%% (i.e., systems whose state ranges on a finite set of values) 
%% whereas PPSV addresses dynamical systems (EDNs) with an infinite number of states.

%% %In our work we exploit the model checking approach decribed in \cite{grosu-etal:2004:isola} e in \cite{grosu-etal:2005:tacas}.
%% %In \cite{grosu-etal:2004:isola} Grosu \textit{et al.} describe their approach to coping with state explosion, typical in the model checking approach, based on the technique of Monte Carlo estimation. They propose the QMC Monte Carlo approximation algorithm for quantitative model-checking. The algorithm is randomized, and a Monte Carlo decision procedure for classical temporal-logic model checking is utilized. They need the computation of an ($\epsilon, \delta$)-approximation $\tilde{p_Z}$ of $p_Z$ ($p_Z$ probability that a Bernoulli random variable $Z$ that takes value 1; intuitively, $p_Z$ is the probability that a random walk in $B$, starting from an initial state and terminating at a cycle, is an accepting lasso, where $B = B_S \times B_{\varphi}$ is the language of the B\"{u}chi automaton) that can be done in a number of samples that is optimal to within a constant factor by appealing to the optimal approximation algorithm (OAA) of \cite{dagum-etal:2000:sicomp}.
%% I%n \cite{grosu-etal:2005:tacas} Grosu \textit{et al.} refine their approach to coping with state explosion based on the technique of random sampling by executing a random walk
%% %through the systems state transition graph. They propose MC2, a randomized Monte Carlo algorithm for temporal-logic model checking, but differently from  \cite{grosu-etal:2004:isola} use an approach based on the basic probability theory of Bernoulli and geometric random variables to derive a decision procedure for the LTL model-checking problem. With this method, the number of samples taken by MC2 is an order of magnitude smaller than that required by OAA.

%% The work in \cite{martins-etal:2011:icfem} applies to a smart grid context the general purpose
%% Bayesian statistical model checking techniques developed \cite{zuliani-etal:2013:fmsd}. 
%% We note however that the approach in \cite{martins-etal:2011:icfem} can only handle abstract (simplified) models
%% of an EDN whereas PPSV, resting on an EDN simulator, can handle a full scale EDN model.

%% %have been used for safety verification of distributed control policies

%% %Similar to our approach is the approach of Martins \textit{et al.} \cite{martins-etal:2011:icfem}. They propose a Distributed Probabilistic-Control Hybrid Automata as a model for hybrid systems with a dynamic number of probabilistic elements. They use Quantified Bounded Linear Temporal Logic to specify properties in the distributed scenario and Bayesian statistical model checking techniques and hypothesis testing algorithm for verifying QBLTL properties, as in \cite{zuliani-etal:2013:fmsd}. They developed a Smart Grid case study to individuate cost-benefit relations relevant to full-scale deployment.
%% %Differently from us, they do not consider a real case, but to describe the behaviour of consumers by assuming they follow certain probability distributions in the use of appliances and on the hour of the day.

%% %%%%%%%%%%%%%%%%%%%%%%%%%%
%% % ADD CITATION TO PRISM
%% %%%%%%%%%%%%%%%%%%%%%%%%%
%% The work in \cite{yuksel-etal:2012:tase} 
%% %Yuksel \textit{et al.} 
%% uses a Markov chain based modelling approach and
%% uses the PRISM model checker to analyse robustness to failures of a smart grid power transmission line.

%% %verify that a power transmission line in a smart grid has an appropriate robustness against failures by using formal verification techniques based on model checking. In particular they adopt algorithmic techniques, known as stochastic model checking. They use Prism, that is the most used stochastic model checkers for model checking of (discrete and continuous time) Markov chains.  Finally, they use a specific Chinese Smart Grid implementation as a case study.

%% To the best of our knowledge, no statistical safety verification approach has ever been developed to handle 
%% safety verification of user demand control policies using a full scale EDN model, like those that PPSV can handle.

%% \subsubsection{Average Case Analysis Methods}

%% Monte Carlo based methods aiming at evaluating the average behaviour of the system under analysis
%% are widely used in \textit{performance evaluation} where, typically, the average case is the 
%% most interesting one. Such methods however, are not very well suited for safety analysis since they
%% cannot address rare (low probability) events and, most importantly, 
%% do not provide any lower bound for the statistical confidence achieved.

%% We note however that many works about user demand control policies focus indeed on performance evaluation,
%% rather than on safety verification, of the control policy, and, to that end,
%% rely on an average case analysis based on Monte Carlo method. 
%% Accordingly, for sake of completeness, we include Monte Carlo based methods in our comparison.

%% The work in \cite{koutitas-tassiulas:2013:tsg} 
%% presents control policies defining time shifts on periodic loads
%% in order to provide peak power and energy cost reduction over a
%% limited time horizon. Effectiveness of the proposed control policies is evaluated 
%% using a Monte Carlo based approach where 100 network topologies are generated at random
%% and smart devices in each smart building are generated by following a suitable stochastic model.

%% %Namely the algorithm is executed on 100 randomly generated independent snapshots of network topologies. For each scenario, the characteristics and the number of smart devices in each smart building are generated by following a stochastic model.
%% %proposes a distributed optimization algorithm for a phase management control scheme and provide an evaluation of its performance using Monte Carlo analysis. 
%% %Namely the algorithm is executed on 100 randomly generated independent snapshots of network topologies. For each scenario, the characteristics and the number of smart devices in each smart building are generated by following a stochastic model.
%% %develop a phase management scheme to define optimal time shifts on the periodic loads, in order to provide peak power and energy cost reduction over a limited time horizon. They propose a centralized and a distributed optimization algorithm for implementing the control scheme and provide an evaluation of the performance using Monte Carlo analysis. Namely the algorithm is executed on 100 randomly generated independent snapshots of network topologies. For each scenario, the characteristics and the number of smart devices in each smart building are generated by following a stochastic model.

%% The work in \cite{chang-etal:2013:tsg} proposes control strategies to improve real-time power balancing with collaborative energy management.
%% %The approach is multi-stage stochastic optimisation problem with customers energy requests random in time. They propose a decentralised stochastic optimisation algorithm, CoHEM, that performs a local computation of scheduling solutions based on domestic user information and message exchange between neighbours. 
%% Effectiveness of the approach is showed by estimating the expected power load using the Monte Carlo method. 
%% %To this end, simulation on 100 randomly generated realizations are executed. Simulation results are averaged, and demonstrate that the proposed CoHEM architecture can  improve real-time power balancing. 

%% While average case analysis approaches aim at evaluating the average behaviour of the system,
%% PPSV, aiming at safety verification, estimates the distribution probability of (aggregated user demand) scenarios and also computes a 
%% statistical confidence for such a distribution. 

%% \subsubsection{Benchmark Based Methods}

%% Performance evaluation can also be done using suitable benchmarks. This is often quite interesting since it guarantees
%% that the system is evaluated on relevant case studies. 
%% We note however, that this approach cannot be used for safety verification since there is no upper bound of any kind on the 
%% probability that a potentially unsafe scenario has not been considered in the analysis.

%% Many control policies in a smart grid context are evaluated using case studies. Accordingly,
%% for sake of completeness, we include benchmark based methods in our comparison.

%% %Several examples of a case study are presented in literature by which the verification of effectiveness of the proposal is shown. This is done by means of  either 
%% % a physical realization or a specific (control or optimisation) algorithm. 

%% %This approach has been used for the design of both smart grid control devices \cite{lee-etal:2013:tsg, lee-hui:2013:tsg} and smart grid control policies 
%% %\cite{guo-etal:2013:tsg, atzeni-etal:2013:tsg, lou-etal:2013:tsg, zhao-etal:2013:tsg}.
%% %An example for the case of the design of smart grid control devices is given in \cite{lee-etal:2013:tsg}. Lee \textit{et al.} study how electric springs can be used to solve the stability problems arising from the intermittent nature of renewable energy sources, to the end of ensuring that the load demand follows the power generation.  

%% In order to ensure that the load demand follows the power generation the work in \cite{lee-etal:2013:tsg} proposes control policies for electric springs aiming at solving the stability problems arising from the intermittent nature of renewable energy sources. Effectiveness of the approach is shown
%% with an experimental evaluation conducted considering different case studies. 

%% %scheme implemented on the control board of each electric spring, based on a theoretical analysis.
%% %An experimental verification is conducted considering different cases. 

%% The work in \cite{lee-hui:2013:tsg} %Lee \textit{et al.} give the mathematical proof that the 
%% presents electric spring control strategies to reduce energy storage requirements in power grids. 
%% Effectiveness of the proposed approach is shown by taking measurements on a smart grid setup in laboratory.

%% The works in \cite{guo-etal:2013:tsg}, \cite{atzeni-etal:2013:tsg}, \cite{lou-etal:2013:tsg}, \cite{zhao-etal:2013:tsg}  propose
%% smart grid control policies and show their effectiveness by performing simulation on meaningful case studies.

%% %Several proposals are available for the case of the design of smart grid control policies. 

%% %In \cite{guo-etal:2013:tsg}, Guo \textit{et al.} propose a collaborative and decentralized energy consumption scheduling algorithm for the reduction of both the impact of the household energy consumption on the power system and the total energy cost. Simulations are performed on different situations. 
%% %Many proposal are derived from the formulation of an optimization problem.

%% %Atzeni \textit{et al.} \cite{atzeni-etal:2013:tsg} model the problem of reducing energy expenses by producing or storing energy rather than purchasing energy from the grid as an optimization process. The optimization problem is modeled as a noncooperative Nash game and the goal is the search of Nash equilibria, when a practical pricing model is applied. The algorithm proposed for the optimization problem is tested by  simulations on a realistic situation employing practical cost functions.

%% %Lou \textit{et al.} \cite{lou-etal:2013:tsg} tackle the problem of optimizing operator profits for different cases of load curtailment, under various constraints, that are properties of the power system, different cost and valuation functions for heterogeneous generation units and loads. They formulate two optimization problems and solution methods, and present extensive numerical results to demonstrate the significant profit gain compared with traditional load shedding approaches. They perform also simulation to quantify the effects of cyber control for load curtailments on the frequency stability of the power system.

%% %In \cite{zhao-etal:2013:tsg}, Zhao \textit{et al.} show how users can schedule the power usage in their home for the purpose of reducing electricity expense and alleviating the power peak-to-average ratio. Authors formulate the power consumption scheduling problem as an optimization problem, and propose a solution based on the use of a genetic algorithm. Simulation results for this approach are presented to show its effectiveness and feasibility for working in the energy management system.

%% Case study based approaches aim at evaluating performance of the system on scenarios that are known to be meaningful.
%% However, safety analysis has the goal of ruling out existence of an unsafe scenario. 
%% Accordingly, case study based approaches are not well suited for safety verification and are, of course, quite different,
%% from PPSV approach. On the other side we note that effectiveness of PPSV approach itself has been evaluated using a case study
%% (namely, the one from Kalundborg demonstration).

